Multi-robot Mission Planning in Dynamic Semantic Environments

This paper addresses a new semantic multi-robot planning problem in uncertain and dynamic environments. Particularly, the environment is occupied with non-cooperative, mobile, uncertain labeled targets. These targets are governed by stochastic dynamics while their current and future positions as well as their semantic labels are uncertain. Our goal is to control mobile sensing robots so that they can accomplish collaborative semantic tasks defined over the uncertain current/future positions and labels of these targets. We express these tasks using Linear Temporal Logic (LTL). We propose a sampling-based approach that explores the robot motion space, the mission specification space, as well as the future configurations of the labeled targets to design optimal paths. These paths are revised online to adapt to uncertain perceptual feedback. To the best of our knowledge, this is the first work that addresses semantic mission planning problems in uncertain and dynamic semantic environments. We provide extensive experiments that demonstrate the efficiency of the proposed method

==> algorithm2e.tex <==
%  algorithm2e.sty --- style file for algorithms
%                      almost everything can be customized by users. See the document for more explanations
%% Copyright 1996-2015 Christophe Fiorio
%
% This work may be distributed and/or modified under the conditions of the LaTeX Project
% Public License, either version 1.3 of this license or (at your option) any later version.
% The latest version of this license is in http://www.latex-project.org/lppl.txt and
% version 1.3 or later is part of all distributions of LaTeX version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is M. Christophe Fiorio
%
% This work consists of the files algorithm2e.sty and algorithm2e.tex 
% and the associated example files algorithm2e_exAlgoDisjdecomp.tex,
% algorithm2e_exIR.tex, algorithm2e_ex01.tex, algorithm2e_exProg.tex,
% algorithm2e_ex02.tex, algorithm2e_exfor.tex, algorithm2e_ex03.tex,
% algorithm2e_exgeneric.tex, algorithm2e_ex04.tex,  algorithm2e_exgeneric2.tex,
% algorithm2e_ex05.tex, algorithm2e_exnlsty.tex, algorithm2e_ex06.tex,
% algorithm2e_exrepeat.tex, algorithm2e_ex07.tex, algorithm2e_exswitch.tex
%  
%  Report bugs and comments to:
%  - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
%  - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
%  subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
%
%  $Id: algorithm2e.sty,v 5.1 2015/10/18 21:37:30 cfiorio Exp $
%
%  PACKAGES REQUIRED:
%
%  - float   (in contrib/supported/float)
%  - ifthen  (in base)
%  - xspace  (in packages/tools)
%  - relsize (in contrib/misc/relsize.sty)
%
%%%%%%%%%%%%%%%  Release 5.1
%
%   Package options: 
%   ---------------
%   - oldcommands                      : to use old command names
%   - french, english, german, ngerman
%      portuguese, czech, italiano,
%      slovak, croatian, spanish       : for the name of the algorithm and some keyword code
%   - onelanguage                      : to simply switch keyword from one language to another without changing
%                                        keyword commands
%   - boxed, boxruled, ruled, tworuled, 
%     algoruled, plain                 : layout of the algorithm
%   - algo2e                           : environment is algorithm2e instead of algorithms and \listofalgorithmes
%                                        instead of \listofalgorithms
%   - slide                            : to use when making slides
%   - noline,lined,vlined              : how block are designed.
%   - shortend, longend, noend         : short or long end keyword as endif for e.g.
%   - linesnumbered                    : auto numbering of the algorithm's lines
%   - linesnumberedhidden              : to hide autonumbered lines (show number on a line with \ShowLn
%   - commentsnumbered, inoutnumbered  : to autonumber comments and inout keywords (by defaut not numbered)
%   - rightnl                          : to have line number on the right instead of on the left as default
%   - algonl                           : line numbers preceded by algo number
%   - scright, scleft                  : right or left justified side comments
%   - fillcomment, nofillcomment       : end mark of comment is flushed to the right so comments fill the line
%   - dotocloa                         : add an entry in the toc for list of algorithms (require tocbibind package)
%   - endfloat                         : add algoendfloat environment pushing algorithm so written to the end of document
%   - resetcount, noresetcount         : start value of line numbers.
%   - algopart,algochapter,algosection : algo numbering within part, chapter or section
%   - titlenumbered,titlenotnumbered   : numbering of title set by \Titleofalgo
%   - figure                           : algorithms are figures, numbered as figures, and put in the list of figures.
%   - procnumbered                     : procedure or function are numbered as algorithm
%   - nokwfunc                         : procedure or function name doens't become a command
%   - norelsize                        : don't use relsize package (useful if it breaks the compatibily)
%   - displayblockmarkers              : display begin, end keywords at start of each block
%  
%   defaults are; english,plain,resetcount,titlenotnumbered
%
%%%%%%%%%%%%%%
%
%   Short summary  
%   -------------
%  
%   algorithm is an environment for writing algorithm in LaTeX2e.
%   Almost all is customizable. You can add keywords, change style, change the layout, ...
%   It provide macros that allow you to create differents sorts of key words, therefore a set of predefined key
%   word is gived.
%
%   IT should be used as follows
%
%   \begin{algorithm}
%       ...
%       ...
%   \end{algorithm}
%
%
%   IMPORTANT : each line MUST end with \;
%
%   Note that if you define macros outside algorithm environment they
%   are avaible in all the document and particulary you can use then
%   inside all algorithms without re-define them.
%  
%   an example:
%
%   \begin{algorithm}
%     \SetAlgoLined
%     \KwIn{this text}
%     \KwOut{how to write algorithm with \LaTeX2e }
%     
%     initialization\;
%     \While{not at end of this document}{
%       read current section\;
%       \eIf{understand}{
%         go to next section\;
%         current section becomes this one\;
%         }{
%         go back to the beginning of current section\;
%         }
%       }
%     \caption{How to write algorithm}
%   \end{algorithm}
%
%
%%%%%%%%%%%%%%         predefined keywords
%
%     \KwIn{input}
%     \KwOut{output}
%     \KwData{input}
%     \KwResult{output}
%     \KwTo                                       % a simple keyword
%     \KwFrom                                     % a simple keyword
%     \KwRet{[value]}
%     \Return{[value]}
%     \Begin{block inside}
%     \eIf{condition}{Then Block}{Else block}     % in blocks
%     \If{condition}{Then block}                  % in a block
%     \uIf{condition}{Then block}                 % in a block unended
%     \lIf{condition}{Else text}                  % on the same line
%     \Else{inside Else}                          % in a block
%     \lElse{Else text}                           % on the same line        
%     \uElse{Else text}                           % in a block unended
%     \ElseIf{inside Elseif}                      % in a block
%     \lElseIf{Elseif text}                       % on the same line        
%     \uElseIf{Elseif text}                       % in a block unended
%     \Switch{Condition}{Switch block}
%     \Case{a case}{case block}                   % in a block
%     \lCase{a case}{case text}                   % on the same line
%     \Other{otherwise block}                     % in a block
%     \lOther{otherwise block}                    % on the same line
%     \For{condition}{text loop}                  % in a block
%     \lFor{condition}{text}                      % on the same line
%     \ForEach{condition}{text loop}              % in a block
%     \lForEach{condition}{text}                  % on the same line
%     \ForPar{condition}{text loop}               % in a block
%     \lForPar{condition}{text}                   % on the same line
%     \While{condition}{text loop}                % in a block
%     \lWhile{condition}{text loop}               % on the same line
%     \Repeat{End condition}{text loop}           % in a block
%     \lRepeat{condition}{text}                   % on the same line
%
%%%%%%%%%%%%%%
%
%   History: 
%
%   -  October 19 2015 - revision 5.1
%                   * CHANGE/ADD: l commands  (the ones as \lIf) can now be used with a
%                              star. If done, no end of line are done, so you can enclose
%                              l command into another one. For example, you can write:
%                              \lForEach{$i$}{\lIf*{foo}{bar}}.
%                               Note that when you use a star, side comments are not allowed.
%                   * CHANGE/ADD: Now you can have a side comment at end of macros which
%                               have a block. For example you can do : 
%                               \Begin(\tcc*[h]{side comment for begin}{text}(\tcc*[h]{side comment after end})
%                               Note: there are some side effects for some commands:
%                              \SetKwProg : macro defined thanks to \SetKwProg are allowed
%                                                   to have no end marker. In this case,
%                                                   beware to end side comment, this can
%                                                   do weird output (but no error)
%                   * CHANGE: \SetKwSwitch defines also an \uOther command which was not
%                               the case until this release.
%                   * CHANGE: \SetStartEndCondition{typo1}{typo2}{typo3} defined two end
%                               conditions (type2 and typo3) : typo3 is no more used for
%                               case condition as typo2 is used which is more consistent
%                               since there is a condition followed by a keyword as for
%                               if-then or other command that are defined using typo2.
%                   * CHANGE: keywords was not language dependant to allow to use multiple
%                               languages in the same document, but some keywords in
%                               different language were having the same keyword that lead
%                               last one declared to replace first one and so you could have some
%                               spanish keywords printed as you were in portuguese. So
%                               this behavior is changed from now:
%                               - localized keywords are defined if according language
%                                  option is defined ; 
%                               - if you want to keep old behaviour and use localized
%                                  keywords without using language option (keep old
%                                  behavior), you can use languagekw option
%                                  (e.g. frenchkw, germankw, ...). Note that you can use
%                                  multiple languagekw options at the same time, in
%                                  contrary of language option. Note also that if you use
%                                  multiple languagekw options, you can get back the same
%                                  problem as previously when keywords was not language
%                                  dependant.
%                   * ADD: new typo styles:
%                               - Arguments of functions have now their own style. By
%                                  default, FuncArgSty is the same as ArgSty. 
%                               - Name of KwProg have now their own sty (they used ArgSty
%                                  previously). By default, ProgSty is still ArgSty.
%                               As usual, \SetFuncArgSty{}, FuncArgSty{} and
%                               \SetProgSty{}, ProgSty{} are macros to set and use these
%                               typo styles.
%                   * ADD: Options to manage algorithm hangindent
%                            Until this revision, long statement acts as classical text and
%                            continue on next line starting from the same point. This makes
%                            difficult to notice that the new lines of text is not a new
%                            statement. Now, hangindent is managed and when a long
%                            statement continue on next lines, lines, except the first,
%                            are indented.
%                            Option: noalgohanging
%                               By default, long statement are indented on subsequent
%                               lines; with this option you get old behavior and lines are
%                               no more indented
%                            Option: hangingcomment 
%                               Comment that are alone on a line (not side comment) are
%                               not driven by algo hanging: subsequent lines of long
%                               comments are indented according to width of start comment
%                               marker. With this option, comment are indented like normal
%                               statement.
%                            Option: hanginginout
%                               As for comment, by default, in/out keywords and input
%                               keywords (defined by \SetKwInOut or \SetKwInput) are not
%                               indented by algorithm hangindent. They are indented
%                               according to width of input keyword. If you want that these
%                               keywords acts like normal statement, use this option.
%                            \SetAlgoHangIndent{length}
%                               This macro allows you to set your own indent length. By
%                               default, \SetAlgoHangIndent{0.5em}
%                   * ADD: Group markers. 
%                            This option is related to block markers of release 5.0. Some
%                            have ask to put also block markers for single line
%                            command. This new feature has been implemented to do this.
%                            So, you can now ask package to put begin and end keywords
%                            automatically at start and end of single line command (see
%                            example in documentation).
%                            These new group markers macros are:
%                            - \AlgoDisplayGroupMarkers and \AlgoDontDisplayGroupMarkers
%                            Note that a new option has also been added: displaygroupmarkers
%                   * ADD: \SetCustomAlgoRuledWidth{length}
%                             set a custom ruled width of ruled and algoruled options ;
%                             note that by the moment you use this macro, rules will have
%                             this fixed length: this can cause strange behavior in
%                             multicolumn mode or other layout that change the line
%                             width. 
%                   * ADD: turkish language option
%                   * FIX: a spurious whitespace which results in a spurious indent in the
%                            user's text right after the end of the algorithm environment
%                            was introduced  in release 5.0. This is fixed now thanks to
%                            Alexander Malkis.
%                   * FIX: there was a problem with margins in caption when option figure
%                            was use with caption package. This is fixed.
%                   * FIX: when changing font size in caption with, interline skip stayed
%                            unchanged and so with a small font was to large. This is fixed.
%                   * FIX: in contrary of that is written in the documentation, ':' what
%                            not in KwSty typo for KwIn and KwOut command. This is fixed. 
%                   * FIX: strange behaviour with label and lines numbered: @currentlabel
%                            was updated according to algo line number not in all
%                            situation. For e.g, with hyperref package, always updated ;
%                            with \nlset also updated, but with \nl or linesnumbered
%                            option, not updated. This "feature" causes different output
%                            with \label command according to options used which is not
%                            that one want. This is solved now, and @currentlabel is
%                            always updated so \label command works always is the same way.
%                   * FIX: some czech keywords
%                   * FIX: some spanish keywords
%                   * FIX: some croatian keywords
%                   * FIX: krantz class changes definition of chapter and get one more
%                            option that classical classes as book.cls or report.cls and
%                            broke fix for hyperref on chapter definition. This is now
%                            fixed and algorithm detects use of krantz class and use then
%                            a definition of chapter working with krantz class.
%                   * FIX: an issue with internal macro which causes ([Q]) use as argument
%                            of some environment to be misprinted (thanks to Martin Schr?der).
%                   * FIX: mispelled name of hyperrefcounter inside internal macro.
%
%   - January 06 2013 - revision 5.0
%                     * CHANGE: SetKwSwitch takes now 9 args: 9th arg is the same as
%                                previous 8th arg ('end of switch' keyword). New 8th arg is
%                                'end of case' keyword. This is due to change of release
%                                3.2 which introduce end after case block... as I never
%                                test with longend option, I never see that the 'end
%                                switch' used for case was not good.
%                     * CHANGE: when no end keyword is defined in a block macro, then
%                                algorithm2e does no more try to print it. So even with lined or noline
%                                option, no empty line is printed (before: a blank end was
%                                printed, so a blank line appeared)
%                     * Internal Change: add some internal function to improve readibility
%                                        (thanks to Philip K. F. H\?lzenspies)
%                     * ADD: Block markers. 
%                            You can now ask package to put begin and end keywords automatically at begin
%                            and end of blocks, it means each group of commands shifted and enclosed in
%                            braces.
%                            This is tricky to use but, combined with \SetStartEndCondition and
%                            redefinition of keywords, you should be abble to simulate any syntax. See
%                            examples in documentation where a generic example is derived in pseudo-code,
%                            python and C by keeping code and changing only style using block markers
%                            macros, \SetStartEndCondition and some redefinition of keywords.
%                            These new block markers macros are:
%                            - \AlgoDisplayBlockMarkers and \AlgoDontDisplayBlockMarkers
%                            - \SetAlgoBlockMarkers{begin marker}{end marker}
%                            - \BlockMarkersSty{text} and \SetBlockMarkersSty
%                            Note that a new option has also been added: displayblockmarkers
%                     * ADD: \leIf macro automatically defined by \SetKwIF: allow to define
%                            an if-then-else on a single line.
%                     * ADD: new macro \SetStartEndCondition{typo1}{typo2}{typo3} which
%                            sets typo around condition in For, If, Switch, Case and
%                            Repeat macros. First two are used around For, If, Swith
%                            conditions, First and third are used for Case and Repeat
%                            condition where condition ends the line. Default definition
%                            is \SetStartEndCondition{ }{ }{}. 
%                            A common alternative is \SetStartEndCondition{ (}{) }{)}
%                            Can also be used to remove space around condition, for
%                            example if you want python style commands:
%                            \SetStartEndCondition{ }{}{} and \SetKwFor{For}{for}{:}{}
%                     * ADD: new environment algomathdisplay which allow display math (like inside \[ \] or $$ $$) 
%                            handling end line and line number
%                     * ADD: new command \SetKwProg{Env}{Title}{is}{end} which defines a macro
%                            \Env{args}{text}. Env is a block with 'Title' (in \CapSty) at the beginning
%                            followed by args followed by 'is' then 'text' is put below inside a block ended
%                            by 'end'. If no 'end' is specified, nothing is written (no
%                            blank line is inserted). Useful to typeset function or prog for example:
%                            \SetKwProg{Fn}{Function}{ is}{end} makes \Fn{afunc(i: int) : int}{return 0\;}                    
%                            writes: 
%                            Function afunc(i: int) : int is
%                            | return 0;
%                            end
%                            or \SetKwProg{Def}{def}{:}{} makes \Def{afunc(i: int)}{return 0\;} writes:
%                            def afunc(i: int):
%                            | return 0
%                            Tip: combine it with \SetKwFunction to write recursive function algorithm. With
%                            example above, you could define \SetKwFunction{\Afunc}{afunc} and then write:
%                            \Def{\Afunc{i:int}{\eIf{i>0}{\KwRet \Afunc{i-1}}{\KwRet 0\;}} that writes:
%                            def afunc(i: int):
%                            | if(i>0):
%                            |     return afunc(i-1)
%                            | else:
%                            |     return 0
%                            with appropriate typo.
%                     * ADD: option croatian: croatian keywords (thanks to Ivan Gavran)
%                     * ADD: option ngerman: same as german option but so can be used with global option ngerman
%                            of babel
%                     * ADD: option spanish: Spanish support (thanks to Mario Abarca)
%                     * ADD: unterminated block: useful to add part separator that doesn't necessary need an end
%                            keyword.  
%                            Designed on the pattern of unterminated if (see \uIf macro) allowing to
%                            add a block that is not terminated by a keyword. Such block are defined in the same
%                            time as a block is defined by adding a macro beginning with u. So, for example,
%                            predefined \SetKwBlock{Begin}{begin}{end} defines now two commands:
%                            - \Begin{} as previously which print a begin - end block
%                            - \uBegin{} that defines a begin only block
%                     * FIX: problem when numbering line inside until condition of
%                            \SetKwRepeat macro: line number was not correctly aligned.
%                     * FIX: dotocloa option which was broken
%                     * FIX: uIf and uCase didn't have same behavior when used with
%                            noline, vlined or lined option. This is fixed. Side effect: no empty
%                            line after an uIf or uCase when used with options lined or vlined
%                     * FIX: a bug with Repeat Until command when use with side comment on Until
%                     * FIX: a bug with side text -- text put into () -- of command macro (SetKwIf and so on)
%                            which was always setting a ';' even after a \DontPrintSemicolon
%                     * FIX: a bug with hyperref and chapter definition (thanks to Hubert Meier)
%                     * FIX: bugs with l macro and side comment
%                     * FIX: revision number
%                     * FIX: fix non ascii character (utf8 not yet recognized by all latex engine)
%                     * FIX: fnum@algocf had an useless parameter which sometimes broke expansion and output an error
%                     * FIX: works now with multicol package
%
%   - december 14 2009 - revision 4.1
%                     * ADD: new command \SetKwHangingKw{Name}{text} (hanging indent with keyword): This creates a
%                            hanging indent much like \texttt{SetKwInput}, except that it removes the trailing `:'
%                            and does not reset numbering (thanks to Nathan Tallent)
%
%   - november 17 2009  - revision 4.00 -
%
%                      * CHANGE: IMPORTANT: some commands have been renamed to have consistent naming (CamlCase
%                                syntax) and old commands are no more available. If you doesn't want to change
%                                your mind or use old latex files, you can use oldcommands option to enable old
%                                commands back.
%                                text. Here are these commands:
%                                - \SetNoLine becomes \SetAlgoNoLine
%                                - \SetVline  becomes \SetAlgoVlined
%                                - \Setvlineskip  becomes \SetVlineSkip
%                                - \SetLine   becomes \SetAlgoLined
%                                - \dontprintsemicolon becomes \DontPrintSemicolon
%                                - \printsemicolon becomes \PrintSemicolon
%                                - \incmargin becomes \IncMargin
%                                - \decmargin becomes \DecMargin
%                                - \setnlskip becomes \SetNlSkip
%                                - \Setnlskip becomes \SetNlSkip
%                                - \setalcapskip becomes \SetAlCapSkip
%                                - \setalcaphskip becomes \SetAlCapHSkip
%                                - \nlSty becomes \NlSty
%                                - \Setnlsty becomes \SetNlSty
%                                - \linesnumbered becomes \LinesNumbered
%                                - \linesnotnumbered becomes \LinesNotNumbered
%                                - \linesnumberedhidden becomes \LinesNumberedHidden
%                                - \showln becomes \ShowLn
%                                - \showlnlabel becomes \ShowLnLabel
%                                - \nocaptionofalgo becomes \NoCaptionOfAlgo
%                                - \restorecaptionofalgo becomes \RestoreCaptionOfAlgo
%                                - \restylealgo becomes \RestyleAlgo
%                                - gIf macros and so on do no more exist
%                      * NEW: - Compatibily with other packages improven by changing name of internal
%                               macros. Algorithm2e can now be used with arabtex for example, if this last is
%                               loaded after algorithm2e package.
%                      * ADD: - OPTION endfloat: endfloat packages doesn't allow float environment inside other
%                               environment. So using it with figure option of algorithm2e makes error. This
%                               option enables a new environment algoendfloat to be used instead of algorithm
%                               environment that put algorithm at the end. algoendfloat environment make
%                               algorithm acting as endfloat figures. This option requires endfloat packages.
%                      * ADD: - OPTION norelsize: starting from this release (v4.00), algorithm2e package uses
%                               relsize package in order to get relative size for lines numbers; but it seems
%                               that some rare classes (such as inform1.cls) are not compatible with relsize; to
%                               have algorithm2e working, this option makes algorithm2e not to load relsize
%                               package and go back to previous definition by using \scriptsize font for lines
%                               numbers.
%                      * ADD: - OPTION onelanguage: allow, if using standard keywords listed below, to switch
%                               from one language to another without changing keywords by using appropriate
%                               language option:
%                               . KwIn, KwOut, KwData, KwResult
%                               . KwTo KwFrom
%                               . KwRet, Return
%                               . Begin
%                               . Repeat
%                               . If, ElseIf, Else
%                               . Switch, Case, Other
%                               . For, ForPar, ForEach, ForAll, While
%                               .
%                      * ADD: - OPTION rightnl: put lines numbers to the right of the algorithm instead of left.
%                      * ADD:   new commands \setRightLinesNumbers and \setLeftLinesNumbers which sets the lines
%                               numbers to the right or to the left of the algorithm.
%                      * ADD: - new kind of keywords: KwArray used to define arrays:
%                               \SetKwArray{Kw}{array} defines an array keywords Kw called array and printed in
%                               DataSty style when call with \Kw. It can be used with one argument which
%                               denotes the element index: \Kw{n} prints array[n] with array in DataSty and n in
%                               ArgSty.
%                      * ADD/FIX: rules of ruled, algoruled, tworuled styles used rules of different sizes! This
%                                 is now fixed. Moreover size of the rules is now controlled by a length and so
%                                 can be customized by the user.
%                                 \algoheightrule is the height of the rules and can be changed via \setlength
%                                 \algoheightruledefault is the default height of he rules (0.8pt)
%                                 \algotitleheightrule is the height of the rule that comes just after the
%                                 caption in ruled and algoruled style; it can be changed via \setlength
%                                 \algotitleheightruledefault is the default height of this rules (0.8pt)
%                                 Thanks to Philippe Dumas who reports the bug and make the suggestion.
%                      * ADD: - \SetAlgoCaptionSeparator which sets the separator between Algorithm 1 and the
%                               title. By default it's ':' and caption looks like "Algorithm 2: title" but now
%                               you can change it by using for example \SetAlgoCaptionSeparator{.} which will
%                               give "Algorithm 3. title"
%                      * ADD: - \SetAlgoLongEnd and \SetAlgoShortEnd and \SetAlgoNoEnd commands which act as
%                               corresponding package options
%                      * ADD: - OPTIONS italiano and slovak as new language (thanks to Roberto Posenato and
%                               Miroslav Binas) 
%                      * CHANGE: - Fnt and Sty macro to have consistent use and naming (see below)
%                      * ADD: - \AlCapSty, \AlCapNameSty, \AlCapFnt, \AlCapNameFnt, \ProcSty, \ProcFnt,
%                               \ProcNameSty, \ProcNameFnt, \ProcArgSty, ProcArgFnt and corresponding "set macro" 
%                               \SetAlCapSty, \SetAlCapNameSty, \SetAlCapFnt, \SetAlCapNameFnt, \SetProcSty,
%                               \SetProcFnt, \SetProcNameSty, \SetProcNameFnt, \SetProcArgSty, \SetProcArgFnt which
%                               control the way caption is printed. Sty macro use command taking one parameter as
%                               argument, Fnt macros use directly command. In Fact caption is printed as follow:
%                               \AlCapSty{\AlCapFnt Algorithm 1:}\AlCapNameSty{\AlCapNameFnt my algorithm}
%                               By default, \AlCapSty is textbf and \AlCapFnt is nothing. \AlCapNameSty keep text 
%                               as it is, and \AlCapNameFnt do nothing also.
%                               You can redefine \AlCapFnt and \AlCapNameFnt by giving macro to \Set commands. For
%                               example, you can do \SetAlCapFnt{\large} to see Algorithm printed in \large font.
%                               You can redefine \AlCapSty, \AlCapFnt, \AlCapNameSty and \AlCapNameFnt with the
%                               corresponding \Set command. For the Sty commands, you have to give in parameter
%                               name of a macro (whithout \)  which takes one argument. For example,
%                               \SetAlCapFnt{textbf} defines the default behaviour. If you want to do more
%                               complicated thing, you should define your own macro and give it to \SetAlCapFnt or
%                               \SetAlCapNameFnt. Here are two examples:
%                               - \newcommand{\mycapsty}[1]{\tiny #1}\SetAlCapNameSty{mycapsty}
%                               - \newcommand{\mycapsty}[1]{\textsl{\small #1}}\SetAlCapNameSty{mycapsty}
%                               Or you can combine the two, for the last example you can also do:
%                               \SetAlCapNameSty{textsl}\SetAlCapNameFnt{\small}
%                               Thanks to Jan Stilhammer who gives me the idea of \AlCapNameFnt.
%                      * CHANGE \AlTitleFnt to match definition of all other Fnt macros and add a \AlTitleSty 
%                               macro (see below) . Now you set \AlTitleFnt by calling \SetAlTitleFnt with 
%                               directly a macro without parameter in argument:
%                               Example: \SetAlTitleFnt{\small} to set title in small font.
%                      * ADD: - \AlTitleSty and \SetAlTitleSty commands to set a style for title. These commands
%                               are defined from a macro taking the text in argument, as \textbf for example. 
%                               To set the TitleSty you have to give name of the macro (without the '\') 
%                               to \SetAlTitleSty. For example \SetAlTitleSty{textbf} to set \textbf style.
%                      * ADD: - new command \SetAlgorithmName{algorithmname}{list of algorithms name} which
%                               redefines name of the algorithms and the sentence list of algorithms. Second
%                               argument is the name that \autoref, from hyperref package, will use. Example:
%                               \SetAlgorithmName{Protocol}{List of protocols} if you prefer protocol than
%                               algorithm.
%                      * ADD: - new \SetAlgoRefName{QXY} which change the default ref (number of the algorithm) by
%                               the name given in parameter (QXY in the example). 
%                      * ADD: - new command \SetAlgoRefRelativeSize{-2} which sets the output size of refs, defined
%                               by \SetAlgoRefName, used in list of algorithms.
%                      * ADD: - two dimensions to control the layout of caption in ruled, algoruled and boxruled
%                               algorithms:
%                               - interspacetitleruled (2pt by defaut) which controls the vertical space between
%                                 rules and title in ruled and algoruled algorithms.
%                               - interspaceboxruled (2\lineskip by default) which controls the vertical space
%                                 between rules and title in boxruled algorithms.
%                               These two dimensions can be changed by using \setlength command.
%                      * ADD: - With the fix (see below) of procedure and function environments, a new feature has
%                               been added: the name of the procedure or function set in caption is automatically
%                               defined as a KwFunction and so can be used as a macro. For example, if inside a
%                               procedure environment you set \caption{myproc()}, you can use \myproc macro in you
%                               main text. Beware that the macro is only defined after the \caption!
%                      * ADD: - OPTION nokwfunc to unable the new feature described above in function and
%                               procedure environment. Useful if you use name of procedure or function that cannot
%                               be a command name as a math display for example.
%                      * ADD: - \SetAlgoNlRelativeSize{number} command which sets the relative size of line
%                               numbers. By default, line numbers are two size smaller than algorithm text. Use
%                               this macro to change this behavior. For example, \SetAlgoNlRelativeSize{0} sets it
%                               to the same size, \SetAlgoNlRelativeSize{-1} to one size smaller and
%                               \SetAlgoNlRelativeSize{1} to one size bigger
%                      * ADD: - \SetAlgoProcName{aname} command which sets the name of Procedure printed by
%                               procedure environment (the environment prints Procedure by default). Second
%                               argument is the name that \autoref, from hyperref package, will use.
%                      * ADD: - \SetAlgoFuncName{aname} command which sets the name of Function printed by
%                               procedure environment (the environment prints Function by default). Second
%                               argument is the name that \autoref, from hyperref package, will use. 
%                      * ADD: - \SetAlgoCaptionLayout{style} command which sets style of the caption; style must
%                               be the name of a macro taking one argument (the text of the caption). Examples
%                               below show how to use it:
%                               . \SetAlgoCaptionLayout{centerline} to have centered caption
%                               . \SetAlgoCaptionLayout{textbf} to have bold caption
%                               If you want to apply two styles in the same time, such as centered bold, you have
%                               to define you own macro and then use \SetAlgoCaptionLayout with its name.
%                      * ADD: - OPTION procnumbered: which makes the procedure and function to be numbered as
%                               algorithm
%                      * ADD: - OPTIONS tworuled and boxruled
%                               these are two new layouts: tworuled acts like ruled but doesn't put a line after
%                               caption ; boxruled surround algorithm by a box, puts caption above and add a line
%                               after caption.
%                      * REMOVE: - SetKwInParam has been deleted since not useful itself because of different
%                                macros which can do the same in a better and a more consistent way as
%                                SetKwFunction or SetKw.
%                      * FIX: - line number is now correctly vertically aligned with math display.
%                      * FIX: - references with hyperref. No more same identifier or missing name error. BUT now
%                               you must NOT use naturalnames option of hyperref packages if you do PdfLaTeX
%                      * FIX: - autoref with hyperref package (thanks to J?rg Sommer who notices the problem).
%                      * FIX: - titlenumbered was not working! fixed.
%                      * FIX: - Else(){} acted like uElse. Corrected.
%                      * FIX: - noend management: when a block was inside another and end of block was following
%                               each other, a blank line was added: it's now corrected.
%                      * FIX: - Function and Procedure environment was no more working as defined originally: the
%                               label was no more name of the procedure, it acts always as if procumbered option
%                               has been used.
%                      * FIX: - line numbers had a fixed size which can be bigger than algorithm text accordingly
%                               to \AlFnt set (see also new command \SetAlgoNlRelativeSize above)
%                      * FIX: - semicolon in comments when dontprintsemicolon is used.
%                      * FIX: - listofalgorithms adds a vertical space before first algo of a chapter as for
%                               listoffigures or listoftables
%                      * FIX: - listofalgorithms with twocolumns mode and some classes which don't allow onecolumn
%                               and so don't define \if@restonecol as prescribed in LaTeX (sig-alternate for
%                               example)
%                      * FIX: - algorithm2e now works with elsart cls and some more classes.
%                      * FIX: - blocks defined by SetKwBlock act now as other blocks (if for instance) and don't
%                               write end in vlined mode, instead they print a small horizontal line as required
%                               by the option.
%                      * FIX: - underfull hbox warning at each end of algorithm environment removed.
%
%                      * INTERNAL CHANGE: - short end keyword are deduce from long end keyword by keeping the
%                                           first one. Allows to avoid double definition.
%                      * INTERNAL CHANGE: - procedure, function and algorithm are now resolved by the same
%                               environment to avoid code duplication. 
%
%   - October  04 2005  - revision 3.9 -
%                      * ADD: - \setalcaphskip command which sets the horizontal skip before Algorithm: in caption
%                               when used in ruled algorithm.
%                      * ADD: - \SetAlgoInsideSkip command which allows to add an extra vertical space before and
%                               after the core of the algorithm (ie: \SetAlgoInsideSkip{bigskip}) 
%                      * CHANGE: - caption, when used with figure option, is no more controlled by algorithm2e
%                                  package and so follows the exact behaviour of figures. The drawback is that you
%                                  cannot change the typo with AlTitleFnt or CapFnt. The avantage is that if you
%                                  use caption package, it works.
%                      * FIX: - problem with numbering line and pdflatex
%                      * FIX: - error when algorithm2e package was used with beamer and listings together
%   - February 12 2005  - revision 3.8 -
%                      * FIX: - extra line with noend option.
%   - February 10 2005  - revision 3.7 -
%                      * ADD: - sidecomment: different macros allowing to put text right after code on the same
%                               line. They are defined in the same time comment macros are defined with a star
%                               after the macro name. By default comments are right justified but this can be
%                               change with appropriate option in the macro. Ex:
%                               . default: \tcc*{side comment}
%                               . same as previous: \tcc*[r]{side comment}
%                               . left justify: \tcc*[l]{side comment}
%                               . here: \tcc*[h]{side comment} don't put the end of line mark before
%                                       comment (; by default) and don't end the line.
%                               . flushed: \tcc*[f]{side comment} same as the precedent but right
%                                 justified
%                      * ADD: - OPTION scright (default): right justified side comments (side comments
%                               are flushed to the righr)
%                      * ADD: - OPTION scleft: left justified side comments (side comments are put right after the
%                               code line)
%                      * ADD: - \SetSideCommentLeft acts as scleft option
%                      * ADD: - \SetSideCommentRight acts as scright option
%                      * ADD: - block like macro side text: all macro defining a block allows now to put text right
%                               after key words by putting text into (). Done to be used with sidecomment macros,
%                               but all text can be used. 
%                               Ex: \eIf(\tcc*[f]{then comment}){test}{then text}(else side text){else text}
%                      * ADD: - OPTION fillcomment (default): end mark of comment is flushed to the right so
%                               comments fill all the width of text.
%                      * ADD: - OPTION nofillcomment: end mark of comment is put right after the comment.
%                      * ADD: - \SetNoFillComment acts as nofillcomment option.
%                      * ADD: - \SetFillComment acts as fillcomment option.
%                      * ADD: - OPTION dotocloa: which adds an entry in the toc for the list of algorithms. This
%                               option load package tocbibind if not already done and so list of figures and list
%                               of tables are also added in the toc. If you want to control which ones of the lists
%                               will be added in the toc, please load package tocbibind before package algorithm
%                               and give it the options you want.
%                      * FIX: - vertical spacing for uif macro with noend option
%                      * FIX: - all the compatibility problems between caption and other packages
%                      * FIX: - typographical differences between list of algorithms and other lists  when in
%                               report or book 
%
%   - January 24 2005  - revision 3.6 -
%                      * FIX: - vertical spacing and space characters at the beginning or end of comments.
%                               line numbers of comments not in the NlSty.
%                               Thanks to Arnaud Giersch for his comments and suggestions.
%                      * FIX: - Set*Sty macro: the styles defined was not protected and was modified by surrounding
%                               context. For example KwTo in a \For{}{} was in bold AND italic instead of just in
%                               bold.
%                      * FIX: - line number misplacement after \Indp
%
%   - January 21 2005  - revision 3.5 -
%                      * ADD: - hidden numbering of the lines. Lines are auto-numbered but numbers are shown only
%                               on lines you specify:
%                               * linesnumberedhidden option or \LinesNumberedHidden macro activate this
%                                 functionnality.
%                               * \ShowLn and \ShowLnLabel{lab} macros make the number visible on the
%                               line. \ShowLnLabel{lab} allows to set a label for this line. 
%                               Thanks to Samson de Jager who makes this suggestion and provides the macros.
%                      * ADD: - \AlCapFnt and \SetAlCapFnt which allow to have a different font for
%                               caption. Works like \AlFnt and \SetAlFnt and by default is the same.
%                      * ADD: - \AlCapSkip skip length. This vertical space is added before caption in plain ou
%                               boxed mode. It allows to change distance between text and caption.
%                      * FIX: - caption compatible with IEEEtran class. 
%                      * FIX: - some vertical spacing error with \uIf macros (Thanks to Arnaud Giersch)
%                      * FIX: - Procedure and Function: lines are also numbered like algorithms
%                      * FIX: - CommentSty was not used for Comments
%
%   - January 10 2005  - revision 3.4 -
%                      * FIX: - caption compatible with new release of Beamer class. 
%
%   - June 16 2004     - revision 3.3 - 
%                      * FIX: - Hyperlink references of Hyperref package works now if compiled with pdflatex 
%                               and [naturalnames] option of hyperref package is used.
%                      * FIX: - algorithm[H] had problem in an list environment - corrected
%                      * FIX: - interline was not so regular in nested blocks - corrected
%                      * ADD  - \SetVlineSkip macro which sets the vertical skip after the little horizontal 
%                               rule which closes a block in Vlined mode. By default 0.8ex
%
%   - June 11 2004     - revision 3.2 - AUTO NUMBERING LINES !!!
%                      * ADD: auto numbering of the lines (the so asked and so long awaiting feature)
%                             this feature is managed by 3 options and 3 commands:
%                             - linesnumbered option: lines of the algo are numbered except for comments and
%                               input/output (KwInput and KwInOut)
%                             - commentsnumbered option: makes comments be numbered
%                             - inoutnumbered option: makes data input/output be numbered
%                             - \nllabel{lab} labels the line so you can cite with \ref{lab}
%                             - \LinesNumbered make the following algorithms having auto-numbered lines
%                             - \linesnotnumbered make the following algorithms having no auto-numbered lines
%                      * Change: algo2e option renames listofalgorithms in listofalgorithmes
%                      * FIX: new solution for compatibility with color package, more robust and not tricky.
%                             Many thanks to David Carlisle for his advices
%
%   - June 09 2004     - revision 3.1 -
%                      * Change: \SetKwSwitch command defines an additionnal macro \uCase and \Case prints end
%                      * Change: now macros SetKw* do a renewcommand if the keyword is already defined. So you can
%                                redefine default definition at your own convenience or change your definition
%                                without introducing a new macro and changing your text.
%                      * ADD: new macro \SetKwIF which do \SetKwIf and
%                             \SetKwIfElseIf.The following default definition has been added:
%                             \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
%                             and so you get the macros;
%                             \If \eIf \lIf \uIf \ElseIf \uElseIf \lElseIf \Else \uElse \lElse
%                      * ADD: new macro \SetAlgoSkip which allow to fix the vertical skip before and after the
%                             algorithms. Default is smallskip, do \SetAlgoSkip{} if you don't want an extra space
%                             or \SetAlgoSkip{medskip} or \SetAlgoSkip{bigskip} if you want bigger space.
%                      * ADD: macro \SetKwIf defines in addition a new macro \uElse  (depending on wat name you
%                             have given in #2 arg).
%                      * ADD: macro \SetKwIfElseIf defines in addition a new macro \uElse and \ugElseIf (depending
%                             on what name you have given in #2 and #3 arg).
%                      * Change: baseline of algorithm is now top, so two algorithms can be put side by side.
%                      * FIX: Compatibility with color package solved. The problem was due to a redefinition of
%                             standard macros by color package. This solves compatibility problem with other
%                             packages as pstcol or colortbl. (notified by Dirk Fressmann, Antti Tarvainen and Koby
%                             Crammer)
%                      * Fix: extra little shift to the right with boxed style algorithm removed (notified by
%                             P. Tanovski)
%                      * Fix: algoln option was buggy (notified bye Jiaying Shen)
%                      * Fix: german and portuges option didn't work due to bad typo (notified by Martin Sievers,
%                             Thorsten Vitt and Jeronimo Pellegrini)
%                      
%   - February 13 2004 - revision 3.0 -
%                      * Major revision which makes the package independent from float.sty, so now
%                        - algorithm* works better, in particular can be used in multicols environments
%                        - (known bug corrected)
%                          [H] works now for all sort of environment but is handled differently for classic
%                          environment and star environment (algorithm, figure, procedure and function). For star
%                          environment, H acts like for classical figure environment, so it doesn't stay here
%                          absolutely.
%                        - (known bug corrected)
%                          you can use now floatflt package with algorithm package and even with figure
%                          option. Beware that if you want to put an algorithm inside a floatingfigure, it cannot
%                          be floating, so [H] is required and then figure option should not be used, since
%                          standard figure[H] are still floating with LaTeX.
%                      * boxruled: a new style added. Possible now since no style no more defined by the float
%                        package.
%                      * nocaptionofalgo: dosen't print Algorithm #: in the caption for algorithm in ruled or
%                        algoruled style.
%                        note: this is just documentation of a macro which was already in the package.
%   - December 14 2003 - revision 2.52 -
%                      * output message shorter
%                      * French keyword macro \PourTous was missing for longend option, it has been added.
%                      * TitleofAlgo prints Function or Procedure in corresponding environments.
%
%   - October 27 2003  - revision 2.51 - Revision submitted to CTAN archive
%                      * correction of a minor which make caption in procedure
%                        and function to be blanck with pdfscreen package
%                        (thanks to Joel Gossens for the notification)
%                      * add two internal definition to avoid some errors when
%                        used with Hyperref package (Hyperref package need to
%                        define new counter macro from existing ones, and
%                        don't do it for algorithm2e package, so we do it)
%
%   - October 17 2003  - revision 2.50 - first revision for CTAN archive
%                      * add \AlFnt and \SetAlFnt{font} macros: \AlFnt is used at the beginning of the caption and
%                        the body of algorithm in order to define the fonts used for typesetting algorithms. You
%                        can use it elsewhere you want to typeset text as algorithm. For example you can do
%                        \SetAlFnt{\small\sf} to have algorithms typeset in small sf font. Default is nothing so
%                        algorithm is typeset as the text of the document.
%                      * add \AlTitleFnt{text} and \SetAlTitleFnt{font} macros: The {Algorithm: } in the caption is
%                        typeset with \AlTitleFnt{Algorithm:}. You can use it to have text typeset as {Algorithm:}
%                        of captions. Default is textbf.  Default can be redefined by \SetAlTitleFnt{font}, for
%                        example you can do \SetAlTitleFnt{emph}
%                      * add CommentSty typo for text comment.  
%                      * add some compatibility with hyperref package (still an error on multiply defined refs but
%                        pdf correctly generated)
%                      * flush text to left in order to have correct indentation even with class as amsart which
%                        center all figures
%                      * add german, portuguese and czech options for title of algorithms and typo.
%                      * add portuguese translation of predefined keywords * add czech translation of some
%                        predefined keywords
%
%   - December 23 2002 - revision 2.40
%                      * add some French keyword missing
%                      * add function* and procedure* environment like algorithme* environment: print in one column
%                        even if twocolumn option is specified for the document.
%                      * add a new macro \SetKwComment to define macro which writes comments in the text. First
%                        argument is the name of the macro, second is the text put before the comment, third is the
%                        text put at the end of the comment.Default are \tcc and \tcp
%                      * add new options to change the way algo are numbered:
%                        [algopart] algo are numbered within part (counter must exist)
%                        [algochapter] algo are numbered within chapter
%                        [algosection] algo are numbered within section
%
%   - March 27 2002   - revision 2.39
%                      * Gilles Geeraerts: added the \SetKwIfElseIf to manage
%                        if (c)
%                             i;
%                        else if (c)
%                             i;
%                        ...
%                        else
%                             i;
%                        end
%                      * Also added \gIf \gElseIf \gElse.
%
%   - January 02 2001 - revision 2.38
%                      * bugs related to the caption in procedure and function
%                        environment are corrected.
%                      * bug related to option noend (extra vertical space added
%                        after block command as If or For) is corrected.
%                      * czech option language added (thanks to Libor Bus: l.bus@sh.cvut.cz).
%  
%   - October 16 2000 - revision 2.37
%                      * option algo2e added: change the name of environment
%                        algorithm into algorithm2e. So allow to use the package
%                        with some journal style which already define an algorithm
%                        environment.
%  
%   - September 13 2000 - revision 2.36
%                      * option slide added: require package color
%                      * Hack for slide class in order to have correct
%                        margins
%  
%   - November 25 1999 - revision 2.35
%                      * revision number match RCS number
%                      * Thanks to David A. Bader, a new option is added:
%                        noend: no end keywords are printed.
%  
%   - November 19 1999 - revision 2.32
%                      * minor bug on longend option corrected.
%  
%   - August 26 1999 - revision 2.31
%                      * add an option: figure
%                        this option makes algorithms be figure and so are numbered
%                        as figures, have Figure as caption and are put in 
%                        the \listoffigures
%  
%   - January 21 1999 - revision 2.3 beta
%                    add 2 new environments: procedure and function.
%                    These environments works like algorithm environment but:
%                    - the ruled (or algoruled) style is imperative.
%                    - the caption now writes Procedure name....
%                    - the syntax of the \caption command is restricted as
%                      follow: you MUST put a name followed by 2 braces like
%                      this ``()''. You can put arguments inside the braces and
%                      text after. If no argument is given, the braces will be
%                      removed in the title. 
%                    - label now puts the name (the text before the braces in the
%                      caption) of the procedure or function as reference (not
%                      the number like a classic algorithm environment).
%                    There are also two new styles: ProcNameSty and
%                    ProcArgSty. These style are by default the same as FuncSty
%                    and ArgSty but are used in the caption of a procedure or a
%                    function.
%                    
%   - November 28 1996 - revision 2.22
%                    add a new macro \SetKwInParam{arg1}{arg2}{arg3}:
%                    it defines a macro \arg1{name}{arg} which prints name in keyword
%                    style followed byt arg surrounded by arg2 and arg3. The main
%                    application is to a function working as \SetKwInput to be used
%                    in the head of the algorithm. For example
%                    \SetKwInParam{Func}{(}{)} allows
%                    \Func{functionname}{list of arguments} which prints:
%                    \KwSty{functioname(}list of arguments\KwSty{)}
%       
%
%   - November 27 1996 - revision 2.21:
%                    minor bug in length of InOut boxes fixed.
%                    add algorithm* environment.
%
%   - July 12 1996 - revision 2.2: \SetArg and \SetKwArg macros removed.
%                        
%                    \SetArg has been removed since it never has been
%                    documented.
%                    \SetKwArg has been removed since \SetKw can now
%                    take an argument in order to be consistent with
%                    \SetKwData and \SetKwFunction macros.
%
%   - July 04 1996 - revision 2.1: still more LaTeX2e! Minor compatibility break
%
%                    Macros use now \newcommand instead of \def, use of \setlength, 
%                    \newsavebox, ... and other LaTeX2e specific stuff.
%                    The compatibility break:
%                    - \SetData becomes \SetKwData to be more consistent. So the old 
%                      \SetKwData becomes \SetKwInput
%                    - old macros \titleofalgo, \Freetitleofalgo and \freetitleofalgo
%                      from LaTeX209 version which did print a warning message and call 
%                      \Titleofalgo in version 2.0 are now removed!
%
%   - March 13 1996 - revision 2.0: first official major revision.
%   
%
%%%%%%%%%%%%%%
%
%   Known bugs: 
%   -----------
%   - horizontal spacing (indent) doesn't work with revtex4 class.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% for more complete informations you can see algorithm2e.tex
%
%
%%%%%%%%%%%%%%%%%%%%%%%% Identification Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\NeedsTeXFormat{LaTeX2e}[1994/12/01]
%
\ProvidesPackage{algorithm2e}[2013/01/06 v5.00 algorithms environments]
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%% Initial Code %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\@makeother\*% some package redefined it as a letter (as color.sty)
\def\@firstword#1 #2\@nil{#1}% an useful fonction
%%%%%%% Utilities:
% \ifArgumentEmpty<c><t><e> ; if c is empty, i.e. {}, then t, else e.
%    Function used internally, but may as well expose it to the user; it's useful
\begingroup
\catcode`\Q=3
\catcode`\T=3
\long\gdef\ALGOCF@argemptyaux#1#2Q#3#4#5T{#4}
\long\gdef\ifArgumentEmpty#1{%
  \begingroup\long\edef\@tempa{\endgroup
    \ALGOCF@argemptyaux#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T%
  }\@tempa
}
\endgroup
% \long\def\ifArgumentEmpty#1{\bgroup
% 	\catcode`\Q=3
% 	\catcode`\T=3
% 	\long\def\@tempa##1##2Q##3##4##5T{##4}%
% 	\xdef\@tempa{\@tempa#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T}%
% \egroup\@tempa}
%%%%%%%%%%%
%
% \algocf@longdef -> shorthand to reduce
%    \expandafter\long\expandafter\def
% to
%    \expandafter\algocf@longdef
% may look insignificant, but reads that much better ;)
\def\algocf@longdef{\long\def}
%
% \algocf@newcommand (and helper \algocf@new@command) behaves like LaTeX's newcommand,
% with two differences:
%  - the argument is not "\<name>", but rather "<name>"; i.e. one level of indirection
%  - if the command exists already, then \renewcommand, rather than \newcommand
\def\algocf@newcommand#1{\expandafter\algocf@new@command\csname#1\endcsname}
\def\algocf@new@command#1{%
	\begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
	\expandafter\@ifundefined\@gtempa\newcommand\renewcommand#1}%
%
% \algocf@newcmdside<name><arity><body>
%   The largest time-saver; many commands we define have the pattern:
%     \<name>(<side_text>)<argX><argY>...
%   where "(<side_text>)" is optional. By defining them with this function,
%   the arguments are parsed and renumbered, i.e. the body works as if the
%   command was:
%     \<name><side_text><argX><argY>...
%   and can use \ifArgumentEmpty to see whether its #1 exists (default case
%   for the side text is (), so there's no difference between calling
%     \foo{bar}
%   or
%     \foo(){bar}
%   Technically this is new behaviour, but it shouldn't really occur...
\algocf@longdef\algocf@newcmdside#1#2#3{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3}%
}
%
% a serie of newcmdside macro for block that allows a comment after the end
%     \<name>(<side_text>)<argX><argY>...(<side_text>)% 
%
% 1. kind of begin-end : for command with only one block as begin-end 
\algocf@longdef\algocf@newcmdside@kobe#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2{\csname algocf@#1checkcomfol\endcsname{##1}{##2}}%
  % now check for last side comment; args are : <first side com (could be empty)>, <body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}}{\csname algocf@#1noendcom\endcsname{##1}{##2}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2(##3){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2{%
    \csname algocf@#1main\endcsname{##1}{##2}{}}%
  \algocf@newcommand{algocf@#1main}[3]{#2}%
}%
%
% 2. kind of if-else : for command with two blocks as if-then-else 
\algocf@longdef\algocf@newcmdside@koif#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2##3{\csname algocf@#1checkcomfol\endcsname{##1}{##2}{##3}}%
  % now check for last side comment; args are : <1st side com>, <1st body of cmd>, <2nd body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2##3{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}{##3}}{\csname algocf@#1noendcom\endcsname{##1}{##2}{##3}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2##3(##4){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{##4}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2##3{%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{}}%
  \algocf@newcommand{algocf@#1main}[4]{#2}%
}%
%
% \algocf@newcmdsides<name><arity><body><tail><closing>
%   Like the command above, but with an optional side text at the end
%   of the command as well, i.e.:
%     \<name>(<side_text>)<argX><argY>(<end_text>)
%   It may be a bit confusing that <arity> doesn't count <end_text>,
%   but since it is for internal use, the naming can be a little more
%   fuzzy. This function behaves as if:
%     <body'> = <body><if end_text: tail{end_text}><closing>
\algocf@longdef\algocf@newcmdsides#1#2#3#4#5{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3\@ifnextchar({\csname algocf@#1end\endcsname}{#4#5}}%
	\expandafter\algocf@longdef\csname algocf@#1end\endcsname(##1){#4{##1}\strut\par}%
}%
%
% definition of commands which can be redefined in options of the package.
%
\newcounter{AlgoLine}%
\setcounter{AlgoLine}{0}%
%
\newcommand{\algocf@algocfref}{\relax}%
\newcommand{\listalgorithmcfname}{}%
\newcommand{\algorithmcfname}{}%
\@ifundefined{algorithmautorefname}{\newcommand{\algorithmautorefname}{algorithm}}{\renewcommand{\algorithmautorefname}{algorithm}}%
\newcommand{\algorithmcflinename}{}%
\newcommand{\algocf@typo}{}%
\newcommand{\@algocf@procname}{}\newcommand{\procedureautorefname}{}%
\newcommand{\SetAlgoProcName}[2]{\renewcommand{\@algocf@procname}{#1}\renewcommand{\procedureautorefname}{#2}}%
\newcommand{\@algocf@funcname}{}\newcommand{\functionautorefname}{}%
\newcommand{\SetAlgoFuncName}[2]{\renewcommand{\@algocf@funcname}{#1}\renewcommand{\functionautorefname}{#2}}%
\newcommand{\@algocf@titleofalgoname}{\algorithmcfname}%
\newcommand{\@algocf@algotitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algorithmcfname}}%
\newcommand{\@algocf@proctitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algocf@procname}}%
%
\newcommand{\algocf@style}{plain}%
\newcommand{\@ResetCounterIfNeeded}{}%
\newcommand{\@titleprefix}{}%
%
\newcommand{\algocf@numbering}[1]{\newcommand{\algocf@within}{#1}}%
%
\newcommand{\defaultsmacros@algo}{\algocf@defaults@shortend}%
%
\newcommand{\algocf@list}{loa}%
\newcommand{\algocf@float}{algocf}%
%
\newcommand{\algocf@envname}{algorithm}%
\newcommand{\algocf@listofalgorithms}{listofalgorithms}%
%
%
%% redefine chapter so that it adds a vspace in the loa as the original does for lof and lot
% \let\algocf@original@chapter=\chapter%
% \def\chapter{\expandafter\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}%
%
% bug correction with hyperref submitted by Hubert Meier
\begingroup\expandafter\expandafter\expandafter\endgroup 
\expandafter\ifx\csname @chapter\endcsname\relax\else 
% \let\algocf@original@chapter=\chapter% 
% \def\chapter{\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}% 
\let\algocf@original@chapter=\@chapter%
\@ifclassloaded{krantz}{%
\def\@chapter[#1][#2]#3{\algocf@original@chapter[#1][#2]{#3}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}{%
\def\@chapter[#1]#2{\algocf@original@chapter[#1]{#2}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}%
\fi
%
%% if@restonecol is defined in article and book but some other classes don't define it and we need it, so we do
\ifx\if@restonecol\relax\else\newif\if@restonecol\fi%
%
%
%%%%%%%%%%%%%%%%%%%%%% Declaration of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\RequirePackage{ifthen}%
%
\newboolean{algocf@displayblockmarkers}\setboolean{algocf@displayblockmarkers}{false}%
\DeclareOption{displayblockmarkers}{%
  \setboolean{algocf@displayblockmarkers}{true}%
}
\newboolean{algocf@displaygroupmarkers}{\setboolean{algocf@displaygroupmarkers}{false}
\DeclareOption{displaygroupmarkers}{%
  \setboolean{algocf@displaygroupmarkers}{true}%
}
%
\newboolean{algocf@nokwfunc}\setboolean{algocf@nokwfunc}{false}%
\DeclareOption{nokwfunc}{%
  \setboolean{algocf@nokwfunc}{true}%
}%
%
\newboolean{algocf@oldcommands}\setboolean{algocf@oldcommands}{false}%
\DeclareOption{oldcommands}{%
  \setboolean{algocf@oldcommands}{true}%
}%
%
\newboolean{algocf@leftlinenumber}\setboolean{algocf@leftlinenumber}{true}%
\newcommand{\setLeftLinesNumbers}{\setboolean{algocf@leftlinenumber}{true}}%
\newcommand{\setRightLinesNumbers}{\setboolean{algocf@leftlinenumber}{false}}%
\DeclareOption{rightnl}{%
  \setRightLinesNumbers%
}%
%
\newboolean{algocf@endfloat}\setboolean{algocf@endfloat}{false}%
\DeclareOption{endfloat}{%
  \setboolean{algocf@endfloat}{true}%
  \newcounter{postalgo}\setcounter{postalgo}{0}%
}%
%
\newboolean{algocf@procnumbered}\setboolean{algocf@procnumbered}{false}%
\DeclareOption{procnumbered}{%
  \setboolean{algocf@procnumbered}{true}%
}%
%
\DeclareOption{algo2e}{%
  \renewcommand{\algocf@envname}{algorithm2e}%
  \renewcommand{\algocf@listofalgorithms}{listofalgorithmes}%
}%
%
\newboolean{algocf@slide}\setboolean{algocf@slide}{false}%
\DeclareOption{slide}{%
  \setboolean{algocf@slide}{true}%
}%
%
\newboolean{algocf@figurecaption}\setboolean{algocf@figurecaption}{false}%
\DeclareOption{figure}{%
\renewcommand{\algocf@list}{lof}%
\renewcommand{\algocf@float}{figure}%
\AtBeginDocument{\@ifpackageloaded{caption}{\setboolean{algocf@figurecaption}{true}}{}}%
}%
%
\newboolean{algocf@optonelanguage}\setboolean{algocf@optonelanguage}{false}%
\DeclareOption{onelanguage}{\setboolean{algocf@optonelanguage}{true}}%
%
\newcommand{\algocf@languagechoosen}{english}%
\newboolean{algocf@localkw@english}\setboolean{algocf@localkw@english}{true}%
\DeclareOption{englishkw}{%
\setboolean{algocf@localkw@english}{true}%
}%
%
\DeclareOption{english}{%
\renewcommand{\listalgorithmcfname}{List of Algorithms}%
\renewcommand{\algorithmcfname}{Algorithm}%
\renewcommand{\algorithmautorefname}{algorithm}%
\renewcommand{\algorithmcflinename}{line}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedure}%
\renewcommand{\@algocf@funcname}{Function}%
\renewcommand{\procedureautorefname}{procedure}%
\renewcommand{\functionautorefname}{function}%
\renewcommand{\algocf@languagechoosen}{english}%
}%
%
%----
\newboolean{algocf@localkw@french}\setboolean{algocf@localkw@french}{false}%
\DeclareOption{frenchkw}{%
\setboolean{algocf@localkw@french}{true}%
}%
%
\DeclareOption{french}{%
\renewcommand{\listalgorithmcfname}{Liste des Algorithmes}%
\renewcommand{\algorithmcfname}{Algorithme}%
\renewcommand{\algorithmautorefname}{algorithme}%
\renewcommand{\algorithmcflinename}{ligne}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Proc\'edure}%
\renewcommand{\@algocf@funcname}{Fonction}%
\renewcommand{\procedureautorefname}{proc\'edure}%
\renewcommand{\functionautorefname}{fonction}%
\renewcommand{\algocf@languagechoosen}{french}%
}%
%
%----
\newboolean{algocf@localkw@czech}\setboolean{algocf@localkw@czech}{false}%
\DeclareOption{czechkw}{%
\setboolean{algocf@localkw@czech}{true}%
}%
%
\DeclareOption{czech}{%
\renewcommand{\listalgorithmcfname}{Seznam algoritm\r{u}}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkce}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{czech}%
}%
%
%----
\newboolean{algocf@localkw@german}\setboolean{algocf@localkw@german}{false}%
\DeclareOption{germankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{german}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\DeclareOption{ngermankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{ngerman}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\newboolean{algocf@localkw@portuguese}\setboolean{algocf@localkw@portuguese}{false}%
\DeclareOption{portuguesekw}{%
\setboolean{algocf@localkw@portuguese}{true}%
}%
%
\DeclareOption{portuguese}{%
\renewcommand{\listalgorithmcfname}{Lista de Algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{linha}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimento}%
\renewcommand{\@algocf@funcname}{Fun\c{c}\~{a}o}%
\renewcommand{\procedureautorefname}{procedimento}%
\renewcommand{\functionautorefname}{fun\c{c}\~{a}o}%
\renewcommand{\algocf@languagechoosen}{portuguese}%
}%
%
%----
\newboolean{algocf@localkw@italiano}\setboolean{algocf@localkw@italiano}{false}%
\DeclareOption{italianokw}{%
\setboolean{algocf@localkw@italiano}{true}%
}%
%
\DeclareOption{italiano}{%
\renewcommand{\listalgorithmcfname}{Elenco degli algoritmi}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{riga}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funzione}%
\renewcommand{\procedureautorefname}{procedura}%
\renewcommand{\functionautorefname}{funzione}%
\renewcommand{\algocf@languagechoosen}{italiano}%
}%
%----
\newboolean{algocf@localkw@spanish}\setboolean{algocf@localkw@spanish}{false}%
\DeclareOption{spanishkw}{%
\setboolean{algocf@localkw@spanish}{true}%
}%
%
\DeclareOption{spanish}{%
\renewcommand{\listalgorithmcfname}{\'Indice de algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{l\'inea}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimiento}%
\renewcommand{\@algocf@funcname}{Funci\'on}%
\renewcommand{\procedureautorefname}{procedimiento}%
\renewcommand{\functionautorefname}{funci\'on}%
\renewcommand{\algocf@languagechoosen}{spanish}%
}%
%----
\newboolean{algocf@localkw@slovak}\setboolean{algocf@localkw@slovak}{false}%
\DeclareOption{slovakkw}{%
\setboolean{algocf@localkw@slovak}{true}%
}%
%
\DeclareOption{slovak}{%
\renewcommand{\listalgorithmcfname}{Zoznam algoritmov}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Proced\'{u}ra}%
\renewcommand{\@algocf@funcname}{Funkcia}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{slovak}%
}%
%
%----
\newboolean{algocf@localkw@croatian}\setboolean{algocf@localkw@croatian}{false}%
\DeclareOption{croatiankw}{%
\setboolean{algocf@localkw@croatian}{true}%
}%
%
\DeclareOption{croatian}{%
\renewcommand{\listalgorithmcfname}{Popis algoritama}%
\renewcommand{\algorithmcfname}{Algoritam}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{redak}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkcija}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{croatian}%
}%
%%% adding 'turkish' option customization
%
%----
\newboolean{algocf@localkw@turkish}\setboolean{algocf@localkw@turkish}{false}%
\DeclareOption{turkishkw}{%
\setboolean{algocf@localkw@turkish}{true}%
}%
\DeclareOption{turkish}{%
\renewcommand{\listalgorithmcfname}{Algoritma Listesi}%
\renewcommand{\algorithmcfname}{Algoritma}%
\renewcommand{\algorithmautorefname}{algoritma}%
\renewcommand{\algorithmcflinename}{?izgi}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Prosed?r}%
\renewcommand{\@algocf@funcname}{Fonksiyon}%
\renewcommand{\procedureautorefname}{prosed?r}%
\renewcommand{\functionautorefname}{fonksiyon}%
\renewcommand{\algocf@languagechoosen}{turkish}%
}%
%
% OPTIONs plain, boxed, ruled, algoruled & boxruled
%
\newcommand{\algocf@style@plain}{\renewcommand{\algocf@style}{plain}}%
\newcommand{\algocf@style@boxed}{\renewcommand{\algocf@style}{boxed}}%
\newcommand{\algocf@style@ruled}{\renewcommand{\algocf@style}{ruled}}%
\newcommand{\algocf@style@algoruled}{\renewcommand{\algocf@style}{algoruled}}%
\newcommand{\algocf@style@boxruled}{\renewcommand{\algocf@style}{boxruled}}%
\newcommand{\algocf@style@tworuled}{\renewcommand{\algocf@style}{tworuled}}%
\newcommand{\algocf@style@plainruled}{\renewcommand{\algocf@style}{plainruled}}%
\newcommand{\RestyleAlgo}[1]{\csname algocf@style@#1\endcsname}%
\DeclareOption{plain}{\algocf@style@plain}%
\DeclareOption{plainruled}{\algocf@style@plainruled}%
\DeclareOption{boxed}{\algocf@style@boxed}%
\DeclareOption{ruled}{\algocf@style@ruled}%
\DeclareOption{algoruled}{\algocf@style@algoruled}%
\DeclareOption{boxruled}{\algocf@style@boxruled}%
\DeclareOption{tworuled}{\algocf@style@tworuled}%
%
% OPTIONs algopart,algochapter & algosection
%
\DeclareOption{algopart}{\algocf@numbering{part}}%       %algo part numbered
\DeclareOption{algochapter}{\algocf@numbering{chapter}}% %algo chapter numbered
\DeclareOption{algosection}{\algocf@numbering{section}}% %algo section numbered
%
% OPTIONs resetcount & noresetcount
%
\DeclareOption{resetcount}{\renewcommand{\@ResetCounterIfNeeded}{\setcounter{AlgoLine}{0}}}%
\DeclareOption{noresetcount}{\renewcommand{\@ResetCounterIfNeeded}{}}%
%
% OPTIONs algorithm hanging for long lines
%
\newlength{\algocf@hangindent}\setlength{\algocf@hangindent}{.5em}
\newcommand{\SetAlgoHangIndent}[1]{\setlength{\algocf@hangindent}{#1}}
%
\newboolean{algocf@hanging}\setboolean{algocf@hanging}{true}% hanging is handle by default
\newboolean{algocf@hanginginout}\setboolean{algocf@hanginginout}{false}% inout are managed as previously: hanging set by inout keywords
\newboolean{algocf@hangingcomment}\setboolean{algocf@hangingcomment}{false}% comment that are not side comment are indented accordingly to comment mark, not as normal text
\newcommand{\algocf@everyparnl}{\relax}%
\newcommand{\algocf@everyparhanging}{\hangafter=1\hangindent=\algocf@hangindent\relax}%
\newcommand{\algocf@everypar}{\algocf@everyparnl\algocf@everyparhanging}%
\newcommand{\algocf@seteverypar}{%
  \ifthenelse{\boolean{algocf@hanging}}{\everypar{\algocf@everypar}}{\relax}%
}%
%
\newcommand{\algocf@seteveryparnl}[1]{\renewcommand{\algocf@everyparnl}{#1}\everypar{\algocf@everypar}}%
\newcommand{\algocf@seteveryparhanging}[1]{%
\let\algocf@oldeveryparhanging=\algocf@everyparhanging%
\renewcommand{\algocf@everyparhanging}{#1}\everypar{\algocf@everypar}%
}%
\newcommand{\algocf@reseteveryparhanging}{%
\let\algocf@everyparhanging=\algocf@oldeveryparhanging%
\everypar{\algocf@everypar}%
}%
\DeclareOption{hanginginout}{\setboolean{algocf@hanginginout}{true}}%
\DeclareOption{hangingcomment}{\setboolean{algocf@hangingcomment}{true}}%
\DeclareOption{noalgohanging}{%
  \setboolean{algocf@hanginginout}{false}%
  \setboolean{algocf@hangingcomment}{false}%
  \setboolean{algocf@hanging}{false}%
}%
%\newcommand{
%
%
% OPTION linesnumbered
%
\newboolean{algocf@linesnumbered}\setboolean{algocf@linesnumbered}{false}%
\newcommand{\algocf@linesnumbered}{\relax}%
\DeclareOption{linesnumbered}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}%
}%
%
% OPTION linesnumberedhidden
%
\DeclareOption{linesnumberedhidden}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}%
}%
%
% OPTION commentsnumbered inoutnumbered
%
\newboolean{algocf@commentsnumbered}\setboolean{algocf@commentsnumbered}{false}%
\DeclareOption{commentsnumbered}{\setboolean{algocf@commentsnumbered}{true}}%
\newboolean{algocf@inoutnumbered}\setboolean{algocf@inoutnumbered}{false}%
\DeclareOption{inoutnumbered}{\setboolean{algocf@inoutnumbered}{true}}%
%
% OPTIONs titlenumbered & titlenotnumbered
%
\DeclareOption{titlenumbered}{%
  \renewcommand{\@titleprefix}{%
    \refstepcounter{\algocf@float}%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\ \expandafter\csname the\algocf@float\endcsname\algocf@typo: }%
  }%
}%
%
\DeclareOption{titlenotnumbered}{\renewcommand{\@titleprefix}{%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\algocf@typo: }}%
}%
%
% OPTIONs algonl
% line numbered with the counter of the algorithm
%
\DeclareOption{algonl}{\renewcommand{\theAlgoLine}{\expandafter\csname the\algocf@float\endcsname.\arabic{AlgoLine}}}%
%
% OPTIONs lined, vlined & noline
%
\DeclareOption{lined}{\AtBeginDocument{\SetAlgoLined}}%   \SetAlgoLined (default)
\DeclareOption{vlined}{\AtBeginDocument{\SetAlgoVlined}}% \SetAlgoVlined
\DeclareOption{noline}{\AtBeginDocument{\SetAlgoNoLine}}%\SetAlgoNoLine
%
% OPTIONs longend, shotend & noend
%
\DeclareOption{longend}{\AtBeginDocument{\SetAlgoLongEnd}}%  \SetAlgoLongEnd
\DeclareOption{shortend}{\AtBeginDocument{\SetAlgoShortEnd}}%\SetAlgoShortEnd
\DeclareOption{noend}{\AtBeginDocument{\SetAlgoNoEnd}}%      \SetAlgoNoEnd
%
\DeclareOption{nosemicolon}{\AtBeginDocument{\DontPrintSemicolon}}%      \SetAlgoNoEnd
%
% OPTION dotoc
%
\newboolean{algocf@dotocloa}\setboolean{algocf@dotocloa}{false}%
\DeclareOption{dotocloa}{%
  \setboolean{algocf@dotocloa}{true}%
}
%
% OPTION comments
%
\newboolean{algocf@optfillcomment}\setboolean{algocf@optfillcomment}{true}%
\DeclareOption{nofillcomment}{%
  \setboolean{algocf@optfillcomment}{false}%
}%
\DeclareOption{fillcomment}{%
  \setboolean{algocf@optfillcomment}{true}%
}%
%
% OPTION sidecommments
%
\newboolean{algocf@scleft}\setboolean{algocf@scleft}{false}%
\DeclareOption{scleft}{%
  \setboolean{algocf@scleft}{true}%
}%
\DeclareOption{sright}{% default
  \setboolean{algocf@scleft}{false}%
}%
%
% OPTION norelsize
%
\newboolean{algocf@norelsize}\setboolean{algocf@norelsize}{false}%
\DeclareOption{norelsize}{%
  \setboolean{algocf@norelsize}{true}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%% Execution of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ExecuteOptions{english,plain,resetcount,titlenotnumbered,lined,shortend}%
%
\ProcessOptions%
%
\@algocf@algotitleofalgo% fix name for \TitleOfAlgo to \algorithmcfname by default
%
%%%%%%%%%%%%%%%%%%%%%%%%%% Package Loading %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
\RequirePackage{xspace}%
%
\ifthenelse{\boolean{algocf@endfloat}}{%
  \RequirePackage{endfloat}%
}{\relax}%
%
\ifthenelse{\boolean{algocf@norelsize}}{%
  \newcommand{\relsize}[1]{\scriptsize}%
}{%
  \RequirePackage{relsize}%
}%
%
\ifthenelse{\boolean{algocf@slide}}{\RequirePackage{color}}{}%
%
%
\AtEndOfPackage{%
  \ifthenelse{\boolean{algocf@dotocloa}}{%
    \renewcommand{\listofalgorithms}{\tocfile{\listalgorithmcfname}{loa}}%
  }{\relax}%
}%
%
% if loa in toc required, load tocbibind package if not already done.
\ifthenelse{\boolean{algocf@dotocloa}}{%
  \ifx\@tocextra\undefined%
  \RequirePackage{tocbibind}%
  \fi%
}{\relax}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Main Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\algocf@name}{algorithm2e}%
\newcommand{\algocf@date}{october 19 2015}%
\newcommand{\algocf@version}{Release 5.1}%
\newcommand{\algocf@id}{\algocf@version\space -- \algocf@date\space --}%
\typeout{********************************************************^^JPackage `\algocf@name'\space\algocf@id^^J%
         - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
         - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
         subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
         - Author: Christophe Fiorio (christophe.fiorio@umontpellier.fr)^^J********************************************************}%
%%
%%
%%
%%
%%
%%
%%%% hyperref compatibility tricks: Hyperref package defines H counters from
   % standard counters (i.e \theHpage from \thepage) and check some particular
   % counters of some packages, unfortunately it doesn't do the same for
   % algorithm2e package but act as Hcounter was defined. To avoid errors we
   % defined \theHalgocf ourself
%%%%
%
\@ifundefined{theHalgocf}{\def\theHalgocf{\thealgocf}}{}%
\@ifundefined{theHAlgoLine}{\def\theHAlgoLine{\theAlgoLine}}{}%
\@ifundefined{theHalgocfproc}{\def\theHalgocfproc{0}}{}%
\@ifundefined{theHalgocffunc}{\def\theHalgocffunc{0}}{}%
\@ifundefined{toclevel@algocf}{\def\toclevel@algocf{0}}{}%
%
% autoref from hyperref needs an autorefname, so we give it.
\def\AlgoLineautorefname{\algorithmcflinename}%
\def\algocfautorefname{\algorithmautorefname}%
\def\algocfprocautorefname{\procedureautorefname}%
\def\algocffuncautorefname{\functionautorefname}%
%%
%%
%%
\newcommand{\@defaultskiptotal}{0.5em}%
\newskip\skiptotal\skiptotal=0.5em%
\newskip\skiplinenumber\skiplinenumber=\hsize\advance\skiplinenumber by-\skiptotal%
\newskip\skiprule%
\newskip\skiphlne%
\newskip\skiptext%
\newskip\skiplength%
\newskip\algomargin%
\newskip\skipalgocfslide\skipalgocfslide=1em%
\newdimen\algowidth%
\newdimen\inoutsize%
\newdimen\inoutindent%
\newdimen\interspacetitleruled\setlength{\interspacetitleruled}{2pt}%
\newdimen\interspacealgoruled\setlength{\interspacealgoruled}{2pt}%
\newdimen\interspacetitleboxruled\setlength{\interspacetitleboxruled}{2\lineskip}%
%
\newcommand{\@algoskip}{\smallskip}%
\newcommand{\SetAlgoSkip}[1]{\renewcommand{\@algoskip}{\csname#1\endcsname}}%
\newcommand{\@algoinsideskip}{\relax}%
\newcommand{\SetAlgoInsideSkip}[1]{\renewcommand{\@algoinsideskip}{\csname#1\endcsname}}%
%
% ruledwidth
%
\newlength{\algocf@ruledwidth}\setlength{\algocf@ruledwidth}{\linewidth}%
\newboolean{algocf@customruledwidth}\setboolean{algocf@customruledwidth}{false}%
\newcommand{\SetCustomAlgoRuledWidth}[1]{%
  \setboolean{algocf@customruledwidth}{true}%
  \ifthenelse{\boolean{algocf@customruledwidth}}{\setlength{\algocf@ruledwidth}{#1}}{\relax}%
}%
%
\newsavebox{\algocf@inoutbox}%
\newsavebox{\algocf@inputbox}%
%%
%%
\newcommand{\arg@e}{}%
\newcommand{\arg@space}{\ }%
\newcommand{\BlankLine}{\vskip 1ex}%
%%
\newcommand{\vespace}{1ex}%
\newcommand{\SetInd}[2]{%
\skiprule=#1%
\skiptext=#2%
\skiplength=\skiptext\advance\skiplength by \skiprule\advance\skiplength by 0.4pt}%
\SetInd{0.5em}{1em}
\algomargin=\leftskip\advance\algomargin by \parindent%
\newcommand{\IncMargin}[1]{\advance\algomargin by #1}%
\newcommand{\DecMargin}[1]{\advance\algomargin by -#1}%
\newcommand{\SetNlSkip}[1]{%
  \renewcommand{\@defaultskiptotal}{#1}%
  \setlength{\skiptotal}{#1}}%
%%
\newskip\AlCapSkip\AlCapSkip=0ex%
\newskip\AlCapHSkip\AlCapSkip=0ex%
\newcommand{\SetAlCapSkip}[1]{\setlength{\AlCapSkip}{#1}}%
\newcommand{\SetAlCapHSkip}[1]{\setlength{\AlCapHSkip}{#1}}%
\SetAlCapHSkip{.5\algomargin}%
%%
%%
\newskip\algoskipindent
\newcommand{\algocf@adjustskipindent}{%
  \algoskipindent=\skiprule%
  \advance\algoskipindent by \skiptext\advance\algoskipindent by 0.4pt}
\algocf@adjustskipindent%
%
\newcommand{\Indentp}[1]{\advance\leftskip by #1}%
\newcommand{\Indp}{\algocf@adjustskipindent\advance\leftskip by \algoskipindent}
\newcommand{\Indpp}{\advance\leftskip by 0.5em}%
\newcommand{\Indm}{\algocf@adjustskipindent\advance\leftskip by -\algoskipindent}
\newcommand{\Indmm}{\advance\leftskip by -0.5em}%
%
%%
%%
%% Line Numbering
%%
%%
% number line style
\newcommand{\algocf@nlrelsize}{-2}\newcommand{\SetAlgoNlRelativeSize}[1]{\renewcommand{\algocf@nlrelsize}{#1}}%
\newcommand{\NlSty}[1]{\textnormal{\textbf{\relsize{\algocf@nlrelsize}#1}}}% default definition
\newcommand{\SetNlSty}[3]{\renewcommand{\NlSty}[1]{\textnormal{\csname#1\endcsname{\relsize{\algocf@nlrelsize}#2##1#3}}}}%
%
% nl definitions
%
\newsavebox{\algocf@nlbox}%
\newcommand{\algocf@printnl}[1]{%
  \ifthenelse{\boolean{algocf@leftlinenumber}}{%
    \skiplinenumber=\skiptotal\advance\skiplinenumber by\leftskip%
    \strut\raisebox{0pt}{\llap{\NlSty{#1}\kern\skiplinenumber}}\ignorespaces%
  }{%
    \sbox\algocf@nlbox{\NlSty{#1}}%
    \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip\advance\skiplinenumber by-\skiptext%
    \advance\skiplinenumber by\algomargin\advance\skiplinenumber by.3em\advance\skiplinenumber by-\wd\algocf@nlbox%
    % to handle particular case of until: printnl is after 'until' keyword has been writen, so we need to substract length of this keyword
    \advance\skiplinenumber by-\algocf@skipuntil%
    \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\NlSty{#1\ignorespaces}}}\ignorespaces%
  }%
}%
\newcommand{\algocf@nl@sethref}[1]{%
  \renewcommand{\theHAlgoLine}{\thealgocfproc.#1}%
  \hyper@refstepcounter{AlgoLine}\gdef\@currentlabel{#1}%
}%
\newcommand{\nl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \algocf@printnl{\theAlgoLine}%
}%
%
\newcommand{\nllabel}[1]{\label{#1}}%
%
\newcommand{\enl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip%
  \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\strut\NlSty{\theAlgoLine}}}\ignorespaces%
}%
%% nlset
\newcommand{\nlset}[1]{%
  \@ifundefined{hyper@refstepcounter}{\protected@edef\@currentlabel{#1}}{\algocf@nl@sethref{#1}}\algocf@printnl{#1}%
}%
%
%% lnl definitions
\newcommand{\lnl}[1]{\nl\label{#1}\ignorespaces}%
%
%% lnlset
\newcommand{\lnlset}[2]{\nlset{#2}\label{#1}}%
%
% set char put at end of each line
%
\newcommand{\algocf@endline}{\string;}
\newcommand{\SetEndCharOfAlgoLine}[1]{\renewcommand{\algocf@endline}{#1}}
%
% end of line definition
%
\newcommand{\@endalgocfline}{\algocf@endline}% default definition: printsemicolon
\newcommand{\DontPrintSemicolon}{\renewcommand{\@endalgocfline}{\relax}}%
\newcommand{\PrintSemicolon}{\renewcommand{\@endalgocfline}{\algocf@endline}}%
\newcommand{\@endalgoln}{\@endalgocfline\hfill\strut\par}%
%
% line numbering
%
\newcommand{\LinesNumbered}{\setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}}%
\newcommand{\LinesNotNumbered}{%
  \setboolean{algocf@linesnumbered}{false}%
  \renewcommand{\algocf@linesnumbered}{\relax}%
}%
%
\newcommand{\LinesNumberedHidden}{%
  \setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}}%
\newcommand{\ShowLn}{\nlset{\theAlgoLine}\ignorespaces}% display the line number on this line (without labelling)
\newcommand{\ShowLnLabel}[1]{\lnlset{#1}{\theAlgoLine}\ignorespaces}% display the line number and label this line
%
%%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Styling text commands
%
\newcommand{\AlFnt}{\relax}% default definition
\newcommand{\SetAlFnt}[1]{\renewcommand{\AlFnt}{#1}}%
\newcommand{\AlTitleFnt}{\relax}% default definition
\newcommand{\SetAlTitleFnt}[1]{\renewcommand{\AlTitleFnt}{#1}}%
%
\newcommand{\AlCapFnt}{\relax}% default definition
\newcommand{\SetAlCapFnt}[1]{\renewcommand{\AlCapFnt}{#1}}%
\newcommand{\AlCapNameFnt}{\relax}% default definition
\newcommand{\SetAlCapNameFnt}[1]{\renewcommand{\AlCapNameFnt}{#1}}%
%
\newcommand{\ProcFnt}{\relax}% default definition
\newcommand{\SetProcFnt}[1]{\renewcommand{\ProcFnt}{#1}}%
\newcommand{\ProcNameFnt}{\relax}% default definition
\newcommand{\SetProcNameFnt}[1]{\renewcommand{\ProcNameFnt}{#1}}%
\newcommand{\ProcArgFnt}{\relax}% default definition
\newcommand{\SetProcArgFnt}[1]{\renewcommand{\ProcArgFnt}{#1}}%
%
\newcommand{\AlTitleSty}[1]{\textbf{#1}\unskip}% default definition
\newcommand{\SetAlTitleSty}[1]{\renewcommand{\AlTitleSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetAlCapSty}[1]{\renewcommand{\AlCapSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapNameSty}[1]{\textnormal{#1}\unskip}% default definition
\newcommand{\SetAlCapNameSty}[1]{\renewcommand{\AlCapNameSty}[1]{\textnormal{\csname #1\endcsname{##1}}\unskip}}%
%
\newcommand{\ProcSty}[1]{\AlCapSty{#1}}%
\newcommand{\SetProcSty}[1]{\renewcommand{\ProcSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcNameSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcNameSty}[1]{\renewcommand{\ProcNameSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcArgSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcArgSty}[1]{\renewcommand{\ProcArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
\newcommand{\KwSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetKwSty}[1]{\renewcommand{\KwSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetArgSty{emph}
\newcommand{\SetArgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetFuncArgSty{emph}
\newcommand{\SetFuncArgSty}[1]{\renewcommand{\FuncArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncSty}[1]{\textnormal{\texttt{#1}}\unskip}%\SetFuncSty{texttt}
\newcommand{\SetFuncSty}[1]{\renewcommand{\FuncSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetProgSty{emphg}
\newcommand{\SetProgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\DataSty}[1]{\textnormal{\textsf{#1}}\unskip}%%\SetDataSty{textsf}
\newcommand{\SetDataSty}[1]{\renewcommand{\DataSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\CommentSty}[1]{\textnormal{\texttt{#1}}\unskip}%%\SetDataSty{texttt}
\newcommand{\SetCommentSty}[1]{\renewcommand{\CommentSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\TitleSty}[1]{#1\unskip}%\SetTitleSty{}{}
\newcommand{\SetTitleSty}[2]{\renewcommand{\TitleSty}[1]{%
\csname#1\endcsname{\csname#2\endcsname##1}}\unskip}%
\newcommand{\BlockMarkersSty}[1]{\KwSty{#1}}%
\newcommand{\SetBlockMarkersSty}[1]{\renewcommand{\BlockMarkersSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Block basic commands
%
\newcommand{\algocf@push}[1]{\advance\skiptotal by #1\moveright #1}%
\newcommand{\algocf@pop}[1]{\advance\skiptotal by -#1}%
\newcommand{\algocf@addskiptotal}{\advance\skiptotal by 0.4pt\advance\hsize by -0.4pt\advance\hsize by -\skiplength}% 0.4 pt=width of \vrule
\newcommand{\algocf@subskiptotal}{\advance\skiptotal by -0.4pt\advance\hsize by 0.4pt\advance\hsize by \skiplength}% 0.4 pt=width of \vrule
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% group of instructions definition
%
\skiphlne=.8ex%
\newcommand{\SetVlineSkip}[1]{\skiphlne=#1}%
\newcommand{\algocf@bblock}{\BlockMarkersSty{begin}}%
\newcommand{\algocf@eblock}{\BlockMarkersSty{end}}%
\newcommand{\AlgoDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{true}}%
\newcommand{\AlgoDontDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{false}}%
\newcommand{\AlgoDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{true}}%
\newcommand{\AlgoDontDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{false}}%
\newcommand{\algocf@bblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@bblock\par}{\relax}%
}%
\newcommand{\algocf@eblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@eblock\par}{\relax}%
}%
\newcommand{\algocf@bgroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@bblock}{\relax}%
}%
\newcommand{\algocf@egroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@eblock}{\relax}%
}%
\newcommand{\SetAlgoBlockMarkers}[2]{%
  \ifArgumentEmpty{#1}{%
    \renewcommand{\algocf@bblock}{\relax}%
  }{%
    \renewcommand{\algocf@bblock}{\BlockMarkersSty{#1}}%
  }% begin marker set
  \ifArgumentEmpty{#2}{%
    \renewcommand{\algocf@eblock}{\relax}%
  }{%
    \renewcommand{\algocf@eblock}{\BlockMarkersSty{#2}}%
  }% end marker set
}
%
%%%%%%%%% block with a vertical line end by a little horizontal line
\newcommand{\algocf@Vline}[1]{%     no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}\Hlne}}\vskip\skiphlne% inside the block
  \algocf@pop{\skiprule}%\algocf@subskiptotal% restore indentation
  \nointerlineskip}% no vskip after
%
%%%%%%%%% block with a vertical line
\newcommand{\algocf@Vsline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%               the vertical rule
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}% restore indentation
  \algocf@eblockcode%
}
%
\newcommand{\algocf@Hlne}{\hrule height 0.4pt depth 0pt width .5em}%
%
%%%%%%%%%  block without line
\newcommand{\algocf@Noline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%
  \hbox{%
    \vtop{\algocf@push{\skiptext}%
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}%
  \algocf@eblockcode%
  % \nointerlineskip% no vskip after
}%
%%%%%%%%%
%
%% default=NoLine
%
\newcommand{\algocf@group}[1]{\algocf@Noline{#1}}% group: set of instruction depending from another (ex: then part of the If)
\newcommand{\algocf@@@eblock}[2]{#1\ifArgumentEmpty{#2}{\relax}{\KwSty{\@algocf@endoption{#2}}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@@block}[3]{#1\ifArgumentEmpty{#2}{\ifArgumentEmpty{#3}{\relax}{ #3\relax}}{\KwSty{\@algocf@endoption{#2}}\ifArgumentEmpty{#3}{\relax}{ #3}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@block}[3]{\algocf@@@block{#1}{#2}{#3}}% block: group with a end keyword.
\newcommand{\algocf@block}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
%\newcommand{\algocf@nblock}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
\newcommand{\algocf@setBlock}{%
  \ifthenelse{\boolean{algocf@optnoend}}{%     if no end option
    \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%     block will be a group
  }{%                                          else
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}% block stays a block
  }%
}%
%
\newcommand{\Hlne}{}% little hrizontal line ending a block in vline mode
%
\newcommand{\@algocf@endoption}[1]{#1}%
\newboolean{algocf@optnoend}\setboolean{algocf@optnoend}{false}%
%
\newcommand{\SetAlgoLongEnd}{%%%%%%%%%%%%%%%%%%%%%%%%% Long End
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{##1}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoShortEnd}{%%%%%%%%%%%%%%%%%%%%%%%% ShortEnd
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{\@firstword##1 \@nil}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoEnd}{%%%%%%%%%%%%%%%%%%%%%%%%%%% NoEnd
  \setboolean{algocf@optnoend}{true}%
  \renewcommand{\@algocf@endoption}[1]{}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoLine}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\algocf@Noline{##1}}{##2}}%
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetAlgoVlined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Vline
\renewcommand{\algocf@@block}[2]{\algocf@Vline{##1}}%
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{\algocf@Hlne}}%
%
\newcommand{\SetAlgoLined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Line
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\strut\algocf@Vsline{##1}}{##2}}% no skip after a block so garantie at least one line
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetNothing}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@Noline{##1}\par}%
%\long
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
%%
%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ``Input:'''s like command 
%
%%%
% text staying at the right of the longer keyword of KwInOut commands 
% (text of KwInOut commands are all vertically aligned)
%
\newcommand{\algocf@newinout}{\par\parindent=\inoutindent}% to put right indentation after a \\ in the KwInOut
\newcommand{\SetKwInOut}[2]{%
  \sbox\algocf@inoutbox{\KwSty{#2\algocf@typo:}}%
  \expandafter\ifx\csname InOutSizeDefined\endcsname\relax% if first time used
    \newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
  \else% else keep the larger dimension
    \ifdim\wd\algocf@inoutbox>\inoutsize%
    \setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
    \fi%
  \fi% the dimension of the box is now defined.
  \algocf@newcommand{#1}[1]{%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
%     {\let\\\algocf@newinout\hangindent=\wd\algocf@inoutbox\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo\hfill:}~##1\par}%
    {\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
%
%% allow to ajust the skip size of InOut
%%
\newcommand{\ResetInOut}[1]{%
  \sbox\algocf@inoutbox{\hbox{\KwSty{#1\algocf@typo:}\ }}%
  \setlength{\inoutsize}{\wd\algocf@inoutbox}%
  }%
%
% 
%%%
% text staying at the right of the keyword.
%
\newcommand{\algocf@newinput}{\par\parindent=\wd\algocf@inputbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwInput}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@inputbox{\hbox{\KwSty{#2\algocf@typo:} }}%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
    {\let\\\algocf@newinput\hangindent=\wd\algocf@inputbox\hangafter=1\unhbox\algocf@inputbox##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
\newcommand{\SetKwData}[2]{%
  \algocf@newcommand{@#1}[1]{\DataSty{#2(}\ArgSty{##1}\DataSty{)}}%
  \algocf@newcommand{#1}{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
  }%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tallent:
%
% Add following macros:
%   \SetKwHangingKw:  [kw] ------------   <= hanging determined by [kw]
%                          ------------
% Should act like a combination of \SetKwInput and \SetKw.
% Based on \SetKwInput:
%   - remove ':' at end of keyword
%   - do not reset numbering
%   - use separate savebox
\newsavebox{\algocf@hangingbox}
\newcommand{\algocf@newhanging}{\par\parindent=\wd\algocf@hangingbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwHangingKw}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@hangingbox{\hbox{\KwSty{#2}\algocf@typo\ }}%
    {\let\\\algocf@newhanging\hangindent=\wd\algocf@hangingbox\hangafter=1\unhbox\algocf@hangingbox##1\;}%
  }%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Comments macros
%
%%%%
% comment in the text, first argument is the name of the macro, second is
% the text put before the comment, third is the text put at the end of the
% comment.
%
% first side comment justification
\newcommand{\SetSideCommentLeft}{\setboolean{algocf@scleft}{true}}%
\newcommand{\SetSideCommentRight}{\setboolean{algocf@scleft}{false}}%
\newcommand{\SetNoFillComment}{\setboolean{algocf@optfillcomment}{false}}%
\newcommand{\SetFillComment}{\setboolean{algocf@optfillcomment}{true}}%
%
% next comment and side comment
%
\newcommand{\algocf@endmarkcomment}{\relax}%
\newcommand{\algocf@fillcomment}{%
  \ifthenelse{\boolean{algocf@optfillcomment}}{\hfill}{\relax}}%
%
\newcommand{\algocf@startcomment}{%
  \hangindent=\wd\algocf@inputbox\hangafter=1\usebox\algocf@inputbox}%
\newcommand{\algocf@endcomment}{\algocf@fillcomment\algocf@endmarkcomment\ignorespaces\par}%
\newcommand{\algocf@endstartcomment}{\algocf@endcomment\algocf@startcomment\ignorespaces}%
%
\newboolean{algocf@sidecomment}%
\newboolean{algocf@altsidecomment}\setboolean{algocf@altsidecomment}{false}%
\newcommand{\algocf@scpar}{\ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\par}}%
\newcommand{\algocf@sclfill}{\ifthenelse{\boolean{algocf@scleft}}{\algocf@fillcomment}{\relax}}%
\newcommand{\algocf@scrfill}{\ifthenelse{\boolean{algocf@scleft}}{\relax}{\hfill}}%
\newcommand{\algocf@startsidecomment}{\usebox\algocf@inputbox}%
\newcommand{\algocf@endsidecomment}{\algocf@endmarkcomment\algocf@scpar}%
\newcommand{\algocf@endstartsidecomment}{%
  \algocf@sclfill\algocf@endsidecomment%
  \algocf@scrfill\algocf@startsidecomment\ignorespaces}%
%
\newcommand{\SetKwComment}[3]{%
  \algocf@newcommand{#1}{\@ifstar{\csname algocf@#1@star\endcsname}{\csname algocf@#1\endcsname}}%
	\algocf@newcommand{algocf@#1}[1]{%
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@seteveryparhanging{\relax}}%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {\renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartcomment%
        \algocf@startcomment\CommentSty{%
          \strut\ignorespaces##1\strut\algocf@fillcomment#3}\par}%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@reseteveryparhanging}%
    }%
  %%% side comment definitions
	\algocf@newcommand{algocf@#1@star}[2][]{%
      \ifArgumentEmpty{##1}\relax{% TODO: Is this even necessary, with all those \ifx's?
        \ifthenelse{\boolean{algocf@scleft}}{\setboolean{algocf@sidecomment}{true}}{\setboolean{algocf@sidecomment}{false}}%
        \ifx##1h\setboolean{algocf@altsidecomment}{true}\SetSideCommentLeft\fi%
        \ifx##1f\setboolean{algocf@altsidecomment}{true}\SetSideCommentRight\fi%
        \ifx##1l\setboolean{algocf@altsidecomment}{false}\SetSideCommentLeft\fi%
        \ifx##1r\setboolean{algocf@altsidecomment}{false}\SetSideCommentRight\fi%
      }%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {%
        \renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartsidecomment%
        % here is the comment
        \ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\@endalgocfline\ }%
        \algocf@scrfill\algocf@startsidecomment\CommentSty{%
          \strut\ignorespaces##2\strut\algocf@sclfill#3}\algocf@scpar%
      }%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifArgumentEmpty{##1}\relax{%
        \ifthenelse{\boolean{algocf@sidecomment}}{\setboolean{algocf@scleft}{true}}{\setboolean{algocf@scleft}{false}}%
        \setboolean{algocf@altsidecomment}{false}%
      }%
	}%
  }%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwProg
%
\newcommand{\SetKwProg}[4]{%\SetKwProg{Env}{Title}{is}{end} 
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\ifArgumentEmpty{#2}\relax{\ }\ProgSty{##2}\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode\@endalgocfline\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Kw
%
\newcommand{\SetKw}[2]{%
	\algocf@newcommand{@#1}[1]{\KwSty{#2} \ArgSty{##1}}
	\algocf@newcommand{#1}{\@ifnextchar\bgroup{\csname @#1\endcsname}{\KwSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwFunction
%
\newcommand{\SetKwFunction}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\FuncSty{#2(}\FuncArgSty{##1}\FuncSty{)}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\FuncSty{#2}\xspace}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwTab
%
\newcommand{\SetKwArray}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\DataSty{#2[}\ArgSty{##1}\DataSty{]}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwBlock
%
\newcommand{\SetKwBlock}[3]{%
	\algocf@newcmdside@kobe{#1}%
    {\KwSty{#2}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#3}{##3}\par}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% condition typo
%
\newcommand{\algocf@scond}{\ }
\newcommand{\algocf@econd}{\ }
\newcommand{\algocf@ucond}{}
\newcommand{\SetStartEndCondition}[3]{%
  \renewcommand{\algocf@scond}{#1}\renewcommand{\algocf@econd}{#2}\renewcommand{\algocf@ucond}{#3}}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For Switch
%
\newcommand{\SetKwSwitch}[9]{% #1=\Switch #2=\Case #3=\Other #4=switch #5=do #6=case #7=otherwise #8=endcase #9=endsw
%	\algocf@newcmdside{#1}{3}%
	\algocf@newcmdside@koif{#1}%
		{\KwSty{#4}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#9} {##4\relax}}%
%%%% Case
	\algocf@newcmdside@koif{#2}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#8}{##4\relax}}%
    %uCase
	\algocf@newcmdside{u#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##3}}%
    %lcase
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\ \relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
%%%% Other 
	\algocf@newcmdside@kobe{#3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#8}{##3\relax}}%
    %lOther
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\algocf@egroupcode}%
    %uOther
	\algocf@newcmdside{u#3}{3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##2}}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% If macros
%
\newcommand{\SetKwIF}[8]{% #1=\If #2=\ElseIf #3=\Else #4=if #5=then #6=elseif #7=else #8=endif
% 
% common text
	\algocf@newcommand{#1@ifthen}[1]{\KwSty{#4}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#1@endif} [2]{\algocf@block{##1}{#8}{##2}}%
	\algocf@newcommand{#1@noend} [1]{\algocf@group{##1}}%
	\algocf@newcommand{#1@else}  [1]{\algocf@group{##1}\KwSty{#7}}%
	\algocf@newcommand{#2@elseif}[1]{\KwSty{#6}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#3@else}     {\KwSty{#7}}%
%%%% If then { } endif
	\algocf@newcmdside@koif{#1}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% If then {} else {} endif
    % first command to handle optional side comment of else (so just after first braces)
 	\algocf@newcmdside@kobe{algocf@e#1thenelse}{\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##2}{##3}}%
    % the definition of if-then-else command using command above 
	\algocf@newcmdside{e#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@else\endcsname{##3}\csname algocf@e#1thenelse\endcsname}%
    %%% leif
    \algocf@newcommand{le#1}{\@ifstar{\csname algocf@le#1star\endcsname}{\csname algocf@le#1\endcsname}}%
    \algocf@newcmdside{algocf@le#1}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\@endalgocfline\ \algocf@egroupcode\ifArgumentEmpty{##1}\relax{##1}\strut\par}%
    \algocf@newcmdside{algocf@le#1star}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\algocf@egroupcode}%
%%%% If then 
	% \algocf@newcmdside{l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\
    % ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@noend\endcsname{##3}}%
%%%% ElseIf {} endif
	\algocf@newcmdside@koif{#2}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% ElseIf
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#2}{3}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{##1}\csname #1@noend\endcsname{##3}}%
%%%% Else {} endif
	\algocf@newcmdside@kobe{#3}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ ##1\csname #1@endif\endcsname{##2}{##3\relax}}%
%%%% Else 
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\algocf@egroupcode}%
	\algocf@newcmdside{u#3}{2}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ {##1\relax}\csname #1@noend\endcsname{##2}}%
}% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For macros
%
\newcommand{\SetKwFor}[4]{%
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4\relax}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Repeat macros
%
\newsavebox{\algocf@untilbox}% to handle width of until keyword needed to have good skip
  % for line numbers
\newskip\algocf@skipuntil
\newcommand{\SetKwRepeat}[3]{%
	\algocf@newcmdsides{#1}{3}{%
      \sbox\algocf@untilbox{\KwSty{#3}\algocf@scond}\algocf@skipuntil=\wd\algocf@untilbox%
      \KwSty{#2}\ifArgumentEmpty{##1}\relax{##1}\algocf@group{##3}%
      \KwSty{#3}\algocf@scond% until keyword and start condition typo
      %\advance\skiptotal by\algocf@skipuntil%
      \ArgSty{##2}%
      %\advance\skiptotal by-\algocf@skipuntil%
      \algocf@ucond%
      \algocf@skipuntil=0pt% reset counter
    }{\@endalgocfline}{\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond\@endalgocfline\ifArgumentEmpty{##1}\relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond}%
}%
%
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%        Environments definitions     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%
%% Caption management
%%
% for the following macros:
% #1 is given by caption and is equal to fnum@algocf
% #2 is the text given in argument by the user in the \caption macro
%
%%%%% text of caption
\newcommand{\algocf@captionlayout}[1]{#1}%
\newcommand{\SetAlgoCaptionLayout}[1]{%
  \renewcommand{\algocf@captionlayout}[1]{\csname #1\endcsname{##1}}}%
\newcommand{\algocf@capseparator}{:}%
\newcommand{\SetAlgoCaptionSeparator}[1]{\renewcommand{\algocf@capseparator}{#1}}%
\newcommand{\algocf@captiontext}[2]{%
  \algocf@captionlayout{\AlCapSty{\AlCapFnt #1\algocf@typo\algocf@capseparator}\nobreakspace%
    \AlCapNameSty{\AlCapNameFnt{}#2\endgraf}}}% text of caption
%
%%%%% default caption of algorithm: used if no specific style caption is defined
\newcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
    \hskip .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
    \global\@minipagefalse%
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}%
%
\newsavebox\algocf@capbox%
\newcommand{\algocf@makecaption@plain}[2]{%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}}%
\newcommand{\algocf@makecaption@boxed}[2]{%
  \addtolength{\hsize}{-\algomargin}%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}%
  \addtolength{\hsize}{\algomargin}%
 }%
%
\newcommand{\algocf@makecaption@plainruled}[2]{\algocf@makecaption@plain{#1}{#2}}%
\newcommand{\algocf@makecaption@tworuled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@algoruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@boxruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@ruled}[2]{%
  \global\sbox\algocf@capbox{\hskip\AlCapHSkip% .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}}% then caption is not centered
}%
%
\newlength{\algoheightruledefault}\setlength{\algoheightruledefault}{0.8pt}%
\newlength{\algoheightrule}\setlength{\algoheightrule}{\algoheightruledefault}%
\newlength{\algotitleheightruledefault}\setlength{\algotitleheightruledefault}{0.8pt}%
\newlength{\algotitleheightrule}\setlength{\algotitleheightrule}{\algotitleheightruledefault}%
\newcommand{\algocf@caption@plain}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@plainruled}{\algocf@caption@plain}%
\newcommand{\algocf@caption@boxed}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@ruled}{\box\algocf@capbox\kern\interspacetitleruled\hrule
  width\algocf@ruledwidth height\algotitleheightrule depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@tworuled}{\box\algocf@capbox\hrule  height0pt depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@algoruled}{\algocf@caption@ruled}%
\newcommand{\algocf@caption@boxruled}{%
  \addtolength{\hsize}{-0.8pt}%
  \hbox to\hsize{%
    \vrule%\hskip-0.35pt%
    \vbox{%
      \hrule\vskip\interspacetitleboxruled%
      \hbox to\hsize{\unhbox\algocf@capbox\hfill}\vskip\interspacetitleboxruled%
    }% 
    %\hskip-0.35pt%
    \vrule%
  }\nointerlineskip%
  \addtolength{\hsize}{0.8pt}%
}%
%
%
%%%% set caption for the environment
\newcommand{\algocf@captionref}{%
  \renewcommand{\fnum@algocf}[1]{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\algocf@algocfref}}%
  \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
  \let\old@thealgocf=\thealgocf\renewcommand{\thealgocf}{{\relsize{\algocf@refrelsize}\algocf@algocfref}}%
  \gdef\@currentlabel{\algocf@algocfref}% let the label use the new ref
}%
%
% Unfortunatly, we also need our own caption to set some specific stuff for special references. But after these
% settings, we call the original caption.
%
\long\def\algocf@caption@algo#1[#2]#3{%
  \ifthenelse{\equal{\algocf@algocfref}{\relax}}{}{\algocf@captionref}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\equal{\algocf@algocfref}{\relax}}{\renewcommand{\theHalgocf}{\thealgocf}}{% take algocf as Href
      \renewcommand{\theHalgocf}{\algocf@algocfref}}%else if SetAlgoRefName done, take this name as ref.
    \hyper@refstepcounter{algocf}%set algocf as category of ref
  }%
   \algocf@latexcaption{#1}[{#2}]{{#3}}% call original caption
}%
%
% beamer define is own caption overrinding latex caption!
% as we need it, we have put here the original definition
% to handle manual ref, unfortunately we have to add one line to handle algocf@algocfref
\long\def\algocf@latexcaption#1[#2]#3{% original definition of caption
  \par%
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
  {\protect\numberline{\csname the#1\endcsname}{\ignorespaces #2}}%
  \begingroup%
  \@parboxrestore%
  \if@minipage%
    \@setminipage%
  \fi%
  \normalsize%
  \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par%
  \endgroup%
}%
%
% \ifx\beamer@makecaption\undefined%
% \else% beamer detected
\ifx\@makecaption\undefined%
\newcommand{\@makecaption}[2]{\relax}%
\fi%
%%

%
% more and more packages redefine \@caption instead of just \@makecaption which makes algorithm2e
% caption not works since based on standard \@caption. So we force the definition of \@caption to be
% the standard one (the one from LaTeX) inside algorithm environment.
%
% unfortunately, makecaption is called with \ignorespace #3 so 
% we can't do the @currentlabel definition inside \algocf@captionproctext
\long\def\algocf@caption@proc#1[#2]#3{%
  \ifthenelse{\boolean{algocf@nokwfunc}}{\relax}{%
    \SetKwFunction{\algocf@captname#3@}{\algocf@captname#3@}%
  }%
  % we tell hyperref to use algocfproc as category and to take the appropriate ref.
  \ifthenelse{\boolean{algocf@func}}{\def\@proc@func{algocffunc}}{\def\@proc@func{algocfproc}}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\boolean{algocf@procnumbered}}{% 
      \expandafter\def\csname theH\@proc@func\endcsname{\thealgocf}%if procnumbered, take \thealgocf as ref
    }{%
      \expandafter\def\csname theH\@proc@func\endcsname{\algocf@captname#3@}%else take procedure or function name
    }%
    \hyper@refstepcounter{\@proc@func}%
  }%
  \ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
    \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
    \gdef\@currentlabel{\algocf@captname#3@}% let the label be the name of the function, not the counter
  }%
  \ifthenelse{\equal{\algocf@captparam#2@}{\arg@e}}{% if no paramater, we remove the ()
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace\algocf@captname#2@]{#3}%
  }{%                                                 else we give the complete name
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace#2]{#3}%
  }%
}%
%%
%%% setcaption
\newcommand{\algocf@setcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment, caption text must be changed
    \let\algocf@oldcaptiontext=\algocf@captiontext%
    \renewcommand{\algocf@captiontext}[2]{%
      \algocf@captionproctext{##1}{##2}%
    }%
  }{}%
  \let\algocf@savecaption=\@caption%
  \ifthenelse{\boolean{algocf@procenvironment}}{\let\@caption=\algocf@caption@proc}{\let\@caption=\algocf@caption@algo}%
  \let\algocf@oldmakecaption=\@makecaption%
  \renewcommand{\@makecaption}[2]{%
    \expandafter\csname algocf@makecaption@\algocf@style\endcsname{##1}{##2}%
  }%
}%
%
%%%%% reset caption
%
% since we have force the LaTeX caption for algorithm environment, we must go back to the caption
% used in the text.
\newcommand{\algocf@resetcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment
    \let\thealgocf=\old@thealgocf% restore normal counter printing
    \let\algocf@captiontext=\algocf@oldcaptiontext% restore normal caption text
  }{}%
  \let\@caption=\algocf@savecaption% now restore caption outside algo/proc/func environment
  \let\@makecaption=\algocf@oldmakecaption% and restore makecaption outside outside algo/proc/func environment
  \algocf@resetfnum%
}%
%
%%%%% nocaptionofalgo and restorecaptionofalgo --
\newcommand{\NoCaptionOfAlgo}{%
  \let\@old@algocf@captiontext=\algocf@captiontext%
  \renewcommand{\algocf@captiontext}[2]{\AlCapNameSty{\AlCapNameFnt{}##2}}%
}%
\newcommand{\RestoreCaptionOfAlgo}{%
  \let\algocf@captiontext=\@old@algocf@captiontext%
}%
%
% ----------------------  algocf environment
%
\newcounter{algocfline}%                    % new counter to make lines numbers be internally 
\setcounter{algocfline}{0}%                 % different in different algorithms
\newcounter{algocfproc}% counter to count all algo environment (proc, func), just used by hyperref to avoir "same
\setcounter{algocfproc}{0}% identifier" error caused by algocf being set to '-' for procedure or function or not
  % changed if no caption is given.
%
\expandafter\ifx\csname algocf@within\endcsname\relax% if \algocf@within doesn't exist
\newcounter{algocf}%                        % just define a new counter
\renewcommand{\thealgocf}{\@arabic\c@algocf}% and the way it is printed
\else%                                     else
\newcounter{algocf}[\algocf@within]%        % counter is numbered within \algocf@within
\renewcommand\thealgocf{\csname the\algocf@within\endcsname.\@arabic\c@algocf}%
\fi%
%
\def\fps@algocf{htbp}%        % default
\def\ftype@algocf{10}%        % float type
\def\ext@algocf{\algocf@list} % loa by default, lof if figure option used
\newcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}%
\newcommand{\algocf@resetfnum}{\renewcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}}%
\newenvironment{algocf}%      % float environment for algorithms
               {\@float{algocf}}%
               {\end@float}%
\newenvironment{algocf*}%     % float* environment for algorithms
               {\@dblfloat{algocf}}%
               {\end@dblfloat}%
%
\def\algocf@seclistalgo{}%
\ifx\l@chapter\undefined\let\algocf@seclistalgo=\section\else\let\algocf@seclistalgo=\chapter\fi%
\@ifundefined{if@restonecol}{\newif\if@restonecol}\relax%
\newcommand\listofalgocfs{%
     \ifx\algocf@seclistalgo\chapter%
      \if@twocolumn\@restonecoltrue\onecolumn\else\@restonecolfalse\fi%
    \fi%
     \algocf@seclistalgo*{\listalgorithmcfname}%
       \@mkboth{\MakeUppercase\listalgorithmcfname}%
               {\MakeUppercase\listalgorithmcfname}%
     \@starttoc{loa}%
    \ifx\algocf@seclistalgo\chapter%
      \if@restonecol\twocolumn\fi%
    \fi%
}
%
\newcommand*\l@algocf{\@dottedtocline{1}{1em}{2.3em}}% line of the list
%
% ----------------------  algorithm environment
%
%%%%%%%
%%
%% Algorithm environment definition
%%
%%%%%%%
%%
%
\newsavebox\algocf@algoframe%
\def\@algocf@pre@plain{\relax}%  action to be done before printing the algo.
\def\@algocf@post@plain{\relax}% action to be done after printing the algo.
\def\@algocf@capt@plain{bottom}% where the caption should be localized.
\def\@algocf@pre@boxed{\noindent\begin{lrbox}{\algocf@algoframe}}
\def\@algocf@post@boxed{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxed{under}%
\def\@algocf@pre@ruled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@ruled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@ruled{top}%
\def\@algocf@pre@algoruled{\hrule width\algocf@ruledwidth height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@algoruled{\kern\interspacealgoruled\hrule width\algocf@ruledwidth height\algoheightrule \relax}%
\def\@algocf@capt@algoruled{top}%
\def\@algocf@pre@tworuled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@tworuled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@tworuled{top}%
\def\@algocf@pre@boxruled{\noindent\begin{lrbox}{\algocf@algoframe}}%
\def\@algocf@post@boxruled{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxruled{above}%
\def\@algocf@pre@plainruled{\@algocf@pre@ruled}%  action to be done before printing the algo.
\def\@algocf@post@plainruled{\@algocf@post@ruled\kern\interspacealgoruled}%  action to be done before printing the algo.
\def\@algocf@capt@plainruled{under}%
%
\newcommand{\noalgocaption}{\def\@algocf@capt@ruled{none}}
%
%% before algocf environment (not figure environment)
\newcommand{\@algocf@init@caption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if we are inside a procedure/function environment
    \@algocf@proctitleofalgo% set Titleofalgo to Procedure: or Function:
                            % accordingly to the environment
    \let\old@thealgocf=\thealgocf\ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
      \renewcommand{\thealgocf}{-}}%
  }{% else inside environment algorithm
    \@algocf@algotitleofalgo% fix name for \Titleofalgo to \algorithmcfname
  }%
  \algocf@setcaption%       set caption to our caption style
}%
%
\newcommand{\@algofloatboxreset}{\@setminipage}
\newcommand{\@algocf@init}{%
  \refstepcounter{algocfline}%
  \stepcounter{algocfproc}%to have a different counter for each environment and being abble to make the difference
    %between href of algoline in different algorithms.
  \ifthenelse{\boolean{algocf@optnoend}}{%
      \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%
    }{%
      \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
    }%
}%
%% after the end of algocf or figure environment
\newcommand{\@algocf@term@caption}{%
  \algocf@resetcaption% restore original caption
}%
%
\newcommand{\@algocf@term}{%
  \setboolean{algocf@algoH}{false}% no H by default
  \ifthenelse{\boolean{algocf@optnoend}}{%
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
  }{%
    \renewcommand{\algocf@block}[2]{\algocf@group{##1}}%
  }%
  \SetAlgoRefName{\relax}%
}%
%
%%%%%%%%%%%%%%%%%
%% makethealgo: macro which print effectively the algo in its box
%% 
\newsavebox\algocf@algobox%
\newcommand{\algocf@makethealgo}{%
  \vtop{%
    % place caption above if needed  bye the style
    \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{above}}%
    {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    % precommand according to the style
    \csname @algocf@pre@\algocf@style\endcsname%
    % place caption at top if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{top}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    \box\algocf@algobox% the algo
    % place caption at bottom if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{bottom}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    % postcommand according to the style
    \csname @algocf@post@\algocf@style\endcsname%
    % place caption under if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{under}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
  }%
}%
%%%%%%%%%%%%%%%%%%%
%
%% at the beginning of algocf or figure environment
\newenvironment{algomathdisplay}{\[}{\@endalgocfline\]\ifthenelse{\boolean{algocf@linesnumbered}}{\nl}{\relax}}%
\newcommand{\@algocf@start}{%
  \@algoskip%
  \begin{lrbox}{\algocf@algobox}%
  \setlength{\algowidth}{\hsize}%
  \vbox\bgroup% save all the algo in a box
  \hbox to\algowidth\bgroup\hbox to \algomargin{\hfill}\vtop\bgroup%
  \ifthenelse{\boolean{algocf@slide}}{\parskip 0.5ex\color{black}}{}%
  % initialization
  \addtolength{\hsize}{-1.5\algomargin}%
  \let\@mathsemicolon=\;\def\;{\ifmmode\@mathsemicolon\else\@endalgoln\fi}%
  \raggedright\AlFnt{}%
  \ifthenelse{\boolean{algocf@slide}}{\IncMargin{\skipalgocfslide}}{}%
  \@algoinsideskip%
%   \let\@emathdisplay=\]\def\]{\algocf@endline\@emathdisplay\nl}%
}%
%
%% at the end of algocf or figure environment
\newcommand{\@algocf@finish}{%
  \@algoinsideskip%
  \egroup%end of vtop which contain all the text
  \hfill\egroup%end of hbox wich contains [margin][vtop]
  \ifthenelse{\boolean{algocf@slide}}{\DecMargin{\skipalgocfslide}}{}%
  %
  \egroup%end of main vbox
  \end{lrbox}%
  \algocf@makethealgo% print the algo
  \@algoskip%
  % restore dimension and macros
  \setlength{\hsize}{\algowidth}%
  \lineskip\normallineskip\setlength{\skiptotal}{\@defaultskiptotal}%
  \let\;=\@mathsemicolon%  
  \let\]=\@emathdisplay%
}%
%
%%%%%%%%%%%%%%%%%%%%
%% basic definition of the environment algorithm
%%
%
\newboolean{algocf@procenvironment}\setboolean{algocf@procenvironment}{false}%
\newboolean{algocf@func}\setboolean{algocf@func}{false}%
\newboolean{algocf@algoH}\setboolean{algocf@algoH}{false}%
\newboolean{algocf@algostar}\setboolean{algocf@algostar}{false}%
%
%%% environment for {algorithm}[H]
\newenvironment{algocf@Here}{\noindent%
  \def\@captype{algocf}% if not defined, caption exit with an error
  \begin{minipage}{\hsize}%
}{%
  \end{minipage}%\par%
}%
%%% real algorithm environment which manages H and * option
%    \let\algocf@originalfloatboxreset=\@floatboxreset%
%    \let\@floatboxreset=\@algofloatboxreset%
\newenvironment{algocf@algorithm}[1][htbp]{%
   \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@figurecaption}}{\captionsetup{margin={-\algomargin,\algomargin}}}{}%
   }{}%
   \@algocf@init%
   \ifthenelse{\equal{\algocf@float}{figure}}{% if option figure set
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \begin{figure*}[#1]% call figure*
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else algorithm environment with figure option
       \begin{figure}[#1]%  call figure
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
          \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }%
   }{% else normal algorithm environment
     \@algocf@init@caption%
     \ifthenelse{\equal{#1}{H}}{% if [H] algorithm
       \if@twocolumn\@latex@error{[H] in two columns mode is not allowed for algorithms}\fi% TODO: SCREAM if H in two colums!
       \setboolean{algocf@algoH}{true}\begin{algocf@Here}% call corresponding environment
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \begin{algocf*}[#1]% call algocf*
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }{% else algorithm environment
         \begin{algocf}[#1]%  call algcf
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }%
     }%
   }% fin test option figure ou pas
   \@algocf@start% 
   \@ResetCounterIfNeeded%
   \algocf@linesnumbered\ignorespaces%
}{%
  \@algocf@finish%
  \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure*}% call figure*
     }{% else algorithm environment with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure}%  call figure
     }%
  }{%
    \@algocf@term@caption%
    \ifthenelse{\boolean{algocf@algoH}}{% if [H] algorithm
      \let\everypar=\algocf@oldeverypar%
      \end{algocf@Here}\par% call corresponding environment
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \let\everypar=\algocf@oldeverypar%
         \end{algocf*}% call algocf*
       }{% else algorithm environment
         \let\everypar=\algocf@oldeverypar%
         \end{algocf}%  call algocf
       }%
     }%
  }%
  \@algocf@term\ignorespacesafterend%
}%
%
%%% user algorithm environment
\newenvironment{\algocf@envname}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%%% user algorithm* environment
\newenvironment{\algocf@envname*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%
%%%
%
\expandafter\newcommand\csname\algocf@listofalgorithms\endcsname{%
  \ifthenelse{\equal{\algocf@float}{figure}}{\listoffigures}{\listofalgocfs}%
}%
%%%
%%%
%
% ----------------------  procedure and function environments
%
%
% -- new style (used in particular in the caption of function and procedure environments)
%
% three macros to extract parts of the caption
\gdef\algocf@captname#1(#2)#3@{#1}  % keep characters before the first brace
\gdef\algocf@captparam#1(#2)#3@{#2} % keep character in between the braces
\gdef\algocf@captother#1(#2)#3@{#3} % keep character after the braces
%
%%% Text of caption for Procedure or Function
\newcommand{\algocf@captionproctext}[2]{%
  {%
    \ProcSty{\ProcFnt\algocf@procname\ifthenelse{\boolean{algocf@procnumbered}}{\nobreakspace\thealgocf\algocf@typo\algocf@capseparator}{\relax}}%
    \nobreakspace\ProcNameSty{\ProcNameFnt\algocf@captname #2@}% Name of the procedure in ProcName Style. 
    \ifthenelse{\equal{\algocf@captparam #2@}{\arg@e}}{}{% if no argument, write nothing
      \ProcNameSty{\ProcNameFnt(}\ProcArgSty{\ProcArgFnt\algocf@captparam #2@}\ProcNameSty{\ProcNameFnt)}%else put arguments in ProcArgSty:
    }% endif
    \algocf@captother #2@%
  }%
}%
%
%
% -- procedure and function environments are defined from algocf@algorithm environment
%
\newenvironment{procedure}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
\newenvironment{procedure*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%
%%%%%%%%%%%%%%%%%%%%
%% definition of algondfloat environment
%%
\ifthenelse{\boolean{algocf@endfloat}}{% if endfloat option then
\newcommand{\algoplace}{% macro which is used to writhe algorithm about there
   \begin{center}%
     [\algorithmcfname~\thepostfig\ about here.]%
   \end{center}%
}%
\newcommand{\algoendfloat}{% use as a \begin{algoendfloat} environment to start scanning of line
%  \immediate\openout\@mainfff\jobname.fff%
  \efloat@condopen{fff}
  \efloat@iwrite{fff}{\string\begin{\algocf@envname}}%
    \if@domarkers%
       \ifthenelse{\equal{\algocf@list}{lof}}{%
         \addtocounter{postfig}{1}%
       }{%
         \addtocounter{postalgo}{1}%
       }%
       \algoplace%
    \fi%
    \bgroup%
    \let\do\ef@makeinnocent\dospecials%
    \ef@makeinnocent\^^L% and whatever other special cases
    \endlinechar`\^^M \catcode`\^^M=12 \ef@xalgocfendfloat}%
}{\relax}%%%% end of endfloat option ifthenelse
%% some macros useful for endfloat option that cannot be defined inside the ifthenelse
%scan algoendfloat algorithm and write the text into .fff file
{\catcode`\^^M=12 \endlinechar=-1 %
 \gdef\ef@xalgocfendfloat#1^^M{% scan the lines inside algoendfloat environment being read by latex
   \def\test{#1}% test is the line being currently scan by latex
   \ifx\test\ef@endalgocftest% if it is \end{algoendfloat}
     \def\next{% define next as to not continue the scan and write \end{algorithm} into .fff file
       \egroup\end{algoendfloat}%
       \efloat@iwrite{fff}{\string\end{\algocf@envname}}%
       \efloat@iwrite{fff}{\string\efloatseparator}%
       \efloat@iwrite{fff}{ }%
     }%
     \else% else write the current line being scanned by latex and set next to continue the scan
       \efloat@iwrite{fff}{#1}%
       \let\next\ef@xalgocfendfloat%
     \fi% endif
     \next}% next is continue if it was else condition, else it does not continue the scan and write end to file
}%
% test if the scan is finish by looking at the string \end{algoendfloat}
{\escapechar=-1%
 \xdef\ef@endalgocftest{\string\\end\string\{algoendfloat\string\}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
\newcommand{\TitleOfAlgo}[1]{\@titleprefix\ 
  \TitleSty{#1}\par\smallskip}%
%
\newcommand{\SetAlgorithmName}[3]{%
  \renewcommand{\listalgorithmcfname}{#3}%
  \renewcommand{\algorithmcfname}{#1}%
  \renewcommand{\algorithmautorefname}{#2}%
}%
%
\newcommand{\algocf@refrelsize}{-2}\newcommand{\SetAlgoRefRelativeSize}[1]{\renewcommand{\algocf@refrelsize}{#1}}%
\newcommand{\SetAlgoRefName}[1]{%
  \renewcommand{\algocf@algocfref}{#1}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
% -------------------------   Default Definitions
%
%%
%%
%
\SetKwComment{tcc}{/* }{ */}%
\SetKwComment{tcp}{// }{}%
%
%\newcommand{\algocf@defaults@common}{
%
%
% english keywords (default)
%
\SetKwHangingKw{KwHData}{Data$\rightarrow$}
\SetKwInput{KwIn}{Input}%
\SetKwInput{KwOut}{Output}%
\SetKwInput{KwData}{Data}%
\SetKwInput{KwResult}{Result}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
%
% French keywords
%
\ifthenelse{\boolean{algocf@localkw@french}\OR\equal{\algocf@languagechoosen}{french}}{%
%\SetKwInOut{AlgDonnees}{Donn\'ees}\SetKwInOut{AlgRes}{R\'esultat}
\SetKwHangingKw{HDonnees}{Donnees$\rightarrow$}
\SetKwInput{Donnees}{Donn\'ees}%
\SetKwInput{Res}{R\'esultat}%
\SetKwInput{Entree}{Entr\'ees}%
\SetKwInput{Sortie}{Sorties}%
\SetKw{KwA}{\`a}%
\SetKw{Retour}{retourner}%
\SetKwBlock{Deb}{d\'ebut}{fin}%
\SetKwRepeat{Repeter}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{Si}{SinonSi}{Sinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Suivant}{Cas}{Autre}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{Pour}{pour}{faire}{fin pour}%
\SetKwFor{PourPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{PourCh}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{PourTous}{pour tous les}{faire}{fin pour tous}%
\SetKwFor{Tq}{tant que}{faire}{fin tq}%
}{}%
%
% --- German keywords
%
\ifthenelse{\boolean{algocf@localkw@german}\OR\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{Ein}{Eingabe}%KwIn
\SetKwInput{Aus}{Ausgabe}%KwOut
\SetKwInput{Daten}{Daten}%KwData
\SetKwInput{Ergebnis}{Ergebnis}%KwResult
\SetKw{Bis}{bis}%KwTo
\SetKw{KwZurueck}{zur\"uck}%KwRet
\SetKw{Zurueck}{zur\"uck}%Return
\SetKwBlock{Beginn}{Beginn}{Ende}%Begin
\SetKwRepeat{Wiederh}{wiederhole}{bis}%Repeat
%
\SetKwIF{Wenn}{SonstWenn}{Sonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Unterscheide}{Fall}{Anderes}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{Fuer}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{FuerPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{FuerJedes}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{FuerAlle}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{Solange}{solange}{tue}{Ende solange}%While
}{}%
%
% --- Czech keywords
%
\ifthenelse{\boolean{algocf@localkw@czech}\OR\equal{\algocf@languagechoosen}{czech}}{%
\SetKwInput{Vst}{Vstup}%
\SetKwInput{Vyst}{V\'{y}stup}%
\SetKwInput{Vysl}{V\'{y}sledek}%
}{}%
%
% --- Portuguese keywords
%
\ifthenelse{\boolean{algocf@localkw@portuguese}\OR\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{Entrada}{Entrada}%
\SetKwInput{Saida}{Sa\'{i}da}%
\SetKwInput{Dados}{Dados}%
\SetKwInput{Resultado}{Resultado}%
\SetKw{Ate}{at\'{e}}
\SetKw{KwRetorna}{retorna}%
\SetKw{Retorna}{retorna}%
\SetKwBlock{Inicio}{in\'{i}cio}{fim}%
\SetKwRepeat{Repita}{repita}{at\'{e}}%
%
\SetKwIF{Se}{SenaoSe}{Senao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Selec}{Caso}{Outro}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{Para}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ParaPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ParaCada}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ParaTodo}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{Enqto}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
%
% --- Italian keywords
%
\ifthenelse{\boolean{algocf@localkw@italiano}\OR\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIng}{Ingresso}%
\SetKwInput{KwUsc}{Uscita}%
\SetKwInput{KwDati}{Dati}%
\SetKwInput{KwRisult}{Risultato}%
\SetKw{KwA}{a}%
\SetKw{KwRitorna}{ritorna}%
\SetKw{Ritorna}{ritorna}%
\SetKwBlock{Inizio}{inizio}{fine}%
\SetKwRepeat{Ripeti}{ripeti}{finch\'e}%
%
\SetKwIF{Sea}{AltSe}{Altrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{Per}{per}{fai}{fine per}%
\SetKwFor{PerPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{PerCiascun}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{PerTutti}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{Finche}{finch\'e}{fai}{fine finch\'e}%
}{}%
%
% --- Spanish keywords
%
\ifthenelse{\boolean{algocf@localkw@spanish}\OR\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{Datos}{Datos}
\SetKwInput{Resultado}{Resultado}
\SetKwInput{Entrada}{Entrada}
\SetKwInput{Salida}{Salida}
\SetKw{KwA}{a}
\SetKw{KwDevolver}{devolver}
\SetKw{Devolver}{devolver}
\SetKwBlock{Inicio}{inicio}{fin}
\SetKwIF{SSi}{EnOtroCasoSi}{EnOtroCaso}{si}{entonces}{sin\'o, si}{sin\'o}{fin si}
\SetKwSwitch{Seleccionar}{Caso}{Otro}{seleccionar}{hacer}{caso}{sin\'o}{fin caso}{fin seleccionar}
\SetKwFor{Para}{para}{hacer}{fin para}
\SetKwFor{ParaPara}{par}{hacer en paralelo}{fin para}
\SetKwFor{EnParalelo}{para}{hacer en paralelo}{fin para}
\SetKwFor{Mientras}{mientras}{hacer}{fin mientras}
\SetKwFor{ParaCada}{para cada}{hacer}{fin para cada}
\SetKwFor{ParaTodo}{para todo}{hacer}{fin para todo}
\SetKwRepeat{Repetir}{repetir}{hasta que}
}{}%
%
% Croatian keywords
%
\ifthenelse{\boolean{algocf@localkw@croatian}\OR\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwUlaz}{Ulaz}%KwIn
\SetKwInput{KwIzlaz}{Izlaz}%KwOut
\SetKwInput{KwPodaci}{Podaci}%KwData
\SetKwInput{KwRezultat}{Rezultat}%KwResult
\SetKw{KwDo}{do}%KwTo
\SetKw{KwVrati}{vrati}%KwRet
\SetKw{Vrati}{vrati}%Return
\SetKwBlock{Pocetak}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Ponavljaj}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{Ako}{InaceAko}{Inace}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Granaj}{Slucaj}{OstaliSlucajevi}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{Za}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ZaPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ZaSvaki}{za svaki}{\v{c}ini}{kraj za svaki}%mForEach
\SetKwFor{ZaSvaku}{za svaku}{\v{c}ini}{kraj za svaku}%fForEach
\SetKwFor{ZaSvako}{za svako}{\v{c}ini}{kraj za svako}%nForEach
\SetKwFor{ZaSve}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{Dok}{dok}{\v{c}ini}{kraj dok}%While
}{}%

%
% --- Turkish keywords
%
\ifthenelse{\boolean{algocf@localkw@turkish}\OR\equal{\algocf@languagechoosen}{turkish}}{%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
% %
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
% --- End 
%}
%
%\algocf@defaults@common
%
% option onelanguage redefinition
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{french}}{%
\SetKwInput{KwIn}{Entr\'ees}%
\SetKwInput{KwOutSortie}{Sorties}%
\SetKwInput{KwData}{Donn\'ees}%
\SetKwInput{KwResult}{R\'esultat}%
\SetKw{KwTo}{\`a}%
\SetKw{KwRet}{retourner}%
\SetKw{Return}{retourner}%
\SetKwBlock{Begin}{d\'ebut}{fin}%
\SetKwRepeat{Repeat}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Switch}{Case}{Other}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{For}{pour}{faire}{fin pour}%
\SetKwFor{ForPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{ForEach}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{ForAll}{pour tous}{faire}{fin pour tous}%
\SetKwFor{While}{tant que}{faire}{fin tq}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{KwIn}{Eingabe}%KwIn
\SetKwInput{KwOut}{Ausgabe}%KwOut
\SetKwInput{KwData}{Daten}%KwData
\SetKwInput{KwResult}{Ergebnis}%KwResult
\SetKw{KwTo}{bis}%KwTo
\SetKw{KwRet}{zur\"uck}%KwRet
\SetKw{Return}{zur\"uck}%Return
\SetKwBlock{Begin}{Beginn}{Ende}%Begin
\SetKwRepeat{Repeat}{wiederhole}{bis}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Switch}{Case}{Other}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{For}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{ForPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{ForEach}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{ForAll}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{While}{solange}{tue}{Ende solange}%While
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Sa\'{i}da}%
\SetKwInput{KwData}{Dados}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{at\'{e}}
\SetKw{KwRet}{retorna}%
\SetKw{Return}{retorna}%
\SetKwBlock{Begin}{in\'{i}cio}{fim}%
\SetKwRepeat{Repeat}{repita}{at\'{e}}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Switch}{Case}{Other}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{For}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ForPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ForEach}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ForAll}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{While}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIn}{Ingresso}%
\SetKwInput{KwOut}{Uscita}%
\SetKwInput{KwData}{Dati}%
\SetKwInput{KwResult}{Risultato}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{ritorna}%
\SetKw{Return}{ritorna}%
\SetKwBlock{Begin}{inizio}{fine}%
\SetKwRepeat{Repeat}{ripeti}{finch\'e}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{For}{per}{fai}{fine per}%
\SetKwFor{ForPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{ForEach}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{ForAll}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{While}{finch\'e}{fai}{fine finch\'e}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Salida}%
\SetKwInput{KwData}{Datos}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{devolver}%
\SetKw{Return}{devolver}%
\SetKwBlock{Begin}{inicio}{fin}%
\SetKwRepeat{Repeat}{repetir}{hasta que}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{entonces}{si no, si}{en otro caso}{fin si}
\SetKwSwitch{Switch}{Case}{Other}{seleccionar}{hacer}{caso}{si no}{fin caso}{fin seleccionar}
\SetKwFor{For}{para}{hacer}{fin para}%
\SetKwFor{ForPar}{para}{hacer in paralelo}{fin para}%
\SetKwFor{ForEach}{para cada}{hacer}{fin para cada}
\SetKwFor{ForAll}{para todo}{hacer}{fin para todo}
\SetKwFor{While}{mientras}{hacer}{fin mientras}
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwIn}{Ulaz}%KwIn
\SetKwInput{KwOut}{Izlaz}%KwOut
\SetKwInput{KwData}{Podaci}%KwData
\SetKwInput{KwResult}{Rezultat}%KwResult
\SetKw{KwTo}{do}%KwTo
\SetKw{KwRet}{vrati}%KwRet
\SetKw{Return}{vrati}%Return
\SetKwBlock{Begin}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Repeat}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Switch}{Case}{Other}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{For}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ForPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ForEach}{za svaki}{\v{c}ini}{kraj za svaki}%ForEach
\SetKwFor{ForAll}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{While}{dok}{\v{c}ini}{kraj dok}%While
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{turkish}}{%
%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
%
%%%% old commands compatibility
%
\ifthenelse{\boolean{algocf@oldcommands}}{%
\newcommand{\SetNoLine}{\SetAlgoNoLine}%
\newcommand{\SetNoline}{\SetAlgoNoLine}%
\newcommand{\SetVline}{\SetAlgoVlined}%
\newcommand{\SetLine}{\SetAlgoLined}%
%
\newcommand{\dontprintsemicolon}{\DontPrintSemicolon}%
\newcommand{\printsemicolon}{\PrintSemicolon}%
\newcommand{\incmargin}[1]{\IncMargin{#1}}%
\newcommand{\decmargin}[1]{\DecMargin{-#1}}%
\newcommand{\setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\Setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\setalcapskip}[1]{\SetAlCapSkip{#1}}%
\newcommand{\setalcaphskip}[1]{\SetAlCapHSkip{#1}}%
\newcommand{\nlSty}[1]{\NlSty{#1}}%
\newcommand{\Setnlsty}[3]{\SetNlSty{#1}{#2}{#3}}%
\newcommand{\linesnumbered}{\LinesNumbered}%
\newcommand{\linesnotnumbered}{\LinesNotNumbered}%
\newcommand{\linesnumberedhidden}{\LinesNumberedHidden}%
\newcommand{\showln}{\ShowLn}%
\newcommand{\showlnlabel}[1]{\ShowLnLabel{#1}}%
\newcommand{\nocaptionofalgo}{\NoCaptionOfAlgo}%
\newcommand{\restorecaptionofalgo}{\RestoreCaptionOfAlgo}%
\newcommand{\restylealgo}[1]{\RestyleAlgo{#1}}%
%
\newcommand{\Titleofalgo}[1]{\TitleOfAlgo{#1}}%
% \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
\newcommand{\SetKwIf}[6]{\SetKwIF{#1}{#2#1}{#2}{#3}{#4}{#5 #1}{#5}{#6}}
%
\SetKwIF{gSi}{gSinonSi}{gSinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwIF{gIf}{gElsIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gIf}{gElseIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gWenn}{gSonstWenn}{gSonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwIF{gSe}{gSenaoSe}{gSenao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwIF{gSea}{gAltSe}{gAltrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKw{Ret}{return}%
\SetKwInput{Data}{Data}%
\SetKwInput{Result}{Result}%
}{%
  \relax%
}%
%
%
%
%%
%%%
%%%% END

==> files/Intro_Old.tex <==
%\red{(IROS)}
Safe and autonomous robot navigation of robots has received considerable research in the last decades. Particularly, several motion planning algorithms have been proposed to address point-to-point navigation tasks \cite{karaman2011sampling,lavalle2006planning,kavraki1996probabilistic} or more complex tasks, such as sequencing, recurrence, or surveillance, captured by formal languages, such as linear Temporal logic (LTL) \cite{kantaros2018text,leahy2016persistent,fainekos2005temporal,kloetzer2010automatic,baier2008principles}.
%is an important research problem that has gained a lot of traction due to its widespread application in real-world implementation of robots. 
%The goal of motion planning problems is tho generate feasible paths for the robot to follow in a given environment. Point to point robot navigation forms the backbone of this research area and considerable research has been done in this \textbf{cite}. More complex navigation problems have been approached using tasks that can capture temporal and Boolean specifications. These approaches use formal languages like Linear Temporal Logic (LTL) to address various types of navigation missions like sequencing, coverage or surveillance \textbf{cite}. %
Common in these works is that they typically assume robots with known dynamics operating in known and static environments. As a result, these methods cannot be applied to scenarios where the environment is dynamic and uncertain, resulting in limited applicability.\textcolor{red}{[add the missing references throughout the intro]}

%\textcolor{red}{Here have paragraph summarizing our paper along the lines of the abstract.}
In this paper we address a motion planning problem for teams of mobile sensing robots with known dynamics. These robots operate in an uncertain and dynamic semantic environment. Specifically, the environment is assumed to have known and static geometry (e.g., walls) but it is populated by labeled non-cooperative mobile targets of interest (e.g., drones, pedestrians, and ground robots of various types). The targets move as per known dynamics but they are subject to uncertain exogenous disturbances (e.g., wind gusts).
%
The actual labels and positions of these targets are unknown. Instead, the robots have access to a prior belief about the initial positions and the labels of the landmarks captured by Gaussian and arbitrary discrete distribution, respectively, that may be user-specified or computed by semantic mapping methods \cite{rosinol2020kimera,bowman2017probabilistic}. The prior Gaussian and discrete distribution model metric and semantic uncertainty in the environment. 
%The environment has known geometries (e.g., buildings) and static as well as dynamic landmarks which are of interest with respect to the task. We assume the landmarks have positional uncertainty and semantic uncertainty, i.e. uncertainty in the class or label of each landmark. These uncertainties gives rise to a semantic map with known geometries. We also assume prior knowledge of the dynamics of each landmark, thus being able to predict their control input at each time instant.
%\textbf{add figure} 
The robots are equipped with imperfect perception systems (e.g., cameras and learning-based object detectors \textbf{cite}) that allow them to detect, classify, and localize objects.
Given this prior environmental belief, imperfect perception systems, and the stochastic dynamics of the targets, the goal of the robots is to accomplish a complex and long-horizon \textit{semantic task} defined over the uncertain positions and labels of targets. This semantic mission is expressed using a fragment of LTL, called co-safe LTL formulas defined over probabilistic atomic predicates capturing perceptual and environmental uncertainty \textbf{cite}. For instance, consider a task \textcolor{red}{[if space permits, add a very simple example in words...]} 
The considered LTL planning problem gives rise to an optimal control problem that generates offline, i.e., open-loop, control policies. To solve this problem,  building upon our previous work \textcolor{red}{[cite our paper]}, we propose a sampling-based approach that explores the robot motion space, the mission specification space, as well as the uncertain future states of the mobile targets. The offline designed control policies are updated online to react to perceptual feedback. We show that our algorithm is probabilistically complete and asymptotically optimal under linearity and Gaussian assumption. We provide extensive experiments that involve drones that fly over an uncertain semantic city to accomplish complex navigation tasks \textcolor{red}{[edit, if needed, based on the experiments]}.
%Similar to \textbf{cite our paper}, to account for both environmental and perceptual uncertainty, the LTL ta
%The collaborative task is defined using an LTL formula which is made up of smaller individual tasks. Each of these tasks has an associated probabilistic satisfaction requirement. Giving such probabilistic satisfaction requirements is helpful in real-world applications due to the presence of uncertainties. It allows the planner to understand the priority of individual tasks and thus gives some flexibility in the actual execution. For example, our robot might need to avoid certain landmarks in the environment (e.g., enemy security robots) at a certain distance with a very high certainty which will result in the planner generating safer paths around such landmarks. On the other hand, the task can be satisfied by being within a certain distance of a landmark with a lower probability, thus enabling our robot to come close to the landmark without forcing it an exact location. 

%\textcolor{red}{Next have a short paragraph on planning unknown but static environments (See our previous paper)}
\textbf{Related works:} Recently, several reactive and senor-based planning methods have been proposed for both point-to-point navigation tasks \cite{vasilopoulos2018sensor,bansal2019combining,ryll2019efficient,zhai2019path,elhafsi2019map} and temporal logic tasks in unknown but static environments \cite{guo2013revising,guo2015multi,maly2013iterative,lahijanian2016iterative,livingston2012backtracking,livingston2013patching,kantaros2020reactive,vasilopoulos2021reactive}. More recently, motion planning methods for dynamic environments have been proposed \textbf{cite}.\textcolor{red}{[when you cite these works split them into temporal logic and  point-to-point planning methods.]} 
The major challenge in these works is that the robots should not only reason about the current structure of the environment but also predict its future configurations to successfully complete the assigned tasks. For instance, %in \textbf{cite}, the environment is dynamic in the sense that new logic tasks may be announced resulting in mission conflicts that need to be resolved. 
in \textbf{cite}, the obstacles are moving in an a-priori known fashion while in \textbf{cite} they patch the designed paths locally to avoid the obstacles which are a-priori unknown \textcolor{red}{do they do motion prediction? If so, do they incorporate uncertainty from motion prediction into planning? This also another (minor) contribution we need to discuss}. \textcolor{red}{[add 1-2 more works with unknown dynamic obstacles, if space permits.]} Common in these works is that they consider environments with unknown geometry but with known metric/semantic structure. As a result, in these works, the robots are tasked with reaching reaching perfectly known and static regions of interest while avoiding dynamic known/unknown obstacles. To the contrary, in this paper we consider environments with known geometric structure (e.g., walls) but with uncertain dynamic metric/semantic structure. In other words, the labels of regions/objects that should be avoided/approached are unknown while their positions are also uncertain and they may be changing over time. Related are also works on target tracking and active sensing that require to actively decrease uncertain of uncertain mobile targets; see e.g.,  \cite{schlotfeldt2018anytime,kantaros2021sampling,charrow2014approximate,dames2017detecting,hollinger2014sampling,bircher2017incremental} and the references therein. Nevertheless, the control objective in this work is completely different. Particularly, instead of actively localizing and tracking a group of uncertain mobile targets, our goal is to design informative paths that satisfy temporal logic missions defined over these targets. To the best of our knowledge, the most relevant works to the one proposed here is the recent work by the authors \textbf{cite}, which, unlike this work, considers \textit{static} semantic environments.
%Temporal logic planning in uncertain semantic environments has also been considered in our previous work which, however, assumes static landmarks.
%To the best of our knowledge, the closest
%
%As a result, the robots are tasked with approaching or avoiding mobile semantic targets/landmarks of ucnertain positions and semantic labels. 
%This requires online reasoning about the labels and positions of the landmarks to desi

%Common in all above works is that they focus on geometric planning problems, where the robots are tasked with reaching known and static regions of interest


%To address this problem of predicting the trajectories for the objects in the environment, various rule-based or data-driven methods have been used \textbf{cite}. Other methods use Gaussian processes and Bayesian methods \textbf{cite} to account for uncertainty in motion prediction. 

%Al these works however ignore the semantic nature of the environment. Methods have also been developed using logic based planning in dynamic environments \textbf{cite}. In \textbf{cite}, the environment is dynamic in the sense that new logic tasks may be announced resulting in mission conflicts that need to be resolved. In \textbf{cite}, the obstacles are moving in an a-priori known fashion while in \textbf{cite} they patch the designed paths locally to avoid the obstacles which are a-priori unknown. But all these works ignore the semantic structure of the environment and do not consider probabilistic guarantees. But all these works ignore the semantic structure of the environment and do not consider probabilistic guarantees. As we consider this in our approach, we are able to perform more complex sub-missions which might involve tracking a certain landmark while some other sub-mission is completed by another robot. 


%These works consider static environments, focusing on the geometry structure of the environment, requiring the robots to reach known regions/landmarks while navigating through a priori unknown geometries (e.g., windows, walls, buildings, etc). Thus, the environment is assumed to have partially unknown geometry while having full knowledge of the semantic structure. Specifically, the classification/labels of regions/landmarks and their positions in the environment are known a priori without any uncertainty. As a result of not considering any uncertainty in the semantics, the overall safety of the mission reduces in dynamic environments. Even in certain static environments, it could lead to safety violations in critical scenarios (e.g., approaching an injured person). 

%\textcolor{red}{Next have a  paragraph on planning unknown,dynamic environments and add a couple of sentences at the end on target tracking.}



%\textcolor{red}{Finally, summarize our contribution (like bullet points as in our previous paper).}
\textbf{Contributions:} The contributions of the paper can be summarized as follows. \textit{First}, we  formulate a new semantic mission planning problem in dynamic and  uncertain semantic environments.
\textit{Second}, we present a sampling-based approach to design paths that satisfy semantic missions captured by LTL specifications.
\textit{Third}, we show that the proposed sampling-based approach is
probabilistically complete and asymptotically optimal under linearity and Gaussian assumptions.
\textit{Fourth}, we provide extensive experiments that support to demonstrate the efficiency of the proposed algorithm.

==> files/Literature_survey.tex <==
%\red{(IROS)}
\begin{figure}[t]
  \centering
 %    \subfigure[$N=1, M=5$ (slow targets)]{
 %   \label{fig:traj15s}
%  \includegraphics[width=0.48\linewidth]{traj_1vs5_slow.pdf}}
\includegraphics[width=1\linewidth]{figures/PF_edited.png}
\caption{\textcolor{black}{A drone equipped with a noisy downward facing camera (blue rectangle) and an object detector is responsible for delivering supplies to uncertain ground units (e.g., people and cars) in a specific order while always avoiding colliding with uncertain poles and flying over known residential areas. The environment is modeled as an uncertain semantic map with known geometry consisting of static labeled landmarks (e.g., poles, or parked cars) and dynamic landmarks (e.g., walking people with arrow showing current direction of motion) with uncertain positions (metric uncertainty) and labels (semantic uncertainty). Each landmark is associated with a prior Gaussian and a discrete distribution modeling its positional and class uncertainty, respectively while unknown landmarks without prior information may exist, as well.}}
  \label{fig:PF1}
\end{figure}

 The basic motion planning problem consists of generating robot trajectories that reach a known desired goal region starting from an initial configuration while avoiding known obstacles. More recently, a new class of planning approaches have been developed that can handle a richer class of tasks than the classical point-to-point navigation, and can capture temporal and Boolean specifications. Such tasks can be, e.g., sequencing or coverage \cite{fainekos2005temporal}, data gathering \cite{guo2017distributed}, or persistent surveillance \cite{leahy2016persistent}, and can be modeled using formal languages, such as Linear Temporal Logic (LTL) \cite{baier2008principles,clarke1999model}. Several control synthesis methods have been proposed to design correct-by-construction controllers that satisfy temporal logic specifications assuming robots with known dynamics that operate in known environments \cite{fainekos2005hybrid,kress2007s,smith2011optimal,tumova2016multi,chen2012formal,ulusoy2014optimal,shoukry2017linear,vasile2013sampling,kantaros2018text}.
%
As a result, these methods cannot be applied to scenarios where the environment is initially unknown and, therefore, online re-planning may be required as environmental maps are constructed;  resulting in limited applicability. To mitigate this issue, learning-based approaches have also been proposed that consider robots with unknown dynamics operating in fully or partially unknown environments. These approaches learn policies that directly map on-board sensor readings to control commands in a trial-and-error fashion; see e.g., \cite{dorsa2014learning,li2017reinforcement,jones,hasanbeig2019reinforcement}. However, learning-based approaches, in addition to being data inefficient, are specialized to the environment and the robotic platform they were trained on. %and do not generalize well to previously unseen environments.

%This paper addresses a multi-robot mission planning problem in uncertain semantic environments. Specifically, the environment is occupied by static landmarks with known classes but located at uncertain positions. The environmental map is determined by Gaussian distributions over landmark positions that can be continuously learned using existing SLAM algorithms. Our goal is to design control policies for sensing robots so that they can to accomplish complex collaborative high level tasks captured by global temporal logic specifications. To specify tasks in semantic maps we extend Linear Temporal Logic (LTL) by including sensor-based predicates allowing us to incorporate uncertainty and probabilistic satisfaction requirements directly into the task specification. The sensor-based LTL planning problem gives rise to an optimal control problem that generates offline i.e., open-loop control policies. To solve this problem, we propose a new highly scalable sampling-based approach that explores the physical workspace, the map uncertainty, and an automaton space corresponding to the assigned mission. The open loop control policies are updated online to adapt to the map continuously learned by existing SLAM algorithms. We show that the proposed sampling-based algorithm is probabilistically complete, asymptotically optimal and supported by convergence rate bounds under Gaussian and linearity assumptions in the sensor models. Extensions of the proposed algorithm to account for uncertain landmark classes and mobile landmarks are discussed.



%\begin{figure}[t]
%  \centering
%\includegraphics[width=1\linewidth]{figures/task.png}
%\caption{ A team of five drones collaborate to track unknown mobile targets and localize and provide services to injured people in the presence of environmental uncertainty while avoiding flying over residential areas. The red ellipsoids illustrate the uncertainty about the location of static and mobile landmarks of interest. The colored disks represent the sensing range of each drone. [\textcolor{red}{TO BE UPDATED}]}
%  \label{fig:env}
%\end{figure}


% In this paper, we address a motion planning problem for a team of mobile sensing robots with known dynamics which are responsible for accomplishing collaborative tasks, expressed using a fragment of LTL, called co-safe LTL, in the presence of environmental and sensing uncertainty. % In particular, the robots are equipped with 
% %equipped with perception systems and are
% %\textit{metric} and \textit{semantic} environmental uncertainty and perceptual uncertainty. 
% Specifically, the environment is assumed to have known geometry while being occupied by static landmarks with uncertain labels/classes (\textit{semantic} uncertainty) located at uncertain positions (\textit{metric} uncertainty) giving rise to an uncertain semantic map with known geometry; see e.g., Figure \ref{fig:PF1}. The semantic map is determined by Gaussian and arbitrary discrete distributions over the positions and labels of the landmarks, respectively. The robots are equipped with noisy/imperfect perception systems (e.g., cameras and object detectors and classifiers) allowing them to take positional and class measurements about the landmarks. To define mission requirements that account for perceptual and environmental uncertainty, similar to \cite{jones2013distribution,haesaert2018temporal}, we specify temporal logic tasks defined over perception-based probabilistic predicates. Specifically, \textcolor{black}{we incorporate probabilistic satisfaction requirements} at the atomic-predicate level as opposed to probabilistic or metric/signal temporal logic languages that evaluate the probabilistic or the robust satisfaction of temporal logic formulas \cite{bianco1995model,donaldson2008monte,fainekos2009robustness,yoo2015control,lindemann2020barrier}. This way, we allow a user to put different weights on the individual components/requirements comprising an LTL formula (e.g., staying away from a hostile patrolling agent may be more important than reaching a goal destination, which cannot be captured by probabilistic temporal logic languages straightforwardly). Then, our goal is to design perception-based control policies so that the multi-robot system satisfies the co-safe LTL specification. %, such as '\textit{the probability of being close to an object with class 'chair' is greater than 0.9 while the uncertainty of its position and class estimate is less than 0.1}'.


% The problem of synthesizing controllers in the presence of mapping or localization uncertainty typically gives rise to partially observable Markov decision processes (POMDPs) \cite{haesaert2018temporal,sun2020stochastic} that suffer from  the curse of dimensionality and history. To avoid the need for computationally expensive POMDP methods, we formulate the planning problem as a deterministic optimal control problem that designs open-loop perception-based control policies that satisfy the assigned specification. \textcolor{black}{To solve this problem, building upon existing sampling-based planners \cite{hsu1997path,sucan2011sampling,kantaros2019optimal}, we present a sampling-based approach} which, given an uncertain prior belief about the semantic map, explores the robot motion space, a (sub-)space of map uncertainty, and an automaton space corresponding to the assigned mission. During the offline control synthesis process, the robots explore the metric environmental uncertainty, i.e., predict how the metric uncertainty will change based on their future control actions under linearity and Gaussian assumptions on the sensor models \cite{atanasov2014information,atanasov2015decentralized}. Prediction of the evolution of semantic uncertainty in the offline control synthesis phase is not possible, as it requires label measurements (i.e., images) which are impossible to obtain a priori/offline.
% %
% To ensure that the proposed sampling-based approach can efficiently explore this large hybrid space, we adopt the biased sampling strategy, developed in our previous work  \cite{kantaros2019optimal}, that biases exploration towards regions that are expected to be informative and contribute to satisfaction of the assigned specification. We show that the proposed sampling-based algorithm is probabilistically complete and asymptotically optimal under Gaussian and linearity assumptions on the sensor models.
% %

% As the robots execute the designed control policies, they take measurements that allow them to update their belief about both the metric and the semantic uncertainty of the environment using recently proposed semantic Simultaneous Localization And Mapping (SLAM) algorithms \cite{bowman2017probabilistic, rosinol2020kimera}. To adapt to the online learned map, the robots design new paths by re-applying the sampling-based approach. Re-planning occurs only at time instants where the offline predicted map differs significantly from the online constructed map. Formally, the re-planning time instants are determined online by an automaton corresponding to the assigned co-safe LTL formula. The mission terminates when an accepting condition of this automaton is satisfied. The proposed planning architecture over continuously learned semantic maps is also summarized in Figure \ref{fig:overview}. %\footnote{\textcolor{red}{Not sure if I should make this blue text more concise}}
%  %The open loop control policies can be updated online at time instants determined by an automaton to adapt to the semantic map that is continuously learned using semantic SLAM methods.
% % %Note that \cite{kantaros2019optimal,kantaros2019asymptotically} explore a subspace of the considered joint space. Specifically, \cite{kantaros2019optimal} explores the robot motion space and an automaton state space while \cite{kantaros2019asymptotically} searches for informative paths by exploring the robot motion space and the map uncertainty space.
% %
% Extensions of the proposed algorithm to account for nonlinear sensor models and environments with no prior metric/semantic  information are discussed, as well. % uncertain landmark classes and
% %Scenarios where the synthesized open-loop optimal policies are also closed-loop optimal policies are discussed. 
% We provide extensive experiments that corroborate the theoretical analysis and show that the proposed algorithm can address large-scale planning tasks under environmental and sensing uncertainty.
% %
% \begin{figure}[t]
%   \centering
%  %    \subfigure[$N=1, M=5$ (slow targets)]{
%  %   \label{fig:traj15s}
% %  \includegraphics[width=0.48\linewidth]{traj_1vs5_slow.pdf}}
% \includegraphics[width=1\linewidth]{figures/Overview.png}
% \caption{Graphical depiction of the proposed  architecture for planning over continuously learned uncertain semantic maps. First, given a mission specification $\phi$ and an uncertain prior belief about the environment, initial paths are constructed. The robots follow the designed paths while updating the semantic map by fusing the collected measurements. Re-planning is triggered occasionally to adapt planning to the continuously learned map. } 
%   \label{fig:overview}
% \end{figure}
% %
% %
% %Building upon our previous works \cite{kantaros2019information,kantaros2019semantic}, we design biased sampling functions that allow us to quickly address large-scale planning tasks, as shown by extensive numerical experiments. This allows us to quickly re-design control policies, at runtime, in case prior information encapsulated by the semantic maps is inaccurate. %Finally, we show that the proposed sampling-based algorithm is probabilistically complete, asymptotically optimal, and supported by convergence rate bounds under Gaussian and linearity assumptions in the sensor models and the hidden state dynamics. %We provide extensive simulation studies that corroborate the theoretical results and show that the proposed approach can address large-scale temporal logic planning tasks.
% %
\subsection{Related Research}
%Relevant are also the works in multi-task SLAM...
\subsubsection{Sampling-based Temporal Logic Planning}
Sampling-based approaches for temporal logic planning have also been proposed in \cite{karaman2012sampling,vasile2013sampling,bhatia2010sampling,bhatia2011motion,luo2021abstraction,kantaros2018text} but they consider  \textit{known} environments. Typically, these works build upon sampling-based planning algorithms originally developed for reachability tasks \cite{karaman2011sampling}.
%
%
Specifically, in \cite{karaman2012sampling}, a sampling-based algorithm is proposed which incrementally builds a
Kripke structure until it is expressive enough to generate a path that satisfies a task specification expressed in deterministic $\mu$-calculus. In fact, \cite{karaman2012sampling} builds upon the RRG algorithm \cite{karaman2011sampling} to construct an expressive enough abstraction of the environment. To enhance scalability of \cite{karaman2012sampling} a sampling-based temporal logic path planning algorithm is proposed in \cite{vasile2013sampling}, that also builds upon the RRG algorithm, but constructs incrementally sparse graphs to build discrete abstractions of the workspace and the robot dynamics. These abstractions are then composed with an automaton, capturing the task specification, which yields a product automaton. Then, correct-by-construction paths are synthesized by applying graph search methods on the product automaton. However, similar to \cite{karaman2012sampling}, as the number of samples increases, the sparsity of the constructed graph is lost and, as a result, this method does not scale well to large planning problems either. 
%
Similar abstraction-free temporal logic planning algorithms have been presented in \cite{bhatia2010sampling,bhatia2011motion,luo2021abstraction}, as well.
%
A highly scalable sampling-based approach for LTL planning problems is also  presented in \cite{kantaros2018text} that can handle hundreds of robots which, unlike the previous works, requires user-specified discrete abstractions of the robot dynamics \cite{belta2005discrete}. %that also build trees, instead of arbitrary graphs, to search on-the-fly the state space of the discrete abstraction and the automaton. To the contrary, the proposed algorithm is abstraction-free and can be used for planning in  %Finally, notice that common in existing sampling-based algorithms \cite{karaman2011sampling}, used for point-to-point navigation, is that samples are drawn from a continuous state-space, which is not the case in this work; therefore, they cannot be applied straightforwardly in our problem setting.
Note that unlike these works, as discussed earlier, our sampling-based approach explores a map uncertainty space, as well, to account for environmental and sensing uncertainty.
%Moreover, note that unlike \cite{karaman2012sampling,vasile2013sampling}, our proposed sampling-based approach builds \textit{trees} to explore the robot motion space the automaton space that captures the assigned task specification. Therefore, it does not require the application of expensive graph search techniques to find the optimal path, but instead it tracks sequences of parent nodes starting from desired accepting states.  Moreover, we show that our proposed planning algorithm is asymptotically optimal which is not the case in \cite{vasile2013sampling}. 
%%% In this way, we can handle more complex planning problems with more robots and LTL tasks that correspond to larger DFA, compared to the ones that can be solved using the approach in \cite{vasile2013sampling}. 


\subsubsection{Temporal Logic Planning under Map Uncertainty}

Temporal logic planning in the presence of map uncertainty in terms of incomplete environment models is considered in \cite{guo2013revising,guo2015multi,maly2013iterative,lahijanian2016iterative,livingston2012backtracking,livingston2013patching,kantaros2020reactive}. 
%kress2009temporal,alonso2018reactive,
Common in these works is that they consider static environments with unknown geometry but with known metric/semantic structure. As a result, in these works, the regions of interest over which the LTL missions are defined are a priori known. Additionally, to model these partially unknown environments, transition systems \cite{baier2008principles} or occupancy grid maps \cite{grisetti2007improved} are used that are continuously updated assuming perfect sensor feedback; as a result, LTL tasks are defined using deterministic atomic predicates. To the contrary, in this work we consider environments with known geometry but with uncertain metric and semantic structure, i.e., the locations and the labels of regions/objects of interest are uncertain. To account for this novel environmental uncertainty, we model the environment as an uncertain semantic map - which is continuously learned through uncertain perceptual
feedback - and we introduce probabilistic atomic predicates over the uncertain map to define robot missions. %Also, we show that the proposed method can also handle dynamic environments as well. %semantic uncertainty, i.e., uncertainty in the labels of objects of interest, and dynamic environments as well. %
%Common in all these works is that they consider static environments with uncertain geometric structure, i.e., uncertainty in the positions of obstacles, using unknown but continuously learned environmental models in the form of transition systems \cite{baier2008principles} or occupancy grid maps \cite{grisetti2007improved}.
For instance, \cite{guo2013revising,guo2015multi} model the environment as transition systems which are partially known. Then discrete controllers are designed by applying graph search methods on a product automaton. As the environment, i.e., the transition system, is updated assuming perfect sensor feedback, the product automaton is locally updated, as well, and new paths are re-designed by applying graph search approaches on the revised automaton. %However, construction of a product automaton and application of graph search techniques is computationally expensive.
%A conceptually similar approach is proposed in \cite{maly2013iterative,lahijanian2016iterative} too. The works in \cite{livingston2012backtracking,livingston2013patching} propose methods to locally patch paths as transition systems, modeling the environment, change so that GR(1) (General Reactivity of Rank 1) specifications are satisfied. 
Common in all these works is that, unlike our approach, they rely on discrete abstractions of the robot dynamics  \cite{belta2005discrete,pola2008approximately}. Thus, correctness of the generated motion plans is guaranteed with respect to the discrete abstractions resulting in a gap between  the generated discrete motion plans and their physical low-level implementation \cite{desaisoter}. An abstraction-free reactive method for temporal logic planning over continuously learned occupancy grid maps is proposed in \cite{kantaros2020reactive}. Note that \cite{kantaros2020reactive} can handle sensing and environmental uncertainty, as shown experimentally, but completeness guarantees are provided assuming perfect sensors, which is not the case in ouor current work. 

The most relevant works are presented by the authors in \cite{fu2016optimal, kantaros2019optimal} that also address temporal logic motion planning problems in  uncertain environments modeled as uncertain semantic maps. In particular, \cite{fu2016optimal} considers sequencing tasks, captured by co-safe LTL formulas, under the assumption of landmarks with uncertain locations but a priori known labels. This work is extended in \cite{kantaros2019optimal} by considering landmarks with uncertain locations and labels and task specifications captured by arbitrary co-safe temporal logic formulas. Common in both works is that control policies are designed based on a given semantic map - which is never updated - without considering the sensing capabilities of the robots. \textcolor{black}{In contrast, in this work, the proposed algorithm designs \textit{perception-based} control policies that actively decrease the metric uncertainty in the environment to satisfy probabilistic satisfaction requirements that are embedded into the mission specification. In other words, the proposed method may find feasible paths even if such paths do not exist for the initial uncertain semantic map.} Also, unlike \cite{fu2016optimal, kantaros2019optimal}, we show that the proposed algorithm can be extended to environments with no prior metric/semantic information. Furthermore all previous work cited above focus on static environments, while we propose an approach that can be used in both static as well as dynamic environments.  Finally, we provide formal completeness and optimality guarantees that do not exist in \cite{fu2016optimal, kantaros2019optimal}. 
%considers task specifications captured by arbitrary co-safe temporal logic formulas with uncertain landmark labels and mobile landmarks. Also, \cite{fu2016optimal} does not explore the  information space, i.e., it does not exploit sensor measurements that can be used to update the semantic map and, therefore, satisfy the assigned task specification with stronger probabilistic satisfaction guarantees. Finally, we show that the proposed sampling-based algorithm can be applied to large-scale planning tasks that involve large workspaces and number of robots. Finally, we provide formal optimality and convergence rate guarantees that do not exist in \cite{fu2016optimal}. 

%\cite{fainekos2005hybrid,kress2009temporal,bhatia2010sampling,guo2015multi,fu2016optimal,kantaros2017Csampling}. Given a task described by a formal language and discrete model of the robot, such as transition systems or Markov Decision Processes (MDPs), model checking algorithms can be employed to synthesize controllers that satisfy the assigned tasks \cite{baier2008principles,clarke1999model}.


\subsection{Summary of objectives of this rotation}
The objectives of this rotation can be summarized as follows. \textit{First}, we build upon our previous work on perception-based temporal logic planning in uncertain semantic maps\cite{TRO} by extending it to dynamic maps where the landmarks are dynamic.
%
%we propose the first abstraction-free sampling-based approach that can synthesize sensor-based control policies for multi-robot systems that are tasked with accomplishing temporal logic missions in the presence of sensing and environmental uncertainty. 
\textcolor{black}{\textit{Second}, we present a sampling-based approach that can synthesize perception-based control policies for robot teams that are tasked with accomplishing temporal logic missions in uncertain dynamic semantic environments.}
%we propose the first sampling-based approach for temporal logic objectives that can synthesize sensor-based control policies for robot teams operating in uncertain semantic maps. 
%
\textit{Third},  we provide extensive experiments that illustrate the efficiency of the proposed algorithm . 
%we design a sampling strategy that biases exploration towards regions that are expected to contribute to mission accomplishment allowing us to scale to large robot teams that operate in large environments.

==> files/PF_new.tex <==

% ------------------------------------------------------------------------------- %
The Objective of the the rotation was to solve the problem of path planning for a multi-robot system in dynamic and uncertain environment, govenerned by a task captured by an LTL formula. The detailed problem definition is described in the following subsections.
\subsection{Multi-Robot System}
Consider $N$ mobile robots governed by the following dynamics: %$\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t))$,
%
\begin{equation}\label{eq:rdynamics1}
\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t)),
\end{equation}
for all $j\in\ccalN:=\{1,\dots,N\}$. In \eqref{eq:rdynamics1}, $\bbp_{j}(t)\in\mathbb{R}^n$ stands for the state (e.g., position and orientation) of robot $j$ in an environment $\Omega\subseteq\mathbb{R}^m$, $m\in\{2,3\}$, at discrete time $t$.\footnote{For simplicity of notation, hereafter, we also denote $\bbp_{j}(t)\in\Omega$.} Also, $\bbu_{j}(t) \in\ccalU_j$ stands for a control input applied at time $t$ by robot $j$, where $\ccalU_j$ denotes a \textit{finite} space of admissible control inputs. %\NA{state that time is discrete}
%Note that the state $\bbp_{j}$ may belong to a higher dimensional space than $\Omega_{\text{free}}$. For example, this is the case if $\bbp_j(t)$ includes the position and the orientation of robot $j$. Nevertheless, throughout the rest of the paper, for simplicity of notations we denote $\bbp_{j}(t) \in \Omega_{\text{free}}$.\BS{Can we make this into a  remark or just remove it? It's extra clutter for something that is fairly straightforward.} 
%Also, note that the considered dynamics can range from simple graph-based dynamics to arbitrary nonlinear discrete dynamics\NA{This sentence could be removed}. 
Hereafter, we compactly model the team of robots, each equipped with a finite library of motion primitives, as
\begin{equation}\label{eq:rdynamics}
\bbp(t+1)=\bbf(\bbp(t),\bbu(t)),
\end{equation}
where $\bbp(t)\in \Omega^N$, $\forall t\geq 0$, and $\bbu(t)\in\ccalU:=\ccalU_1\times\dots\times\ccalU_N$.
%
\begin{figure}[t]
  \centering
 %    \subfigure[$N=1, M=5$ (slow targets)]{
 %   \label{fig:traj15s}
%  \includegraphics[width=0.48\linewidth]{traj_1vs5_slow.pdf}}
\includegraphics[width=1\linewidth]{figures/mapEx.png}
\caption{An environment with known geometric structure modeled as a uncertain semantic map consisting of $M=7$ landmarks with a set of semantic classes defined as $\ccalC=\{\text{`person'}, \text{`door'}, \text{`supplies'}\}$. Each landmark is determined by a Gaussian distribution and a discrete distribution modeling uncertainty in its position and class, respectively. } %In Section \ref{sec:PF}, we assume that each landmark has a known class. Relaxation of this assumption is discussed in Section \ref{sec:extensions}.
  \label{fig:seMmap}
\end{figure}
\subsection{Uncertain Semantic Maps}
The robots operate in an environment with known geometric structure (e.g., walls, buildings) but with uncertain metric and semantic structure. Specifically, the obstacle-free space $\Omega_{\text{free}}\subseteq\Omega$ is assumed to be known while $\Omega_{\text{free}}$ is cluttered with $M>0$ uncertain, static, and labeled landmarks $\ell_i$ giving rise to an uncertain semantic map $\ccalM=\{\ell_1,\ell_2,\dots,\ell_M\}$. Each landmark $\ell_i=\{\bbx_i,c_i,\psi_i\}\in\ccalM$ is defined by its position $\bbx_i\in \Omega$, its class $c_i\in\ccalC$, where $\ccalC$ is a finite set of semantic classes and $\psi_i\in\Psi$, where $\Psi$ is a set of possible control functions that govern the dynamics of the landmark. The dynamics generate control inputs $\mu_i(t)$ for the landmark $\ell_i$ at every time instant $t$ and thus governs the position of the landmark. Each $\psi_i$ is defined by the type of motion (eg. linear, oscillatory, circular), landmark velocity, direction of motion, and distance whenever applicable (eg. radius of circle or distance of oscillation). Thus we can denote the position update of landmark $\ell_i$ governed by the dynamics $\psi_i$ as $\bbx_i(t+1)=g_i(\bbx_i(t),\mu_i(t))$.  

The robots have prior information about the dynamics of all landmarks. 
%
The robots do not know the true landmark positions and classes but instead they have access to a probability distribution over the space of all possible maps. Such a distribution can be produced by its perceptual capabilities and typically consists of a Gaussian distribution over the landmark positions, modeling metric uncertainty in the environment, and an arbitrary discrete distribution over the landmark classes modeling semantic uncertainty. 
%Hereafter, we assume that the landmarks are static with known classes. A discussion on relaxing this assumption is presented in Section \ref{sec:extensions}. On the other hand, the robots do not know the true landmark positions but instead they initially have access to a probability distribution $\ccalM$ over the space of all possible maps. 
%
%Such a distribution can be user-specified initially and can be updated online by existing SLAM algorithms. Such a map distribution typically consists of a Gaussian distribution over the landmark positions. 
Specifically, we assume that $\ccalM$ is determined by parameters $(\hat{\bbx}_i,\Sigma_i, d_i, \psi_i)$, for all landmarks $\ell_i$, such that $\bbx_i\sim\ccalN(\hat{\bbx}_i,\Sigma_i)$, where $\hat{\bbx}_i$ and $\Sigma_i$ denote the mean and covariance matrix of the position of landmark $\ell_i$, $c_i\sim d_i$, where $d_i:\ccalC\rightarrow [0,1]$ is an arbitrary discrete distribution over the finite set of possible classes and $\psi_i$ is the dynamics that governs landmark $\ell_i$. Hereafter, we compactly denote by $(\hat{\bbx},\Sigma, d, \psi)$ the parameters that determine all landmarks in the semantic map $\ccalM$. 
% In what follows, we assume that an uncertain prior belief about the metric/semantic structure of the environment is available by a user to the robots which can be updated online using SLAM methods. A discussion on relaxing this assumption is provided in Section \ref{sec:extensions}.
\begin{assumption}[Uncertain Prior Map]\label{as:prior}
We assume that initially the robots have access to Gaussian and discrete distributions denoted by $\bbx_i\sim\ccalN(\hat{\bbx}_i(0),\Sigma_i(0))$ and $c_i\sim d_i(0)$, for all landmarks $\ell_i\in\ccalM$, where the number of landmarks and the set of available classes is a priori known. We also assume that the robots have access to the dynamics $\psi_i$ for all landmarks $\ell_i\in\ccalM$.
\end{assumption}
\begin{ex}[Semantic Map]%\label{ex:semMap}
An example of an uncertain semantic map is illustrated in Figure \ref{fig:seMmap} that consists of $M=7$ landmarks with set of classes $\ccalC=\{\text{`person'}, \text{`door'}, \text{`supplies'}\}$. Uncertain semantic maps provide a novel means to define mission objectives in terms of meaningful semantic objects in uncertain environments. For instance, in Figure \ref{fig:seMmap}, consider a task that requires the robots to collect all available supplies and deliver them in a specific order to injured people. %; see also Section \ref{sec:task}. %A formal language to specify robot missions in the presence of metric/semantic environmental and perceptual uncertainty is discussed in Section \ref{sec:task}.
\end{ex}


\subsection{Perceptual Capabilities}
The robots are equipped with sensors (e.g., cameras) to collect measurements associated with the landmark positions $\bbx$ as per the following \textit{linear observation model}: $\bby_j(t) = \bbM_j(\bbp_j(t))\bbx + \bbv_j(t)$, where $\bby_j(t)$ is the measurement signal at discrete time $t$ taken by robot $j\in\ccalN$. For instance, linear observation models with respect to the hidden state have been considered in \cite{freundlich2018distributed}. Also, $\bbv_j(t) \sim \ccalN(\bb0, \bbR_j)$ is sensor-state-dependent Gaussian noise with covariance $\bbR_j$. %Linear observation models have been used, e.g., in \cite{bennetts2013towards} to estimate a gas concentration field.
Hereafter, we compactly denote the observation models of all robots as 
\begin{equation}\label{eq:measModelR}
\bby(t)= \bbM(\bbp(t))\bbx+\bbv(t),~\bbv(t) \sim \ccalN(\bb0, \bbR),
\end{equation}
where $\bby(t)$ collects measurements taken at time $t$ by all robots  associated with any landmark, and $\bbM$ and $\bbR$ are diagonal matrices where their $j$-th diagonal block is $\bbM_j$ and $\bbR_j$, respectively.\footnote{Note that the observation model \eqref{eq:measModelR} is assumed to be linear with respect to the landmark positions as this allows us to employ separation principles developed in estimation theory; see Section \ref{sec:updateMap}. }

Moreover, we assume that the robots are equipped with object recognition systems that allow them to collect measurements associated with the landmark classes $\bbc$. These semantic measurements typically consist of label measurements along with label probabilities \cite{redmon2016you,ren2016faster, guo2017calibration}. Since such algorithms are scale- and orientation-invariant, the class measurement is independent of the robot/sensor position (assuming that the landmark is within the sensing range of the robot). Thus, once a landmark $\ell_i$ is detected, a semantic measurement is generated by the following observation model: $[\bby_{j}^c, \bbs_{j}^c]=\bbg_j(L_i)$ (see also \cite{atanasov2016localization}) where $\bby_{j}^c$ and $\bbs_{j}^c$ represent a class/label measurement and the corresponding probability scores over all available classes, respectively, and $L_i$ stands for the true class of the detected landmark $\ell_i$. More details about modeling sensors generating semantic measurements can be found in \cite{atanasov2016localization}; see also Remark \ref{rem:objRec}. Hereafter, we compactly denote the object recognition model of all robots as  
\begin{equation}\label{eq:measModelC}
[\bby^c(t), \bbs^c(t)]=\bbg(\bbL),
\end{equation}
where $\bbL$ denote the true classes of all landmarks detected at time $t$.
%\begin{equation} \label{eq:measModel}
%\bby(t)= \bbm(\bbp(t),\bbx,\bbv(t)),~\bbv(t) \sim \ccalN(\bb0, \bbR(t) ).
%\end{equation}
%
\subsection{Separation Principle: Offline Update of Semantic Maps}\label{sec:updateMap}
Given measurements generated by the sensors \eqref{eq:measModelR}-\eqref{eq:measModelC}  until a time instant $t\geq0$, the semantic map can be updated online by fusing the collected measurements %that the robots collect according to the sensor models \eqref{eq:measModelR}-\eqref{eq:measModelC} until a time instant $t\geq0$ as they apply a sequence control inputs denoted by $\bbu_{0:t}$. The collected measurements can be fused by 
using recently proposed semantic SLAM algorithms \cite{bowman2017probabilistic,rosinol2020kimera}. Note that updating the map requires knowledge of the measurements that the robots may collect in the field if they apply a sequence of control actions, denoted $\bbu_{0:t}$, which is impossible to obtain during the offline control synthesis process. 

To mitigate this challenge and to design control policies while accounting for their effect on the map uncertainty, we rely on separation principles that have recently been employed in estimation theory \cite{atanasov2014information,atanasov2015decentralized}. Specifically, given a linear observation model with respect to the landmark positions, as  defined in  \eqref{eq:measModelR}, and given a sequence of control inputs until a time instant $t$, denoted by $\bbu_{0:t}$, the a-posteriori covariance matrix can be computed offline using the Kalman filter Riccati equation, i.e., without requiring knowledge of any measurements \cite{atanasov2014information,atanasov2015decentralized}. %In this case, the a-posteriori covariance matrix  can be computed using the Kalman filter Riccati equation using only the current robot position $\bbp(t+1)$. 
Hereafter, with slight abuse of notation, we denote the Kalman filter Riccati map by $\Sigma(t+1)=\rho(\Sigma(t),\bbp(t+1))$ where $\Sigma(t+1)$ and $\Sigma(t)$ denote the a posteriori covariance matrix at consecutive time instants $t$ and $t+1$. Observe that $\Sigma(t+1)$ can be computed directly from $\Sigma(t)$ given the next robot position $\bbp(t+1)$ (or equivalently the control input $\bbu(t)$ applied at $\bbp(t)$).
%
Note that the a posteriori estimates $\hat{\bbx}(t)$ for the positions of the landmarks cannot be updated offline, i.e., without sensor measurements generated by \eqref{eq:measModelR}. Similarly, the semantic uncertainty, captured by the discrete distribution $d$, cannot be updated offline as it requires measurements (i.e., images) that will be processed by the object recognition algorithm \eqref{eq:measModelC}.

Finally, throughout the report we make the following assumption that is required for applying a Kalman filter and, consequently, for offline computation of a posteriori covariance matrices. % and the underlying communication network between the robots.

Since the landmarks are dynamic, it is also necessary for the robots to update their estimates of the semantic map $\ccalM$ until the landmarks are observed. We use an extended kalman filter (EKF) to update our estimates without observation. We denote the update of the landmark estimates using the notation $\hat{\bbx}(t+1),\Sigma(t+1)=\kappa(\hat{\bbx}(t),\Sigma(t),\psi)$. 

\begin{assumption} \label{as:assumption}%[State Model]
%The dynamics of the state $\bbx(t)$ and the control input $\bba(t)$ in \eqref{eq:dynamics}, 
The observation model \eqref{eq:measModelR} and the covariance matrix $\bbR$ of the measurement noise are known.  
\end{assumption}

Assumption \ref{as:assumption} is common in related works and, in practice, it can be satisfied by learning the covariance matrix offline using training data \cite{atanasov2014information,atanasov2015decentralized,bowman2017probabilistic}.


\subsection{Temporal Logic Tasks over Uncertain Semantic Maps}\label{sec:task}
The goal of the robots is to accomplish a complex collaborative task captured by a global co-safe Linear Temporal Logic (LTL) specification $\phi$. To reason about both environmental and perceptual uncertainty, similar to \cite{jones2013distribution,haesaert2018temporal}, we define perception-based atomic predicates that depend on both the multi-robot state and the perceived uncertain semantic map over which the LTL formula is defined. %As it will be discussed later, these predicates require the robots to reason about the both the environmental and perceptual uncertainty.  %Particularly, given a map distribution $\ccalM$, we define atomic predicates $g(\bbp(t),\ccalM)\geq 0$ that reason about the semantic and/or metric uncertainty. %An example of such a predicate follows.
%\begin{align}
%&g(\bbp_j(t),\ell_i,r,\delta)\geq 0: ~~\mathbb{P}(||\bbp_j(t)-\bbx_i||\leq r)\geq 1-\delta.\label{apIROS}
%\end{align}
%Specifically,  predicate \eqref{apIROS} is true at time $t$ if the probability of robot $j$ being within distance less than $r$ from landmark $\ell_i$ is greater than $1-\delta$. In \cite{kantaros2019optimal}, we designed offline control policies that satisfy temporal logic missions defined over such probabilistic predicates without considering the sensing capabilities of the robots and, therefore, without updating the map during the control synthesis process. In this paper, our goal is to design open-loop \textit{sensor-based} control policies that also reason about how the uncertainty in the workspace may decrease if a sequence of control actions is applied. The benefit of this approach is that paths satisfying the assigned mission may be found even if they do not exist for the initial map distribution. 
To define such predicates, first, with slight abuse of notation, we denote by $\ccalM(t)$ the map distribution at time $t$ obtained after the robots apply a sequence of control actions $\bbu_{0:t}$; the offline construction of $\ccalM(t)$ was discussed in Section \ref{sec:updateMap}. %Hereafter we refer to the uncertain map as dynamic map, although the landmarks are static, to account for changes in the map distribution. 

\subsubsection{Perception-based Predicates}
%Similar to the majority of temporal logic planning papers, we can define atomic predicate $\pi_g$  over the robot states $\bbp(t)$ and the known environmental geometry as follows 
%\begin{subequations}
%\begin{align}
%\pi_g^j(\ccalR): \bbp_j\in\ccalR\subseteq\Omega,\label{ap0} %\\
%&\pi_{\ell_i}(\Sigma_i(t|\bby_{0:t}^d),\zeta):\det\Sigma_i(t|\bby_{0:t}^d)\leq\zeta. \label{ap3a}
%\end{align}
%\end{subequations}
%where $\pi_g^j(\ccalR)$ is true only if robot $j$ is within a known region $\ccalR\subseteq\Omega$ (e.g., an obstacle) in the environment. %Similarly, in \eqref{ap3a}, $\pi_{\ell_i}(\Sigma_i(t|\bby_{0:t}^d),\zeta)$ is true if the uncertainty of the position of landmark $\ell_i$, captured by the determinant of the (a-posteriori) covariance matrix $\Sigma_i(t|\bby_{0:t}^d)$, denoted by $ \det\Sigma_i(t|\bby_{0:t}^d)$, is less than a user-specified parameter $\zeta\geq 0$ after fusing the semantic measurements $\bby_{0:t}^d$.

We define perception-based predicates, denoted by $\pi_p(\bbp(t),\ccalM(t),\Delta)$, as follows:
\begin{equation}\label{eq:pip}
  \pi_p(\bbp(t),\ccalM(t),\Delta)=
    \begin{cases}
      \text{true}, & \text{if $p(\bbp(t),\ccalM(t),\Delta)\geq 0$}\\
      \text{false}, & \text{otherwise}
    \end{cases}       
\end{equation}
where $\Delta$ is set of user-specified and case-specific parameters (e.g., probabilistic thresholds or robots indices) and $p(\bbp(t),\ccalM(t),\Delta): \Omega^N\times\ccalM(t)\times\Delta\rightarrow\mathbb{R}$. Hereafter, when it is clear from the context, we simply denote a perception-based predicate by $\pi_p$.

In what follows, we define  functions $p(\bbp(t),\ccalM(t),\Delta)$ that will be used throughout this report. %; see \eqref{eq:pip}. %\footnote{Note that the  perception-based that will be defined next may } 
First, we define the following two functions reasoning about the metric uncertainty of the map:
\begin{align}
&p(\bbp(t),\ccalM(t), \{j,\ell_i,r,\delta\})=\nonumber\\&\mathbb{P}(||\bbp_j(t)-\bbx_i||\leq r)- (1-\delta),\label{ap1} 
\end{align}
and
\begin{equation}\label{apS}  
p(\bbp(t),\ccalM(t),\{j,\ell_i,\delta\})= \delta - \det(\Sigma_i(t)).
\end{equation}
%and
%\begin{equation}\label{apS2}  
%p(\ccalM(t),\{\delta\})= \delta - \det(\Sigma_i(t)). 
%\end{equation}
 %
%where $t\geq t'$.
The predicate associated with \eqref{ap1} is true at time $t$ if the probability of robot $j$ being within distance less than $r$ from landmark $\ell_i$ is greater than $1-\delta$, after applying control actions $\bbu_{0:t}$, for some user-specified parameters $r,\delta>0$. %Note that to compute the probability in \eqref{ap1}, only the Gaussian distribution of $\bbx_i$ and the robot position $\bbp_j(t)$ are required. 
Similarly, \eqref{apS} is true if the determinant of the a-posteriori covariance matrix associated with landmark $\ell_i$ is less than a user-specified threshold $\delta$ after applying control actions $\bbu_{0:t}$. %Recall from the Kalman Filter Ricatti that to compute the a posteriori covariance matrix $\Sigma(t)$, the multi-robot state $\bbp(t)$ is used. 
Note that in \eqref{apS}, robot $j$ is responsible for actively localizing landmark $\ell_i$, although the global multi-robot state $\bbp(t)$ is used to compute the a posteriori covariance matrix $\Sigma(t)$ using the Kalman Filter Ricatti map. The latter predicate allows us to reason about how confident the robots are about the position of landmark $\ell_i$; the smaller the $\det(\Sigma_i(t))$ is, the smaller the metric uncertainty about landmark $i$ is. %Note that \eqref{apS} does not depend on the robot states but only on the current semantic map and, specifically, on the covariance matrix of the Gaussian distribution associated with landmark $\ell_i$. In what follows, with slight abuse of notation, we drop any such unnecessary dependencies from the definitions of $\pi_p$ and $p$.
%Additional predicates can be defined using e.g., risk measures.
%

In a similar way, we can define predicates that reason about both the metric and the semantic uncertainty. For instance, consider the following function:
\begin{align}
    &p(\bbp(t),\ccalM(t),\{j,r,\delta,c\})=\nonumber\\&\max_{\ell_i}[\mathbb{P}(||\bbp_j(t)-\bbx_i||\leq r)d_i(c)]-( 1-\delta),\label{apMS}
\end{align}
In words, the predicate associated with \eqref{apMS} is true at time $t$ if the probability of robot $j$ being within distance less than $r$ from at least one landmark with class $c$ is greater than $1-\delta$. Additional predicates can be defined using e.g., the entropy of the discrete distributions or risk measures defined over the semantic map. For simplicity, in what follows, we restrict our attention on predicates of the form \eqref{ap1}-\eqref{apMS}. We can also introduce atomic predicates defined over the robots states and the known geometric structure that have been widely used in the literature (e.g., atomic predicates that are true if a robot is within a known region of interest). For simplicity of presentation, we abstain from defining such atomic propositions. Finally, given a finite set of available parameters $\Delta$, we define atomic predicates of the form \eqref{ap1}-\eqref{apMS} that are collected in a set $\mathcal{AP}$.

\subsubsection{Syntax \& Semantics}
Given a set $\mathcal{AP}$ of perception-bases atomic predicates, we construct a mission specification expressed in co-safe LTL, which is satisfied by a finite-length robot trajectory. The syntax of co-safe LTL over sequences of robot states and uncertain semantic maps is defined as follows.

%in this paper the map distribution is updated allowing the robots to actively decrease the map uncertainty so that the assigned mission is satisfied.
%\footnote{Note that in \cite{kantaros2019optimal} paths satisfying $\phi$ may not exist given the initial map distribution and the parameters $\delta$ and $r$ in \eqref{apIROS}. To the contrary, in this paper the map distribution is updated allowing the robots to actively decrease the map uncertainty so that the assigned mission is satisfied.}
\begin{definition}[Syntax]\label{syntax}
The syntax of co-safe LTL over a sequence of multi-robot states $\bbp(t)$ and uncertain semantic maps $\ccalM(t)$ is defined as $\phi::=\text{true}~|~\pi_p~|~\neg\pi_p~|~\phi_1\wedge\phi_2~|~\phi_1\vee\phi_2~|~\phi_1~\mathcal{U}~\phi_2,$
%\begin{equation}%~\pi_g~
%\phi::=\text{true}~|~\pi_p~|~\neg\pi_p~|~\phi_1\wedge\phi_2~|~\phi_1\vee\phi_2~|~\phi_1~\mathcal{U}~\phi_2,\nonumber
%\end{equation}
where % (i) $\pi_g$ is a geometric-based predicate depending on the  multi-robot state $\bbp(t)$ and the known geometric structure of the environment; (ii) 
(i) $\pi_p$ is a perception-based predicate defined in \eqref{eq:pip} and (ii) $\wedge$, $\vee$, $\neg$, and $\mathcal{U}$, denote the conjunction, disjunction, negation, and until operator, respectively.
\end{definition}
%
Note that using the `until' operator, the eventually operator, denoted by $\Diamond$, can be defined, as well \cite{baier2008principles}. 

Next, we define the semantics of co-safe LTL over sequences of multi-robot states and semantic maps. We first define a labeling function $L:\Omega^N\times\ccalM(t)\rightarrow 2^{\mathcal{AP}}$ determining which atomic propositions are true given the current robot system state $\bbp(t)\in\Omega^N$ and the current map distribution $\ccalM(t)$ obtained after applying a sequence of control actions $\bbu_{0:t}$.

\begin{definition}[Semantics]\label{semantics}
Let $\sigma=\sigma(0),\sigma(1)\dots$ be an finite sequence of multi-robot states and uncertain semantic maps, where $\sigma(t)=L([\bbp(t),\ccalM(t)])$. The semantics of temporal logic over robot states and semantic maps is defined recursively as:
\begin{align}
&\sigma\models\text{true} \nonumber\\
%&s \models \pi_g \Leftrightarrow \bbp(0)\models\pi_g \nonumber\\
&\sigma\models \pi_p(\bbp,\ccalM,\Delta) \Leftrightarrow p(\underbrace{\bbp(0),\ccalM(0)}_{\text{from~}\sigma(0)},\Delta)\geq 0 \nonumber\\
%&s\models\neg\phi \Leftrightarrow \neg(s\models\phi) \nonumber\\
&\sigma\models \phi_1\wedge\phi_2 \Leftrightarrow (\sigma\models\phi_1)\wedge(\sigma\models\phi_2) \nonumber\\
&\sigma\models \phi_1\vee\phi_2 \Leftrightarrow (\sigma\models\phi_1)\vee(\sigma\models\phi_2) \nonumber\\
&\sigma\models \phi_1\ccalU\phi_2 \Leftrightarrow \exists~t\geq 0~\text{s.t.}~\{\sigma(t)\sigma(t+1)\dots\models\phi_2\}\nonumber\\& \wedge\{\sigma(t')\sigma(t'+1)\dots\models\phi_1\},~\forall 0\leq t'<t.\nonumber
\end{align}
\end{definition}
%Hereafter, we assume that the assigned task $\phi$ is expressed as a \textit{co-safe} formula defined over a set of atomic propositions, denoted by $\mathcal{AP}$, which is satisfied by a finite-length robot trajectory. 
%To interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\Omega^N\times\ccalM(t)\rightarrow 2^{\mathcal{AP}}$ determining which atomic propositions are true given the current robot system state $\bbp(t)\in\Omega^N$ and the current map distribution $\ccalM(t)$ obtained after applying a sequence of control actions $\bbu_{0:t}$.
%, where $\mathcal{AP}$ is a set of atomic predicates of the form \eqref{ap1}-\eqref{apMS}. This labeling function d
%%%%%%%%%%%%%%


\begin{ex}[Mission Specification]\label{ex:LTL}
%\textcolor{red}{[TO BE UPDATED]}
Consider a single-robot mission defined over a semantic map modeled as two landmarks with available classes $\ccalC=\{\text{`Pole'},\text{`Person'}\}$. The robot has to eventually reach a person of interest to deliver supplies while always avoiding colliding with a pole; see e.g., Figure \ref{fig:PF1}. This task can be captured by the following co-safe LTL formula:%; see also Figure \red{(??)}:
%\begin{subequations}
\begin{align}\label{eq:taskEx}
    \phi = &[\Diamond\pi_p(\bbp(t),\ccalM(t),\{1,r_1,\delta_1,\text{`Person'}\})]\\&\wedge[\neg\pi_p(\bbp(t),\ccalM(t),\{1,r_2,\delta_2,\text{`Pole'}\})\nonumber\\&\ccalU \pi_p(\bbp(t),\ccalM(t),\{1,r_1,\delta_1,\text{`Person'}\})]\nonumber
\end{align}
%\end{subequations}
where the atomic predicates are defined as in \eqref{apMS}.
%This specification requires robot $1$ to (i) \textit{eventually}, with probability greater than or equal to $\delta_1$, be within distance $r_1$ from a landmark with class \texttt{Hostage}  in order e.g., to provide supplies (see \eqref{subtask1}) and (ii) \textit{eventually} be confident enough about the position of both landmarks that exist in the environment (see \eqref{subtask2}) and (ii) to always maintain a safe distance $r_2$ from landmarks that are estimated to be hostile (see \eqref{subtask4}).
\end{ex}
%
\subsection{Safe Planning over Uncertain Semantic Maps}
Given a task specification $\phi$, an uncertain prior belief about the semantic map (see Assumption \ref{as:prior}), the observation model \eqref{eq:measModelR}, and the robot dynamics \eqref{eq:rdynamics}, our goal is to select a stopping horizon $H$ and a sequence $\bbu_{0:H}$ of control inputs $\bbu(t)$, for all $t\in\set{0,\dots,H}$, that satisfy $\phi$ while minimizing a user-specified motion cost function. This gives rise to the following optimal control problem:
\begin{subequations}
\label{eq:Prob2}
\begin{align}
& \min_{\substack{H, \bbu_{0:H}}} \left[J(H,\bbu_{0:H}) = \sum_{t=0}^{H}  c(\bbp(t),\bbp(t+1)) \right] \label{obj2}\\
& \ \ \ \ \ \ \  [\bbp_{0:H},\ccalM_{0:H}]\models\phi  \label{constr1b} \\
& \ \ \ \ \ \ \   \bbp(t) \in \Omega_{\text{free}}^N, \label{obsFree}\\
%& \ \ \ \ \ \ \ \bbx(t+1) = \bbg(\bbx,\bbw(t))\label{constr2}\\
& \ \ \ \ \ \ \   \bbp(t+1) = \bbf(\bbp(t),\bbu(t)) \label{constr3b}\\
%& \ \ \ \ \ \ \  \bby^d=\bbm_{\bbx}(\bbp(t),\bbx,\bbv(t)) \label{constr4}\\
%& \ \ \ \ \ \ \  [\bby^c, \bbs^c]=\bbm_c(\bbc) \label{constr5}\\
& \ \ \ \ \ \ \ \hat{\bbx}(t+1)=\hat{\bbx}(0) \label{constr6b}\\
&  \ \ \ \ \ \ \  \Sigma(t+1)=\rho(\Sigma(t),\bbp(t+1)) \label{constr7b}\\
&  \ \ \ \ \ \ \  d(t+1)=d(0) \label{constr8}
\end{align}
\end{subequations}
where the constraints \eqref{constr3b}-\eqref{constr8} hold for all time instants $t\in[0,H]$. In \eqref{obj2}, any motion cost function $c(\bbp(t),\bbp(t+1))$ can be used associated with the transition cost from $\bbp(t)$ to $\bbp(t+1))$ as long as it is positive (e.g., traveled distance). If non-positive summands are selected, then \eqref{eq:Prob2} is not well-defined, since the  optimal terminal horizon $H$ is infinite. The constraints \eqref{constr1b}-\eqref{obsFree} require the robots to accomplish the mission specification $\phi$ and always avoid the known obstacles/walls respectively. With slight abuse of notation, in \eqref{constr1b}, $[\bbp_{0:H},\ccalM_{0:H}]$ denotes a finite sequence of length/horizon $H$ of multi-robot states and semantic maps while $[\bbp_{0:H},\ccalM_{0:H}]\models\phi$ means that the symbols generated along this finite sequence satisfy $\phi$ (see also Definition \ref{semantics}). The constraint \eqref{constr3b} requires the robots to move according to their known dynamics \eqref{eq:rdynamics}. Also, the constraints in \eqref{constr6b}-\eqref{constr7b} require the metric uncertainty to be updated as per the Kalman filter Ricatti map, discussed in Section \ref{sec:updateMap}, while the semantic uncertainty is not updated during the control synthesis process captured by \eqref{constr8}; instead, as it will be discussed in Section \ref{sec:samplingAlg}, it is updated online as semantic measurements are collected as per \eqref{eq:measModelC}.
%Recall that satisfaction of $\phi$ depends on the sequence semantic maps $\ccalM(t)$, $t\in[0,\dots,H]$ while the constraints \eqref{constr6b}-\eqref{constr8b} capture the evolution of the (estimated/predicted) semantic map $\ccalM(t)$. 
Then, the problem addressed in the work done in this rotation can be summarized as follows:
\begin{problem} \label{prob}
Given (i) an initial robot configuration $\bbp(0)$, (ii) a prior distribution of maps $\ccalM(0)$ (see Assumption \ref{as:prior}), (iii) a linear sensor model \eqref{eq:measModelR}, and (iv) a task  captured by a co-safe formula $\phi$, compute a horizon $H$ and compute control inputs $\bbu(t)$ for all time instants $t\in\{0,\dots,H\}$ as per \eqref{eq:Prob2}.
\end{problem}

%known environmental geometry; and (iii)

\begin{rem}[Online Re-planning \& Object Recognition]\label{rem:objRec}
The object recognition method modeled in \eqref{eq:measModelC} is not required to solve \eqref{eq:Prob2} as, therein, the semantic uncertainty is not updated. In fact, \eqref{eq:Prob2} is an offline problem yielding open-loop/offline robot paths that are agnostic to the object recognition model \eqref{eq:measModelC}. A sampling-based algorithm to solve \eqref{eq:Prob2} is presented in Sections \ref{sec:sampling}-\ref{sec:constructTree}. The online execution of these paths is discussed in Section \ref{sec:replan}. Specifically, in that section, we discuss when the offline synthesized paths may need to be revised online to adapt to the semantic map that is continuously learned using perceptual feedback captured by \eqref{eq:measModelR}-\eqref{eq:measModelC}; see Figure \ref{fig:overview}, as well.
%to solve \eqref{eq:Prob2} along with a method to revise paths online are presented in Section \ref{sec:samplingAlg} and they are illustrated
\end{rem}

\begin{rem}[Arbitrary LTL formulas]
Recall that the optimal control problem \eqref{eq:Prob2} generates a finite sequence of control actions that satisfies a co-safe LTL specification. Arbitrary LTL formulas can be considered, as well, which, however, are satisfied by infinite-length paths.
%
%To synthesize a feasible infinite-length path, an infinite horizon optimal control problem, along the lines of \eqref{eq:Prob2}, needs to be solved. 
Nevertheless, infinite-length paths cannot be manipulated in practice. Typically, to mitigate this issue, these paths are expressed in a prefix-suffix form, where the prefix path is executed once followed by the indefinite execution of the suffix path; see e.g., \cite{kantaros2018text}. Following this approach, to account for arbitrary LTL formulas, two separate optimal control problems, which have a similar form to \eqref{eq:Prob2}, can be defined where the first one generates a (finite) prefix path while the second one generates the corresponding (finite) suffix path. Both optimal control problems can be solved by the proposed sampling-based approach.
%
In this report, for simplicity, we consider only co-safe LTL formulas that are satisfied by finite-horizon paths.
\end{rem}

%that the landmarks are static and that the observation model \eqref{eq:measModelR} is linear is provided in Section \ref{sec:extensions}. %Finally, throughout the paper we make the following assumption that is required for applying a Kalman filter.% and the underlying communication network between the robots.
%\begin{assumption} \label{as:assumption}%[State Model]
%The dynamics of the state $\bbx(t)$ and the control input $\bba(t)$ in \eqref{eq:dynamics}, 
%The observation model \eqref{eq:measModelR} and the covariance matrix $\bbR(t)$ of the measurement noise   are known.  
%\end{assumption}

% In order to interpret an LTL formula over the trajectories of the robot system, we use a labeling function $\ccalL:\Omega^N\times\ccalM\rightarrow \Sigma$ that determines which atomic propositions are true given the current robot system state $\bbp(t)\in\Omega^N$ and the distribution of maps $\ccalM$.

%\begin{equation}\label{ap1}
%\pi_j^i(r,\delta): \mathbb{P}(||\bbp_j-\bbx_i||\leq r)\geq 1-\delta, 
%\end{equation}
%
%\begin{equation}\label{ap2}
%\pi_j^{\ell_i}(r,\delta,\ccalC_m): \mathbb{P}(||\bbp_j-\bbx_i||\leq r)\geq 1-\delta, c_i\in\bar{\ccalC}\subseteq\ccalC
%\end{equation}

%\begin{equation}\label{ap4}
%\pi_j^{\ell_i}(r,\delta,\zeta,\ccalC_m): [\mathbb{P}(||\bbp_j-\bbx_i||\leq r)\geq 1-\delta]\wedge \det\Sigma_i\leq\zeta, c_i\in\bar{\ccalC}\subseteq\ccalC
%\end{equation}
%
%\begin{equation}\label{ap3}
%\pi_j(\delta, \ccalR): \bbp_i\in\ccalR\subseteq\Omega.
%\end{equation}




%\section{Probabilistic Map Temporal Logic}

%The map uncertainty in problem \eqref{eq:Prob12} leads to uncertainty in the evaluation of the atomic propositions and hence to uncertainty in the robot trajectory labeling. Moreover, due to map uncertainty the DFA state cannot be observed. Instead of solving the optimal control problem  \eqref{eq:Prob12} with partial observability, we propose an alternative solution that allows us to convert  \eqref{eq:Prob12}  into a deterministic optimal control problem with full observability that we can solve efficiently and still provide a correctness guarantee. This avoids the need for employing available techniques to solve POMDP problems that are computationally expensive \cite{agha2014firm,vasile2016control}. To this end, motivated by the Gaussian Distribution Temporal Logic (GDTL) proposed in \cite{vasile2016control} for control in belief space, we introduce the Probabilistic Map Temporal Logic (PMTL) for control in probabilistic maps. The syntax of PMTL is defined as follows:




==> files/PF_short_v3.tex <==

% ------------------------------------------------------------------------------- %
\subsection{Robot, Environment, \& Sensor Model}
Consider $N$ mobile robots governed by the following dynamics: $\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t))$,
%
%\begin{equation}\label{eq:rdynamics}
%\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t)),
%\end{equation}
for all $j\in\ccalN:=\{1,\dots,N\}$, where $\bbp_{j}(t) \in\Omega\subseteq\mathbb{R}^n$ stands for the state (e.g., position and orientation) of robot $j$ in an environment $\Omega$ at discrete time $t$, $\bbu_{j}(t) \in\ccalU_j$ stands for a control input in a \textit{finite} space of admissible controls $\ccalU_j$. %\NA{state that time is discrete}
%Note that the state $\bbp_{j}$ may belong to a higher dimensional space than $\Omega_{\text{free}}$. For example, this is the case if $\bbp_j(t)$ includes the position and the orientation of robot $j$. Nevertheless, throughout the rest of the paper, for simplicity of notations we denote $\bbp_{j}(t) \in \Omega_{\text{free}}$.\BS{Can we make this into a  remark or just remove it? It's extra clutter for something that is fairly straightforward.} 
%Also, note that the considered dynamics can range from simple graph-based dynamics to arbitrary nonlinear discrete dynamics\NA{This sentence could be removed}. 
Hereafter, we compactly denote the dynamics of all robots as
\begin{equation}\label{eq:rdynamics}
\bbp(t+1)=\bbf(\bbp(t),\bbu(t)),
\end{equation}
where $\bbp(t)\in \Omega^N$, $\forall t\geq 0$, and $\bbu(t)\in\ccalU:=\ccalU_1\times\dots\times\ccalU_N$.

The robots operate in a environment modeled by a semantic map $\ccalM=\{\ell_1,\ell_2,\dots,\ell_M\}$ consisting of $M$ static landmarks. Each landmark $\ell_i=\{\bbx_i(t),c_i\}\in\ccalM$ is defined by its position $\bbx_i\in \Omega$ and its class $c_i\in\ccalC$, where $\ccalC$ is a finite set of classes. Hereafter, we assume that the landmarks are static with known classes. A discussion on relaxing these assumptions is presented in Section \ref{sec:relax}. On the other hand, the robots do not know the true landmark positions but instead they initially have access to a probability distribution $\ccalM(t)$ over the space of all possible maps. 
%
Such a distribution can be user-specified initially and it can be updated by a SLAM algorithm and typically consists of a Gaussian distribution over the
landmark positions. Specifically, we assume that $\ccalP(t)$ is determined by parameters $(\hat{\bbx}_i(t),\Sigma_i(t))$, for all landmarks $\ell_i$, such that $\bbx_i\sim\ccalN(\hat{\bbx}_i(t),\Sigma_i(t))$, where $\hat{\bbx}_i(t)$ and $\Sigma_i(t)$ denote the estimated mean and covariance matrix of the position of landmark $i$. Hereafter, we compactly denote by $(\hat{\bbx}(t),\Sigma(t))$ the parameters that determine $\ccalP(t)$. 


Moreover, the robots are equipped with sensors to collect measurements associated with $\bbx(t)$ as per the \textit{observation model}: $\bby_j(t) = \bbg_j(\bbp_j(t),\bbx, \bbv_j(t))$, where $\bby_j(t)$ is the measurement signal at discrete time $t$ taken by robot $j\in\ccalN$ that e.g., consists of a range (or bearing) measurements. Also, $\bbv_j(t) \sim \ccalN(\bb0, \bbR_j(t) )$ is sensor-state-dependent Gaussian noise with covariance $\bbR_j(t)$. %Linear observation models have been used, e.g., in \cite{bennetts2013towards} to estimate a gas concentration field.
Hereafter, we compactly denote the observation models of all robots as 
\begin{equation} \label{eq:measModel}
\bby(t)= \bbg(\bbp(t),\bbx,\bbv(t)),~\bbv(t) \sim \ccalN(\bb0, \bbR(t) ).
\end{equation}

\subsection{Temporal Logic Tasks over Uncertain Maps}
The goal of the robots is to accomplish a complex collaborative task captured by a global Linear Temporal Logic (LTL) specification $\phi$. To account for environmental and sensing uncertainty, we extend LTL by including probabilistic atomic predicates with the following syntax.
\begin{definition}[Syntax]\label{syntax}
The syntax of Linear Temporal Logic with probabilistic predicates is defined as 
\begin{equation}
\phi::=\text{true}~|~\pi~|~g(\bbp(t),\ccalP(t))\geq0~|~\phi_1\wedge\phi_2~|~\neg\phi~|~\phi_1~\mathcal{U}~\phi_2,\nonumber
\end{equation}
where $\pi$ is a predicate over the robot state $\bbp(t)$, and $g(\bbp(t),\ccalP(t))\geq0$ is a predicate over the robot state $\bbx(t)$ and the map distribution $\ccalP(t)$, where $g(\bbp(t),\ccalP(t)): \Omega^N\times\ccalP(t)\rightarrow\mathbb{R}$.
\end{definition}

An example of an atomic predicate $\pi$ defined over the robot states $\bbp(t)$ is 
%\begin{subequations}
\begin{align}
\pi_j(\ccalR): \bbp_j\in\ccalR\subseteq\Omega,\label{ap0} %\\
%&\pi_{\ell_i}(\Sigma_i(t|\bby_{0:t}^d),\zeta):\det\Sigma_i(t|\bby_{0:t}^d)\leq\zeta. \label{ap3a}
\end{align}
%\end{subequations}
where $\pi_j(\ccalR)$ is true only if robot $j$ is within a region $\ccalR$. %Similarly, in \eqref{ap3a}, $\pi_{\ell_i}(\Sigma_i(t|\bby_{0:t}^d),\zeta)$ is true if the uncertainty of the position of landmark $\ell_i$, captured by the determinant of the (a-posteriori) covariance matrix $\Sigma_i(t|\bby_{0:t}^d)$, denoted by $ \det\Sigma_i(t|\bby_{0:t}^d)$, is less than a user-specified parameter $\zeta\geq 0$ after fusing the semantic measurements $\bby_{0:t}^d$.
Moreover, given a map distribution $\ccalP(t)$, in this paper we consider atomic predicates $g(\bbp(t),\ccalP(t))\geq 0$ that reason about the uncertainty of the workspace defined as follows:
\begin{subequations}
\begin{align}
&g(\bbp_j(t),\ell_i,r,\delta)\geq 0: ~~\mathbb{P}(||\bbp_j(t)-\bbx_i||\leq r)\geq 1-\delta,\label{ap1} \\
&g(\Sigma_i(t|\bby_{0:t}),\delta)\geq 0:~~~ \det(\Sigma_i(t|\bby_{0:t}))\leq \delta. \label{apS} 
\end{align}
\end{subequations}
%where $t\geq t'$.
The predicate \eqref{ap1} is true at time $t$ if the probability of robot $j$ being within distance less than $r$ from landmark $\ell_i$ is greater than $1-\delta$, after fusing all measurements $\bby_{0:t}$, for some user-specified parameters $r,\delta>0$. Note that to compute the probability in \eqref{ap1}, only the Gaussian distribution of $\bbx_i(t)$ and the robot position $\bbp_j(t)$ are required. Similarly, \eqref{apS} is true of the determinant of the covariance matrix associated with landmark $\ell_i$ is less than a user-specified threshold $\delta$ after fusing the range measurements taken by all robots up to time $t$ using e.g., a Kalman filter. The latter predicate allows us to reason about the uncertainty associated with target $i$; the smaller the $\delta$ is, the smaller the uncertainty (captured by $\det(\Sigma_i(t|\bby_{0:t}))$) about landmark $i$ should be. Note that additional predicates can be defined using e.g., risk measures.


Using these predicates, we define temporal logic tasks over probabilistic semantic maps. For instance, consider a search-and-rescue task where $c_1=\texttt{Hostage}$ and $c_2=\texttt{Hostile}$ captured by the following temporal logic formula:%; see also Figure \red{(??)}:
\begin{subequations}
\begin{align}
    \phi = &\Diamond\{[g(\bbp_j(t),\ell_1,r_1,\delta_1)\geq 0]\label{subtask1}\\
    &\wedge[g(\Sigma_1(t|\bby_{0:t}),\delta)\geq 0]\label{subtask2}\\
    &\wedge \{(\neg g(\bbp_j(t),\ell_2,r_2,\delta)\geq 0)\}.\label{subtask4}
\end{align}
\end{subequations}
This specification requires a robot $j$ to (i) \textit{eventually}  approach a target $\ell_1$ with class \texttt{Hostage} in order e.g., to provide supplies (see \eqref{subtask1}) and at the same time be confident enough about the position of this landmark (see \eqref{subtask2}) and (ii) to always maintain a safe distance $r$ from the hostile landmark $\ell_2$ that is patrolling the environment (see \eqref{subtask4}).

%
The semantics of the proposed specification language over probabilistic semantic maps is defined as follows.
\begin{definition}[Semantics]\label{semantics}
Let $p=[\bbp(0),\ccalP(0)][\bbp(1),\ccalP(1)]\dots$ be an infinite sequence of robot states and semantic maps. The semantics of temporal logic over semantic maps is defined recursively as:
\begin{align}
&p\models\text{true} \nonumber\\
&p \models \pi \Leftrightarrow \bbp(0)\models\pi \nonumber\\
&p\models g\geq 0 \Leftrightarrow g(\bbp(0),\ccalP(0))\geq 0 \nonumber\\
&p\models\neg\phi \Leftrightarrow \neg(p\models\phi) \nonumber\\
&p\models \phi_1\wedge\phi_2 \Leftrightarrow (p\models\phi_1)\wedge(p\models\phi_2) \nonumber\\
&p\models \phi_1\ccalU\phi_2 \Leftrightarrow \exists~t\geq 0~\text{s.t.}~\\&\{[\bbp(t),\ccalP(t)][(\bbp(t+1),\ccalP(t+1))]\dots\models\phi_2\} \nonumber\\
&\wedge\{[\bbp(t'),\ccalP(t')][\bbp(t'+1),\ccalP(t'+1)]\dots\models\phi_1\},~\forall 0\leq t'<t.\nonumber
\end{align}
\end{definition}

Hereafter we assume that the assigned task $\phi$ is expressed as a \textit{co-safe} formula defined over a set of atomic propositions $\mathcal{AP}$, which is satisfied by a finite-length robot trajectory. In order to interpret a temporal logic formula over the trajectories of the robot system, we use a labeling function $L:\Omega^N\times\ccalP(t)\rightarrow 2^{\mathcal{AP}}$ that determines which atomic propositions are true given the current robot system state $\bbp(t)\in\Omega^N$ and the current map distribution $\ccalP(t)$ obtained after fusing all robot measurements.
%%%%%%%%%%%%%%

\subsection{Mission Planning Problem in Probabilistic Semantic Maps}


Given a task specification $\phi$, our goal is to select a stopping time $H$ and a sequence $\bbu_{0:H}$ of control inputs $\bbu(t)$, for all $t\in\set{0,\dots,H}$, that satisfy $\phi$ while minimizing a user-specified motion cost function. This gives rise to the following stochastic optimal control problem:

\begin{subequations}
\label{eq:Prob1}
\begin{align}
& \min_{\substack{H, \bbu_{0:H}}} \left[J(H,\bbu_{0:H}) = \sum_{t=0}^{H}  c(\bbp(t),\bbp(t+1)) \right] \label{obj1}\\
& \ \ \ \ \ \ \  [\bbp_{0:H},\ccalP_{0:H}]\models\phi  \label{sat1} \\
& \ \ \ \ \ \ \   \bbp(t+1) = \bbf(\bbp(t),\bbu(t)) \label{rdyn1}\\
& \ \ \ \ \ \ \ P(t+1|\bby_{0:t+1})=K(P(t|\bby_{0:t}), \bby_{t+1}) \label{map1}\\
& \ \ \ \ \ \ \  \bby=\bbm(\bbp(t),\bbx(t),\bbv(t)) \label{meas1}\\
%& \ \ \ \ \ \ \ \hat{\bbx}(t+1|\bby_{0:t+1}^r)=U(\hat{\bbx}(t|\bby_{0:t}^r)) \label{constr6}\\
%&  \ \ \ \ \ \ \  \Sigma(t+1|\bby_{0:t+1}^r)=\rho(\Sigma(t|\bby_{0:t}^r),\bbp_{t+1}) \label{constr7}\\
%&  \ \ \ \ \ \ \ d_c(t+1|\bby_{0:t+1}^c, \bbs_{0:t+1}^c)=B(d_c(t|\bby_{0:t}^c),\bbs_{0:t}^c) \label{constr8}
\end{align}
\end{subequations}
The objective function \eqref{obj1} captures an accumulated motion cost objective, such as total traveled distance. The first constraint in \eqref{sat1} requires the robot trajectory from $t=0$ until $t=H$ along with the corresponding sequence of semantic maps, denoted by $[\bbp_{0:H},\ccalP_{0:H}]$, to satisfy the assigned specification $\phi$. The constraint \eqref{rdyn1} capture the robot dynamics while \eqref{map1} captures the map update using a Kalman filter, denoted by $K$, after fusing the collected measurements; however, any other inference method can be used.  The last constraint constraints requires measurements to be generated by the mesaurement model defined in \eqref{eq:measModel}.
%
%In particular, the sixth constraint in \eqref{constr6} requires the estimate of the target positions to be updated using the Kalman-filter update step; however, any other inference method can be used. Similarly, the seventh constraint in \eqref{constr7} requires the covariance matrix associated with the landmark positions to be updated as per the Kalman filter Ricatti map when new range measurements are collected. The last constraint in \eqref{constr6} requires that the class distribution is updated using the class-related meausurements $\bby_{0:t}^c$, as per a Bayes filter .%
%

\subsection{Problem Reformulation}

Note that \eqref{eq:Prob2} is a stochastic optimal control problem with partial observability and asks for closed-loop control policies. To avoid employing computationally expensive methods, such as POMDP-based methods, we reformulate it as a deterministic optimal control problem that asks for open-loop control policies. Specifically, given a linear observation model \eqref{eq:measModelR} in terms of the hidden state $\bbx(t)$, the a-posteriori covariance matrix in \eqref{constr7} can be computed offline i.e., without requiring knowledge of the measurements $\bby_{0:t}^r$ \cite{atanasov2015decentralized}. In this case, the covariance matrix $\Sigma(t)$ can be computed  


To this end, first we replace the Kalman-filter update-step \eqref{constr6} with the Kalman-filter prediction step, i.e.,  $\hat{\bbx}(t+1)=\bbg(\hat{\bbx}(t),\bba(t))$ (i.e., process noise is ignored). Second, note that for linear landmark dynamics and a linear observation model \eqref{eq:measModelR} in terms of the hidden state $\bbx(t)$, the a-posteriori covariance matrix in \eqref{constr7} can be computed offline i.e., without requiring knowledge of the measurements $\bby_{0:t}^r$ \cite{atanasov2015decentralized}. Therefore, in this case, we can replace \eqref{constr7} with $\Sigma(t+1)=\rho(\Sigma(t),\bbp(t+1))$. Finally, since we are interested in open-loop control policies, we replace the last constraint \eqref{constr8} with $d_c(t+1)=d_c(t)$, i.e., class-related measurements are ignored. Thus, we reformulate the \eqref{eq:Prob2} into the following deterministic optimal control problem that does not depend on any hidden variables.
%Specifically, by considering a linearized observation model for \eqref{eq:measModelR} about the current robot states, we can compute the a-posteriori covariance matrices offline, i.e., without requiring knowledge of the measurements $\bby_{0:t}^d$ \cite{atanasov2015decentralized}. 

\begin{subequations}
\label{eq:Prob2}
\begin{align}
& \min_{\substack{H, \bbu_{0:H}}} \left[J(H,\bbu_{0:H}) = \sum_{t=0}^{H}  c(\bbp(t),\bbp(t+1)) \right] \label{obj2}\\
& \ \ \ \ \ \ \  [\bbp_{0:H},\ccalP_{0:H}]\models\phi  \label{constr1b} \\
%& \ \ \ \ \ \ \ \bbx(t+1) = \bbg(\bbx,\bbw(t))\label{constr2}\\
& \ \ \ \ \ \ \   \bbp(t+1) = \bbf(\bbp(t),\bbu(t)) \label{constr3b}\\
%& \ \ \ \ \ \ \  \bby^d=\bbm_{\bbx}(\bbp(t),\bbx,\bbv(t)) \label{constr4}\\
%& \ \ \ \ \ \ \  [\bby^c, \bbs^c]=\bbm_c(\bbc) \label{constr5}\\
& \ \ \ \ \ \ \ \hat{\bbx}(t+1)=\hat{\bbx}(0) \label{constr6b}\\
&  \ \ \ \ \ \ \  \Sigma(t+1)=\rho(\Sigma(t),\bbp(t+1)) \label{constr7b}
\end{align}
\end{subequations}

%Recall that satisfaction of $\phi$ depends on the sequence semantic maps $\ccalP(t)$, $t\in[0,\dots,H]$ while the constraints \eqref{constr6b}-\eqref{constr8b} capture the evolution of the (estimated/predicted) semantic map $\ccalP(t)$. 
Then, the problem addressed in this paper can be summarized as follows:
\begin{problem} \label{prob}
Given (i) an initial robot configuration $\bbp(0)$, (ii) an initial distribution of maps $\ccalP(0)$, (iii) a task specification captured by a co-safe formula $\phi$, compute a horizon $H$ and compute control inputs $\bbu(t)$ for all time instants $t\in\{0,\dots,H\}$ as per \eqref{eq:Prob2}.
\end{problem}

Finally, throughout the paper we make the following assumption that is required for applying a Kalman filter.% and the underlying communication network between the robots.
\begin{assumption} \label{as:assumption}%[State Model]
%The dynamics of the state $\bbx(t)$ and the control input $\bba(t)$ in \eqref{eq:dynamics}, 
The observation model \eqref{eq:measModelR}, and process and measurement noise covariances $\bbQ(t)$ and $\bbR(t)$ are known.  
\end{assumption}

% In order to interpret an LTL formula over the trajectories of the robot system, we use a labeling function $\ccalL:\Omega^N\times\ccalP\rightarrow \Sigma$ that determines which atomic propositions are true given the current robot system state $\bbp(t)\in\Omega^N$ and the distribution of maps $\ccalP$.

%\begin{equation}\label{ap1}
%\pi_j^i(r,\delta): \mathbb{P}(||\bbp_j-\bbx_i||\leq r)\geq 1-\delta, 
%\end{equation}
%
%\begin{equation}\label{ap2}
%\pi_j^{\ell_i}(r,\delta,\ccalC_m): \mathbb{P}(||\bbp_j-\bbx_i||\leq r)\geq 1-\delta, c_i\in\bar{\ccalC}\subseteq\ccalC
%\end{equation}

%\begin{equation}\label{ap4}
%\pi_j^{\ell_i}(r,\delta,\zeta,\ccalC_m): [\mathbb{P}(||\bbp_j-\bbx_i||\leq r)\geq 1-\delta]\wedge \det\Sigma_i\leq\zeta, c_i\in\bar{\ccalC}\subseteq\ccalC
%\end{equation}
%
%\begin{equation}\label{ap3}
%\pi_j(\delta, \ccalR): \bbp_i\in\ccalR\subseteq\Omega.
%\end{equation}




%\section{Probabilistic Map Temporal Logic}

%The map uncertainty in problem \eqref{eq:Prob12} leads to uncertainty in the evaluation of the atomic propositions and hence to uncertainty in the robot trajectory labeling. Moreover, due to map uncertainty the DFA state cannot be observed. Instead of solving the optimal control problem  \eqref{eq:Prob12} with partial observability, we propose an alternative solution that allows us to convert  \eqref{eq:Prob12}  into a deterministic optimal control problem with full observability that we can solve efficiently and still provide a correctness guarantee. This avoids the need for employing available techniques to solve POMDP problems that are computationally expensive \cite{agha2014firm,vasile2016control}. To this end, motivated by the Gaussian Distribution Temporal Logic (GDTL) proposed in \cite{vasile2016control} for control in belief space, we introduce the Probabilistic Map Temporal Logic (PMTL) for control in probabilistic maps. The syntax of PMTL is defined as follows:




==> files/Sim4mobileTargets.tex <==
\subsection{Temporal Logic Planning in Uncertain and Dynamic Environments}\label{sec:dyn}

Next, we illustrate the performance of Algorithm \ref{alg:RRT} in an environment with mobile landmarks. Specifically, we consider a team of $N=20$ robots with differential drive dynamics, as in \eqref{eq:nonlinRbt} with $\tau=0.1$ secs, that need to accomplish a collaborative task in an environment with the same geometric structure as in Section \ref{sec:scale}. Moreover, there are $M=15$ targets, among which $12$ are governed by noisy linear time invariant dynamics in the form of $\bbx_i(t+1)=\bbA_i\bbx_i(t)+\bbB_i\bba_i(t)+\bbw_i(t)$ (e.g., target $2$) or by Gaussian noise i.e., $\bbx_i(t+1)=\bbx_i(t)+\bbw_i(t)$ (targets $5$, and $11$) while $3$ targets (targets $11$, $12$ and $15$) are static. The trajectories of all targets are shown in Figure \ref{fig:traj}.
As in Section \ref{sec:scale}, the true class of each target is uncertain; instead the robots have access to a discrete distribution $d(0)$ over the labels that is designed by randomly selecting a probability within the range $[0.7,1]$ that a target has the correct label, and by randomly selecting probabilities for the remaining classes.
%$1$ target is a hostile unit that is patrolling the area, and $1$ (static) target corresponds to the exit location of the building i.e., the set of available classes is defined as $\ccalC=\{\texttt{hostage1},\dots,\texttt{hostage13},\texttt{hostile},\texttt{Exit}\}$. The true class of each target is unknown; instead the robots have access to a discrete distribution $d(0)$ over the labels that is designed by randomly selecting a probability within the range $[0.7,1]$ that a target has the correct label, and by randomly selecting probabilities for the remaining classes.

The initial estimates $\hat{\bbx}_i(0)$ of the target states are selected so that $\lVert\hat{\bbx}_i(0)-\bbx_i(0)\rVert\leq 0.25$ while the covariance matrix $\bbQ\in\mathbb{R}^{30\times30}$ of the process noise is a diagonal matrix designed as follows:
\begin{align}
\bbQ=&10^{-3}\times\diag(0.02,0.02, 0.01, 0.2, 0.02,0.1,0.01,0.7,0.7,\nonumber\\&0.04,0.02,0.02,0.1,0.01,0.01,0.1,0.2,0.02,0.02,0,\nonumber\\&0,0,0,0.002,0.02, 0.002,0.02, 0, 0)    
\end{align}
where notice that the process noise for static targets is zero. 

%where the probability that the class of target $i$ is the true one is randomly generated so that it belongs in the interval $[0.7,1)$ and 

The robots are responsible for accomplishing a collaborative task captured by a temporal logic formula $\phi$. To define $\phi$, we first divide the robots into $10$ teams $\ccalT_m$, $m\in\{1,2,\dots,10\}$, as follows:
\begin{itemize}
    %xi1
    \item $\ccalT_1=\{1,2,11,12,13,14,15,16\}$, %hostage1
    %xi2
    \item $\ccalT_2=\{3,4,14\}$,%hostage8 AND
    \item $\ccalT_3=\{5,6,7,15,16,17,18,19\}$,%hostage4
    %xi3
    \item $\ccalT_4=\{1,2,11,12\}$, %hostage 3
    \item $\ccalT_5=\{9,10,19,20\}$, %hostage 6
    %xi4
    \item $\ccalT_6=\{1,4,7,17\}$, %hostage 2
    \item $\ccalT_7=\{12,13,18\}$, %hostage 5
    %xi5
    \item $\ccalT_8=\{9,10\}$, %hostage 8
    \item $\ccalT_9=\{6,8\}$, %hostage 7
    %xi6
    \item $\ccalT_{10}=\{3,4,7,13,15,16\}$. %hostage 9
\end{itemize}

The assigned task is described by the following temporal logic formula which has the same structure as \eqref{eq:task0}.
\begin{align}\label{eq:task1}
\phi &= \Diamond(\xi_{\ccalT_1}^{1}\vee\xi_{\ccalT_1}^{2})%xi1
%
\wedge \Diamond(\xi_{\ccalT_2}^{8}\wedge\xi_{\ccalT_3}^{4})%x2
%
\wedge(\neg (\xi_{\ccalT_1}^{1}\vee\xi_{\ccalT_1}^{2})\ccalU(\xi_{\ccalT_4}^{3}\wedge\xi_{\ccalT_5}^{6}))\nonumber\\
%
&\wedge\{\Diamond[(\xi_{\ccalT_6}^{2}\wedge\xi_{\ccalT_7}^{5})\wedge(\Diamond(\xi_{\ccalT_8}^{8}\wedge\xi_{\ccalT_9}^{7})\wedge(\Diamond(\xi_{\ccalT_{10}}^{9})))]\}\nonumber\\
%
&\wedge\Diamond\square(\xi^{\text{Exit}})\wedge \square( \neg \xi^{\text{obs}}))\wedge\square(\neg \xi^{\text{hostile}})),
%
%\Diamond(\phi_1 \wedge \Diamond(\phi_2 \wedge \Diamond \phi_3))  \wedge (\neg \phi_1 \ccalU \phi_4)\nonumber\\ &\wedge \Diamond(\phi_5) \wedge \square(\neg\phi_6) \wedge \square(\neg\phi_7).\nonumber
\end{align}
where $\xi_{\ccalT_m}^i$ is a Boolean formula that is true if all robots in team $\ccalT_m$ are within $0.2$ meters from target $i$ with probability greater than $0.8$ (see \eqref{ap1}) and the uncertainty about this target is less than 0.01 (see \eqref{apS}). The Boolean formulas $\xi^{\text{Exit}}$, $\xi^{\text{obs}}$, and $\xi^{\text{hostile}}$ are defined as in Section \ref{sec:scale}.

In words, \eqref{eq:task1} requires (i) team $\ccalT_1$ to eventually visit either hostage $1$ or $2$; (ii) sub-task (i) to never happen until teams $\ccalT_4$ and $\ccalT_5$ visit hostages $3$ and $6$, respectively, at the same time; (iii) teams $\ccalT_2$ and $\ccalT_3$ to visit hostages $8$ and $4$, respectively, at the same time; (iv) eventually (iv.1), (iv.2) and (iv.3) to happen in this order, where in (iv.1) teams $\ccalT_6$ and $\ccalT_7$ should visit hostages $2$ and $5$, respectively, at the same time; in (iv.2)  teams $\ccalT_8$ and $\ccalT_9$ should visit hostages $8$ and $7$, respectively, at the same time; (iv.3) team $\ccalT_{10}$ should visit hostage $9$; (v) all robots to always avoid the hostile unit; (vi) all robots to eventually go to the exit of the building and remain there forever; (vii) all robots to always avoid the obstacles. The sub-tasks (i)-(vi) should be satisfied according the uncertainty and probabilistic satisfaction guarantees discussed before.

Algorithm \ref{alg:RRT} generated a sequence of control inputs with terminal horizon $H=421$ in $14.2$ minutes. The resulting trajectories are shown in Figure \ref{fig:traj} and the simulation video can be found in \cite{dynSem}. Observe in this figure that the robots avoid the hostile target $10$ while they learn only the parts of the environment that are necessary to accomplish the assigned task. For instance, none of the robots tries to actively decrease the uncertainty of targets $13$ and $15$ as this is not required by the mission specification in \eqref{eq:task1}.



\begin{figure}[t]
  \centering
 %    \subfigure[$N=1, M=5$ (slow targets)]{
 %   \label{fig:traj15s}
%  \includegraphics[width=0.48\linewidth]{traj_1vs5_slow.pdf}}
\includegraphics[width=0.9\linewidth]{figures/trajDyn.pdf}
\caption{ Robot trajectories that satisfy the LTL task \eqref{eq:task1}. The robots are initially located at the top left corner of the workspace. The green and red squares represent the initial and final locations of the targets while the black paths correspond to the target trajectories (ground truth).}
  \label{fig:traj}
\end{figure}



\subsection{Controlling UAVs over Semantic Cities}

Algorithm \ref{alg:RRT} generates paths that satisfy a given mission specification while respecting the robot dynamics as captured in \eqref{constr3c}. A common limitation of sampling-based algorithms is that the more complex the robot dynamics is, the longer it takes to generate feasible paths; see e.g., \cite{kantaros2019asymptotically}. To mitigate this issue, an approach that we investigate in this section, is to generate paths for simple robot dynamics that need to be followed by robots with more complex dynamics. Particularly, in this section, we present simulation studies that involve a team of $N=5$ AsTech Firefly Unmanned Aerial Vehicles (UAVs) that operate over a city with dimensions $200\times 200$ with $M=5$ landmarks among which four are static and one flies over the city as per noisy linear dynamics; see e.g., Figure \ref{fig:env}. The UAVs are tasked with providing services to injured people and tracking mobile targets while avoiding flying over certain residential areas according. Specifically, the UAVs are respnsible for accomplishing a mission captured by the following LTL formula:
%
%'F(p1) & F(p2) & F(p3) & FG(p4)'
\begin{align}\label{eq:task3}
    \phi=&(\Diamond \xi^1_{\ccalT_1}) \wedge (\Diamond \xi^2_{\ccalT_2}) \wedge (\Diamond \xi^3_{\ccalT_3})\wedge (\Diamond\square (\xi^4_{\ccalT_4}\wedge \xi^5_{\ccalT_5})) \wedge(\square \neg \xi^{\text{res}}), 
\end{align}
where the $\xi_{\ccalT_m}^i$ is a Boolean formula defined as before. In words, \eqref{eq:task3} requires (i) sub-teams $\ccalT_m$ of robots to eventually visit the injured people with index $1$, $2$, $3$ in any order; (ii) the sub-team $\ccalT_4$ to eventually  visit the injured person $4$ and stay there forever and eventually the sub-team $\ccalT_5$ to approach the unknown target $5$ that is flying over the city and stay close to it forever; (iii) all robots to always avoid flying over certain residential areas; see Figure \ref{fig:init1}.

The initial configuration of the robots and the map are shown in Figure \ref{fig:init1} while the nominal paths generated by Algorithm \ref{alg:RRT}, considering the dynamics in \eqref{eq:nonlinRbt},  are illustrated in Figure \ref{fig:final1}. Given the waypoints, generated by Algorithm \ref{alg:RRT}, we compute minimum jerk trajectories, defined by fifth-order polynomials, that connect consecutive waypoints in the nominal paths. To determine the coefficients of this polynomial, we impose boundary conditions on the UAV positions that require the travel time between consecutive waypoints in the nominal paths to be $T=2$ seconds for all UAVs \cite{lavalle2006planning}. The latter ensures that all UAVs will execute the synthesized paths synchronously, as required by proposed method. %; see Figure \ref{fig:sync}. 
%Note that the minimum jerk trajectories are smooth enough for the UAVs to follow.  Observe in Figure \ref{fig:paths} that deviation between the nominal paths generated by Algorithm \ref{alg:RRT} and the minimum jerk paths is quite small. %and, in fact, the latter paths still satisfy the assigned specification.
%
The UAVs are controlled to follow the resulting trajectories using the ROS package developed in \cite{Furrer2016}. The corresponding video along with simulation results involving $N=20$ robots and $M=16$ landmarks can be found in \cite{dynSem2}.


%\red{explain how the paths are executed syncrhonously (add fig) and how you account for uav dynamics}


\begin{figure}[t]
  \centering
    \subfigure[Initial Configuration]{
    \label{fig:init1}
  \includegraphics[width=0.89\linewidth]{figures/init.png}}
      \subfigure[Robot and Target Trajectories]{
    \label{fig:final1}
  \includegraphics[width=0.9\linewidth]{figures/final.png}}
\caption{Case Study $N=5, M=5$: The green block correspond to regions where the UAVs are not allowed to fly over. The red ellipsoids illustrate the uncertainty about the location of static and mobile landmarks of interest. The colored disks represent the sensing range of each drone.}
  \label{fig:gaz5_5m}
\end{figure}

%\begin{figure}[t]
%  \centering
% %    \subfigure[$N=1, M=5$ (slow targets)]{
% %   \label{fig:traj15s}
%%  \includegraphics[width=0.48\linewidth]{traj_1vs5_slow.pdf}}
%\includegraphics[width=1\linewidth]{figures/paths.pdf}
%\caption{Graphical illustration of minimum jerk trajectories (dashed lines) along with the paths (solid lines) generated by Algorithm \ref{alg:RRT}.}
%  \label{fig:paths}
%\end{figure}

%\begin{figure}[t]
%  \centering
% %    \subfigure[$N=1, M=5$ (slow targets)]{
% %   \label{fig:traj15s}
%%  \includegraphics[width=0.48\linewidth]{traj_1vs5_slow.pdf}}
%\includegraphics[width=0.9\linewidth]{figures/cumulative_time.png}
%\caption{ Graphical illustration of the total time required for each UAV to reach the $k$-th waypoint. Notice that all curves are aligned implying that the UAVs execute their paths synchronously.}
%  \label{fig:sync}
%\end{figure}



%To describe the proposed modified algorithm, we need first to introduce the following notation. Specifically, let $q_D(t)$ be the DFA state of the robots at time $t$ initialized as $q_D(0)=q_D^0$.


%Given the deterministic nature of the DFA and the Boolean conditions that enable DFA transitions, we can extract all atomic propositions that if satisfied, the LTL formula will be violated, i.e., no transitions from $q_D(t)$ will be enabled if such atomic propositions are satisfied. Given, such atomic propositions we define the set $\ccalA(t)$ that collects all associated landmarks; see Example \ref{ex:exUn}.



%Next, we follow a similar approach as in \cite{leung2012decentralized,atanasov2015decentralized} to define an exploration strategy that will be incorporated into Algorithm \ref{alg:RRT}. Particularly, we define a grid $C=\{c_1,c_2,\dots,c_L\}$ over the environment where $c_k$ corresponds to the $k$-th grid cell. Then, we split the grid cells into `explored' (i.e., cells that have been visited by the robots) and 'unexplored'. Then, we introduce dummy `exploration' landmarks at the frontiers of the explored grid map. The robots move towards to the unexplored cells until a landmark is detected. Once a landmark $\ell_i$is detected by a robot $j$, a Gaussian and a discrete distribution associated with this landmark are defined.

%this robot checks if there exists an atomic proposition associated with landmark $\ell_i$ that needs to be satisfied to enable a tr

%\begin{example}\label{ex:exUn}
%Note that a combination of atomic propositions may need to be satisfied to violate an LTL formula. For instance, assume that the robot has to always avoid being close enough to two landmarks, \textit{simultaneously}. In other words, being close enough .
%\end{example}


%collect in the set $\ccalA(t)$, the atomic propositions that 
%%



%
%Following a similar approach as in \cite{leung2012decentralized,atanasov2015decentralized}
%To describe the exploration strategy, we define a grid $C=\{c_1,c_2,\dots,c_L\}$ over the environment where $c_k$ corresponds to the $k$-th grid cell. Then, we split the grid cells into `explored' (i.e., cells that have been visited by the robots) and 'unexplored'. Then, we introduce dummy `exploration' landmarks at the frontiers of the explored grid map with a known Gaussian prior on their locations. This fake uncertainty in the exploration-landmark locations promises information gain to the robots. 

%Given these exploration landmarks, Algorithm \ref{alg:RRT} is applied to design informative paths. As the robots follow the designed paths, they update the explored part of the grid world and accordingly introduce new exploration landmarks. If an a-priori unknown landmark is detected, then a Gaussian distribution is assigned to its location. Algorithm \ref{alg:RRT} is applied in an MPC-fashion every few time units, to account for new exploration or actual landmarks that are detected on-the-fly. The algorithm terminates once all grid cells are considered explored and all detected landmarks are localized as per the user-specified uncertainty threshold. \textcolor{blue}{The same idea can be applied to cases pertaining to a \textit{known} number of mobile targets with no prior information. The difference is that in this case the algorithm should terminate when all mobile targets are localized as per a user-specified accuracy and. Note that if the number of mobile targets is unknown, it is non-trivial to design a termination criterion for the proposed algorithm as grid cells of the unknown environment should be visited repetitively to detect potentially new targets.} A simulation study with $2$ robots that are responsible for localizing $13$ fully unknown static landmarks is presented in Figure \ref{fig:unknown}.

==> files/alg.tex <==
%\subsection{Planning for Information Acquisition}
%Solving the planning problem in \eqref{eq:Prob2} in practice can be very challenging particularly because of the temporal logic constraint \eqref{constr1b} and the nonlinear constraints \eqref{constr3b} and \eqref{constr7b}.
In this section we build upon our previous work in perception based planning in uncertain semantic maps \cite{TRO} by extending the work to dynamic environments. The major addition over the previous work is taking into account the motion of the landmarks, predicting their future positions and planning a path accordingly. In this section, first we show that \eqref{eq:Prob2} can be converted into a reachability problem defined over a hybrid and uncertain space; see Section \ref{sec:reach}. In Sections \ref{sec:sampling}-\ref{sec:constructTree}, we present a sampling-based algorithm that can efficiently explore hybrid and uncertain state-spaces and solve Problem \ref{prob}. Then in Section \ref{sec:replan} we discuss the online execution of the synthesized paths and we present a re-planning method to adapt to the continuously learned semantic map; see also Figure \ref{fig:overview}.%Note that reachability planning problems in known and continuous spaces can be solved using existing sampling-based approaches such as RRT \cite{karaman2011sampling} and, therefore, they cannot be directly used to solve the considered problem.
%
\subsection{Reachability in Uncertain Hybrid Spaces}\label{sec:reach}
To convert \eqref{eq:Prob2} into a reachability problem, we first convert the specification $\phi$, defined over a set of atomic predicates $\mathcal{AP}$, into a Deterministic Finite state Automaton (DFA), defined as follows \cite{baier2008principles}. 

\begin{definition}[DFA]
A Deterministic Finite state Automaton (DFA) $D$ over $\Sigma=2^{\mathcal{AP}}$ is defined as a tuple $D=\left(\ccalQ_{D}, q_{D}^0,\Sigma,\delta_D,q_F\right)$, where $\ccalQ_{D}$ is the set of states, $q_{D}^0\in\ccalQ_{D}$ is the initial state, $\Sigma$ is an alphabet, $\delta_D:\ccalQ_D\times\Sigma\rightarrow\ccalQ_D$ is a deterministic transition relation, and $q_F\in\ccalQ_{D}$ is the accepting/final state. 
\end{definition}

Given a robot trajectory $\bbp_{0:H}$ and a corresponding sequence of maps $\ccalM_{0:H}$, we get the labeled sequence $L(\bbp_{0:H}, \ccalM_{0:H}) =L([\bbp(0), \ccalM(0)])\dots L([\bbp(H), \ccalM(H)])$. This labeled sequence satisfies the specification $\phi$, if starting from the initial state $q_D^0$, each symbol/element in $L(\bbp_{0:H}, \ccalM_{0:H})$ yields a DFA transition so that eventually -after $H$ DFA transitions- the final state $q_F$ is reached \cite{baier2008principles}. %With slight abuse of notation we denote this compactly by $q_F=\delta_D(q_D^0,w)$. 
As a result, we can equivalently re-write \eqref{eq:Prob2} as follows:
%\footnote{\textcolor{red}{Not sure if you plan to edit this or if this is th final version but you should be a bit more careful here. The landmarks are moving and during offline planning you predict their future state using their dynamics. The fourth constraint says that you never predict their future states. }}
%
\begin{subequations}
\label{eq:ProbR}
\begin{align}
& \min_{\substack{H, \bbu_{0:H}}} \left[J(H,\bbu_{0:H}) = \sum_{t=0}^{H}  c(\bbp(t),\bbp(t+1)) \right] \label{obj4}\\
& \ \ \ \ \ \ \  q_D(t+1) = \delta_D(q_D(t),\sigma(t)),\label{constr1c}\\
& \ \ \ \ \ \ \   \bbp(t+1) = \bbf(\bbp(t),\bbu(t)) \label{constr3c}\\
& \ \ \ \ \ \ \   \bbp(t) \in \Omega_{\text{free}}^N, \label{obsFree2}\\
& \ \ \ \ \ \ \ \hat{\bbx}(t+1)=\hat{\bbx}(t)+ \label{constr6c}\\
&  \ \ \ \ \ \ \  \Sigma(t+1)=\rho(\Sigma(t),\bbp(t+1)) \label{constr7c}\\
&  \ \ \ \ \ \ \  d(t+1)=d(0) \label{constr8c}\\
&  \ \ \ \ \ \ \  q_D(H)=q_F \label{constr9c}
\end{align}
\end{subequations}
where $q_D(0)=q_D^0$, $\sigma(t)=L([\bbp(t),\ccalM(t)])$ and $\ccalM(t)$ is determined by $\hat{\bbx}(t)$, $\Sigma(t)$, and $d(t)$. Note that the constraint in \eqref{constr1c} captures the automaton dynamics, i.e., the next DFA state that will be reached from the current DFA state under the observation/symbol $\sigma(t)$.
%
In words, \eqref{eq:ProbR}, is a reachability problem defined over a joint space consisting of the automaton state-space (see \eqref{constr1c}), the robot motion space (see \eqref{constr3c}-\eqref{obsFree2}), and the metric uncertainty space (see \eqref{constr6c}-\eqref{constr8c}) while the terminal constraint requires to reach the final automaton state (see \eqref{constr9c}).

%Next, we define the accepting run of a DFA that will be used in Algorithm \ref{alg:RRT}. A run of $\rho_D$ of $D$ over a finite word $\sigma=\sigma(1)\sigma(2)\dots\sigma(K)$, is a sequence $\rho_D=q_D^0q_D^1q_D^2\dots,q_D^K$, where $\delta(q_D^{k},\sigma(k))=q_D^{k+1}$, and $\sigma(k)\in 2^\mathcal{AP}$, $\forall k\in\mathbb{N}$. A run $\rho_D$ is called \textit{accepting} if $q_D^K=q_F$. A sequence of robot states $\bbp_{0:H}$ satisfies $\phi$, i.e., $\bbp_{0:H}\models\phi$, if the word $\sigma=L(\bbp(0),\ccalM(0))L(\bbp(1),\ccalM(1))\dots L(\bbp(H),\ccalM(H))$ yields an accepting DFA run.

\subsection{\textcolor{black}{Sampling-based Planning in Uncertain Semantic Maps}}\label{sec:sampling}

%The reachability problem in \eqref{eq:ProbR} is computationally challenging to solve as it requires to explore a uncertain hybrid state space.
%As discussed before, existing sampling-based approaches, such as $\text{RRT}^*$, \cite{karaman2011sampling,luders2010chance}, cannot directly solve \eqref{eq:ProbR} due to the hybrid state-space that needs to be explored. To address this challenge,  we propose a new sampling-based approach to solve \eqref{eq:ProbR}.\footnote{We note that \cite{karaman2011sampling,luders2010chance} explore different state spaces from the one considered in this paper and, as a result, they cannot be applied directly to solve \eqref{eq:ProbR}. The proposed sampling-based algorithm is conceptually similar to \cite{hsu1997path}; however, \cite{hsu1997path} focuses on reachability tasks in known environments and, therefore, it explores only the robot configuration space. 
%, as they both rely on building trees by following two steps. First, a node in existing tree structure is sampled. Second, the tree is extended to states that lie in the vicinity of the selected tree node. Nevertheless,
%Also, unlike \cite{hsu1997path}, we show that the proposed sampling-based planner is both probabilistically complete and asymptotically optimal.}

%\footnote{We note that the proposed sampling-based planner is similar to \cite{hsu1997path}}
%\footnote{We emphasize that \cite{karaman2011sampling,luders2010chance} explore different state spaces from the one considered in this paper. Also, unlike \cite{csucan2009kinodynamic}, we show that the proposed algorithm is both probabilistically complete and asymptotically optimal.}
%To address these challenges, we propose a new sampling-based algorithm to solve \eqref{eq:Prob2}. Note that several sampling-based methods have been proposed to solve safe planning problems for reachability-avoidance  \cite{karaman2011sampling} or temporal logic specifications \cite{vasile2013sampling,kantaros2018text} in known environments, or for information gathering tasks \cite{kantaros2019asymptotically}. Hereafter, we build upon these methods to solve the temporal logic planning problem in uncertain semantic environments discussed in \eqref{eq:Prob2}. 
In this section, we propose a sampling-based algorithm to solve \eqref{eq:ProbR} which incrementally builds trees that explore simultaneously the robot motion space, the  space of covariance matrices (metric uncertainty), and the automaton space that corresponds to the assigned specification. The proposed algorithm is summarized in Algorithm \ref{alg:RRT}. 

%The proposed algorithm relies on incrementally constructing a directed tree that explores both the robot motion space, the space of semantic maps  $\ccalM(t)$, and the state-space of the DFA $D$ that corresponds to $\phi$. 
In what follows, we provide some intuition for the steps of Algorithm \ref{alg:RRT}. First, we denote the constructed tree by $\mathcal{G}=\{\mathcal{V},\mathcal{E},J_{\ccalG}\}$, where $\ccalV$ is the set of nodes and $\ccalE\subseteq \ccalV\times\ccalV$ denotes the set of edges. The set of nodes $\mathcal{V}$ contains states of the form $\bbq(t)=[\bbp(t), \ccalM(t), q_D(t)]$, where $\bbp(t)\in\Omega$ and $q_D(t)\in\ccalQ_D$.\footnote{Throughout the report, when it is clear from the context, we drop the dependence of $\bbq(t)$ on $t$.} The function $J_{\ccalG}:\ccalV\rightarrow\mathbb{R}_{+}$ assigns the cost of reaching node $\bbq\in\mathcal{V}$ from the root of the tree. The root of the tree, denoted by $\bbq(0)$, is constructed so that it matches the initial robot state $\bbp(0)$, the initial semantic map $\ccalM(0)$, and the initial DFA state, i.e., $\bbq(0)=[\bbp(0), \ccalM(0), q_D^0]$. %\footnote{In case the DFA has more than one initial state, then there is more than one state $\bbq(0)$ that can be used as a root. In this case, a separate tree is build for each one of possible roots.}
%
By convention the cost of the root $\bbq(0)$ is $J_{\ccalG}(\bbq(0)) = 0$, %[\bbp(t+1), \ccalM(t+1), q_D(t+1)]
while the cost of a node $\bbq(t+1)\in\ccalV$, given its parent node $\bbq(t)\in\ccalV$, is computed as 
\begin{equation}\label{eq:costUpd}
J_{\ccalG}(\bbq(t+1))= J_{\ccalG}(\bbq(t)) +  c(\bbp(t),\bbp(t+1)).
\end{equation}
Observe that by applying \eqref{eq:costUpd} recursively, we get that $J_{\ccalG}(\bbq(t+1)) = J(t+1,\bbu_{0:t+1})$ which is the objective function in \eqref{eq:Prob2}.


\begin{algorithm}[t]
%\footnotesize
\caption{Mission Planning in Probabilistic Maps}
\LinesNumbered
\label{alg:RRT}
\KwIn{ (i) maximum number of iterations $n_{\text{max}}$, (ii) dynamics \eqref{eq:rdynamics}, (iii) map distribution $\ccalM(0)$, (iv) initial robot configuration $\bbp(0)$, (v) task $\phi$;}
\KwOut{Terminal horizon $H$, and control inputs $\bbu_{0:H}$}
Convert $\phi$ into a DFA\label{rrt:dfa}\;
Initialize $\ccalV = \set{\bbq(0)}$, $\ccalE = \emptyset$, $\ccalV_{1}=\set{\bbq(0)}$, $K_1=1$, and $\ccalX_g = \emptyset$\;\label{rrt:init}
\For{ $n = 1, \dots, n_{\text{max}}$}{\label{rrt:forn}
	 Sample a subset $\ccalV_{k_{\text{rand}}}$ from $f_{\ccalV}$\;\label{rrt:samplekrand}
     %
     \For{$\bbq_{\text{rand}}(t)=[\bbp_{\text{rand}}(t),\ccalM_{\text{rand}}(t),q_D]\in\ccalV_{k_{\text{rand}}}$}{\label{rrt:forq}
     Sample a control input $\bbu_{\text{new}}\in\ccalU$ from $f_{\ccalU}$\;\label{rrt:sampleu}
     %Compute 
     $\bbp_{\text{new}}(t+1)=\bbf(\bbp_{\text{rand}}(t),\bbu_{\text{new}})$\;\label{rrt:pnew}
     \If{$\bbp_{\text{new}}(t+1)\in\Omega_{\text{free}}^N$}{\label{rrt:obsFree}
     %Estimated landmark positions %$\hat{\bbx}_{\text{new}}(t+1)=\bbg(\hat{\bbx}_{\text{rand}}(t),\bba(t))$\;\label{rrt:xnew}
     $\hat{\bbx}_{\text{new}}(t+1),\Sigma_{\text{kf}}(t+1)=\kappa(\hat{\bbx}_{\text{rand}}(t),\Sigma_{\text{rand}}(t),\Psi)$\;\label{rrt:xnew}
     %Compute 
     $\Sigma_{\text{new}}(t+1)=\rho(\Sigma_{\text{kf}}(t),\bbp_{\text{new}}(t+1))$\;\label{rrt:Sigmanew}
     $d_{\text{new}}(t+1)=d(0)$\;\label{rrt:dnew}
     $\psi_{\text{new}}(t+1)=\psi(0)$\;\label{rrt:psinew}
     Construct map: $\ccalM_{\text{new}}(t+1) = (\hat{\bbx}_{\text{new}}(t+1),\Sigma_{\text{new}}(t+1), d_{\text{new}}(t+1),\psi_{\text{new}}(t+1))$\;\label{rrt:updmap}
     Compute $q_D^{\text{new}}=\delta_D(q_D^{\text{rand}},L([\bbp_{\text{rand}}(t),\ccalM_{\text{rand}}(t)]))$\label{rrt:feasTrans}\;
     %\For{$q_D^{\text{new}}\in\ccalQ_D$}{\label{rrt:forqB}
     \If{$\exists q_D^{\text{new}}$}{\label{rrt:feasTrans}
     Construct $\bbq_{\text{new}}=[\bbp_{\text{new}},\ccalM_{\text{new}},q_D^{\text{new}}]$\;\label{rrt:qnew}
     Update set of nodes: $\ccalV= \ccalV\cup\{\bbq_{\text{new}}\}$\;\label{rrt:updV}
     Update set of edges: $\ccalE = \ccalE\cup\{(\bbq_{\text{rand}},\bbq_{\text{new}})\}$\;\label{rrt:updE}
     Compute cost of new state: $J_{\ccalG}(\bbq_{\text{new}})=J_{\ccalG}(\bbq_{\text{rand}})+c(\bbp_{\text{rand}},\bbp_{\text{new}})$\;\label{rrt:updCost}
     \If{$q_D^{\text{new}}=q_F$}{\label{rrt:updXg1}
     $\ccalX_g=\ccalX_g\cup\{\bbq_{\text{new}}\}$\;\label{rrt:updXg2}
     }
     Update the sets $\ccalV_{k}$\;\label{rrt:updVk}
     }}}
	 %
}
Among all nodes in $\ccalX_g$, find $\bbq_{\text{end}}(t_{\text{end}})$ \; \label{rrt:node}
$H=t_{\text{end}}$ and recover $\bbu_{0:H}$ by computing the path $\bbq_{0:t_{\text{end}}}= \bbq(0), \dots, \bbq(t_{\text{end}}) $\;\label{rrt:solution}
%Project $\bbQ$ onto the workspace of robot $j$ to get the local path $\bbP_{j}$\;\label{rrt:projP}
%return: \;\label{rrt:path}
\end{algorithm}

\normalsize
The tree $\ccalG$ is initialized so that $\ccalV=\{\bbq(0)\}$, $\ccalE=\emptyset$, and $J_{\ccalG}(\bbq(0)) = 0$ [line \ref{rrt:init}, Alg. \ref{alg:RRT}]. Also, the tree is built incrementally by adding new states $\bbq_\text{new}$ to $\ccalV$ and corresponding edges to $\ccalE$, at every iteration $n$ of Algorithm \ref{alg:RRT}, based on a \textit{sampling} [lines \ref{rrt:samplekrand}-\ref{rrt:sampleu}, Alg. \ref{alg:RRT}] and \textit{extending-the-tree} operation [lines \ref{rrt:pnew}-\ref{rrt:updVk}, Alg. \ref{alg:RRT}]. 
%
After taking $n_{\text{max}}\geq 0$ samples, where $n_{\text{max}}$ is user-specified, Algorithm \ref{alg:RRT} terminates and returns a feasible solution to \eqref{eq:ProbR} (if it has been found), i.e., a terminal horizon $H$ and a sequence of control inputs $\bbu_{0:H}$. 

To extract such a solution, we need first to define the set $\ccalX_g\subseteq\ccalV$ that collects all states $\bbq(t)=[\bbp(t), \ccalM(t), q_D(t)]\in\ccalV$ of the tree that satisfy %$\bbp(t)\in\ccalM_{\text{goal}}$ and %%\eqref{constr21}-
$q_D(t)=q_F$, which captures the terminal constraint \eqref{constr9c} [lines \ref{rrt:updXg1}-\ref{rrt:updXg2}, Alg. \ref{alg:RRT}]. Then, among all nodes $\ccalX_g$, we select the node $\bbq(t)\in\ccalX_g$, with the smallest cost $J_{\ccalG}(\bbq(t))$, denoted by $\bbq(t_{\text{end}})$ [line \ref{rrt:node}, Alg. \ref{alg:RRT}]. %\NA{Note that if you relate the biasing to consistent heuristic the search can stop as soon as you find the first terminal state and you will not need to compare all such states. A consistent heuristic allows biasing the search even more by inflating the heurstic (multiplying by a constant $\epsilon$) and still guaranteeing $\epsilon$-suboptimality}. 
Then, the terminal horizon is $H=t_{\text{end}}$, and the control inputs $\bbu_{0:H}$ are recovered by computing the path $\bbq_{0:t_{\text{end}}}$ in $\ccalG$ that connects $\bbq(t_{\text{end}})$ to the root $\bbq(0)$, i.e., $\bbq_{0:t_{\text{end}}}= \bbq(0), \dots, \bbq(t_{\text{end}})$ [line \ref{rrt:solution}, Alg. \ref{alg:RRT}]; see also Figure \ref{fig:overview}.
%
Note that satisfaction of the constraints in \eqref{eq:ProbR} is guaranteed by construction of $\ccalG$; see Section \ref{sec:constructTree}. In what follows, we describe the core operations of Algorithm \ref{alg:RRT}, `\textit{sample}' and `\textit{extend}' that are used to construct the tree $\ccalG$.

\subsection{Incremental Construction of Trees}\label{sec:constructTree}
At every iteration $n$ of Algorithm \ref{alg:RRT}, a new state $\bbq_\text{new}(t+1) =[\bbp_{\text{new}}, \ccalM_{\text{new}}, , q_D^{\text{new}}]$ is sampled. The construction of the state $\bbq_\text{new}(t+1)$ relies on three steps. Specifically, first we sample a state $\bbp_{\text{new}}$; see Section \ref{sec:sample}. Second, given $\bbp_{\text{new}}$ and its parent node, we compute the corresponding new semantic map $\ccalM_{\text{new}}$. Third, we append to $\bbp_{\text{new}}$ and $\ccalM_{\text{new}}$ a DFA state $q_D^{\text{new}}$ giving rise to $\bbq_{\text{new}}(t+1)$ which is then added to the tree structure, if possible; see Section \ref{sec:extend}. %The third step is repeated for all DFA states $q_D^{\text{new}}$.

%To do this, we first sample a state $\bbp_{\text{new}}$; see Section \ref{sec:sample} [lines \ref{rrt:samplekrand}-\ref{rrt:sampleu}, Alg. \ref{alg:RRT}]. Then, we select a state $\bbq_{\text{rand}}(t)=[\bbp_{\text{rand}}(t),\bbd_{\text{rand}}(t)]\in\ccalV$ that will be the parent node of $\bbq_{\text{new}}(t+1)$[line \eqref{rrt:for2}, Alg. \ref{alg:RRT}]. Note that the time instant $t+1$ which $\bbq_{\text{new}}$ is associated with, is determined by the parent node $\bbq(t)$. Given $\bbp_{\text{new}}$ and the parent node $\bbq_{\text{rand}}(t)$, we compute $\bbd_{\text{new}}(t+1)$ which then gives rise to the new state $\bbq_\text{new}(t+1) =[\bbp_{\text{new}}(t+1),\bbd_{\text{new}}(t+1)]$ that will be added to the tree at iteration $n$ [lines \ref{rrt:dnew}-\ref{rrt:updCost}, Alg. \ref{alg:RRT}]; see Section \ref{sec:extend}.

\subsubsection{Sampling Strategy}\label{sec:sample} 
To construct the state $\bbp_{\text{new}}$, we first divide the set of nodes $\ccalV$ into a \textit{finite} number of sets, denoted by $\ccalV_{k}\subseteq\ccalV$, based on the robot state $\bbp$ and the DFA state $q_D$ that comprise the states $\bbq\in\ccalV$. Specifically, $\ccalV_{k}$ collects all states $\bbq\in\ccalV$ that share the same DFA state and the same robot state (or in practice, robot states that very close to each other). %As a result, the set of nodes $\ccalV$ is divided into $|\ccalQ_D|$ subsets. %\footnote{Decomposition of $\ccalV$ into subsets $\ccalV_k$ is required to ensure completeness and optimality of Algorithm \ref{alg:RRT}; see Appendix \ref{sec:prop}.}
%$\bbq(t)=[\bbp(t),\Sigma(t)]\in\ccalV$ that have the same robot configuration $\bbp$ but possibly different covariance matrices $\Sigma(t)$ and different time stamps $t$; see Figure \ref{fig:tree}. %Also, note that the states $\bbq\in\ccalV_k$ do not necessarily have the same time stamp $t$, since, in general, there are multiple paths that connect the root $\bbq(0)$ to $\bbq$.
%
By construction of $\ccalV_{k}$, we get that $\ccalV = \cup_{k=1}^{K_n}\{\ccalV_{k}\}$, where $K_n$ is the number of subsets $\ccalV_{k}$ at iteration $n$.
Also, notice that $K_n$ is finite for all iterations $n$, due to the finite number of available control inputs $\bbu$ and the finite DFA state-space. %for all robots $j$, i.e., the number of all possible different robot configurations contained in $\ccalV$ is finite for all iterations $n$. 
At iteration $n=1$ of Algorithm \ref{alg:RRT}, it holds that $K_1=1$, $\ccalV_1=\ccalV$ [line \ref{rrt:init}, Alg. \ref{alg:RRT}]. %\red{[maybe a figure would make this definition much cleaner]}%%the (global) set V can be 'infinite'!
% 

Second, given the sets $\ccalV_k$, we first sample from a given discrete distribution $f_{\ccalV}(k|\ccalV):\set{1,\dots,K_n}\rightarrow[0,1]$ an index $k\in\set{1,\dots,K_n}$ that points to the set $\ccalV_{k}$ [line \ref{rrt:samplekrand}, Alg. \ref{alg:RRT}]. The mass function $f_{\ccalV}(k|\ccalV)$ defines the probability of selecting the set $\ccalV_{k}$ at iteration $n$ of Algorithm \ref{alg:RRT} given the set $\ccalV$. 

%Next, given the set $\ccalV_{k_{\text{rand}}}$ sampled from $f_{\ccalV}$, we sample a state $\bbq_\text{rand}\in\ccalV_{k_{\text{rand}}}$ from a desnity function $f_{\bbq}(\bbq|\ccalV_{k}):\set{1,\dots,|\ccalV_{k}|}\rightarrow[0,1]$. This \textcolor{black}{mass} function defines the probability of selecting a node $\bbq$ at iteration $n$ from the set $\ccalV_{k}$. Any \textcolor{black}{mass} function $f_{\bbq}$ can be used to draw samples $\bbq_{\text{rand}}$ from the set $\ccalV_{k_{\text{rand}}}$ as long as it satisfies the following assumption.
%\begin{assumption}[Probability \textcolor{black}{mass} function $f_{\bbq}$]\label{fq}
%(i) The probability \textcolor{black}{mass} function $f_{\bbq}(\bbq|\ccalV_{k}):\set{1,\dots,|\ccalV_{k}|}\rightarrow[0,1]$ satisfies $f_{\bbq}(\bbq|\ccalV_{k})\geq \xi$, $\forall\bbq\in\ccalV_k$ and for all $n\geq 0$, for some $\xi>0$ that remains constant across all iterations $n$. 
%(ii) Independent samples $\bbq_{\text{rand}}$ can be drawn from $f_{\bbq}$.
%\end{assumption}
%Next, given a state $\bbq_\text{rand}\in\ccalV_{k_{\text{rand}}}$, 

Next, given the set $\ccalV_{k_{\text{rand}}}$ sampled from $f_{\ccalV}$, we perform the following steps for all $\bbq\in \ccalV_{k_{\text{rand}}}$. Specifically, given a state $\bbq_{\text{rand}}$, we sample a control input $\bbu_{\text{new}}\in\ccalU$ from a discrete distribution $f_{\ccalU}(\bbu):\ccalU\rightarrow [0,1]$ [line \ref{rrt:sampleu}, Alg. \ref{alg:RRT}]. 
%
Given a control input $\bbu_{\text{new}}$ sampled from $f_{\ccalU}$, we construct the state $\bbp_{\text{new}}$ as $\bbp_{\text{new}}=\bbf(\bbp_{\text{rand}},\bbu_{\text{new}})$ [line \ref{rrt:pnew}, Alg. \ref{alg:RRT}]. If $\bbp_{\text{new}}$ belongs to the obstacle-free space, as required by \eqref{obsFree2}, then the `extend' operation follows [line \ref{rrt:obsFree}, Alg. \ref{alg:RRT}].

Any mass functions $f_{\ccalV}$ and $f_{\ccalU}$ can be used to generate $\bbp_{\text{new}}$ as long as they satisfy the following two assumptions. These assumptions are useful to show completeness and optimality of the proposed sampling-based algorithm.
%We make the following assumptions for $f_{\ccalV}$:
\begin{assumption}[Probability mass function $f_{\ccalV}$]\label{frand}
(i) The probability mass function $f_{\ccalV}(k|\ccalV):\set{1,\dots,K_n}\rightarrow[0,1]$ satisfies $f_{\ccalV}(k|\ccalV)\geq \epsilon$, $\forall$ $k\in\set{1,\dots,K_n}$ and for all $n\geq 0$, for some $\epsilon>0$ that remains constant across all iterations $n$. 
(ii) Independent samples $k_{\text{rand}}$ can be drawn from $f_{\ccalV}$.
\end{assumption}
%
%Any \textcolor{black}{mass} function $f_{\ccalU}$ can be used to draw samples $\bbu_{\text{new}}\in\ccalU$ as long as it satisfies the following assumption.
%The \textcolor{black}{mass} function $f_{\ccalU}$ should be designed so that it satisfies the following assumption.
\begin{assumption}[Probability mass function $f_{\ccalU}$]\label{fnew}
(i) The distribution $f_{\ccalU}(\bbu)$ satisfies $f_{\ccalU}(\bbu)\geq \zeta$, for all $\bbu\in\ccalU$, for some  $\zeta>0$ that remains constant across all iterations $n$. (ii) Independent samples $\bbu_{\text{new}}$ can be drawn from the probability mass function $f_{\ccalU}$.
\end{assumption}
%
\begin{rem}[Mass functions $f_{\ccalV}$ and $f_{\ccalU}$]
Assumptions \ref{frand}(i) and \ref{fnew}(i) also imply that the mass functions $f_{\ccalV}$ and $f_{\ccalU}$ are bounded away from zero on $\set{1,\dots,K_n}$ and $\ccalU$, respectively. Also, observe that 
Assumptions \ref{frand} and \ref{fnew} are very flexible, since they also allow $f_{\ccalV}$ and $f_{\ccalU}$ to change with iterations $n$ of Algorithm \ref{alg:RRT}, as the tree grows.
\end{rem}
%
\begin{rem}[Sampling Strategy]
An example of a distribution $f_{\ccalV}$ that satisfies Assumption \ref{frand} is the discrete uniform distribution $f_{\ccalV}(k|\ccalV )=\frac{1}{k}$, for all $k\in\set{1,\dots,K_n}$. Observe that the uniform mass function trivially satisfies Assumption \ref{frand}(ii). Also, observe that Assumption \ref{frand}(i) is also satisfied, since there exists a finite $\epsilon>0$ that satisfies Assumption \ref{frand}(i), which is $\epsilon =\frac{1}{|\ccalR|}$, where $\ccalR$ is a set that collects all robot configurations $\bbp$ that can be reached by the initial state $\bbp(0)$. Note that $\ccalR$ is a finite set, since the set $\ccalU$ of admissible control inputs is finite, by assumption. Similarly, uniform mass functions $f_{\ccalU}$ satisfy Assumption \ref{fnew}. Note that any functions $f_{\ccalV}$ and $f_{\ccalU}$ can be employed as long as they satisfy Assumptions \ref{frand} and \ref{fnew}. Nevertheless, the selection of $f_{\ccalV}$ and $f_{\ccalU}$ affects the performance of Algorithm \ref{alg:RRT}; see the numerical experiments in Section \ref{sec:Sim}. %The latter allows us to solve large-scale active information acquisition problems.
\end{rem}

\subsubsection{Extending the tree}\label{sec:extend}

To build incrementally a tree that explores both the robot motion space, the space of metric uncertainty, and the DFA state space, we need to append to $\bbp_\text{new}$ the corresponding semantic map $\ccalM_{\text{new}}$ determined by the parameters $(\hat{\bbx}_{\text{new}},\Sigma_{\text{new}},d_{\text{new}})$ and DFA state $q_D^{\text{new}}$. Particularly, $\ccalM_{\text{new}}$ is constructed so that $\hat{\bbx}_{\text{new}}=\hat{\bbx}(0)$,
%\begin{equation}\label{eq:updX}
%  \hat{\bbx}_{\text{new}}=\hat{\bbx}(0),  
%\end{equation}
%$$\hat{\bbx}_{\text{new}}(t+1)=\hat{\bbx}(0),$$ 
as required in \eqref{constr6c}, and computing $\Sigma_{\text{new}}$ as per the Kalman filter Ricatti map, i.e.,
%\begin{equation}
%  \Sigma_{\text{new}}=\rho(\Sigma_{\text{rand}},\bbp_{\text{new}}),
%\end{equation}
%$$\Sigma_{\text{new}}(t+1)=\rho(\Sigma_{\text{rand}}(t),\bbp_{\text{new}}(t+1)),$$ 
$\Sigma_{\text{new}}=\rho(\Sigma_{\text{rand}},\bbp_{\text{new}})$, as required in \eqref{constr7c}, and $d_{\text{new}}=d(0)$,
%\begin{equation}
%  d_{\text{new}}=d(0),  
%\end{equation}
as required in \eqref{constr8c} [lines \ref{rrt:xnew}-\ref{rrt:updmap}, Alg. \ref{alg:RRT}]. %Thus, we get that $\ccalM_{\text{new}}(t+1) =(\hat{\bbx}_{\text{new}}(t+1),\Sigma_{\text{new}}(t+1))$ [line \ref{rrt:updmap}, Alg. \ref{alg:RRT}].
%
Next, to construct the state $\bbq_{\text{new}}$ we append to $\bbp_\text{new}$ and $\ccalM_{\text{new}}$ the DFA state $q_D^{\text{new}}=\delta_D(q_D^{\text{rand}},L([\bbp_{\text{rand}},\ccalM_{\text{rand}}]))$,
%\begin{equation}
%    q_D^{\text{new}}=\delta_D(q_D^{\text{rand}},L([\bbp_{\text{rand}},\ccalM_{\text{rand}}])),
%\end{equation}
as required by \eqref{constr1c}.
%$$q_D^{\text{new}}=\delta_D(q_D^{\text{rand}},L([\bbp_{\text{rand}}(t),\ccalM(t)])).$$ 
In words, $q_D^{\text{new}}$ is the automaton state that that can be reached from the parent automaton state $q_D^{\text{rand}}$ given the observation $L([\bbp_{\text{rand}},\ccalM_{\text{rand}}])$. 
If such a DFA state does not exist, then this means the observation $L([\bbp_{\text{rand}},\ccalM_{\text{rand}}])$ results in violating the LTL formula and this new sample is rejected. Otherwise, the state $\bbq_{\text{new}}=(\bbp_\text{new},\ccalM_{\text{new}},q_D^{\text{new}})$ is constructed [line \ref{rrt:qnew}, Alg. \ref{alg:RRT}] which is then added to the tree.
%to $\bbp_\text{new}(t+1)$ and $\ccalM_{\text{new}}(t+1)$, a state $q_D^{\text{new}}\in\ccalQ_D$ giving rise to a state $\bbq_{\text{new}}=(\bbp_\text{new},\ccalM_{\text{new}}(t+1),q_D^{\text{new}})$ [lines \ref{rrt:forqB}-\ref{rrt:qnew}, Alg. \ref{alg:RRT}]. Specifically, for each state $q_D^{\text{new}}\in\ccalQ_D$, we check if $\delta(q_D^{\text{rand}},L(\bbp_{\text{rand}}(t),\ccalM_{\text{rand}}(t)))=q_D^{\text{new}}$ [lines \ref{rrt:forqB}-\ref{rrt:feasTrans}, Alg. \ref{alg:RRT}]. If so, then we construct the corresponding state $\bbq_{\text{new}}$ which is then added to the tree.

Given a state $\bbq_{\text{new}}$, we update the set of nodes and edges of the tree as $\ccalV = \ccalV\cup\{\bbq_{\text{new}}\}$ and $\ccalE = \ccalE\cup\{(\bbq_{\text{rand}},\bbq_{\text{new}})\}$, respectively [lines \ref{rrt:updV}-\ref{rrt:updE}, Alg. \ref{alg:RRT}]. The cost of the new node $\bbq_{\text{new}}$ is computed as in \eqref{eq:costUpd}, i.e., $J_{\ccalG}(\bbq_{\text{new}})=J_{\ccalG}(\bbq_{\text{rand}})+c(\bbp_{\text{rand}},\bbp_{\text{new}})$ [line \ref{rrt:updCost}, Alg. \ref{alg:RRT}]. Finally, the sets $\ccalV_{k}$ are updated, so that if there already exists a subset $\ccalV_k$ associated with both the DFA state  $\bbq_D^{\text{new}}$ and the robot state $\bbp_{\text{new}}$, then $\ccalV_{k}=\ccalV_{k}\cup\set{\bbq_{\text{new}}}$. Otherwise, a new set $\ccalV_{k}$ is created, i.e., $K_n = K_n +1$ and $\ccalV_{K_n}=\set{\bbq_{\text{new}}}$ [line \ref{rrt:updVk}, Alg. \ref{alg:RRT}]. Recall that this process is repeated for all states  $\bbq_{\text{rand}}\in\ccalV_{k_{\text{rand}}}$ [line \ref{rrt:forq}, Alg. \ref{alg:RRT}]. 


%\begin{rem}[\textcolor{black}{mass} functions $f_{\ccalV}$ and $f_{\ccalU}$]
%Observe that Assumptions \ref{frand}(i) and \ref{fnew}(i) imply that the \textcolor{black}{mass} functions $f_{\ccalV}$ and $f_{\ccalU}$ are bounded away from zero on $\set{1,\dots,K_n}$ and $\ccalU$, respectively. Also, observe that 
%Assumptions \ref{frand} and \ref{fnew} are very flexible, since they also allow $f_{\ccalV}$ and $f_{\ccalU}$ to change with iterations $n$ of Algorithm \ref{alg:RRT}, as the tree grows.
%\end{rem}

%\begin{rem}[Sampling Strategy]
%An example of a distribution $f_{\ccalV}$ that satisfies Assumption \ref{frand} is the discrete uniform distribution $f_{\ccalV}(k|\ccalV )=\frac{1}{k}$, for all $k\in\set{1,\dots,K_n}$. Observe that the uniform function trivially satisfies Assumption \ref{frand}(ii). Also, observe that Assumption \ref{frand}(i) is also satisfied, since there exists an $\epsilon>0$ that satisfies Assumption \ref{frand}(i), which is $\epsilon =\frac{1}{|\ccalQ_D|}$. Similarly, uniform \textcolor{black}{mass} functions $f_{\ccalU}$ satisfy Assumption \ref{fnew}. Note that any functions $f_{\ccalV}$ and $f_{\ccalU}$ can be employed as long as they satisfy Assumptions \ref{frand} and \ref{fnew}. Nevertheless, the selection of $f_{\ccalV}$ and $f_{\ccalU}$ affects the performance of Algorithm \ref{alg:RRT}; see the numerical experiments in Section \ref{sec:Sim}. In Section \ref{sec:biasedSampling}, we design (nonuniform) \textcolor{black}{mass} functions $f_{\ccalV}$ and $f_{\ccalU}$ that bias the exploration towards regions that are expected/predicted to `contribute' in satisfying the task specification $\phi$. %The latter allows us to solve large-scale active information acquisition problems.
%\end{rem} 

\begin{rem}[Finite Decomposition of $\ccalV$]\label{rem:finite}
In Section \ref{sec:sample}, we decomposed the set of nodes $\ccalV$ into $K_n$ finite sets, where $K_n$ remains finite as $n\to\infty$, by construction. The \textit{finite} decomposition of the set of nodes is required to ensure probabilistic completeness and optimality of the proposed sampling-based algorithm. Any alternative decomposition of $\ccalV$ that always results in a finite number of subsets $\ccalV_k$ can be employed without affecting correctness of Algorithm \ref{alg:RRT}.
\end{rem}
%
\begin{figure}[t]
  \centering
 %    \subfigure[$N=1, M=5$ (slow targets)]{
 %   \label{fig:traj15s}
%  \includegraphics[width=0.48\linewidth]{traj_1vs5_slow.pdf}}
\includegraphics[width=1\linewidth]{figures/Overview.png}
\caption{Graphical depiction of the proposed  architecture for planning over continuously learned uncertain semantic maps. First, given a mission specification $\phi$ and an uncertain prior belief about the environment, initial paths are constructed. The robots follow the designed paths while updating the semantic map by fusing the collected measurements. Re-planning is triggered occasionally to adapt planning to the continuously learned map. } 
  \label{fig:overview}
\end{figure}

\subsection{Online Execution and Re-planning}\label{sec:replan}
Algorithm \ref{alg:RRT} generates an open-loop sequence $\bbq_{0:H}=\bbq(0),\bbq(1),\dots,\bbq(H)$, where $\bbq(t)=[\bbp(t),\ccalM(t),q_D(t)]$, so that the resulting robot trajectory $\bbp_{0:H}$ and sequence of maps $\ccalM_{0:H}$ satisfy $\phi$. %Recall that $\ccalM(t)$ is the semantic map at time $t$ constructed offline by computing the a posteriori covariance matrices . %Particularly, recall that the semantic map $\ccalM(t)=(\hat{\bbx}(t),\Sigma(t))$ is built using the Kalman-filter prediction step to compute $\bbx(t)$, the Kalman-filter Ricatti map to  compute $\Sigma(t)$ (which is an approximation if the landmark dynamics is not linear and/or the sensor model is not linear with respect to the hidden state), and $d_c(t)=d_c(0)$. %Hereafter, we denote the semantic map generated offline by $\hat{\ccalM}(t)$.
%
As the robots execute synchronously their respective paths in $\bbp_{0:H}$, synthesized by Algorithm \ref{alg:RRT}, they take measurements (see \eqref{eq:measModelR}-\eqref{eq:measModelC}) which are used to update both the metric and the semantic environmental uncertainty using a semantic SLAM method. In other words, every time the robots move towards their next waypoint, they take measurements which are then used to update (i) the a posteriori mean and covariance matrix associated with the landmark positions and (ii) the discrete distribution associated with the landmark classes yielding a new semantic map denoted by $\ccalM_{\text{online}}(t)$. \textcolor{black}{Note that the online constructed map $\ccalM_{\text{online}}(t)$ may be different from the corresponding offline map $\ccalM(t)$, as the latter is constructed by predicting only the metric environmental uncertainty by computing the a posteriori covariance matrices.}
%expected landmark positions and their covariances using e.g., any existing SLAM algorithm giving rise to a map denoted by $\ccalM_{\text{online}}(t)$. Note that this map may be different from the corresponding offline-generated map $\ccalM(t)$ due to the fact that landmark states are updated (which is not the case during the construction of $\ccalM(t)$). 

As a result, given the new map, the previously designed paths may not be feasible and, therefore, re-planning may be required to adapt to the updated map $\ccalM_{\text{online}}(t)$; see also Figure \ref{fig:overview}. Specifically, re-planning is needed only if the observations/symbols that the robots generate online do not allow them to follow the sequence of DFA states that appears in $\bbq_{0:H}$. Formally, re-planning at time $t$ is required only if the observation $L([\bbp(t),\ccalM_{\text{online}}(t)])$ does not enable a transition from $q_D(t)$ to $q_D(t+1)$, where $q_D(t)$ and $q_D(t+1)$ are determined by $\bbq_{0:H}$ computed by Algorithm \ref{alg:RRT}. In this case, Algorithm \ref{alg:RRT} is initialized with the current robot state $\bbp(t)$, the current DFA state $q_D(t)$, and the current map $\ccalM_{\text{online}}(t)$ to generate a new path. This process is repeated until the accepting DFA state is reached. Once this happens, the LTL formula has been satisfied and the mission terminates. We note that it is possible that at time $t$, as the robots follow their paths, the LTL formula may get violated. This happens if $L([\bbp(t),\ccalM_{\text{online}}(t)])$ does not yield any DFA transition from the current DFA state $q_D(t)$ (or if it yields a transition to an absorbing DFA state, in case DFA is complete). In this scenario, least violating paths can be found as e.g., in \cite{lahijanian2016specification}.\footnote{Intuitively, violation of an LTL formula as the robots follow their paths depends on their sensing capabilities. For instance, an LTL formula may get violated during execution of the synthesized paths, if the robot sensing range is significantly smaller than then proximity requirements captured by the atomic predicates. Consider e.g., the specification in Example \ref{ex:LTL}; see also Fig. \ref{fig:PF1}. Assume that a robot has to always keep a distance of $2$m from the pole. If the sensing capabilities allow the robot to detect objects that are within $d<2$ m, then it is possible that the pole avoidance requirement may get violated, as the pole may get detected only when its distance from the robots is less than $d<2$ m.} %A more computationally efficient re-planning approach, at the expense of sacrificing completeness, is to terminate Algorithm \ref{alg:RRT} when a DFA state $q_D'$ is reached that is closer to $q_F$ than $q_D(t)$ is, as per the distance function defined in Section \ref{sec:biasedSampling}.
%
%\subsection{Environments with Unknown Obstacles}
%
%...
% \textcolor{black}{\begin{rem}[Prior Map \& Re-planning]
% First, recall from Assumption \ref{as:prior} that we assume that there exists a known number of landmarks in the environment. This assumption can be relaxed due to the SLAM capability included in the proposed architecture; see Fig. \ref{fig:overview}. In fact, a prior semantic map is used to initialize Algorithm \ref{alg:RRT} and to guide the planning phase. Once the robots follow the designed paths, they may discover/sense new landmarks. Once this happens, the employed SLAM method will generate a probabilistic belief about these landmarks, which will then be included in the semantic map. Second, it is possible that the prior distribution may guide the robots towards locations in the environment where no landmarks exist. For instance, consider a case where, as per the prior distribution, a landmark of interest is expected to be in a certain room. Due to this prior distribution, Algorithm \ref{alg:RRT} will design paths towards this room. If no landmarks exist in this room, i.e., if this prior distribution is wrong, then it can be discarded from the current semantic map, so that design of mission paths is not guided by this wrong prior. For instance, a prior belief about a landmark can be considered wrong, if the robot approaches the expected position of the landmark within some distance $\eta>0$, and no landmarks are sensed. The parameter $\eta$ is user-specified and it can be associated with the sensing range of the robots. Both scenarios may trigger re-planning as discussed above to account for the new map. 
% \end{rem}}
% \begin{rem}[Re-planning Frequency]
% The frequency with which re-planning is triggered depends on how different the offline predicted map is from the online learned map. In Section \ref{sec:Sim}, we illustrate through simulations that the more inaccurate the initial semantic map is, the more often re-planning is triggered. \textcolor{black}{A potential approach towards minimizing the re-planning frequency is to incorporate semantic map prediction methods into the offline planning process \cite{narasimhan2020seeing} or to design paths that are robust to uncertainty \cite{yel2020gp,lindemann2021robust}.} 
% %
% Also, throughout the paper, we have assumed that the geometric structure of the environment is known; note that the geometry of the environment can be learned using SLAM methods, as well \cite{grisetti2007improved}. This assumption can be relaxed by re-planning every time the robots detect new obstacles/walls that interfere with the paths designed by Algorithm \ref{alg:RRT}. Nevertheless, this may result in rather frequent re-planning, especially, in cluttered environments, increasing the online computational burden \cite{ryll2019efficient}. %and under complex LTL tasks that may require long planning horizons. 
% Our future work will focus on designing more efficient re-planning frameworks in the presence of both geometric and metric/semantic environmental uncertainty by e.g., locally patching the designed paths, or decomposing the global LTL task into smaller sub-tasks \cite{kantaros2020reactive}, or incorporating data-driven map prediction methods in the planning process \cite{elhafsi2020map}.
% \end{rem}

%\textcolor{black}{
%\begin{rem}[Unknown Environmental Geometry]
%\end{rem}}



% \section{Discussion and Extensions}\label{sec:extensions}
% In this section, we discuss how assumptions made in Section \ref{sec:PF} can be relaxed.  \textcolor{black}{Specifically, in Section \ref{sec:unexpl} we discuss how the robots should behave in case feasible - either initial or online revised - paths do not exist. This way, we can relax Assumption \ref{as:prior} requiring an informative enough prior  belief so that there exists a feasible solution to \eqref{eq:Prob2}.} Then, in  Section \ref{sec:nonlin}, we show how Algorithm \ref{alg:RRT} can account for sensor models \eqref{eq:measModelR} that may be nonlinear in the positions of landmarks (e.g., range sensors) \textcolor{black}{or subject to  noise of unknown distribution}.
% \subsection{Reactive Planning in Unexplored Semantic Environments}\label{sec:unexpl}
% \textcolor{black}{In this section, we discuss how the robots should behave in case feasible paths do not exist and, therefore, Alg.\ref{alg:RRT} cannot generate paths. %Algorithm \ref{alg:RRT} can be applied when Assumption \ref{as:prior} does not hold, i.e., to previously unexplored semantic environments where prior information about the metric/semantic environmental structure may be highly uncertain or even unavailable. Note that by highly uncertain map, we mean that a solution to \eqref{eq:Prob2} does not exist given the imposed probabilistic requirements captured by the mission specification. %In what follows we exclude the negation operator from the syntax
% %that object recognition model \eqref{eq:measModelC} is deterministic and perfect, i.e., once a landmark falls into the sensor field-of-view, the object recognition method will always detect it returning its corresponding true class with probability $1$.
% %
% %
% In fact, initial feasible paths may not exist if a prior map is unavailable or highly uncertain; see Assumption \ref{as:prior}. The latter may hold for the online learned map when re-planning is triggered, as well. 
% %
% %may be highly uncertain and, therefore, a solution to \eqref{eq:Prob2} may not exist. T
% %
% %Consider an environment with either no prior information about its metric/semantic structure or a highly uncertain prior. 
% %In both cases, as discussed before, Algorithm \ref{alg:RRT} cannot return a feasible solution, as it does not exist. 
% To mitigate this challenge, we couple Algorithm \ref{alg:RRT} with existing exploration and information gathering methods \cite{leung2012decentralized,atanasov2015decentralized, kantaros2019asymptotically}. 
% %yamauchi1997frontier
% The key idea is that the robots switch back and forth between an exploration and exploitation mode depending on the mission status. In particular, first the robots follow an exploration strategy aiming to spread in the environment to detect landmarks and decrease the environmental uncertainty. Once a user-specified condition about the exploration mode is satisfied, the robots switch to an exploitation mode by applying Algorithm \ref{alg:RRT} aiming to find paths satisfying the assigned mission by exploiting the semantic map constructed during exploration. If such paths still do not exist, the robots switch back to the exploration mode. This process is repeated until the robots accomplish their mission. }
% %Note that in this way we can also account for cases where a prior map is already given to the robots but it turns out to be highly inaccurate. In this case, if Algorithm \ref{alg:} 
% %The same idea also applied if when re-planning is triggered, feasible paths cannot be found given the online learned map (see  Section \ref{sec:replan}). In this case, the robots switch to an exploration mode and then the above process follows.


% %we denote by $q_D(t)$ the DFA state of the robots at time $t$ initialized as $q_D(0)=q_D^0$. 
% %leung2012decentralized
% In what follows, we describe an exploration strategy, adopted from \cite{leung2012decentralized,atanasov2015decentralized}, along with its interaction with Algorithm \ref{alg:RRT} in more detail. First, we define a grid $C=\{c_1,c_2,\dots,c_L\}$ over the environment, where $c_k$ corresponds to the $k$-th grid cell, and we split the grid cells into `explored' (i.e., cells that have been visited by the robots) and 'unexplored'. Then, we introduce dummy `exploration' landmarks at the frontiers of the explored grid map for which uniform discrete and Gaussian distributions are defined for their labels and positions, respectively.  Given the `exploration' and any already detected landmarks, the robots design informative open-loop/offline paths that aim to minimize the metric uncertainty of these landmarks within a pre-determined finite horizon $F>0$; more details about designing these paths can be found in  \cite{atanasov2015decentralized}. Note that the fake uncertainty in the exploration-landmark locations promises information gain to the robots motivating them to move towards the unexplored part of the environment and, therefore, detect new landmarks.
% %
% As the robots start following the designed paths while taking measurements and updating the semantic map, they may detect new landmarks. Once a  new landmark $\ell_i$ is detected by a robot $j$, a Gaussian and a discrete distribution associated with this landmark are initialized. %\footnote{The prior distributions can initialized randomly or in a sensor specific way. For example, if a robot is equipped with a stereo vision sensor that can measure directly the landmark positions, then the mean of the Gaussian distribution is initialized to be the first positional measurement. The corresponding covariance matrix can be initialized randomly or depending on. The discrete distribution over the landmark classes can be initialized randomly where the highest probability is assigned to first class measurement.} %Once a landmark is detected, the robots can explore the environment to minimize the uncertainty associated with the detected landmark \cite{leung2012decentralized,atanasov2015decentralized}. 
% Once all robots have finished the execution of their paths, they should determine whether they should keep exploring the environment or design mission-based paths over the constructed semantic map using Algorithm \ref{alg:RRT}. 
% %
% We require mission-based planning to be triggered once $K(t)\geq 0$ new landmarks are detected, where $K(t)$ is user-specified and it depends on the assigned mission. %Note that selection of $K(t)$ can be mission-specific i.e., it may depend on the number and classes of landmarks involved in the LTL specification. 
% Also, additional requirements can be incorporated to trigger Algorithm \ref{alg:RRT} related to e.g., the map uncertainty.
% %and localized as per user-specified accuracy
% %In particular, once a landmark is detected the robots navigate to gather information about the detected landmark $\ell_i$ and eventually drop its metric and semantic uncertainty below user specified thresholds $\zeta(t)$ and $\eta(t)$; the metric uncertainty of landmark can be captured by $\det\Sigma_i(t)$ while the semantic uncertainty can be captured by the entropy of the discrete distribution $d_i$. Once the exploration mode is terminated, the robots execute Algorithm \ref{alg:RRT} to compute paths satisfying the assigned LTL task. If such paths cannot be found, the robots switch back to the exploration mode where more landmarks may be detected (if there are unexplored cells $c_k$) and/or uncertainty about the already detected landmarks may decrease. 
% Note that during the exploration phase, as the robots detect and localize landmarks, they may  satisfy certain atomic propositions enabling a transition from the current DFA state to a new DFA state; see also Remark \ref{rem:safeExpl}. Thus, when Algorithm \ref{alg:RRT} is executed, it is initialized with the DFA state that the exploration mode has ended up. %At the first execution of the exploration strategy, the DFA state is initialized to be the initial automaton state $q_D^0$.
% %
% %
% \begin{rem}[Safe Exploration]\label{rem:safeExpl}
% %There two main challenges that arise in the proposed framework. First of all
% A particular challenge that arises in the proposed framework is that of safe exploration. In fact, as the robots explore the environment to detect and localize previously unknown landmarks they may satisfy atomic propositions that violate the assigned LTL specification. Specifically, let $q_D(t)$ be the automaton state the robots are at time $t$ and assume that the robots are currently in exploration mode. During exploration, the robots may generate a symbol that does not enable any transition originating from $q_D(t)$ resulting in violation of the LTL task. An empirical approach towards mitigating this issue is to ensure that the robots always satisfy the Boolean formula that enables them to remain in $q_D(t)$.\footnote{By construction of the DFA, there exists a Boolean formula defined over $\mathcal{AP}$ that needs to be satisfied to enable a DFA transition.} For instance, assume that the robots can remain in $q_D(t)$ if with probability greater than $0.9$, they keep a distance of at least $1$m from any landmark with class `table'. Then, we can compute $\epsilon$-confidence intervals, for some $\epsilon>0$, centered at the expected positions of detected landmarks whose most likely class is `table'; $\epsilon$-confidence intervals are then treated as virtual obstacles that should be avoided. %A less conservative approach would be to allow the robots to transition to other DFA states without violating the LTL formula. 
% %Given $q_D(t)$, this can be accomplished by extracting the atomic propositions that if satisfied, then no transitions from $q_D(t)$ will be enabled; in other words, these are the atomic propositions that if satisfied, the LTL formula will be violated. Given, such atomic propositions we define the set $\ccalA(t)$ that collects all associated landmarks. Then, similarly to Section \ref{sec:fu}, we can compute $\epsilon$-confidence intervals centered at the expected positions of these landmarks in $\ccalA(t)$, which are treated as virtual obstacles, as well. 
% If the negation operator is excluded from the syntax, then exploration is always safe as there are no observations that can violate the assigned LTL task. 
% %prevent the robots from visiting locations that result in violations of the assigned task. Particularly, given the deterministic nature of the DFA and the Boolean conditions that enable DFA transitions, we can
% \end{rem}
% %
% %\textcolor{black}{
% %\begin{rem}[Exploration-Exploitation]
% %The proposed framework for planning in unexplored semantic environments requires the robots to switch from exploration to mission-based planning and vice versa controlled by $K(t)$, $\zeta(t)$, and $\eta(t)$. Intuitively, the larger $K(t)$ is and the smaller $\zeta(t)$ and $\eta(t)$ are (i.e., the less uncertain the semantic map is after exploration), the more likely is that Algorithm \ref{alg:RRT} will find a solution without triggering exploration again. Nevertheless, this may lead to long exploration phases that may also compromise safety; see Remark \ref{rem:safeExpl}. 
% %\end{rem}}
% %
% %
% %\subsection{Mobile Targets} First, we assumed that the environment is occupied by \textit{static} landmarks. Mobile landmarks can also be considered that are governed by the following known but noisy dynamics:
% %\begin{equation} \label{eq:dynamics}
% %\bbx_i(t+1) =\bbg_i(\bbx_i(t),\bba_i(t), \bbw_i(t)), 
% %\end{equation}
% %where $\bba_i(t)$ and $\bbw_i(t) \in\reals^{d_w}$ are the control input and the process noise for target $i$ at discrete time $t$. We assume that the process noise $\bbw_i(t)$ is uncertain and follows a normally distributed as $\bbw(t) \sim \ccalN(0, \bbQ(t))$, where $\bbQ(t)$ is the covariance matrix at time $t$. To account for dynamic targets, the optimal control problem in \eqref{eq:Prob2} can be reformulated by replacing the constraint in \eqref{constr6b} with 
% %\begin{equation}\label{eq:predict}
% %  \hat{\bbx}_i(t+1) =\bbg_i(\hat{\bbx}_i(t),\bba_i(t)),  
% %\end{equation}
% %which is, in fact, the prediction step of a Kalman filter. Assuming that the control inputs $\bba_i(t)$ and the covariance matrices $\bbQ(t)$ are known to the robots for all $t\geq 0$, Algorithm \ref{alg:RRT} can be used to solve the new formulation of \eqref{eq:Prob2}. The only difference is that \eqref{eq:predict} will be used to construct the landmark states $\hat{\bbx}_{\text{new}}(t)$, instead of \eqref{eq:updX}, which are then used to define the map $\ccalM_{\text{new}}(t)$.
% %
% %\subsubsection{Semantic Uncertainty} Second, we assumed that the class of each landmark is known. This assumption can be relaxed as in \cite{kantaros2019optimal}. Specifically, we can assume that the class of landmark $i$ follows an arbitrary discrete distribution $d_i:\ccalC\rightarrow [0,1]^{|\ccalC|}$ where $d_i(c)$ denotes the probability of landmark $i$ having the class $c$. To account for semantic map uncertainty we can introduce additional probabilistic predicates related to the distributions $d_i$; see \cite{kantaros2019optimal}. Note that these distributions cannot be updated offline by Algorithm \ref{alg:RRT} but they can be updated online as the robots collect semantic perceptual measurements using a semantic SLAM algorithm \cite{bowman2017probabilistic}.
% %
% \subsection{Nonlinear Sensor Models and Unknown Noise Distribution}\label{sec:nonlin}
% In Section \ref{sec:PF}, we assumed that the sensor model \eqref{eq:measModelR} is linear with respect to the landmark positions $\bbx$ allowing us to compute offline the a-posteriori covariance matrix without the need of measurements. Nevertheless, this assumption may not hold in practice e.g., in case of range sensors. In this case, during the execution of Algorithm \ref{alg:RRT}, similar to \cite{atanasov2015decentralized}, we compute the a-posteriori covariance matrices $\Sigma_{\text{new}}$ using the linearized observation model about the estimated landmark positions [line \ref{rrt:Sigmanew}, Alg. \ref{alg:RRT}]. Such case studies are presented in Section \ref{sec:Sim}.

% \textcolor{black}{Additionally, in Section \ref{sec:PF}, we assumed that the measurement noise follows a Gaussian distribution. This can be relaxed by leveraging recent distributionally robust planning methods \cite{summers2018distributionally,renganathan2020towards}. Specifically, we can consider measurement noise with unknown distribution assuming that it belongs to an ambiguity set with known mean and covariance matrix. Then, the Kalman filter Ricatti map can be used to update the covariance matrices offline \cite{renganathan2020towards}. A key challenge in this case is to define perception-based predicates capturing probabilistic requirements since the hidden state (e.g., the landmark positions) does not follow a known distribution. To mitigate this challenge, worst-case probabilistic requirements can be defined that are typically translated to linear constraints \cite{renganathan2020towards}.}

%\textcolor{black}{
%\subsection{Distributionally Robust Planning}\label{sec:distrRob}
%as}


==> files/biasedSampling.tex <==
As discussed in Section \ref{sec:samplingAlg}, any density functions $f_{\ccalV}$ and $f_{\ccalU}$ that satisfy Assumptions \ref{frand} and \ref{fnew} can be employed to generate states $\bbq_{\text{new}}(t)$ in Algorithm \ref{alg:RRT}. In what follows, we build upon our previous work \cite{kantaros2018temporal}, to design density functions that allow us to address large-scale planning tasks that involve large teams of robots and workspaces. The  main difference with  \cite{kantaros2018temporal}, in terms of designing sampling functions, is that \cite{kantaros2018temporal} (i) requires discrete abstractions of robot mobility captured by transition systems and (ii) evaluates atomic propositions over a given deterministic map (transition systems).%The main idea is to build $f_{\ccalV}$ and $f_{\ccalU}$ so that the tree is biased to explore regions of $\Omega_{\text{free}}$ where targets are predicted to be. 


\subsection{Pruning the DFA}\label{sec:prune}
We first prune the DFA by removing transitions that are unlikely to be enabled. Particularly, these are DFA transitions enabled when a robot $j$ has to \textit{simultaneously} satisfy atomic propositions of the form \eqref{ap1}-\eqref{ap2} associated with more than one landmark, e.g., $\pi_j^{\ell _i}(r_1,\delta_1) \wedge \pi_j^{\ell _e}(r_2,\delta_2), e\neq i$. Note that existence of a robot position that satisfies $\pi_j^{\ell _i}(r_1,\delta_1) \wedge \pi_j^{\ell _e}(r_2,\delta_2)$ depends on the distribution of the position of landmarks $e$ and $j$. Hereafter, for simplicity, we classify such DFA transitions as \textit{infeasible}.\footnote{Note that this is a conservative approach as \textit{feasible} transitions may be classified as infeasible transitions. Nevertheless, this does not affect the correctness of the proposed algorithm, since the constructed biased sampling functions satisfy Assumptions \eqref{frand} and \eqref{fnew}; see \cite{kantaros2018temporal}. If the pruned DFA is disconnected then this means that the specification is infeasible or the task is feasible but the pruning was very conservative. In this case, a warning message can be returned to the user, and either uniform distributions  can be employed or the proposed biased distributions but using the original (and not the pruned) DFA.} Similarly, DFA transitions that are enabled when a robot is present in more than one disjoint regions simultaneously are also pruned. We denote by $\Sigma_{q_D,q_D'}^\text{feas}\subseteq\Sigma$ the set that collects all `feasible' finite words $\sigma^* \in {\Sigma}$ enabling transition from a state $q_D$ to $q_D'$ according to $\rightarrow_D$.

Second, we define a distance function $d: \ccalQ_D \times \ccalQ_D \rightarrow \mathbb{N}$ between any two DFA states, which captures the minimum number of transitions in the pruned DFA to reach a state $q_D'$ from a state $q_D$. This function is defined as follows
\begin{equation}
d(q_D,q_D')=\left\{
                \begin{array}{ll}
                  |SP_{q_D,q_D'}|, \mbox{if $SP_{q_D,q_D'}$ exists,}\\
                  \infty, ~~~~~~~~~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\normalsize
where $SP_{q_D,q_D'}$ denotes the shortest path (in terms of hops) in the  pruned DFA from $q_D$ to $q_D'$ and $|SP_{q_D,q_D'}|$ stands for its cost (number of hops).%\footnote{Note that since $\ccalG_B$ is a directed graph, it does not necessarily hold that $d(q_B,q_B')=d(q_B',q_B)$ or that $d(q_B,q_B)=0$.}% In other words, $d(q_B,q_B')$ represents the minimum number of (feasible) transitions that are required to reach the state $q_B'$ starting from $q_B'$.

%%%%

\subsection{Density function $f_{\ccalV}$}\label{sec:fv}
First, given the root of the tree we select a \textit{feasible} final state $q_{F}\in\ccalQ_F$, such that $d(q_D^0,q_{F})\neq \infty$. Among all final states that satisfy this condition, we select one randomly denoted by $q_F^{\text{feas}}$. %\footnote{Note that if there are more than one final states $q_B^{F,\text{feas}}$, then Algorithm \ref{alg:tree} can be executed for all such final states in parallel.} 
%If there does not exist such a state $q_F^{\text{feas}}$, then this means that there is no feasible path associated with the initial state $q_D^0$ or the pruning of the DFA was conservative yielding a `disconnected' pruned DFA(see the definition of infeasible DFA transitions in Section \ref{sec:prune}). In this case, either uniform sampling functions can be employed or biased sampling functions can be constrcuted as follows but based on the original DFA (and not the pruned one).
%
We also define the set $\ccalD_{\text{min}}$ that collects the nodes $q=(\bbp,q_D)\in\ccalV$ that have the minimum distance $d(q_D,q_F^{\text{feas}})$ among all nodes in $\ccalV$, i.e., $\ccalD_{\text{min}}=\{\bbq=(\bbp,q_D)\in\ccalV~|~d(q_D,q_F^{\text{feas}})=d_{\text{min}} \}$, where $d_{\text{min}}=\min \cup_{\forall q_D\in\Pi|_{\ccalQ_D}\ccalV}\{d(q_D,q_F^{\text{feas}})\}$ and $\Pi|_{\ccalQ_D}\ccalV\subseteq\ccalQ_D$ stands for the projection of all states $\bbq\in\ccalV$ onto the DFA state space $\ccalQ_D$. The set $\ccalD_{\text{min}}$ initially collects only the root and is updated (along with $d_{\text{min}}$) as new states are added to the tree. Given the set $\ccalD_{\text{min}}$, we define the set $\ccalK_{\text{min}}$ that collects the indices $k$ of the subsets $\ccalV_k$ that satisfy $\ccalV_k\cap\ccalD_{\text{min}}\neq\emptyset$.
%
Given the set $\ccalK_{\text{min}}$, the probability density function $f_{\text{rand}}(k|\ccalV)$ is defined so that it is biased to select more often subsets $\ccalV_k\subseteq\ccalV$ that satisfy $k\in\ccalK_{\text{min}}$. Specifically, $f_{\text{rand}}(k|\ccalV)$ is defined as follows

\begin{equation}\label{eq:frand}
f_{\text{rand}}(k|\ccalV)=\left\{
                \begin{array}{ll}
                  p_{\text{rand}}\frac{1}{|\ccalK_{\text{min}}|}, ~~~~~~~~~~~~\mbox{if}~k\in\ccalK_{\text{min}}\\
                  (1-p_{\text{rand}})\frac{1}{|\ccalV\setminus\ccalK_{\text{min}}|},~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
where $p_{\text{rand}}\in(0.5,1)$ stands for the probability of selecting \textit{any} subset $\ccalV_k$ that satisfies $k\in\ccalK_{\text{min}}$. Note that $p_{\text{rand}}$ can change with iterations $n$ but it should always satisfy $p_{\text{rand}}\in(0.5,1)$ to ensure that subsets $\ccalV_k$ with $k\in\ccalK_{\text{min}}$ are selected more often. 

\subsection{Density function $f_{\ccalU}$}\label{sec:fu}
The sampling function $f_{\ccalU}(\bbu|k_{\text{rand}})$ is designed so that a state $\bbq=(\bbp,q_F^{\text{feas}})$ is reached by following the shortest path (in terms of hops) in the pruned DFA that connects $q_D^0$ to $q_F^{\text{feas}}$. %The proposed biased sampling process is illustrated in Figure \ref{fig:sampling}.%There three main steps to sample such a state $q_{\text{PTS}}^{\text{new}}$. First, given $q_P^{\text{rand}}=(q_{\text{PTS}}^{\text{rand}},q_B^{\text{rand}})$, we construct a set, denoted by $\ccalR_B^{\text{min}}(q_B^{\text{rand}})$ that collects all the states $q_B\in\ccalQ_B$ that can be reached from $q_B^{\text{rand}}$ given the observation $L(q_{\text{PTS}}^{\text{rand}})$. Among all these states we pick the state, denoted by $q_B^{\text{min}}$ that is closer to $q_B^{F,\text{feas}}$ than any other state $q_B\in\ccalR_B^{\text{min}}(q_B^{\text{rand}})$. 

%\begin{figure}[t]
%  \centering
%  \includegraphics[width=0.57\linewidth]{sample.eps}
%   \caption{\footnotesize{Graphical depiction of the proposed sampling function when $N=1$. The thick black arrow ends in the state that will be selected with probability $p_{\text{new}}$. Note that for $\sigma^*=L_{i}(q_{i}^{\ccalL(i)})$, it holds that $(q_B^{\text{min}},\sigma^*, q_B^{\text{decr}})\in \rightarrow_B$. Next to each state $q_B\in\ccalQ_B$, we also note inside parentheses the value of $d(q_B,q_B^{F,\text{feas}})$.}}
%  \label{fig:sampling}
%\end{figure}
%Also, by construction of the sampling and the `extend' operation, all states $(q_i,q_B)\in\ccalQ_B$, for some $q_i\in\ccalR_{\text{wTS}_i}(q_i^{\text{rand}})$ and for all $q_B\in\ccalR_{B}(q_B^{\text{rand}})$ will be added to the tree at iteration $n$; see also Proposition 5.1 in \cite{kantaros2017Csampling}

\paragraph{Selection of $q_B^{\text{min}}\in\ccalQ_B$} First, given  a state $\bbq_{\text{rand}}=(\bbp_{\text{rand}},q_D^{\text{rand}})$, we first construct the reachable set $\ccalR_D(q_D^{\text{rand}})$ that collects all states $q_D\in\ccalQ_D$ that can be reached in one hop in the pruned DFA from $q_D^{\text{rand}}$ given the observation $L(\bbp_{\text{rand}})$, i.e., $\ccalR_D(q_D^{\text{rand}})=\{q_D\in\ccalQ_D~|~(q_D^{\text{rand}},L(\bbp_{\text{rand}}), q_D)  \in\rightarrow_D\}$.
%\begin{equation}\label{eq:RBrand}
%\ccalR_B(q_B^{\text{rand}})=\{q_B\in\ccalQ_B~|~(q_B^{\text{rand}},L_{\text{PTS}}(q_{\text{PTS}}^{\text{rand}}), q_B)  \in\rightarrow_B\}.
%\end{equation}
Given $\ccalR_D(q_D^{\text{rand}})$ we construct the set $\ccalR_D^{\text{min}}(q_D^{\text{rand}})$ that collects the states $q_D\in\ccalR_D(q_D^{\text{rand}})$ that have the minimum distance from $q_F^{\text{feas}}$ among all other nodes $q_D\in\ccalR_D(q_D^{\text{rand}})$, i.e., $\ccalR_D^{\text{min}}(q_D^{\text{rand}})=\{q_D\in\ccalR_D(q_D^{\text{rand}})~|~d(q_D,q_F^{\text{feas}})=\min_{q_D'\in\ccalR_D(q_D^{\text{rand}})} d(q_D',q_F^{\text{feas}}) \}\subseteq\ccalR_D(q_D^{\text{rand}})$; see Figure \ref{fig:sampling}.
%\begin{align}\label{eq:RBmin}
%&\ccalR_B^{\text{min}}(q_B^{\text{rand}})=\{q_B\in\ccalR_B(q_B^{\text{rand}})~|\\&d(q_B,q_B^{F,\text{feas}})=\min_{q_B'\in\ccalR_B(q_B^{\text{rand}})} d(q_B',q_B^{F,\text{feas}}) \}\subseteq\ccalR_B(q_B^{\text{rand}}),\nonumber
%\end{align}
%where $d_{\text{min}}^{\text{reach}}=\min_{q_B\in\ccalR_B(q_B^{\text{rand}})} d_{q_B,q_B^{\text{feas}}}$. 
Among all DFA states in $\ccalR_D^{\text{min}}(q_D^{\text{rand}})$ we select a state  $q_D^{\text{min}}$ for which there is a finite (`feasible') word $\sigma^*$ such that (i) $q_D^{\text{min}}\xrightarrow{\sigma^*}q_D$, and (ii) $q_D$ is closer to $q_F^{\text{feas}}$ than $q_D^{\text{min}}$ is; for more details see in \cite{kantaros2018temporal}. Such a  state $q_D$ is denoted hereafter as $q_B^{\text{decr}}$.


%In what follows, we denote by  $q_D^{\text{cand,min}}$ the states that belong to $\ccalR_D^{\text{min}}(q_D^{\text{rand}})$. For every state $q_D^{\text{cand,min}}\in\ccalR_D^{\text{min}}(q_D^{\text{rand}})$, we construct the set $\ccalR_D^{\text{decr}}(q_D^{\text{cand,min}})$ that collects all states $q_D\in\ccalQ_D$, for which (i) there exists a feasible word $\sigma^*\in\Sigma_{q_D^{\text{cand,min}},q_D}^{\text{feas}}$ such that $q_D^{\text{cand,min}}\xrightarrow{\sigma^*}q_D$, and (ii) $q_D$ is closer to $q_F^{\text{feas}}$ than $q_D^{\text{cand,min}}$ is, i.e., $\ccalR_D^{\text{decr}}(q_D^{\text{cand,min}})=\{q_D\in\ccalQ_D~|~(\Sigma_{q_D^{\text{cand,min}},q_D}^{\text{feas}}\neq\emptyset)\wedge
%d(q_D,q_D^{F,\text{feas}})=d(q_D^{\text{cand,min}},q_F^{\text{feas}})-1 \}\subseteq\ccalQ_D.$
%
%
%We collect all states $q_D^{\text{cand,min}}\in\ccalR_D^{\text{min}}(q_D^{\text{rand}})$ that satisfy $\ccalR_D^{\text{decr}}(q_D^{\text{cand,min}})\neq\emptyset$ in the set $\ccalM(q_D^{\text{rand}})$, i.e., $\ccalM(q_D^{\text{rand}})=\set{q_D^{\text{cand,min}}~|~ \ccalR_D^{\text{decr}}(q_D^{\text{cand,min}})\neq\emptyset }\subseteq \ccalR_D^{\text{min}}(q_D^{\text{rand}})$ [line \ref{s:M}, Alg.\ref{alg:sample1}].
%
%Next, given the set $\ccalM(q_D^{\text{rand}})$, we sample a state $q_D^{\text{min}}\in\ccalM(q_D^{\text{rand}})$ from a discrete distribution $f_D^{\text{min}}(q_D|\ccalM(q_D^{\text{rand}})):\ccalM(q_D^{\text{rand}})\rightarrow[0,1]$ defined as $f_D^{\text{min}}(q_D|\ccalM(q_D^{\text{rand}}))=\frac{1}{|\ccalM(q_D^{\text{rand}})|}$ [line \ref{s:qBmin}, Alg.\ref{alg:sample1}] .
%
%Here, we assume that every time a given state $q_P$ is selected to be $q_P^{\text{rand}}$, we always select the same state $q_B^{\text{min}}\in\ccalR_B(q_B^{\text{rand}})$, for all $q_P\in\ccalV_T$. 
%Note that if $\ccalM(q_D^{\text{rand}})=\emptyset$, then no sample will be taken at this iteration [line \ref{s:empty2}, Alg. \ref{alg:sample1}].
%
%
%The following steps ensure that a state $q_{\text{PTS}}^{\text{new}}$ will be sampled so that a final state $(q_{\text{PTS}},q_B^{F,\text{feas}})\in\ccalQ_P^F$ will be added to the tree as soon as possible. %This will be formally shown in \red{Proposition \ref{prop:distDeacr}}.
%\normalsize
%
%\paragraph{Selection of $q_D^{\text{decr}}\in\ccalR_D^{\text{decr}}(q_D^{\text{min}})$} Given the state $q_D^{\text{min}}$ and its respective set $\ccalR_D^{\text{decr}}(q_D^{\text{min}})$, we sample a state $q_D^{\text{decr}}\in\ccalR_D^{\text{decr}}(q_D^{\text{min}})$ from a given discrete distribution $f_D^{\text{decr}}(q_D|\ccalR_D^{\text{decr}}(q_D^{\text{min}})):\ccalR_D^{\text{decr}}(q_D^{\text{min}})\rightarrow[0,1]$ [line \ref{s:qBfeas}, Alg. \ref{alg:sample1}] defined as
%$f_D^{\text{decr}}(q_D|\ccalR_D^{\text{decr}}(q_D^{\text{min}}))=\frac{1}{|\ccalR_D^{\text{decr}}(q_D^{\text{min}})|}, \forall q_D\in \ccalR_D^{\text{decr}}(q_D^{\text{min}})$; see also Figure \ref{fig:sampling}. %Alternative sampling methods are discussed in \red{Remark \ref{rem:sample-qB}.} 
%
%Note that if $\ccalR_D^{\text{decr}}(q_D^{\text{min}})=\emptyset$, then no sample $\bbu_{\text{new}}$ is generated [line \ref{s:empty1}, alg. \ref{alg:sample1}].

\normalsize{Given $q_D^{\text{min}}$ and $q_D^{\text{decr}}$, we select a word $\sigma^*$ from $\Sigma_{q_D^{\text{min}},q_D^{\text{decr}}}\neq\emptyset$.\footnote{To speed up the detection of final states, we always select the same word
$\sigma^*\in\Sigma_{q_D^{\text{min}},q_D^{\text{decr}}}$ for a given pair of states $q_D^{\text{min}}$ and $q_D^{\text{decr}}$. Also, by construction of $q_D^{\text{decr}}$, it holds that $\Sigma_{q_D^{\text{min}},q_D^{\text{decr}}}\neq\emptyset$.} Given the word $\sigma^*$, we construct the set $\Pi_j$ that collects all atomic propositions that appear in $\sigma^*$ and are associated with robot $j$. 
%
For instance, the set $\Pi_j$ corresponding to the word $\sigma^*=\pi_{j}(r,\delta,\bar{\ccalC})\pi_{z}^{\ell_e}(r,\delta)$ collects only the atomic proposition $\pi_{j}(r,\delta,\bar{\ccalC})$. Also, observe that $\Pi_s=\varnothing$ for all robots $s\neq j,z$.  
%
Next, given $\Pi_j$, and for each atomic proposition $\pi$ in $\Pi_j$, we compute all possible landmarks or regions that if robot $j$ visits, then $\pi$ may be satisfied, collected in a set $\ccalL_j(\pi)$. For instance,  if $\Pi_j=\set{\pi_{j}(r,\delta,\bar{\ccalC})}$, then all landmarks that have a non-zero probability of having a class that belongs to $\ccalC_m$ are collected in a set denoted by $\ccalL_j(\pi_{j}(r,\delta,\bar{\ccalC}))$. Among all landmarks (or regions) in the set $\ccalL_j$, we select one landmark/region, denoted by $t_j$. This landmark/region is used to design $f_{\text{new},i}(\bbu_i|k)$ so that control inputs that drive robot $j$ toward $t_j$ are selected more often. In particular, from each set $\ccalL_j(\pi)$, indexed by $\pi\in\Pi_j$ we select one landmark/region denoted by $r_j^{\ccalL_j(\pi)}$. Then among all landmark regions $r_j^{\ccalL_j(\pi)}$, indexed by  $\ccalL_j(\pi)$, we select as $t_j$ the landmark/region based on any criterion  e,g., proximity to robot $j$. In what follows, we discuss, how $r_j^{\ccalL_j(\pi)}$ is selected from $\ccalL_j$.\footnote{For simplicity we denote $r_j^{\ccalL_j(\pi)}$ by $r_j^{\ccalL_j}$.} 
If the atomic proposition $\pi\in \Pi_j$ is in the form of \eqref{ap1}, i.e., $\pi=\pi_j^{\ell_i}$, then it trivially holds that $\ccalL_j(\pi_{j}^{\ell_i}(r,\delta))=\ell_i$ and, therefore, $r_j^{\ccalL_j}=\ell_j$. The same argument also applies to atomic propositions  in the form of \eqref{ap3}.
%
If the atomic proposition $\pi\in \Pi_j$ is in the form of \eqref{ap2}, then we select as $r_j^{\ccalL_j}$ from $\ccalL_j(\pi)$ the landmark $\ell_i$ with maximum value $\frac{d_{c_i}(c_i\in\ccalC)}{\det\Sigma_i}$, where $\det\Sigma_i$ is the determinant of the covariance matrix $\Sigma_i$. In words, the larger the value of $\frac{d_{c_i}(c_i\in\ccalC)}{\det\Sigma_i}$ is, the smaller the uncertainty about the position and the class of landmark $\ell_i$. Similarly, we construct $r_j^{\ccalL_j}$ for atomic propositions $\pi$ in the form of \eqref{ap4}.

Given the assigned landmark/region denoted by $t_j$, we construct the density function $f_{\text{new},j}(\bbu_j|k)$ from which we sample a control input $\bbu_j$ as follows: 

\footnotesize{
\begin{equation}\label{eq:fnew}
f_{\text{new},j}(\bbu_j|k)=\left\{
                \begin{array}{ll}
                \frac{1}{|\ccalU_j|},~\mbox{if}~\ccalL(j)=\emptyset,\\
                 p_{\text{new}},\mbox{if}~(L(j)\neq\varnothing)\wedge
                   (\bbu_j=\bbu_j^*)\\
                  (1-p_{\text{new}})\frac{1}{|\ccalU_j\setminus\set{\bbu_j^*}|},\mbox{if}~(L(j)\neq\varnothing)\wedge
                   (\bbu_j\neq \bbu_j^*),
                \end{array}
              \right.
\end{equation}}
\normalsize
\noindent where $\bbu_j^{*}\in\ccalU_j$ is the control input that minimizes the \textit{geodesic} distance between $\bbp_j(t+1)$ and the location of the assigned landmark (or, e.g., the center of an assigned region) $t_j$. To compute the \textit{geodesic} distance between $\bbp_j(t+1)$  and the assigned landmark $t_j$, we first treat all landmarks that if visited, then the Boolean condition under which transition from $q_D^{\text{min}}$ to $q_D^{\text{decr}}$ is enabled, is false, as `virtual' obstacles. For example, assume that transition from  $q_D^{\text{min}}$ to $q_D^{\text{decr}}$ is possible if the following Boolean condition is true $\pi_j^{\ell_i}(r,\delta)\wedge \pi_z^{\ell_e}(r,\delta)\wedge(\neg \pi_j^{\ell_e}(r,\delta))$, which is satisfied by the following word $\sigma^*=\pi_j^{\ell_i}(r,\delta)\pi_z^{\ell_e}(r,\delta)$ and is violated if $\pi_j^{\ell_e}(r,\delta)$ is observed. For such `virtual' obstacles, we compute the $\delta$-confidence interval around the mean, which is then treated as an (known) obstacle in the workspace. Then, we compute the \textit{geodesic} distance between $\bbp_j(t+1)$ and $t_j$ given such virtual obstacles. Essentially, this minimizes the probability of generating an observation that violates the assigned task specification. Note that the `virtual' obstacles are different for each robot.

% \begin{rem}
% As it will be discussed in Section \ref{sec:extend}, a state $q_P^{\text{new}}=(q_{\text{PTS}}^{\text{new}},q_B^{\text{min}})\in\ccalQ_P$ will be added to the tree, if it has not already been added. By construction of $q_B^{\text{min}}$, when the state $q_P^{\text{new}}$ is selected to be $q_P^{\text{rand}}$
% \end{rem}
%\begin{rem}[Selection of  $q_B^{\text{reach}}$, $q_B^{\text{rand}}$, $\sigma^*$]
%Note that given $q_P^{\text{rand}}$ the states $q_B^{\text{reach}}$ and $q_B^{\text{rand}}$ can also be selected probabilistically from the sets $\ccalR_B(q_B^{\text{rand}})$ and $\ccalR_B^{\text{feas}}(q_B^{\text{reach}})$. However, for simplicity of notations, we avoid presenting such analysis. Also, the word $\sigma^*\in\Sigma_{q_B^{\text{reach}},q_B^{\text{feas}}}$ does not need to remain fixed every time a node $q_P$ is selected to be $q_P^{\text{rand}}$; however, this can slow down the detection of final states. 
%\end{rem}

%\begin{rem}[selection of rrand]
%Note that if $SP_{q_{i}^{\text{rand}},q_{i}^{\ccalL(i)}}(2))$ is a region that robot $i$ should always avoid, then for high values of $p_{\text{new}}$, a state q_{PTS}^{new} will be constructed that will be rejected in the step. 
%\end{rem}

%\begin{algorithm}[t]
%\footnotesize
%\caption{Biased Sampling of $\bbu_{\text{new}}$}
%\label{alg:sample1}
%\If{$\ccalR_D(q_D^{\text{rand}})\neq\emptyset$}{
%Compute $\ccalM(q_D^{\text{rand}})\subseteq \ccalR_D(q_D^{\text{rand}})$\;\label{s:M}
%\If{$\ccalM(q_D^{\text{rand}})\neq\emptyset$}{
%Sample $q_D^{\text{min}}\in\ccalM(q_D^{\text{rand}})$ from $f_D^{\text{min}}$\;\label{s:qBmin}
%Select $q_D^{\text{decr}}\in\ccalR_D^{\text{decr}}(q_D^{\text{min}})$\;\label{s:qBfeas}% from $f_B^{\text{feas}}(q_B|\ccalR_B^{\text{feas}}(q_B^{\text{reach}})):\ccalR_B^{\text{feas}}(q_B^{\text{reach}})\rightarrow[0,1]$\;\label{s:qBfeas}
%Pick $\sigma^*\in\Sigma_{q_D^{\text{min}},q_D^{\text{decr}}}$\;\label{s:sigmamin}
%Compute the target location $t_{j}$ for each robot\;\label{s:sigmamin}
%}
%\Else{$\bbu_{\text{new}}=\varnothing$\;}}\label{s:empty1}
%\Else{$\bbu_{\text{new}}=\varnothing$\;}\label{s:empty2}
%\If{$(\ccalR_D(q_D^{\text{rand}})\neq\emptyset)\wedge(\ccalM(q_D^{\text{rand}})\neq\emptyset)$}{
%\For{$i=1:N$}{
%Pick  $\bbu_{j,\text{new}}$ from $f_{\text{new},j}$, for all robots $i$\;\label{s:fnewi}%(q_{i}^{\text{new}}|q_{\text{PTS}}^{\text{rand}}):\ccalR_{\text{wTS}_i}(q_i^{\text{rand}})\rightarrow[0,1]$
%$f_{\text{new},i}(q_{\text{wTS}_i}^{\text{new}}|q_{\text{PTS}}^{\text{rand}},q_B^{\text{reach}}, q_B^{\text{feas}}):\ccalR_{\text{wTS}_i}(q_{\text{wTS}_i}^{\text{rand}})\rightarrow[0,1]$\;
%}
%Construct $\bbu_{\text{new}}=(\bbu_{1,\text{new}},\dots,\bbu_{N,\text{new}})$\;}\label{s:line5}
%\Return {$q_{\text{PTS}}^{new}$}\;
%\end{algorithm}


==> files/biasedSampling_v2.tex <==
As discussed in Section \ref{sec:complOpt}, any mass functions $f_{\ccalV}$ and $f_{\ccalU}$ that satisfy Assumptions \ref{frand} and \ref{fnew}, respectively, can be employed in Algorithm \ref{alg:RRT} without sacrificing its completeness and optimality guarantees. %to generate states $\bbq_{\text{new}}(t)$ in Algorithm \ref{alg:RRT}.
In what follows, we describe a non-uniform/biased sampling strategy, originally developed in \cite{kantaros2019optimal}, allowing us to address large-scale planning tasks. %that involve large teams of robots and workspaces.
%In what follows, we build upon our previous works \cite{kantaros2019optimal,kantaros2019asymptotically}, to design \textcolor{blue}{mass} functions that allow us to address large-scale planning tasks that involve large teams of robots and workspaces. 

%The  main difference with  \cite{kantaros2018temporal}, in terms of designing sampling functions, is that \cite{kantaros2018temporal} (i) requires discrete abstractions of robot mobility captured by transition systems and (ii) evaluates atomic propositions over a given deterministic map (transition systems).%The main idea is to build $f_{\ccalV}$ and $f_{\ccalU}$ so that the tree is biased to explore regions of $\Omega_{\text{free}}$ where targets are predicted to be. 
%\textcolor{red}{EXPLAIN HOW IT IS DIFFERENT}

\subsection{Pruning the DFA}\label{sec:prune}

We first prune the DFA by removing transitions that are unlikely to be enabled. Particularly, these are DFA transitions that are enabled when a robot $j$ has to satisfy atomic propositions that require it to be present in more than one location \textit{simultaneously}. Hereafter, these DFA transitions are called \textit{infeasible}. %For instance, if a transition is enabled only when a robot $j$ has to satisfy more than one atomic proposition of the form \eqref{ap1}-\eqref{ap2} associated with more than one landmark, then such a transition may be \textit{infeasible}. 
For instance, a DFA transition that is enabled if a robot is required to be simultaneously in more than one known disjoint region of interest, is classified as infeasible; see \cite{kantaros2018text} for more details. %Hereafter, for simplicity, we assume that all regions $\ccalR_e$ are disjoint. 
%Note that detecting transitions that are enabled based on predicates defined over the known environmental geometry can be determined by solving Boolean formulas that are true if at least one robot is required to be in more than region simultaneously; see \cite{kantaros2018text} for more details. 
%
Determining infeasible transitions becomes more challenging for transitions that depend on probabilistic predicates as e.g., in \eqref{ap1}. The reason is that search over the space of distributions is required to determine if there exist robot positions that satisfy a Boolean formula defined over such predicates; recall that the map distribution is updated during the execution of Algorithm \ref{alg:RRT}. 
%
%For instance, consider a transition from $q_D$ to $q_D'$ that is enabled when the following Boolean formula is true: $\pi_p(\bbp(t),\ccalM(t),\{j, \ell_i,r_1,\delta_1\}) \wedge \pi_p(\bbp(t),\ccalM(t),\{j, \ell_e,r_2,\delta_2\}), e\neq i$ which requires robot $j$ to be close to landmarks $\ell_i$ and $\ell_e$, simultaneously, with certain probabilistic requirements determined by $\delta_1$ and $\delta_2$. Note that existence of a robot position $\bbp_j$ that satisfies this depends on the distribution of the position of landmarks $\ell_e$ and $\ell_j$ - which may change during the offline control synthesis process - and the parameters $r_1,\delta_1,r_2,\delta_2$.
%
Hereafter, for simplicity, we classify such DFA transitions that require a robot to be close to more than one landmark at the same time as \textit{infeasible}.\footnote{Note that this is a conservative approach as transitions that are in fact feasible may be classified as infeasible transitions. Nevertheless, this does not affect the correctness of the proposed algorithm, since the biased sampling functions that will be constructed next still satisfy Assumptions \ref{frand} and \ref{fnew}. If in the pruned DFA, there is no path from the initial to the final state then this means that either the specification is infeasible or the task is feasible but the pruning was very conservative. In this case, a warning message can be returned to the user, and either uniform distributions  or the proposed biased distributions can be employed but using the original (and not the pruned) DFA.} 
%  Similarly, DFA transitions that are enabled when a robot is present in more than one disjoint regions simultaneously are also pruned. %We denote by $\Sigma_{q_D,q_D'}^\text{feas}\subseteq\Sigma$ the set that collects all `feasible' finite words $\sigma^* \in {\Sigma}$ enabling transition from a state $q_D$ to $q_D'$ according to $\rightarrow_D$.

Second, along the lines of \cite{kantaros2018text} we define a distance function $d: \ccalQ_D \times \ccalQ_D \rightarrow \mathbb{N}$ between any two DFA states, which captures the minimum number of transitions in the pruned DFA to reach a state $q_D'$ from a state $q_D$. This function is defined as follows
\begin{equation}
d(q_D,q_D')=\left\{
                \begin{array}{ll}
                  |SP_{q_D,q_D'}|, \mbox{if $SP_{q_D,q_D'}$ exists,}\\
                  \infty, ~~~~~~~~~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
%\normalsize
where $SP_{q_D,q_D'}$ denotes the shortest path (in terms of hops) in the  pruned DFA from $q_D$ to $q_D'$ and $|SP_{q_D,q_D'}|$ stands for its cost (number of hops).%\footnote{Note that since $\ccalG_B$ is a directed graph, it does not necessarily hold that $d(q_B,q_B')=d(q_B',q_B)$ or that $d(q_B,q_B)=0$.}% In other words, $d(q_B,q_B')$ represents the minimum number of (feasible) transitions that are required to reach the state $q_B'$ starting from $q_B'$.
%
%%%%
\subsection{Mass function $f_{\ccalV}$}\label{sec:fv}
%First, given the root of the tree we select a \textit{feasible} final state $q_{F}\in\ccalQ_F$, i.e., a final state that is reachable from $q_D^0$ in the pruned DFA. In other words, feasible final states are the ones that satisfy  $d(q_D^0,q_{F})\neq \infty$. Among all final states that satisfy this condition, we select one randomly denoted by $q_F^{\text{feas}}$. %\footnote{Note that if there are more than one final states $q_B^{F,\text{feas}}$, then Algorithm \ref{alg:tree} can be executed for all such final states in parallel.} 
%If there does not exist such a state $q_F^{\text{feas}}$, then this means that there is no feasible path associated with the initial state $q_D^0$ or the pruning of the DFA was conservative yielding a `disconnected' pruned DFA(see the definition of infeasible DFA transitions in Section \ref{sec:prune}). In this case, either uniform sampling functions can be employed or biased sampling functions can be constrcuted as follows but based on the original DFA (and not the pruned one).
%
To construct a non-uniform mass function $f_{\ccalV}$, first, we define the set $\ccalD_{\text{min}}$ that collects all tree nodes $\bbq=(\bbp,\ccalM,q_D)$ with the smallest distance $d(q_D,q_F)$, denoted by $d_{\text{min}}$, among all nodes in the tree, i.e., $\ccalD_{\text{min}}=\{\bbq=(\bbp,\ccalM,q_D)\in\ccalV~|~d(q_D,q_F)=d_{\text{min}} \}$. The set $\ccalD_{\text{min}}$ initially collects only the root and is updated (along with $d_{\text{min}}$) as new states are added to the tree. Given the set $\ccalD_{\text{min}}$, we define the set $\ccalK_{\text{min}}$ that collects the indices $k$ of the subsets $\ccalV_k$ that satisfy $\ccalV_k\cap\ccalD_{\text{min}}\neq\emptyset$.
%
Given the set $\ccalK_{\text{min}}$, the probability mass function $f_{\text{rand}}(k|\ccalV)$ is defined so that it is biased to select more often subsets $\ccalV_k\subseteq\ccalV$ that satisfy $k\in\ccalK_{\text{min}}$. Specifically, $f_{\text{rand}}(k|\ccalV)$ is defined as follows:
%
\begin{equation}\label{eq:frand}
f_{\text{rand}}(k|\ccalV)=\left\{
                \begin{array}{ll}
                  p_{\text{rand}}\frac{1}{|\ccalK_{\text{min}}|}, ~~~~~~~~~~~~\mbox{if}~k\in\ccalK_{\text{min}}\\
                  (1-p_{\text{rand}})\frac{1}{|\ccalV\setminus\ccalK_{\text{min}}|},~\mbox{otherwise},
                \end{array}
              \right.
\end{equation}
where $p_{\text{rand}}\in(0.5,1)$ stands for the probability of selecting \textit{any} subset $\ccalV_k$ that satisfies $k\in\ccalK_{\text{min}}$. Note that $p_{\text{rand}}$ can change with iterations $n$ but it should always satisfy $p_{\text{rand}}\in(0.5,1)$ to ensure that subsets $\ccalV_k$ with $k\in\ccalK_{\text{min}}$ are selected more often. 
%
\subsection{Mass function $f_{\ccalU}$}\label{sec:fu}
The sampling function $f_{\ccalU}(\bbu|k_{\text{rand}})$ is designed so that a state $\bbq=(\bbp,\ccalM,q_F)$ is reached by following the shortest path (in terms of hops) in the pruned DFA that connects $q_D^0$ to $q_F$.  %The proposed biased sampling process is illustrated in Figure \ref{fig:sampling}.%There three main steps to sample such a state $q_{\text{PTS}}^{\text{new}}$. First, given $q_P^{\text{rand}}=(q_{\text{PTS}}^{\text{rand}},q_B^{\text{rand}})$, we construct a set, denoted by $\ccalR_B^{\text{min}}(q_B^{\text{rand}})$ that collects all the states $q_B\in\ccalQ_B$ that can be reached from $q_B^{\text{rand}}$ given the observation $L(q_{\text{PTS}}^{\text{rand}})$. Among all these states we pick the state, denoted by $q_B^{\text{min}}$ that is closer to $q_B^{F,\text{feas}}$ than any other state $q_B\in\ccalR_B^{\text{min}}(q_B^{\text{rand}})$. 
%
%\begin{figure}[t]
%  \centering
%  \includegraphics[width=0.57\linewidth]{sample.eps}
%   \caption{\footnotesize{ depiction of the proposed sampling function when $N=1$. The thick black arrow ends in the state that will be selected with probability $p_{\text{new}}$. Note that for $\sigma^*=L_{i}(q_{i}^{\ccalL(i)})$, it holds that $(q_B^{\text{min}},\sigma^*, q_B^{\text{decr}})\in \rightarrow_B$. Next to each state $q_B\in\ccalQ_B$, we also note inside parentheses the value of $d(q_B,q_B^{F,\text{feas}})$.}}
%  \label{fig:sampling}
%\end{figure}
%Also, by construction of the sampling and the `extend' operation, all states $(q_i,q_B)\in\ccalQ_B$, for some $q_i\in\ccalR_{\text{wTS}_i}(q_i^{\text{rand}})$ and for all $q_B\in\ccalR_{B}(q_B^{\text{rand}})$ will be added to the tree at iteration $n$; see also Proposition 5.1 in \cite{kantaros2017Csampling}
%
%\paragraph{Selection of $q_B^{\text{min}}\in\ccalQ_B$} 
First, given  a state $\bbq_{\text{rand}}=(\bbp_{\text{rand}},\ccalM_{\text{rand}},q_D^{\text{rand}})$, we compute the next DFA state defined as $q_D^{\text{next}}=\delta_D(q_D^{\text{rand}},L(\bbp_{\text{rand}},\ccalM_{\text{rand}}))$. 
%
Next, we construct the reachable set $\ccalR_D(q_D^{\text{next}})$ that collects all states $q_D\in\ccalQ_D$ that can be reached in one hop in the \textit{pruned} DFA from $q_D^{\text{next}}$, for any observation/symbol $\sigma\in 2^{\mathcal{AP}}$, defined as $\ccalR_D(q_D^{\text{next}})=\{q_D\in\ccalQ_D|\exists  \sigma\in 2^{\mathcal{AP}}~\text{s.t.}~\delta_D(q_D^{\text{next}},\sigma)=q_D\}.$
%\begin{equation}\label{eq:reachable}
%\ccalR_D(q_D^{\text{next}})=\{q_D\in\ccalQ_D|\exists  \sigma\in 2^{\mathcal{AP}}~\text{s.t.}~\delta_D(q_D^{\text{next}},\sigma)=q_D\}.    
%\end{equation}
%
Among all states in $\ccalR_D(q_D^{\text{next}})$ we select the state, denoted by $q_D^{\text{min}}$, with the minimum distance from $q_F$. 

\normalsize{Given $q_D^{\text{next}}$ and $q_D^{\text{min}}$, we select a symbol $\sigma$ that enables a transition from $q_D^{\text{next}}$ to $q_D^{\text{min}}$ in the pruned DFA. %Essentially, the word $\sigma^*$ satisfies the Boolean condition associated with the transition from $q_D^{\text{min}}$ to $q_D^{\text{decr}}$ in the DFA. %\footnote{To speed up the detection of final states, we always select the same word$\sigma^*\in\Sigma_{q_D^{\text{min}},q_D^{\text{decr}}}$ for a given pair of states $q_D^{\text{min}}$ and $q_D^{\text{decr}}$. %Also, by construction of $q_D^{\text{decr}}$, it holds that $\Sigma_{q_D^{\text{min}},q_D^{\text{decr}}}\neq\emptyset$.
} 
Based on the selected symbol $\sigma$, we select locations that if every robot visits, then $\sigma$ is generated and transition from $q_D^{\text{next}}$ to $q_D^{\text{min}}$ is achieved.
%
To this end, first we select the atomic proposition that appears in $\sigma$ and is associated with robot $j$. Note that by definition of the feasible transitions and by construction of the pruned DFA, there is only one (if any) atomic proposition in $\sigma$ related to robot $j$. With slight abuse of notation, we denote this atomic proposition by $\pi_j\in\mathcal{AP}$.
%first we construct the set $\Pi_j$ that collects all atomic propositions that appear in $\sigma^*$ and are associated with robot $j$. 
%
For instance, the atomic proposition $\pi_j$ corresponding to the word $\sigma=\pi_p(\bbp,\ccalM,\{j, r_1,\delta_1,c_1\})\pi_p(\bbp,\ccalM,\{z,r_2,\delta_2,c_2\})$ is $\pi_j=\pi_p(\bbp,\ccalM,\{j,r_1,\delta_1,c_1\})$. Also, observe that there is no atomic proposition $\pi_s$ associated with any robot $s\neq j,z$.  
%                                                       
%
%
Next, given $\pi_j$, we select a landmark that if robot $j$ approaches/localizes, then $\pi_j$ may be satisfied. The selected landmark is denoted by $L_j$ and is used to design $f_{\text{new},i}(\bbu_i|k)$ so that control inputs that drive robot $j$ toward $L_j$ are selected more often than others. Note that for robots $j$ for which there is no predicate $\pi_j$ associated with them in $\sigma$, we have that $L_j=\varnothing$. In other words, the location of such robots $j$ does not play any role in generating the word $\sigma$. For instance, following the previous example, $L_j$ is selected to be the landmark that has the highest probability of having the label $c_1$, based on the discrete distribution $\bbd$, while for all other robots $s\neq j,z$ it holds $L_s=\varnothing$.

%Next, we discuss how we select $L_j$ from $\ccalL_j$ for robot $j$.  If the atomic proposition $\pi_j$ is in the form of \eqref{ap1}, i.e., $\pi_j=g(\bbp_j,\ell_i,r,\delta)$, then it trivially holds that $\ccalL_j=\set{\ell_i}$ and, therefore, $L_j=\ell_i$. 
%
%If the atomic proposition $\pi_j$ is in the form of \eqref{ap4}, i.e., $\pi_j=g(\bbp_j,r,\delta,c)$, then we select as $L_j$ from $\ccalL_j$ the landmark $\ell_i$ with maximum value $\frac{d_{c_i}(c_i\in\bar{\ccalC})}{\det\Sigma_i}$, where recall that $\det\Sigma_i$ is the determinant of the covariance matrix $\Sigma_i$. In words, the larger the value of $\frac{d_{c_i}(c_i\in\bar{\ccalC})}{\det\Sigma_i}$ is, the smaller the uncertainty about the position and the class of landmark $\ell_i$. 
%
%Similarly, we construct $L_j$ for atomic propositions $\pi_j$ in the form of \eqref{ap0}. Note that for robots $j$ for which it holds that $\pi_j=\varnothing$, we have that $L_j=\varnothing$, as well. In other words, the location of such robots $j$ does not play any role in generating the word $\sigma$. %The same argument also applies to atomic propositions  in the form of \eqref{ap3}.

Given a landmark $L_j$, we construct the mass function $f_{\text{new},j}(\bbu_j|k)$ from which we sample a control input $\bbu_j$ as follows: 
%
%\footnotesize{
\begin{equation}\label{eq:fnew}
f_{\text{new},j}(\bbu_j|k)=\left\{
                \begin{array}{ll}
                \frac{1}{|\ccalU_j|},~\mbox{if}~L_j=\varnothing,\\
                 p_{\text{new}},\mbox{if}~(L_j\neq\varnothing)\wedge
                   (\bbu_j=\bbu_j^*)\wedge (d_j\geq R_j)\\
                  (1-p_{\text{new}})\frac{1}{|\ccalU_j\setminus\set{\bbu_j^*}|},\mbox{if}~(L_j\neq\varnothing)\\ 
                  ~~~~~~~~~~~~~\wedge(\bbu_j\neq \bbu_j^*)\wedge (d_j\leq R_j),
                \end{array}
              \right.
\end{equation}
%}
\normalsize
where (i) $d_j$ denotes the \textit{geodesic} distance between robot $j$ and the estimated position of landmark $L_j$, i.e., $d_j=\left\lVert\hat{\bbx}_{L_j}(t+1) - \bbp_j(t+1) \right\rVert_g$ \cite{kantaros2016global}, (ii) $R_j$ denotes the sensing range of robot $j$, and (iii) $\bbu_j^{*}\in\ccalU_j$ is the control input that minimizes the geodesic distance between $\bbp_j(t+1)$ and $\hat{\bbx}_i(t+1)$, i.e., $\bbu_j^*=\argmin_{\bbu_j\in\ccalU_j} \left\lVert \hat{\bbx}_i(t+1) - \bbp_j(t+1) \right\rVert_g,$
%\begin{equation}\label{eq:ujstar}
%\bbu_j^*=\argmin_{\bbu_j\in\ccalU_j} \left\lVert \hat{\bbx}_i(t+1) - \bbp_j(t+1) \right\rVert_g,
%\end{equation}
where $\left\lVert \cdot \right\rVert_g$ denotes the geodesic norm/distance. In words, in the first case of \eqref{eq:fnew}, a control input $\bbu_j$ is drawn from a uniform distribution if $L_j=\varnothing$. In the second case, the input $\bbu_j^{*}\in\ccalU_j$ is selected, if the (predicted) distance between robot $j$ and the assigned landmark $L_j$ is greater than the sensing range. In the third case, if the assigned landmark is  within the sensing range, random inputs are selected to get different views of the assigned landmark, which will contribute to decreasing the uncertainty of the assigned landmark. %Note that the only difference if $L_j$ corresponds to a region of interest (i.e., $\pi_j$ is a deterministic atomic proposition as in \eqref{ap0}), is that the sensing range and the distance to the region are not considered.
 
%Also, to compute $\hat{\bbx}_{L_j}(t+1)$, we execute the Kalman-filter prediction step. 
Finally, to compute the geodesic distance between $\bbp_j(t+1)$  and the estimated location of $L_j$, we first treat as `virtual/temporal' obstacles all landmarks that if visited, the Boolean condition under which transition from $q_D^{\text{next}}$ to $q_D^{\text{min}}$ is enabled, is false. For example, assume that transition from  $q_D^{\text{next}}$ to $q_D^{\text{min}}$ is possible if the following Boolean condition is true 
$\pi_p(\bbp,\ccalM,\{j, r_1,\delta_1,c_1\})\wedge\pi_p(\bbp,\ccalM,\{z,r_2,\delta_2,c_2\})\wedge[\neg \pi_p(\bbp,\ccalM,\{j, \ell_1, r_1,\delta_1\})]$
%$\pi_j(\ccalR_1)\wedge \pi_z(\ccalR_2)\wedge(\neg g(\bbp_j,\ell_i,r,\delta))$,
which is satisfied by the following symbol $\sigma=\pi_p(\bbp,\ccalM,\{j, r_1,\delta_1,c_1\})\pi_p(\bbp,\ccalM,\{z,r_2,\delta_2,c_2\})$ and is violated if $\pi_p(\bbp,\ccalM,\{j, \ell_1, r_1,\delta_1\}$ is observed, i.e., if robot $j$ approaches the landmark $\ell_1$ as per the probabilistic requirements captured by $\pi_p(\bbp,\ccalM,\{j, \ell_1, r_1,\delta_1\}$. For such `virtual' obstacles, we first compute a $\epsilon$-confidence interval around the mean position of landmark $\ell_1$, for some $\epsilon>0$ (e.g., $\epsilon=90\%$). This $\epsilon$-confidence interval is then treated as a (known) physical obstacle in the workspace. Then, we compute the \textit{geodesic} distance between $\bbp_j(t+1)$ and  such virtual obstacles. 
%
Essentially, this empirical approach minimizes the probability of generating an observation that violates the assigned task specification. Observe that the `virtual' obstacles are different for each robot while they may also depend on the global state $\bbp(t)$ (and not solely on individual robot states $\bbp_j(t)$). For instance, consider the Boolean condition 
$\pi_p(\bbp,\ccalM,\{j, r_1,\delta_1,c_1\})\wedge\pi_p(\bbp,\ccalM,\{z,r_2,\delta_2,c_2\})\wedge\{[\neg \pi_p(\bbp,\ccalM,\{j, \ell_1, r_1,\delta_1\})] \wedge [\neg \pi_p(\bbp,\ccalM,\{z, \ell_2, r_2,\delta_2\})]\}$
%$\pi_j(\ccalR_1)\wedge \pi_z(\ccalR_2)\wedge(\neg \pi_j(\ccalR_1)\wedge \neg \pi_z(\ccalR_1))$. 
%
This is violated only if \textit{both} robots $j$ and $z$ are sufficiently close to landmarks $\ell_1$ and $\ell_2$, respectively. Such `virtual' obstacles are ignored, i.e., in this case, $\ell_1$ is not treated as an obstacle for robot $j$.

%\red{to be polished}
%Note that if the \textcolor{blue}{mass} functions $f_\text{rand}^n$ and $f_{\text{new},i}^n$ are biased towards states that violate the LTL formula, i.e., states $q_P^{\text{new},n}$ with $\ccalR_P^{\rightarrow}(q_P^{\text{new},n})=\emptyset$, then the parameters $\alpha_n(\texttt{p})$, associated with a \textit{feasible} path $\texttt{p}$, will have low values, by construction of  $f_\text{rand}^n$ and $f_{\text{new},i}^n$. As a result, a large number of iterations is expected until $\texttt{p}$ is detected due to Theorem \ref{thm:conv}. Also, note that in general, it is not possible to know \textit{a priori} whether the states in the PBA which the sampling process is biased to are feasible or not; therefore, in practice, values for $p_{\text{rand}}^n$ and $p_{\text{new}}^n$ that are arbitrarily close to 1 should be avoided, as they might significantly slow down the synthesis part. 
%Finally, observe that if 

%case: never in room1 and room2 at the same time: here room1 and room2 are not obstacles 

% \begin{rem}
% As it will be discussed in Section \ref{sec:extend}, a state $q_P^{\text{new}}=(q_{\text{PTS}}^{\text{new}},q_B^{\text{min}})\in\ccalQ_P$ will be added to the tree, if it has not already been added. By construction of $q_B^{\text{min}}$, when the state $q_P^{\text{new}}$ is selected to be $q_P^{\text{rand}}$
% \end{rem}
%\begin{rem}[Selection of  $q_B^{\text{reach}}$, $q_B^{\text{rand}}$, $\sigma^*$]
%Note that given $q_P^{\text{rand}}$ the states $q_B^{\text{reach}}$ and $q_B^{\text{rand}}$ can also be selected probabilistically from the sets $\ccalR_B(q_B^{\text{rand}})$ and $\ccalR_B^{\text{feas}}(q_B^{\text{reach}})$. However, for simplicity of notations, we avoid presenting such analysis. Also, the word $\sigma^*\in\Sigma_{q_B^{\text{reach}},q_B^{\text{feas}}}$ does not need to remain fixed every time a node $q_P$ is selected to be $q_P^{\text{rand}}$; however, this can slow down the detection of final states. 
%\end{rem}

%\begin{rem}[selection of rrand]
%Note that if $SP_{q_{i}^{\text{rand}},q_{i}^{\ccalL(i)}}(2))$ is a region that robot $i$ should always avoid, then for high values of $p_{\text{new}}$, a state q_{PTS}^{new} will be constructed that will be rejected in the step. 
%\end{rem}

%\begin{algorithm}[t]
%\footnotesize
%\caption{Biased Sampling of $\bbu_{\text{new}}$}
%\label{alg:sample1}
%\If{$\ccalR_D(q_D^{\text{rand}})\neq\emptyset$}{
%Compute $\ccalM(q_D^{\text{rand}})\subseteq \ccalR_D(q_D^{\text{rand}})$\;\label{s:M}
%\If{$\ccalM(q_D^{\text{rand}})\neq\emptyset$}{
%Sample $q_D^{\text{min}}\in\ccalM(q_D^{\text{rand}})$ from $f_D^{\text{min}}$\;\label{s:qBmin}
%Select $q_D^{\text{decr}}\in\ccalR_D^{\text{decr}}(q_D^{\text{min}})$\;\label{s:qBfeas}% from $f_B^{\text{feas}}(q_B|\ccalR_B^{\text{feas}}(q_B^{\text{reach}})):\ccalR_B^{\text{feas}}(q_B^{\text{reach}})\rightarrow[0,1]$\;\label{s:qBfeas}
%Pick $\sigma^*\in\Sigma_{q_D^{\text{min}},q_D^{\text{decr}}}$\;\label{s:sigmamin}
%Compute the target location $t_{j}$ for each robot\;\label{s:sigmamin}
%}
%\Else{$\bbu_{\text{new}}=\varnothing$\;}}\label{s:empty1}
%\Else{$\bbu_{\text{new}}=\varnothing$\;}\label{s:empty2}
%\If{$(\ccalR_D(q_D^{\text{rand}})\neq\emptyset)\wedge(\ccalM(q_D^{\text{rand}})\neq\emptyset)$}{
%\For{$i=1:N$}{
%Pick  $\bbu_{j,\text{new}}$ from $f_{\text{new},j}$, for all robots $i$\;\label{s:fnewi}%(q_{i}^{\text{new}}|q_{\text{PTS}}^{\text{rand}}):\ccalR_{\text{wTS}_i}(q_i^{\text{rand}})\rightarrow[0,1]$
%$f_{\text{new},i}(q_{\text{wTS}_i}^{\text{new}}|q_{\text{PTS}}^{\text{rand}},q_B^{\text{reach}}, q_B^{\text{feas}}):\ccalR_{\text{wTS}_i}(q_{\text{wTS}_i}^{\text{rand}})\rightarrow[0,1]$\;
%}
%Construct $\bbu_{\text{new}}=(\bbu_{1,\text{new}},\dots,\bbu_{N,\text{new}})$\;}\label{s:line5}
%\Return {$q_{\text{PTS}}^{new}$}\;
%\end{algorithm}




==> files/proofs.tex <==
%\section{Proof of Completeness \& Optimality}\label{sec:prop}

In what follows, we denote by $\mathcal{G}^n=\{\mathcal{V}^{n}, \mathcal{E}^{n}, \ccalJ_{\ccalG}\}$ the tree that has been built by Algorithm \ref{alg:RRT} by the $n$-th iteration. The same notation also extends to $f_{\ccalV}$, $f_{\ccalU}$, and $\bbu_{\text{new}}$. %We also denote by $f_{\ccalV}^n$ and $f_{\ccalU}^n$ the density functions used at iteration $n$ of Algorithm \ref{alg:RRT}. The same notations extends to subsets $\ccalV_{k}$ $k_{\text{rand}}$, and $\bbu_{\text{new}}$. For simplicity of notations, we denote by $\ccalV_{k_{\text{rand}}}^n\subseteq \ccalV^n$ (instead of  $\ccalV_{k_{\text{rand}}^n}^n$) the subset of nodes selected by $f_{\ccalV}^n$ at iteration $n$.
%
%
%
To prove Theorems \ref{thm:probCompl} and \ref{thm:asOpt}, it suffices to show that Algorithm \ref{alg:RRT} can find all possible paths $\bbq_{0:H}$, for any $H>0$, whether they are feasible or not, with probability $1$ as $n\to\infty$. Showing this result means that if there exists a feasible (including the optimal) path $\bbq_{0:H}$, then Algorithm \ref{alg:RRT} will find it with probability $1$ as $n\to\infty$. The key idea is to prove that once any node is added to the tree, then eventually this node will be extended towards all possible feasible directions as per the set of control inputs $\ccalU$. A key assumption to show this is that of finite control space $\ccalU$. %any feasible path that satisfies all constraints of \eqref{eq:Prob2} and, therefore, the optimal one. 
To show this result, we first need to state the following results. %Their proofs are omitted due to space limitations. %that rely on the Borel-Cantelli lemma \cite{grimmett2001probability}.

%\begin{lem}[Borel-Cantelli \cite{grimmett2001probability}]\label{lem:bc}
%Consider a sequence of independent events $A=\{A^n\}_{n=1}^{\infty}$. If $\sum_{n=1}^{\infty}\mathbb{P}(A^n)=\infty$ then $\mathbb{P}(\limsup_{n\to\infty} A^n)=1$, i.e., the probability that infinitely many events $A^n$ occur is 1.  
%i.e., the events $A^n$ occur infinitely often meaning that $A^n$ is true for an infinite number of indices $n\in\mathbb{N}_{+}$.
%\end{lem}


\begin{lem}[Sampling $\ccalV_{k_{\text{rand}}}^n$]
Consider any subset $\ccalV_{k}^n$ and any fixed iteration index $n$ and any fixed $k\in\set{1,\dots,K_n}$. Then, there exists an infinite number of subsequent iterations $n+w$,  where $w\in\mathcal{W}\subseteq\mathbb{N}$ and $\ccalW$ is a subsequence of $\mathbb{N}$, at which the subset $\ccalV_{k}^n$ is selected to be the set $\ccalV_{k_{\text{rand}}}^{n+w}$. %\footnote{The subsequences $\ccalK$ and $\ccalK'$}
\label{lem:qrand}
\end{lem}

\begin{proof}
Let $A^{\text{rand},n+w}(k)=\{\ccalV_{k_{\text{rand}}}^{n+w}=\ccalV_{k}^n\}$, with $w\in\mathbb{N}$, denote the event that at iteration $n+w$ of Algorithm \ref{alg:RRT} the subset $\ccalV_{k}^n\subseteq\ccalV^n$ is selected by the sampling operation to be the set $\ccalV_{k_{\text{rand}}}^{n+w}$ [line \ref{rrt:samplekrand}, Alg. \ref{alg:RRT}]. Also, let $\mathbb{P}(A^{\text{rand},n+w}(k))$ denote the probability of this event, i.e., $\mathbb{P}(A^{\text{rand},n+w}(k))=f_{\ccalV}^{n+w}(k)$. 

Next, define the infinite sequence of events $A^{\text{rand}}=\{A^{\text{rand},n+w}(k)\}_{w=0}^{\infty}$, for a given subset $\ccalV_{k}^n\subseteq\ccalV^n$. In what follows, we show that the series $\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))$ diverges and then we complete the proof by applying the Borel-Cantelli lemma \cite{grimmett2001probability}. %Lemma \ref{lem:bc}. 
%
%Recall first that the size of $K_{n+e}$, i.e., the number of  subsets $\ccalV_{T,k}^{n+e}$ cannot grow arbitrarily large as $e\to\infinity$, since it holds that $|\ccalU|=|\ccalU_1\times\ccalU_2\times\dots\times\ccalU_n|<\infty$, by assumption. Also, 

Recall that by Assumption \ref{frand}(i) we have that  given any subset $\ccalV_{k}^n\subseteq\ccalV^n$, the probability $f_{\ccalV}^n(k|\ccalV^n)$ satisfies $f_{\ccalV}^n(k|\ccalV^n)\geq \epsilon$, for any iteration $n$. Thus we have that $\mathbb{P}(A^{\text{rand},n+w}(k))=f_{\ccalV}^{n+w}(k|\ccalV^{n+w})\geq \epsilon>0, 
$
%\begin{equation}\label{ineq1}
%\mathbb{P}(A^{\text{rand},n+w}(k))=f_{\ccalV}^{n+w}(k|\ccalV^{n+w})\geq \epsilon> 0, 
%\end{equation} 
for all $w\in\mathbb{N}$. Note that this result holds for any $k\in\set{1,\dots,K_{n+w}}$ due to Assumption \ref{frand}(i). 
%
%Since \eqref{ineq1} holds for all $w\in\mathbb{N}$, 
Therefore, we have that $\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))\geq\sum_{w=0}^{\infty}\epsilon.$
%\begin{equation}\label{ineq2}
%\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))\geq\sum_{w=0}^{\infty}\epsilon.
%\end{equation}
Since $\epsilon$ is a strictly positive constant, we have that $\sum_{w=0}^{\infty}\epsilon$ diverges. Then, %by the comparison test \cite{marsden1993elementary}, 
we conclude that $\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))=\infty.$
%\begin{equation}\label{res1}
%\sum_{w=0}^{\infty}\mathbb{P}(A^{\text{rand},n+w}(k))=\infty.
%\end{equation}
%
Combining this result with the fact that the events $A^{\text{rand},n+w}(k)$ are independent by Assumption \ref{frand}(ii), we get that $\mathbb{P}(\limsup_{k\to\infty} A^{\text{rand},n+w}(k))=1,$ by the Borel-Cantelli lemma. In other words, the events $A^{\text{rand},n+w}(k)$ occur infinitely often, for all $k\in\{1,\dots,K_n\}$. This equivalently means that for every subset $\ccalV_{k}^n\subseteq\ccalV^n$, for all $n\in\mathbb{N}_{+}$, there exists an infinite subsequence $\mathcal{W}\subseteq \mathbb{N}$ so that for all $w\in\mathcal{W}$ it holds $\ccalV_{k_{\text{rand}}}^{n+w}=\ccalV^{n}$, completing the proof.
\end{proof}

    
%Using Lemma \ref{lem:qrand} we can show the following result for the control input.
\begin{lem}[Sampling $\bbu_{\text{new}}$]
Consider any  subset $\ccalV_{k_{\text{rand}}}^n$ selected by $f_{\ccalV}$ and any fixed iteration index $n$. Then, for any given control input $\bbu\in\ccalU$, there exists an infinite number of subsequent iterations $n+w$, where $w\in\mathcal{W}'$ and $\mathcal{W}'\subseteq\mathcal{W}$ is a subsequence of the sequence of $\mathcal{W}$ defined in Lemma \ref{lem:qrand}, at which the control input $\bbu\in\ccalU$ is selected to be $\bbu_{\text{new}}^{n+w}$.
\label{lem:qnew}
\end{lem}

\begin{proof}
Define the infinite sequence of events $A^{\text{new}}=\{A^{\text{new},n+w}(\bbu)\}_{w=0}^{\infty}$, for $\bbu\in\ccalU$, where $A^{\text{new},n+w}(\bbu)=\{\bbu_{\text{new}}^{n+w}=\bbu\}$, for $w\in\mathbb{N}$, denotes the event that at iteration $n+w$ of Algorithm \ref{alg:RRT} the control input $\bbu\in\ccalU$ is selected by the sampling function to be the input $\bbu_{\text{new}}^{n+w}$, given the subset $\ccalV_{k_{\text{rand}}}^n\in\ccalV_{k_{\text{rand}}}^{n+w}$. Moreover, let $\mathbb{P}(A^{\text{new},n+w}(\bbu))$ denote the probability of this event, i.e., $\mathbb{P}(A^{\text{new},n+w}(\bbu))=f_{\ccalU}^{n+w}(\bbu| \ccalV_{k_{\text{rand}}}^{n+w})$. 
%
Now, consider those iterations $n+w$ with $w\in\mathcal{W}$ such that $k_{\text{rand}}^{n+w}=k_{\text{rand}}^n$ by Lemma \ref{lem:qrand}. We will show that the series $\sum_{w\in\ccalW}\mathbb{P}(A^{\text{new},n+w}(\bbu))$ diverges and then we will use the Borel-Cantelli lemma to show that any given $\bbu\in\ccalU$ will be selected infinitely often to be control input $\bbu_{\text{new}}^{n+w}$.
%
By Assumption \ref{fnew}(i)  we have that $\mathbb{P}(A^{\text{new},n+w}(\bbu))=f_{\ccalU}^{n+w}(\bbu| \ccalV_{k_{\text{rand}}}^{n+w})$ is bounded below by a strictly positive constant $\zeta>0$ for all $w\in\ccalW$. 
Therefore, we have that $\sum_{w\in\ccalW}\mathbb{P}(A^{\text{new},n+w}(\bbu))$ diverges, since it is an infinite sum of a strictly positive constant term. Using this result along with the fact that the events $A^{\text{new},n+w}(\bbu)$ are independent, by Assumption \ref{fnew}(ii), we get that $\mathbb{P}(\limsup_{w\to\infty} A^{\text{new},n+w}(\bbu))=1,$ due to the Borel-Cantelli lemma. In words, this means that the events $A^{\text{new},n+w}(\bbu)$ for $w\in\mathcal{W}$ occur infinitely often. Thus, given any subset $\ccalV_{k_{\text{rand}}}^n$, for every control input $\bbu$ and for all $n\in\mathbb{N}_{+}$, there exists an infinite subsequence $\mathcal{W}' \subseteq \mathcal{W}$ so that for all $w\in\mathcal{W}'$ it holds $\bbu_{\text{new}}^{n+w}=\bbu$. %, completing the proof.
\end{proof}
Before stating the next result we first define the \textit{reachable} state-space of a state $\bbq(t)=[\bbp(t),\ccalM(t), q_D(t)]\in\ccalV_{k}^n$, denoted by $\ccalR(\bbq(t))$, that collects all states $\bbq(t+1)=[\bbp(t+1),\ccalM(t+1), q_D(t+1)]$ that can be reached within one time step from $\bbq(t)$.%, where recall that  $\bbp_j(t+1)=\bbf_j(\bbp_j(t),\bbu_j)\in\Omega_{\text{free}}$, $d_i(t+1)=\det\Sigma_i(t+1)=\det\rho(\Sigma_i(t))$. In math, $\ccalR(\bbq(t))$ is defined as follows. 

%\begin{align}\label{eq:reachableSet}
%\ccalR(\bbq(t))&=\{\bbq(t+1)=[\bbp(t+1), \bbd(t+1)]~|~\nonumber \\ &\bbp_j(t+1)=\bbg(\bbp_j(t),\bbu_j), \forall j,\\& d_i(t+1)=\Sigma_i(t+1)=\det\rho(\Sigma_i(t)), \forall i, \forall \bbu\in\ccalU \}\nonumber.
%\end{align}

%\subsection{Proof of Corollary \ref{cor:reach}}
%Algorithm \ref{alg:RRT} will add to $\ccalV^n$
\begin{cor}[Reachable set $\ccalR(\bbq)$]\label{cor:reach}
Given any state $\bbq=[\bbp,\ccalM,q_D]\in\ccalV_{k}^n$, for any $k\in\{1,\dots,K_n\}$, all states that belong to the reachable set $\ccalR(\bbq)$ will be added to $\ccalV^{n+w}$, with probability 1, as $w\to\infty$, i.e., $\lim_{w\rightarrow\infty} \mathbb{P}\left(\{\ccalR(\bbq)\subseteq\mathcal{V}^{n+w}\}\right)=1.$
%\begin{equation}\label{eq:reach2}
%\lim_{w\rightarrow\infty} %\mathbb{P}\left(\{\ccalR(\bbq(t))\subseteq\mathcal{V}^{n+w}\}%\right)=1.
%\end{equation}
Also, edges from $\bbq(t)$ to all reachable states $\bbq'\in\ccalR(\bbq)$ will  be added to $\ccalE^{n+w}$, with probability 1, as $w\to\infty$, i.e., $\lim_{w\rightarrow\infty} \mathbb{P}\left(\{\cup_{\bbq'\in\ccalR(\bbq)}(\bbq,\bbq')\subseteq\mathcal{E}^{n+w}\}\right)=1.$
%\begin{equation}\label{eq:reachedge}
%\lim_{w\rightarrow\infty} %\mathbb{P}\left(\{\cup_{\bbq'\in\ccalR(\bbq)}(\bbq,\bbq')\sub%seteq\mathcal{E}^{n+w}\}\right)=1.
%\end{equation}
\end{cor}

\begin{proof}
We show this result by contradiction. Let $\bbq\in\ccalV_{k}^n$ and $\bbq'\in\ccalR(\bbq)$. Since $\bbq'\in\ccalR(\bbq)$ we have that there exists a control input $\bbu$ so that $\bbq'$ can be reached from $\bbq$.
%
Assume that the edge from $\bbq$ to $\bbq'$ will never be added to the tree. This can happen in the following two cases. (i) There exists no subsequent iteration $n+w$, for some $w>0$, where the set $\ccalV_{k}^n$ will be selected to be $\ccalV_{{k_{\text{rand}}}}^{n+w}$ and, therefore, no edges starting from $\bbq$ will ever be constructed. However, this contradicts Lemma \ref{lem:qrand}. (ii) There exists no subsequent iteration $n+w$, for some $w>0$, where the control input $u$ will be selected to be $\bbu_{\text{new}}^{n+w}$ and, therefore, the edge from $\bbq$ to $\bbq'$ will never be considered to be added to the tree. However, this contradicts Lemma \ref{lem:qnew}. Therefore, we conclude that all states that belong to the reachable set $\ccalR(\bbq)$ along with edges from $\bbq$ to the states in $\ccalR(\bbq)$ will eventually be added to the tree structure. In mathematical terms this can be written as $\lim_{w\rightarrow\infty} \mathbb{P}\left(\{\ccalR(\bbq(t))\subseteq\mathcal{V}^{n+w}\}\right)=1$ and %Also, edges from $\bbq\in\ccalV$ to nodes $\bbq'\in\ccalR(\bbq)$ will eventually be added to the tree structure with probability 1, i.e.,  
$\lim_{w\rightarrow\infty} \mathbb{P}\left(\{\cup_{\bbq'\in\ccalR(\bbq)}(\bbq,\bbq')\subseteq\mathcal{E}^{n+w}\}\right)=1$, completing the proof.
%
%This result straightforwardly holds due to Lemmas \ref{lem:qrand} and \ref{lem:qnew}. Specifically, recall from Lemma \ref{lem:qrand}, that for any given and fixed iteration index $n$ of Algorithm \ref{alg:RRT}, there exists an infinite sequence of iterations $n+w$, $w\in\ccalW$, where the subset $\ccalV_{k}^{n+w}$, for any given and fixed $k$, will be selected to be the subset $\ccalV_{{k_{\text{rand}}}}^{n+w}$. Also, given a control input $\bbu_{\text{new}}^{n+w}$ sampled by $f_{\ccalU}^{n+w}$, we have that the state $\bbq'=[\bbp'(t+1),\ccalM(t+1), q_D']$, where $\bbp(t+1)=\bbg(\bbp(t),\bbu_{\text{new}}^{n+w})$, will be added to the tree, if $\bbp'(t+1)\in\Omega_{\text{free}}^N$. By Lemma \ref{lem:qnew}, we get that there exist an infinite sequence number of iterations $n+w$, $w\in\ccalW'\subseteq \ccalW$, where any given control input $\bbu\in\ccalU$ will be selected to be $\bbu_{\text{new}}^{n+w}$. %%%Since it holds that if $\bbq\in\ccalV_{k}^{n}$, then it trivially holds that $\bbq\in\ccalV_{k}^{n+w}$, for all $n+w\geq n$. 
%Thus, we conclude that all states that belong to the reachable set $\ccalR(\bbq(t))$ will eventually be added to the tree structure. In mathematical terms this can be written as $\lim_{w\rightarrow\infty} \mathbb{P}\left(\{\ccalR(\bbq(t))\subseteq\mathcal{V}^{n+w}\}\right)=1.$, completing the first part of the proof. 
%
%Moreover, observe that when a state $\bbq'\in\ccalR(\bbq)$ (where $\bbq$ is selected to be the node $\bbq_{\text{rand}}^{n+w}$) is added to the set of nodes $\ccalV^{n+w}$, then the edge $(\bbq,\bbq')$ is also added to the set of edges $\ccalE^{n+w}$ by construction of Algorithm \ref{alg:RRT}. This means that $\lim_{w\rightarrow\infty} \mathbb{P}\left(\{\cup_{\bbq'\in\ccalR(\bbq)}(\bbq,\bbq')\subseteq\mathcal{E}^{n+w}\}\right)=1$, completing the proof.
\end{proof}

%Given the above results we are now ready to prove that Algorithm \ref{alg:RRT} is probabilistically complete and asymptotically optimal.
%\subsection{Probabilistic Completeness - Proof of Theorem \ref{thm:probCompl}}\label{app:compl}

%To show this result it suffices to show that $\lim_{n\rightarrow\infty} \mathbb{P}\left(A^n(\bbq_{0:H})\right)=1,$
%\begin{equation}\label{eq:show}
%\lim_{n\rightarrow\infty} %\mathbb{P}\left(A^n(\bbq_{0:H})\right)=1,
%\end{equation}
%where  $A^n(\bbq_{0:H})=\{(\bbq(h)\in\ccalV^n) \wedge ((\bbq(f-1), \bbq(h))\in\mathcal{E}^{n}), \forall f\in\{1,\dots,F\} \}$ denotes the event that at iteration $n$ of Algorithm \ref{alg:RRT} the path $\bbq_{0:H}$ in \eqref{eq:path} has been included in the tree $\ccalG^n$, i.e.,  the states $\bbq(h)$ have been added to the set of nodes $\ccalV^n$ and the edges  $(\bbq(f-1), \bbq(h))$ have been to set of edges $\mathcal{E}^{n}$ for all $f\in\{1,\dots,F\}$. %In words, \eqref{eq:show} says that the path \eqref{eq:path} will be detected with probability $1$ as $n\to\infty$.


\begin{cor}\label{cor:paths}
Consider any (feasible or not) path $\bbq_{0:H}=\bbq(0),\bbq(1),\dots,\bbq(H)$, where $\bbq(h)\in\ccalR(\bbq(h-1))$, for all $h\in\{1,\dots,H\}$. Then Algorithm \ref{alg:RRT} will find $\bbq_{0:H}$ with probability $1$ as $n\to\infty$.
\end{cor}
\begin{proof}
By construction of the path $\bbq_{0:H}$, it holds that $\bbq(h)\in\ccalR(\bbq(h-1))$, for all $h\in\{1,\dots,H\}$. Since $\bbq(0)\in\ccalV^1$, it holds that all states $\bbq\in\ccalR(\bbq(0))$, including the state $\bbq(1)$ (i.e., the second state in the path $\bbq_{0:H}$), will be added to $\ccalV^n$ with probability $1$, as $n\to\infty$, due to Corollary \ref{cor:reach}. %; see \eqref{eq:reach2}. 
Once this happens, the edge $(\bbq(0),\bbq(1))$ will be added to set of edges $\ccalE^n$ due to Corollary \ref{cor:reach}. %; see \eqref{eq:reachedge}.
Applying Corollary \ref{cor:reach} inductively, we get that $\lim_{n\rightarrow\infty} \mathbb{P}\left(\{\bbq(h)\in\mathcal{V}^{n}\}\right)=1$ and $\lim_{n\rightarrow\infty} \mathbb{P}\left(\{(\bbq(h-1), \bbq(h))\in\mathcal{E}^{n}\}\right)=1$, for all $h\in\{1,\dots,H\}$ meaning that the path $\bbq_{0:H}$ will be added to the tree $\ccalG^n$ with probability $1$ as $n\to\infty$.
\end{proof}

{\bf{Proof of Theorem \ref{thm:probCompl}}:}  
Probabilistic completeness directly follows from Corollary \ref{cor:paths}. Specifically, since Algorithm \ref{alg:RRT} can find all possible paths $\bbq_{0:H}$, it will also find any feasible path (if they exist), that satisfy $\phi$. %, including the optimal one
 %\red{[similar to the argument for prob completeness of rrt]}.% Therefore, \eqref{eq:show} holds completing the proof. 
%\begin{equation}\label{eq:prob3}
%\lim_{n\rightarrow\infty} \mathbb{P}\left(A^n(\texttt{path})\right)=1,
%\end{equation}
%for any finite path $\texttt{path}$ that resides in $\Omega_{\text{free}}^N\times\mathbb{R}_{+}$ generated as per the observation model \eqref{eq:measModel} and the robot dynamics \eqref{eq:rdynamics}. This means that if there exists feasible solution to Problem \ref{prob}, then Algorithm \ref{alg:RRT} will detect it with probability $1$ as $n\to\infty$. Therefore, \eqref{eq:show} holds for any feasible path $\texttt{path}$ completing the proof.

%\subsection{Asymptotic optimality - Proof of Theorem \ref{thm:asOpt}}\label{app:opt}
{\bf{Proof of Theorem \ref{thm:asOpt}}:} The proof of this result follows from Theorem \ref{thm:probCompl}. Specifically, recall from Theorem \ref{thm:probCompl} that Algorithm \ref{alg:RRT} can find any feasible path and, therefore, the optimal path, as well, with probability $1$, as $n\to\infty$. 

%{\bf{Proof of Theorem \ref{thm:conv}}:}
%To prove this result, we model the sampling strategy employed by Algorithm \ref{alg:RRT} as a Poisson binomial process. Specifically, we define Bernoulli random variables $Y_n$ at every iteration $n$ of Algorithm \ref{alg:RRT} so that $Y_n=1$ only if the edge $(\bbq(h-1), \bbq(h))$ is added to the tree at iteration $n$, where $h$ is the smallest element of the set $\set{1,\dots,H}$ that satisfies $\bbq(h-1)\in\ccalV^{n-1}$ and $\bbq(h)\notin\ccalV^{n-1}$. Then, using the random variables $Y_n$, we define the random variable $Y=\sum_{n=1}^{n_{\text{max}}}Y_n$ which captures the total number of successes of the random variables $Y_n$ and we show that it follows a Poisson binomial distribution. Finally, we show that $  \mathbb{P}(A^{n_{\text{max}}}(\bbq_{0:H}^*))=\mathbb{P}(Y\geq H)$ which yields \eqref{eq:bnd1} by applying the Chernoff bounds to $Y$. The detailed proof is omitted due to space limitations \red{[will be added later]}.%-\eqref{eq:bnd2}.


==> files/sim.tex <==
% N=20, M=15, H=564, 514.328759
%N=20, M=30, H=570, 635.502483 
%N=40, M=30, H=453, 943.722735
%N=40, M=15,H=453, 924.520976



%\begin{figure}[t]
%  \centering
% %    \subfigure[$N=1, M=5$ (slow targets)]{
% %   \label{fig:traj15s}
%%%  \includegraphics[width=0.48\linewidth]{traj_1vs5_slow.pdf}}
%\includegraphics[width=0.9\linewidth]{figures/map_mobile_landmarks.png}
%\caption{\red{[this is for the case study with mobile landmarks]}Initial Semantic Map.}
%  \label{fig:map_ML}
%3456787`-1Q\
%\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.75\linewidth]{figures/map1_30.png}
\caption{Initial semantic map $\ccalM(0)$ with $30$ landmarks considered in Table \ref{tab:scaleSum}. The map with the $15$ landmarks considered in the same table consists of the landmarks $\ell_i$ with indices $i\in\{1,\dots,15\}$ shown in this figure.}
  \label{fig:maps_tables}
\end{figure}


%\begin{figure}[t]
%  \centering
%    \subfigure[$M=15$]{
%    \label{fig:map15}
%  \includegraphics[width=0.48\linewidth]{figures/map1_15.png}}
%      \subfigure[$M=30$]{
%    \label{fig:map30}
%  \includegraphics[width=0.48\linewidth]{figures/map1_30.png}}
%\caption{Initial semantic maps $\ccalM(0)$ used to generate the results in Tables \ref{tab:scale}-\ref{tab:scale2}. }
%  \label{fig:maps_tables}
%\end{figure}

In this section, we present experimental case studies that illustrate the performance of Algorithm \ref{alg:RRT} and show that it can solve large-scale planning tasks in uncertain environments. In Section \ref{sec:scale}, we demonstrate scalability of Algorithm \ref{alg:RRT} with respect to the number of landmarks and robots. In particular, given an initial semantic map and an initial multi-robot state, we report the time required by Algorithm \ref{alg:RRT} to find the first feasible solution along with the corresponding terminal horizon (without considering re-planning). \textcolor{black}{The scalability analysis has been conducted using MATLAB 2016b on a computer with Intel Core i7 3.1GHz and 16Gb RAM.}
%
In Section \ref{sec:replanSim}, we demonstrate in a Gazebo simulated semantic city the re-planning framework, discussed in Section \ref{sec:replan}, for various initial semantic maps. %In particular, we show that the more uncertain/inaccurate the initial semantic map is, the more often re-planning is triggered. 
\textcolor{black}{These experiments have been conducted on Gazebo (ROS, python3) on a computer with Intel Core i5 - 8350U 1.7GHz and 16Gb RAM.}
%
Finally, in Section \ref{sec:noMap}, we show how Algorithm \ref{alg:RRT} can be applied in environments with no prior information about their metric/semantic structure, as per the discussion provided in Section \ref{sec:extensions}. The experimental videos can be found in \cite{SimSemMaps}.
%https://youtu.be/g2euNw_KmYU
%The software simulation stack used is based on the Robot Operating System (ROS).
%
 %and we select a distance-based motion cost function: $w(\bbp(t),\bbp(t+1))=\sum_{j=1}^N||\bbp_j(t)-\bbp_j(t+1)||$. 
%
%\subsection{Robot Dynamics \& Sensors}\label{sec:rmodel}
%Throughout this section, we consider robots that reside in a non-convex environment $\Omega\subset\mathbb{R}^2$ with obstacles; see e.g., Figure \ref{fig:traj15s}. Also, 
%
\subsection{Scalability Analysis: Offline Planning over Prior Semantic Maps}\label{sec:scale}
In what follows, we examine the scalability performance of Algorithm \ref{alg:RRT} with respect to the number $N$ of robots, and the number $M$ of landmarks. We first describe the robot dynamics, the sensor model, the setup of the initial semantic map, the structure of the assigned LTL task, and then we conclude with the scalability analysis summarized in Tables \ref{tab:scaleSum}-\ref{tab:scale3}.
\normalsize
\subsubsection{Robot Dynamics} We consider robots with the following differential drive dynamics:

%The linear dynamics are defined as  
%\begin{equation}\label{eq:linRbt}
%\bbp_j(t+1)=\bbp_j(t)+\bbu_j(t),
%\end{equation}
%where $\bbp_j(t)\in\mathbb{R}^2$ denotes the position of robot $j$, and 
%$\left\lVert\bbu_j(t) \right\rVert\in\{0, 0.2\}$, for all robots $j$.
%The nonlinear dynamics are defined as 
%
\footnotesize{
\begin{equation}\label{eq:nonlinRbt}
\begin{bmatrix}
   p_j^1(t+1) \\
  p_j^2(t+1)\\
  \theta_j(t+1)
  \end{bmatrix}=  
  \begin{bmatrix}
   p_j^1(t) \\
  p_j^2(t)\\
  \theta_j(t)
  \end{bmatrix}+    
   \begin{cases}
        \begin{bmatrix}
   \tau u \cos(\theta_j(t)+\tau\omega/2) \\
   \tau u \sin(\theta_j(t)+\tau\omega/2)\\
     \tau  \omega
     \end{bmatrix}, \text{if} ~\tau\omega<0.001\\
  \\
 \begin{bmatrix}
   \frac{u}{\omega} (\sin(\theta_j(t)+\tau\omega)-\sin(\theta_j(t))) \\
   \frac{u}{\omega} (\cos(\theta_j(t)) - \cos(\theta_j(t)+\tau\omega)) \\
  \tau \omega
  \end{bmatrix}, \text{else},
    \end{cases}      
\end{equation}}
\normalsize
where the robot state $\bbp_j(t)=[p_j^1(t),p_j^2(t),\theta_j]^T$ captures both the position $[p_j^1(t),p_j^2(t)]$ and the orientation $\theta_j(t)$ of robot $j$ and $\tau$ is the sampling period. The available motion primitives are $u\in\{0,1\}\text{m/s}$ and $\omega\in\set{0,\pm 1,\pm 2,\dots, \pm 180}\text{degree/s}$.
%where $u\in\{0,0.2\}\text{m/s}$ and $\omega\in\set{0,\pm \pi/4,\pm \pi/2, \pm \pi/1.33, \pm \pi}$. Note in \eqref{eq:nonlinRbt}, that the state $\bbp_j(t)$ includes both the position $[p_j^1(t),p_j^2(t)]^T$ and the orientation  $\theta_j(t)$ of the robots, i.e., $\bbp_j(t)=[p_j^1(t),p_j^2(t),\theta_j(t)]^T$.

\subsubsection{Sensor Model \eqref{eq:measModelR}} All robots are equipped with omnidirectional, range-only, line-of-sight sensors with limited range of $1$m. Every robot can take noisy range measurements, i.e., measure its distance from all landmarks that lie within its sight and range. Specifically, the measurement associated with robot $j$ and landmark $i$ is given by %$y_{j,i}^r = \ell_{j,i}(t) + v(t) \ ~\mbox{if}~ \ (\ell_{j,i}(t) \leq R_j) \wedge (i\in\texttt{FOV}_j)$,
\begin{equation}\label{eq:meassim}
y_{j,i} = \ell_{j,i}(t) + v(t) \ ~\mbox{if}~ \ (\ell_{j,i}(t) \leq R_j) \wedge (i\in\texttt{FOV}_j).
\end{equation}
%
where $\ell_{j,i}(t)$ is the distance between landmark $\ell_i$ and robot $j$, $R_j$ denotes the sensing range of robot $j$ which is equal to $1$m, $\texttt{FOV}_j$ denotes its corresponding field-of-view, and $v(t) \sim \ccalN(0,\sigma(\bbx_i(t),\bbp_j(t)))$ is the measurement noise. 
%schlotfeldt2018anytime
Also, we model the measurement noise so that $\sigma$ increases linearly with $\ell_{j,i}(t)$, with slope $0.5$, as long as $\ell_{j,i}(t)\leq R_j$; if $\ell_{j,i}(t)> R_j$, then $\sigma$ is infinite. This model captures the fact that range readings become more inaccurate as the distance increases \cite{schlotfeldt2018anytime}; nevertheless, any other model can be used, such as uniform noise within the sensing range. Observe that the considered observation model is nonlinear and, therefore, the a-posteriori covariance matrix, cannot be estimated optimally offline; see \eqref{constr7c}.
%
In this case, at every iteration of Algorithm \ref{alg:RRT},  we approximately compute the a-posteriori covariance matrices $\Sigma_{\text{new}}$ using the linearized observation model about the predicted positions of the landmarks [line \ref{rrt:Sigmanew}, Alg. \ref{alg:RRT}].\footnote{We avoid defining an object recognition method as per \eqref{eq:measModelC}, as the main focus of this section is to demonstrate scalability of Algorithm \ref{alg:RRT} in terms of solving \eqref{eq:Prob2} without considering re-planning. Recall that \eqref{eq:Prob2} does not depend on the object recognition method. In fact, the latter is needed only for learning online the semantic map and accordingly re-planning; see Section \ref{sec:replan}.}


\subsubsection{Sampling strategy} Hereafter, we employ the mass functions $f_{\ccalV}$ and $f_{\ccalU}$ designed in Appendix \ref{sec:biasedSampling} with $p_{\text{rand}}=0.9$ and $p_{\ccalU}=0.9$. Note that uniform sampling functions failed to solve the considered planning problems within three hours due to the large joint state space that needs to be explored. In fact, using uniform sampling strategies, Algorithm \ref{alg:RRT} was able to solve only small-scale problems e.g., single-agent planning problems in $4\times4$ environments with $3$ landmarks.
%
Also, notice that the computational complexity of Algorithm \ref{alg:RRT} per iteration depends linearly on the size of the selected subset $\ccalV_{k_{\text{rand}}}$ (see [line \ref{rrt:forq}, Alg. \ref{alg:RRT}]). Therefore, to speed up the construction of a feasible solution, a new set $\ccalV_k$ is constructed for every new sample, for the first $100$ iterations/samples (i.e., the first $100$ sets $\ccalV_k$ are singleton). After that, the sets $\ccalV_k$ are constructed as described in Section \ref{sec:samplingAlg}. This way the number of subsets $\ccalV_k$ remains finite as Algorithm \ref{alg:RRT}; see also Remark \ref{rem:finite}.


\subsubsection{Initial Semantic Map} 
%In what follows, we examine the performance of Algorithm \ref{alg:RRT} with respect to the number $N$ of robots, and the number $M$ of static landmarks along with the effect of robot velocities (parameter $\tau$ in \eqref{eq:nonlinRbt}). The results are summarized in Tables \ref{tab:scale} and \ref{tab:scale2} for $\tau=0.1$ and $\tau=0.5$ seconds. 
We have evaluated the performance of Algorithm \ref{alg:RRT} on two different initial semantic maps consisting of $M=15$ and $M=30$ landmarks illustrated in Figure \ref{fig:maps_tables}. Particularly, this figure shows the Gaussian distributions determining the initial semantic map $\ccalM(0)$ along with the known geometric structure. We assume that the set of classes is $\ccalC=\set{1,2,\dots,M}$,
while the true class of each landmark is uncertain. In fact, the robots have access to a discrete distribution $d(0)$ over the labels that is designed by randomly selecting a probability within the range $[0.8,1]$ that a landmark has the correct label, and by randomly selecting probabilities for the remaining classes.

\subsubsection{Mission Specification} The robots are responsible for accomplishing a search-and-rescue task captured by the following LTL formula: $\phi=\Diamond\xi_{1}\wedge\Diamond\xi_{2}\wedge\neg \xi_1 \ccalU \xi_3\wedge\Diamond(\xi_{4}\wedge\Diamond(\xi_{5}\wedge(\Diamond \xi_{6})))\wedge\Diamond\xi_{7}$
% %
%FG(p7) & F(p1) & F(p2) & (!p1 U p3) & F(p4 & F(p5 & F(p6)))
%OLD TASK
%\begin{align}\label{eq:task0}
%\phi &= \Diamond\xi_{1}\wedge\Diamond\xi_{8}\wedge (\neg \xi_1 \ccalU \xi_3)\wedge\Diamond(\xi_{2}\wedge\Diamond(\xi_{6}\wedge(\Diamond \xi_{4})))\\&\Diamond\square\xi_{\text{exit}} \wedge \square(\neg\xi_{\text{obs}})\wedge \square(\neg\xi_{1})\nonumber%xi1
%\end{align}
%NEW TASK
%\begin{align}\label{eq:task0}
%\phi &= \Diamond\xi_{1}\wedge\Diamond\xi_{2}\wedge\neg \xi_1 \ccalU \xi_3\wedge\Diamond(\xi_{4}\wedge\Diamond(\xi_{5}\wedge(\Diamond \xi_{6})))\wedge\Diamond\xi_{7}%xi1 %\wedge \square(\neg\xi_{1})\\&
%\end{align} %- defined over predicates defined in Section \ref{sec:PF} - 
%\phi &= \Diamond\xi_{1}\wedge\Diamond\xi_{8}\wedge (\neg \xi_1 \ccalU \xi_3)\wedge\Diamond(\xi_{2}\wedge\Diamond(\xi_{6}\wedge(\Diamond \xi_{4})))\\&\Diamond\square\xi_{\text{exit}} \wedge \square(\neg\xi_{\text{obs}})\wedge \square(\neg\xi_{1})\nonumber%xi1
where $\xi_i$ is a Boolean formula. Specifically, to define $\xi_i$, we decompose the robot team into smaller sub-groups where each sub-group is associated with a specific landmark. Each $\xi_i$ is associated with a finite number of pairs of robot sub-groups and an assigned landmark. We collect such pairs in a set denoted by $\ccalP_i$.
%
The Boolean formula $\xi_i$ is true if the following is true for all pairs in $\ccalP_i$: given a pair in $\ccalP_i$, all robots within a sub-group should be within $r=0.2$ meters from a specific landmark $\ell_k$ with probability greater than $1-\delta=0.75$ (see \eqref{ap1}) while the uncertainty about the position of this landmark is less than $\delta=0.01$ (see \eqref{apS}). %In other words, $\xi_i$ is expressed as a conjunction and/or disjunction of atomic predicates $g(\bbp_j,\ell_i, 0.2, 0.8)$, defined in  \eqref{apS}, over robot indices $j$.
%
%The Boolean formula $\xi_{\text{Exit}}$ is defined similarly. Specifically, it requires \textit{all} robots to reach the exit location (landmark $\ell_{11}$) with the same probabilistic requirements, i.e., following the notation of \eqref{ap1}, $\xi_{\text{Exit}}$ is defined as $\xi_{\text{Exit}}=\wedge_{j\in\ccalN}\pi_p(\bbp(t),\ccalM(t),\{j,\ell_{11}, 0.2, 0.25\})$.
%
%Also, $\xi_{\text{hostile}}$ is true if any robot approaches within $r=1$ meter a static hostile unit (any landmark with class $10$) with probability greater than $1-\delta=0.8$ that is patrolling the area, i.e., following the notation of \eqref{apMS} $\xi_{\text{hostile}}=\vee_{j\in\ccalN}\pi_p(\bbp(t),\ccalM(t),\{j,\ell_{11}, 1, 0.2, `10'\})$.
%
%Finally, $\xi_{\text{obs}}$ is true if any robot hits an obstacle. Recall that the geometric structure of the environment is assumed to be known and, therefore, $\xi_{\text{obs}}$ is a Boolean formula that does not depend on the uncertain semantic map but, instead, only on the positions of the robots and the known environmental geometric structure. 
%For instance, for a case study that involves $N=5, M=15$, each $\xi_i$ is associated with a single sub-group and, 
In words, the specification $\phi$ requires (i) sub-groups of robots to eventually satisfy $\xi_1$ (see $\Diamond\xi_1$); (ii) sub-task (i) to never happen until certain sub-groups satisfy $\xi_3$ (see $(\neg \xi_1 \ccalU \xi_3)$); (iii) robot sub-groups to eventually satisfy $\xi_2$ (see $\Diamond\xi_2$); (iii) robot sub-groups to eventually satisfy $\xi_7$ (see ($\Diamond\xi_7$)); (iv) robot sub-groups  to eventually satisfy $\xi_4$, $\xi_5$, and $\xi_6$ in this order (see $\Diamond(\xi_{4}\wedge\Diamond(\xi_{5}\wedge(\Diamond \xi_{6})))$); %(v) all robots to always avoid hostile landmarks and obstacles (see $\square(\neg\xi_{\text{obs}})\wedge \square(\neg\xi_{\text{hostile}})$); (vi) all robots to eventually exit the building and remain there forever (see $\Diamond\square\xi_{\text{exit}}$). 
The sub-tasks (i)-(iv) should be satisfied according to the probabilistic satisfaction requirements discussed above. 

Observe that the LTL task $\phi$ does not capture the requirement for obstacle avoidance. Recall that obstacle avoidance is considered during the offline path design in [line \ref{rrt:obsFree}, Alg. \ref{alg:RRT}]. Additional safety constraints can be added to line \ref{rrt:obsFree}. For instance, consider a safety property that requires all robots to always avoid approaching landmark with class $10$ within distance of $r=1$m with probability greater than $1-\delta=0.2$. This requirement can be captured by the following Boolean formula $\xi_{\text{safety}}=\wedge_{j\in\ccalN}\neg\pi_p(\bbp(t),\ccalM(t),\{j, 1, 0.8, `10'\})$, where the atomic predicate $\pi_p$ is defined as per \eqref{apMS}. Given such a safety property, every time a new sample $\bbp_{\text{new}}$ is generated, we can compute the corresponding semantic map $\ccalM_{\text{new}}$, and check if the current pair of the multi-robot state $\bbp_{\text{new}}$  and the semantic map $\ccalM_{\text{new}}$ satisfies the Boolean formula $\xi_{\text{safety}}$. If it does, the state $\bbq_{\text{new}}$ can be constructed as discussed in Algorithm \ref{alg:RRT}. Otherwise, the current sample is discarded. In this case study, we execute Alg. \ref{alg:RRT} for the specification $\phi$ along with the additional safety constraint $\xi_{\text{safety}}$ defined above.
%Observe that \eqref{eq:task0} is not a co-safe LTL formula as it includes the 'always' operator and, therefore, it is satisfied by infinite paths. To account for this, we modify the DFA corresponding to \eqref{eq:task0} as follows. First, we ignore the parts in the specification that include the `always' operator and convert the resulting formula into a DFA. Recall that a DFA transition is enabled if a Boolean formula defined over atomic predicates is satisfied. To account for the safety properties included in \eqref{eq:task0}, we augment all these Boolean formulas by including the following Boolean formula $\wedge (\neg\xi_{\text{obs}})\wedge (\neg\xi_{\text{hostile}})$ that requires the robots to always avoid obstacles and the hostile unit. Second, we add a new DFA state  and a transition from the final DFA state to this new state that is activated when the following Boolean formula is true $(\xi_{\text{exit}})\wedge(\neg\xi_{\text{obs}})\wedge(\neg\xi_{\text{hostile}})$. This Boolean formula is satisfied if all robots visit the exit of the building while avoiding obstacles and the hostile unit. Once the added DFA state is visited, the assigned LTL specification \eqref{eq:task0} is satisfied. 
\subsubsection{Scalability Results}
In what follows, we examine the performance of Algorithm \ref{alg:RRT} with respect to the number $N$ of robots, and the number $M$ of  landmarks along with the effect of robot velocities (parameter $\tau$ in \eqref{eq:nonlinRbt}). 
%
In this scalability analysis, for a fixed number $M$ of landmarks, as we increase the number of robots, we associate each $\xi_i$ in $\phi$ with more pairs of robot sub-teams and landmarks. %, i.e., we augment the set $\ccalP_i$ by adding more pairs of robot sub-teams and landmarks.
The same holds as we increase the number of landmarks given a fixed number $N$ of robots, as well. Also, we note that the mission specification does not necessarily involve all landmarks that may exist in the environment. The results are summarized in Table \ref{tab:scaleSum} for $\tau=0.1$ and $\tau=0.5$ seconds. 
% B$\ddot{\text{u}}$cchi}
%
First, using available online toolboxes \cite{duret2004spot}, we convert $\phi$ into a deterministic automaton that has $48$ states and $540$ transitions. The pruning process finished in less than a second for all cases studies considered in Table \ref{tab:scaleSum}, which e.g., for the case study $N=100, M=30$, yielded a pruned automaton with $172$ edges.
%
%
%
Observe in Table \ref{tab:scaleSum}, that as the robot velocities increase, the terminal horizon and the runtime of Algorithm \ref{alg:RRT} decrease. Also, observe in Table \ref{tab:scale3} that for a fixed number of number of robots, as the number of landmarks increase, the total runtime of Algorithm \ref{alg:RRT} increases, as the robots have to adapt planning to a `larger' map.
%
Notice that Algorithm \ref{alg:RRT} can solve large-scale tasks that may involve hundreds of robots in a reasonable time due to the biased sampling process. Recall that the employed biased sampling strategy requires computing the geodesic distance between the position of robot $j$ to the expected position of a landmark, for all robots $j$. In our implementation, to compute the geodesic distances, we first discretize the workspace and, then, we use the Dijkstra algorithm to compute the corresponding shortest paths sequentially across the robots. As a result, the runtimes can significantly decrease if the geodesic distances are computed in parallel.% across the robots while using more efficient approaches that do not involve discretization of the environment; see e.g., \cite{VisiLibity:08}.



%'FG(p7) & F(p1) & F(p2) & (!p1 U p3) & F(p4 & F(p5 & F(p6)))'

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Scalability Analysis}
\label{tab:scaleSum}
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{N} & \multirow{2}{*}{M} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Matlab Runtimes (mins)\\ (First feasible path)\end{tabular}}                                                                                          & \multicolumn{2}{c|}{H}                            \\ \cline{3-6} 
                   &                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}$\tau=0.1$\\ \end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}$\tau=0.5$\\ 
                   \end{tabular}} & $\tau=0.1$ & $\tau=0.5$ \\ \hline
1                  & 15                 & 0.66                                                                                          & 0.12                                                                                          & 461                     & 105                     \\ \hline
1                  & 30                 & 0.88                                                                                          & 0.21                                                                                          & 465                     & 107                     \\ \hline
5                  & 15                 & 1.94                                                                                          & 0.48                                                                                          & 389                     & 94                      \\ \hline
5                  & 30                 & 2.68                                                                                          & 0.58                                                                                          & 389                     & 102                     \\ \hline
20                 & 15                 & 8.74                                                                                          & 2.33                                                                                          & 561                     & 132                     \\ \hline
20                 & 30                 & 10.32                                                                                         & 2.65                                                                                          & 565                     & 121                     \\ \hline
40                 & 15                 & 14.68                                                                                         & 7.77                                                                                          & 457                     & 151                     \\ \hline
40                 & 30                 & 16.43                                                                                         & 7.81                                                                                          & 456                     & 151                     \\ \hline
100                & 15                 & 33.32                                                                                         & 15.41                                                                                         & 533                     & 147                     \\ \hline
100                & 30                 & 38.42                                                                                         & 20.56                                                                                         & 543                     & 146                     \\ \hline
\end{tabular}
\end{table}

%\begin{table}[t]
%\caption{Scalability Analysis - $\tau = 0.1$}
%\label{tab:scale}
%\centering
%\begin{tabular}{|l|l|l|l|}
%\hline
%N  & M  & MatLab runtime & H    \\ \hline
%1  & 15 & ~~~0.66 mins       & 461  \\ \hline
%1  & 30 & ~~~0.88  mins      & 465   \\ \hline
%5 & 15 & ~~~1.94 mins       & 389    \\ \hline
%5  & 30 & ~~~2.68 mins       & 389      \\ \hline
%20 & 15 & ~~~8.74  mins      & 561  \\ \hline
%20 & 30 & ~~~10.32 mins       & 565    \\ \hline
%40 & 15 & ~~~14.68  mins      & 457    \\ \hline
%40 & 30 & ~~~16.43 mins       & 456    \\ \hline
%100 & 15 & ~~~33.32 mins       & 533   \\ \hline
%100 & 30 & ~~~38.42 mins       & 543    \\ \hline
%\end{tabular}
%\end{table}
% N=20, M=15, H=564, 514.328759
%N=20, M=30, H=570, 635.502483 
%N=40, M=30, H=453, 943.722735
%N=40, M=15,H=453, 924.520976


%begin{table}[t]
%\caption{Scalability Analysis - $\tau = 0.5$}
%\label{tab:scale2}
%\centering
%\begin{tabular}{|l|l|l|l|}
%\hline
%N  & M  & MatLab runtime & H    \\ \hline
%1  & 15 & ~~~0.12 mins      & 105  \\ \hline
%1  & 30 & ~~~0.21  mins     & 107   \\ \hline
%5 & 15 & ~~~0.48 mins       & 94    \\ \hline
%5  & 30 & ~~~0.58 mins    & 102     \\ \hline
%20 & 15 & ~~~2.33  mins   & 132  \\ \hline
%20 & 30 & ~~~2.65 mins    & 121    \\ \hline
%40 & 15 & ~~~7.77  mins   & 151   \\ \hline
%40 & 30 & ~~~7.81 mins    & 151    \\ \hline
%100 & 15 & ~~~15.41 mins  & 147   \\ \hline
%100 & 30 & ~~~20.56 mins  & 146   \\ \hline
%\end{tabular}
%\end{table}

\begin{table}[t]
\caption{Scalability Analysis - $\tau = 0.5$}
\label{tab:scale3}
\centering
\begin{tabular}{|l|l|l|l|}
\hline
N  & M  & MatLab Runtime & H   \\ \hline
10 & 10 & 0.94 mins                 & 106 \\ \hline
10 & 45 & 2.98 mins                 & 146 \\ \hline
10 & 60 & 3.94 mins                 & 121 \\ \hline
10 & 75 & 5.41 mins                 & 133 \\ \hline
\end{tabular}
\end{table}

\begin{figure}[t]
 \centering
  %\includegraphics[width=1\linewidth]{figures/Drone1.png}
  \includegraphics[width=0.9\linewidth]{figures/envDrone1.png}
\caption{A drone is responsible for delivering supplies to a landmark with class `person' while always avoiding hitting landmarks with class `pole' as per \eqref{eq:taskEx}. The prior information about two landmarks is also illustrated. Observe that the prior discrete distribution for the `pole' is inaccurate in the sense that, initially, the most likely class of this landmark is `person'. }
  \label{fig:EnvDrone1}
\end{figure}

\begin{figure}[t]
  \centering
%\subfigure[$N/M=1/5$, Cost = $34.47$, $F=374$,  Runtime = 23.74secs]{
%\label{fig:traj15f}
%\includegraphics[width=0.45\linewidth]{figures/traj_1vs5_fast.pdf}}
%
%\subfigure[Initial Configuration]{
   % \label{fig:t0drone1}
  %\includegraphics[width=0.48\linewidth]{figures/t0drone1.png}
    %\includegraphics[width=0.48\linewidth]{figures/t0Drone.png}}
  \subfigure[Heading towards the `pole']{
    \label{fig:2Pole}
  %\includegraphics[width=0.48\linewidth]{figures/t1drone1replanning1.png}
  \includegraphics[width=0.47\linewidth]{figures/towardsPole.png}
  }
      \subfigure[Re-planning ]{
    \label{fig:t2drone1}
  \includegraphics[width=0.47\linewidth]{figures/replan1.png}}
        \subfigure[Re-planning ]{
    \label{fig:t3drone1}
  \includegraphics[width=0.47\linewidth]{figures/replan2.png}}
%        \subfigure[$t=220$]{
%    \label{fig:t220}
%  \includegraphics[width=0.48\linewidth]{figures/t220.png}}
          \subfigure[Avoiding `pole' \& heading towards `person']{
    \label{fig:t3drone1replan}
  \includegraphics[width=0.47\linewidth]{figures/avoidPole2Person.png}}
\subfigure[Heading towards the `person']{
    \label{fig:t3a}
  \includegraphics[width=0.47\linewidth]{figures/2Person.png}}
   \subfigure[Mission accomplished]{
    \label{fig:trajDrone1}
  %\includegraphics[width=0.45\linewidth]{traj_10vs35.pdf}
  \includegraphics[width=0.47\linewidth]{figures/traj.png}}  
 %
% \subfigure[$N/M=1/5$, Cost = $75.03$, $F=374$,  Runtime = 4.19 mins]{
%    \label{fig:biasedGreedy15}
%  \includegraphics[width=0.45\linewidth]{figures/biasedGreedy.pdf}}
 \caption{Snapshots of a drone navigating an environment towards accomplishing the task in \eqref{eq:taskEx}. The green solid line shows the path the drone currently plans to follow. The drone initially heads towards the `pole' (Fig. \ref{fig:2Pole}) believing that this landmark is a `person' due to its inaccurate prior information (see also Fig. \ref{fig:EnvDrone1}). Once the `pole' is approached, the robot updates its belief about this landmark and it re-plans so that the `pole' is avoided while heading to another landmark that is (correctly) believed to be a `person' (Fig. \ref{fig:t2drone1}-\ref{fig:t3drone1}). Once the person is detected, the belief about the position and the class of this landmark is updated, the drone re-plans, and moves towards the person (Figs. \ref{fig:t3drone1replan}-\ref{fig:t3a}). Once the person is approached as per the imposed probabilistic requirements, the mission terminates (Fig. \ref{fig:trajDrone1}).}
  \label{fig:Drone1}
\end{figure}

\subsection{Effect of Prior Map Uncertainty on Replanning Frequency}\label{sec:replanSim}
In this section, we present experimental studies that involve AsTech Firefly Unmanned Aerial Vehicles (UAVs) that operate over a semantic city with dimensions $150\times 150$. There are $M=5$ landmarks in the city and the available classes are `pole' and `person'.

\subsubsection{Robot Dynamics} 
The AsTech Firefly UAV is governed by first order dynamics where the UAV state includes the position, velocity, orientation, and biases in the measured angular velocities and acceleration; more details can be found in \cite{Furrer2016}. 
%%%
In general, the more complex the robot dynamics is, the longer it takes for sampling-based methods to generate feasible paths as they have to explore a larger state- and control- space. %; see e.g., \cite{kantaros2019asymptotically}. 
To mitigate this issue, an approach that we investigate in this section, is to generate paths for simple robot dynamics that need to be followed by robots with more complex dynamics. Specifically, in what follows, we use Algorithm \ref{alg:RRT} to synthesize  paths considering the differential drive dynamics defined in \eqref{eq:nonlinRbt} that are simpler than the actual AsTech Firefly UAV dynamics. Given the waypoints, generated by Algorithm \ref{alg:RRT}, we compute minimum snap trajectories that smoothly transition through all waypoints every $T=2$ seconds \cite{mellinger2011minimum}.
%
%Particularly, to construct them,  we model each segment connecting consecutive waypoints as the following polynomial on each segment:
%\begin{equation*}
%    \bbs(t) = \bbc_5t^5+\bbc_4t^4+\bbc_3t^3+\bbc_2t^2+\bbc_1t+\bbc_0
%\end{equation*}
%where $\bbs(t)$ denotes the position of a point on this segment at a time instant $t$, where $t$ is considered to be $0$ when the robot is at the starting waypoint of the segment. The coefficients are computing by solving an optimal control problem minimizing the jerk subject to constraints related to the positions of waypoints, the continuity of the polynomial, and boundary conditions requiring the UAVs to travel between consecutive waypoints within $T=2$ seconds. More details about computing minimum jerk trajectories can be found in \textcolor{red}{[??]}.
%To determine the coefficients of this polynomial, we impose boundary conditions on the UAV positions that require the travel time between consecutive waypoints in the nominal paths to be $T=2$ seconds for all UAVs \cite{lavalle2006planning}. 
The UAVs are controlled to follow the synthesized trajectories using the ROS package developed in \cite{Furrer2016}. %The synthesized paths allow the UAVs to always approach the original waypoints within distance less than $0.8$m.
%%%

\subsubsection{Perception System \eqref{eq:measModelR}-\eqref{eq:measModelC}}\label{sec:objRecDrone}
We assume that the drones are equipped with a downward facing sensor with rectangular field of view with dimensions $24\times16$ m that can take noisy positional measurements of landmarks falling inside its field-of-view (see e.g., Figure \ref{fig:EnvDrone1} and  \cite{freundlich2018distributed}), i.e., the measurement of landmark $\ell_i$ by robot $j$ is:
\begin{equation}\label{eq:measPosDrone}
    \bby_{j,i}=\bbx_j + \bbv,
\end{equation}
where $\bbv$ is Gaussian noise with covariance matrix with diagonal entries equal to $2$.

As for the object recognition method \eqref{eq:measModelC}, we assume that the robot is equipped with a neural network that is capable of detecting  classes of interest which are, for this case study, `car', `pole', and `person' and returning a discrete distribution over the available classes (see e.g. \cite{guo2017calibration}). Also, we model the confusion matrix of the object recognition method as follows:
\[ \left( \begin{array}{ccc}
0.8 & 0.23 & 0.06  \\
0.18  & 0.75 & 0.04 \\
0.02 & 0.02 & 0.9 \end{array} \right),\] 
where the first, second, and third row and column correspond to the classes `person', `car', and `pole', respectively. The entries in this confusion matrix capture the conditional probabilities $\mathbb{P}(\text{predicted class (row)}|\text{actual class (column)})$.
%
For instance, if the drone sees a person then with probability $0.8$, $0.18$, and $0.02$, it will generate a discrete distribution where the most likely class is `person', `car', and `pole', respectively. The confusion matrix can be learned offline based on training data. We note that any other object recognition/classification method can be used in place of the simulated one as this is used only to update the environmental belief.


\subsubsection{Mission Specifications \& Reacting to the Learned Map}

First, we consider a single drone that is responsible for accomplishing the task \eqref{eq:taskEx} described in Example \ref{ex:LTL} with parameters $r_1=r_2=0.2$ m, $\delta_1=0.2$, and $\delta_2=0.8$. The prior semantic semantic map that is available to the drone is illustrated in Figure \ref{fig:EnvDrone1}. \textcolor{black}{As per the prior Gaussian distribution, it holds that $||\hat{\bbx}_1(0)-\bbx_i||=4.9$m, $||\hat{\bbx}_2(0)-\bbx_i||= 5$m where $\ell_1$ and $\ell_2$ refer to the landmarks with true classes 'person' and 'pole', respectively. Also, the semantic prior is inaccurate as the most likely class for landmark $\ell_2$, i.e., the pole (that has to be avoided), is `person'  (who has to be approached). %with probabilility $0.66$. The prior probability that $\ell_2$ is a pole is $0.32$.  
Also, the most likely class for landmark $\ell_1$, i.e., the person, is 'person'. %with probability $0.5$. The prior probability that $\ell_1$ is a pole is $0.28$.
}
%
Due to this (partially) wrong semantic prior, the  drone initially heads towards the `pole' (see Fig. \ref{fig:2Pole}). As the drone navigates the environment, it updates the semantic map and it accordingly re-plans so that eventually the person is approached and the pole is avoided as per the imposed probabilistic requirements (see Figs. \ref{fig:t2drone1}-\ref{fig:trajDrone1}).\footnote{In our implementation, when re-planning is triggered a new tree is constructed from scratch. A more efficient approach would be to exploit the previously constructed tree structure. For instance, given the new online learned map, the a-posteriori covariance matrices for all tree nodes that are reachable from the current one (where re-planning was triggered) can be computed along with the corresponding DFA states. Then re-planning may start using this sub-tree. This way previously sampled obstacle-free multi-robot states are not discarded.} In total re-planning was triggered $5$ times. Snapshots of the robot trajectory along with instances where re-planning was triggered are provided and discussed in Figure \ref{fig:Drone1}. Additional simulations for various initial semantic maps can be found in \cite{SimSemMaps} where it can be observed that the more inaccurate the initial semantic map is, the more often re-planning is triggered. \textcolor{black}{For instance, re-planning was never triggered when the prior means of the two landmarks (i.e., person and pole) were close enough to the actual positions, i.e., $||\hat{\bbx}_1(0)-\bbx_1||= 0.7$m and $||\hat{\bbx}_2(0)-\bbx_2||=1$m, and the most likely class, as per the prior distribution $d(0)$, for each landmark, is the true one. Similar observations were made for case studies involving a team of five drones; see Figure \ref{fig:multiDrone} and \cite{SimSemMaps}.}

\begin{figure}[t]
 \centering
  \includegraphics[width=1\linewidth]{figures/MultiDrone.png}
\caption{A team of drones equipped with downward facing cameras (colored rectangles) is responsible for accomplishing a collaborative mission.}
  \label{fig:multiDrone}
\end{figure}

%Second, we also consider a team of $N=5$ drones flying over a semantic city; see e.g., Figure \ref{fig:multiDrone}. The assigned LTL task is described by the following LTL formula $\phi= (\Diamond\xi_{1})\wedge\Diamond(\xi_{2}\wedge \Diamond \xi_3)$
%\begin{align}\label{eq:taskDrone2}
%\phi= (\Diamond\xi_{1})\wedge\Diamond(\xi_{2}\wedge \Diamond \xi_3)
%\end{align} %- defined over predicates defined in Section 
%where $\xi_i$ is a Boolean formula defined as the conjunction of atomic predicates of the form \eqref{ap1} requiring a robot $j$ to be close enough to a specific landmark $\ell_i$ (regardless of its class). For instance, $\xi_1$ is defined as
%\begin{align}\label{eq:xi1}
%    &\xi_1=\pi_p(\bbp(t),\ccalM(t),\{1,1.5, 0.2, \ell_1\})\nonumber\\&\wedge\pi_p(\bbp(t),\ccalM(t),\{2,1.5, 0.2, \ell_3\})\nonumber\\&\wedge\pi_p(\bbp(t),\ccalM(t),\{1,1.5, 0.2, \ell_4\})\nonumber\\&\wedge\pi_p(\bbp(t),\ccalM(t),\{1,1.5, 0.2, \ell_7\})\nonumber\\&\wedge\pi_p(\bbp(t),\ccalM(t),\{1,1.5, 0.2, \ell_{13}\}),
%\end{align}
%which is true if at the same time the robots $1, 2, 3, 4$ and $5$ are within distance of $1.5$ m from the landmarks $\ell_1, \ell_3, \ell_4, \ell_7$ and $\ell_{13}$ with probability greater than or equal to $0.8$, respectively. In words, this task requires (i) eventually $\xi_1$ to become true; and (ii) eventually $\xi_2$ and $\xi_3$ to become true in this order. We also impose a safety constraint, as discussed in Section \ref{sec:scale}, requiring all drones to avoid landmark $\ell_{12}$ as per user-specified probabilistic requirements.
%
%Initially, we assume that the robots have access to an uncertain semantic map where the expected landmark positions are very close to the true positions. Then, we re-ran the same experiment in a more uncertain semantic map where the difference between the initially expected and the true landmark positions has increased. We observe that the more uncertain the initial semantic map is, the more often re-planning is triggered. Specifically, in the first case re-planning was triggered twice while in the second re-planning occurred seven times.

\textcolor{black}{\subsection{Effect of Map Density on Re-planning Frequency}\label{sec:ObsDensity}
In this section, we build upon the case study considered in Section \ref{sec:replanSim} and we examine how the density of uncertain obstacles/poles affect the re-planning frequency and runtimes. Specifically, we consider a single-drone with the dynamics, perceptual capabilities, and the mission specification discussed in Section \ref{sec:replanSim}. Recall that the assigned mission \eqref{eq:taskEx} requires the drone to eventually reach a person while always avoiding all poles with a user-specified probability; see also Figure \ref{fig:FourObstacles}. In Figure \ref{fig:replanRuntime}, we report the average (re-)planning runtimes as the number of the poles increases. Specifically, to design the initial or revised paths, we run Algorithm \ref{alg:RRT} five times and we report the average runtime. Observe in this figure, that as the number of uncertain poles increases, the re-planning frequency increases. Additionally, notice that as the mission progresses (i.e., as the re-planning counter increases), the runtimes tend to decrease, as the robot gets 'closer' to accomplishing the assigned task.}

\begin{figure}[t]
 \centering
  %\includegraphics[width=1\linewidth]{figures/FourObstacles.png}
   \subfigure[Initial Map]{
    \label{fig:InitMap4}
  %\includegraphics[width=0.48\linewidth]{figures/t1drone1replanning1.png}
  \includegraphics[width=0.45\linewidth]{figures/FourObst_Init.png}
  }
  \subfigure[Approaching the person ]{
    \label{fig:FinalMap44}
  %\includegraphics[width=0.48\linewidth]{figures/t1drone1replanning1.png}
  \includegraphics[width=0.45\linewidth]{figures/FourObst_End.png}
  }
\caption{\textcolor{black}{A drone tasked with reaching a person while avoiding four poles.}}
  \label{fig:FourObstacles}
\end{figure}

\begin{figure}[t]
 \centering
  \includegraphics[width=0.70\linewidth]{figures/replanRuntime.pdf}
\caption{\textcolor{black}{Graphical depiction of replanning frequency and average (re-)planning runtime. The runtime when the re-planning counter is zero refers to the runtime to design the initial paths. Each curve corresponds to a different number of poles. The markers along the curves correspond to re-planning events. The average total planning runtime for $1, 2, 3,$ and $4$ poles is $0.961, 1.176, 1.518,$ and $2.024$ secs. Note that these average runtimes are significantly smaller (between $0.1$ and $0.3$ secs) when Algorithm \ref{alg:RRT} is not executed in the Gazebo simulation environment.}}
  \label{fig:replanRuntime}
\end{figure}

\textcolor{black}{\subsection{Benefit of Predicting Offline the Metric Uncertainty}\label{sec:PredUnc}
In this section, we compare the proposed method against \cite{kantaros2019optimal}. Recall that Algorithm \ref{alg:RRT} updates the covariance matrices of the semantic map as per \eqref{constr7c} as opposed to \cite{kantaros2019optimal} where the map remains fixed during the synthesis phase. Particularly, we consider the case study discussed in Section \ref{sec:replanSim} evaluated on two semantic maps shown in Figures \ref{fig:InfoMap}-\ref{fig:UnInfoMap}. The only difference between these two maps is that the prior Gaussian distributions in Figure \ref{fig:InfoMap} are more informative (or less uncertain) than the ones in Figure \ref{fig:UnInfoMap}. When the informative map in Figure \ref{fig:InfoMap} is considered both \cite{kantaros2019optimal} and Alg. \ref{alg:RRT} generate feasible initial paths after $1.152$ and $1.548$ seconds, with costs $47$m and $46$m and terminal horizons for both equal to $13$, respectively, while re-planning was triggered three times for both algorithms. When the less informative map in Figure \ref{fig:UnInfoMap} is considered, Alg. \ref{alg:RRT} found a feasible path after $4.824$ secs. To the contrary, \cite{kantaros2019optimal} failed to design feasible initial paths as the imposed probabilistic requirements cannot be satisfied under the considered prior metric uncertainty. In other words, due to updating offline the covariance matrices, Alg. \ref{alg:RRT} can find feasible paths in prior maps with high metric uncertainty.}

\begin{figure}[t]
 \centering
  %\includegraphics[width=1\linewidth]{figures/FourObstacles.png}
    \subfigure[Informative Prior Map]{
    \label{fig:InfoMap}
  %\includegraphics[width=0.48\linewidth]{figures/t1drone1replanning1.png}
  \includegraphics[width=0.46\linewidth]{figures/InfoMap.png}
  }
    \subfigure[Uninformative Prior Map ]{
    \label{fig:UnInfoMap}
  %\includegraphics[width=0.48\linewidth]{figures/t1drone1replanning1.png}
  \includegraphics[width=0.46\linewidth]{figures/UninfoMap.png}
  }
\caption{\textcolor{black}{Semantic maps of an environment with two poles and a person. Figure \ref{fig:InfoMap} shows a semantic map with an informative metric prior distribution while Figure \ref{fig:UnInfoMap} shows a less informative map; observe the flatter Gaussian distributions.}}
  \label{fig:OfflineUpd}
\end{figure}

\subsection{Safe Planning in Semantically Unexplored Environments }\label{sec:noMap}
In this section, we evaluate Algorithm \ref{alg:RRT} in environments with known geometric structure but with no prior semantic map, i.e., when Assumption \ref{as:prior} does not hold. Specifically, in this case, the number $M$ of landmarks is unknown while a prior uncertain semantic map $\ccalM(0)$ is not available. In this case, Algorithm \ref{alg:RRT} is applied as discussed in Section \ref{sec:extensions}.
%and the set of possible classes $\ccalC$

In what follows, we consider a single ground robot with the dynamics defined in \eqref{eq:nonlinRbt} equipped with (i) a camera capable of taking noisy positional measurements (as in \eqref{eq:measPosDrone}) of all landmarks that are within range of $1$ m where the covariance matrix of the Guassian measurement noise has diagonal entries equal to $0.3$ and (ii) an object recognition method as defined in Section \ref{sec:objRecDrone}. The robot operates in an $10\times10$ m environment with the semantic and geometric structure presented in Figure \ref{fig:environmentUnexpl}. The robot is responsible for eventually finding a landmark with class `resource center' to pick up supplies, and then eventually find an `injured person' where the collected supplies will be delivered, while always avoiding known obstacles. Formally, this sequencing mission can be expressed by the following LTL formula
%
\begin{align}\label{eq:task1}
\phi = &\Diamond \{\pi_p(\bbp(t),\ccalM(t),\{1,0.2,0.1, \text{'resource center'}\})\wedge \nonumber\\ &\Diamond [\pi_p(\bbp(t),\ccalM(t),\{1,0.2,0.1, \text{'injured person'}\})]\},
\end{align}
where $\pi_p(\bbp(t),\ccalM(t),\{1,0.2,0.1, \text{'resource center'}\})$ and $\pi_p(\bbp(t),\ccalM(t),\{1,0.2,0.1, \text{'injured person'}\})$ are atomic predicates defined as per \eqref{apMS}. For instance, the latter requires the robot, with probability greater than $0.9$ to be within distance of $0.2$m from a landmark with class `injured person'. In this case study, we assume that landmarks $\ell_9$ and $\ell_{14}$ are the landmarks with classes `injured person' and 'resource center', respectively; see also Fig. \ref{fig:environmentUnexpl}.

We emphasize that initially the robot does not have any prior information about where the landmarks of interest are. As a result, the robot initially adopts an exploration mode aiming to detect landmarks of interest; see Fig. \ref{fig:t0}. Here, since the mission involves two distinct landmarks, we require the robot to switch from exploration to exploitation (i.e., application of Algorithm \ref{alg:RRT} over the currently learned semantic map) for the first time when the first two landmarks are detected. This happens at the time instant $t=225$ (see Fig. \ref{fig:t225}). Algorithm \ref{alg:RRT} fails to design a path satisfying the assigned task based on the currently learned map within $1000$ iterations. Thus, the robot keeps being in exploration mode and switches to exploitation mode every time a new landmark is detected. At $t=335$, both landmark $\ell_9$ and $\ell_5$ are detected and then Algorithm \ref{alg:RRT} is triggered generating feasible paths over the currently learned semantic map. Then the robot switches to an exploitation mode following the synthesized paths; see Fig. \ref{fig:ExploitationMode}. Observe in Figure \ref{fig:ExploitationMode} that the robot does not explore the whole environment but, instead, it only partially learns/explores the environment to accomplish the assigned mission. This simulation required in total $51.2$ \text{seconds}.


\begin{figure}[t]
 \centering
  \includegraphics[width=0.60\linewidth]{figures/EnvironmentUnexplored.png}
\caption{Graphical depiction of the environment considered in Section \ref{sec:noMap}. The gray polygons represent known obstacles while the red squares denote the true positions of the landmarks. The numbers next to the landmarks denote their respective indices. Each index correspond to a different label, i.e., there are $|\ccalC|=14$ available classes. For instance, $14$ (bottom right corner) corresponds to 'resource center' while $9$ (top right corner) corresponds to 'injured person'. The robot does not know either the positions or the classes of the landmarks.}
  \label{fig:environmentUnexpl}
\end{figure}


\begin{figure}[t]
  \centering
%\subfigure[$N/M=1/5$, Cost = $34.47$, $F=374$,  Runtime = 23.74secs]{
%\label{fig:traj15f}
%\includegraphics[width=0.45\linewidth]{figures/traj_1vs5_fast.pdf}}
%
\subfigure[$t=0$]{
    \label{fig:t0}
  \includegraphics[width=0.48\linewidth]{figures/t0.png}}
  \subfigure[$t=40$]{
    \label{fig:t40}
  \includegraphics[width=0.48\linewidth]{figures/t40.png}}
%    \subfigure[$t=100$]{
%    \label{fig:t100}
%  \includegraphics[width=0.48\linewidth]{figures/t100.png}}
%      \subfigure[$t=160$]{
 %   \label{fig:t160}
%  \includegraphics[width=0.48\linewidth]{figures/t160.png}}
%        \subfigure[$t=220$]{
%    \label{fig:t220}
%  \includegraphics[width=0.48\linewidth]{figures/t220.png}}
          \subfigure[$t=225$]{
    \label{fig:t225}
  \includegraphics[width=0.48\linewidth]{figures/t225.png}}
%\subfigure[$t=280$]{
%    \label{fig:t280}
%  \includegraphics[width=0.48\linewidth]{figures/t280.png}}
%  \subfigure[$t=320$]{
%    \label{fig:t320}
%  \includegraphics[width=0.48\linewidth]{figures/t320.png}}
%   \subfigure[$t=330$]{
 %   \label{fig:t330}
%  \includegraphics[width=0.48\linewidth]{figures/t330.png}}
   \subfigure[$t=335$]{
    \label{fig:t335}
  %\includegraphics[width=0.45\linewidth]{traj_10vs35.pdf}
  \includegraphics[width=0.48\linewidth]{figures/t335.png}}  
 %
% \subfigure[$N/M=1/5$, Cost = $75.03$, $F=374$,  Runtime = 4.19 mins]{
%    \label{fig:biasedGreedy15}
%  \includegraphics[width=0.45\linewidth]{figures/biasedGreedy.pdf}}
 \caption{Exploration Mode: Figures \ref{fig:t0}-\ref{fig:t335} illustrate the robot path towards exploring the environment. The green disk, red square, and the green solid line represent the initial robot location, the current robot location, and the followed trajectory, respectively. The green circle centered at the current robot position denotes the sensing range. The green squares denote the actual position of the detected landmarks. Gaussian distributions for landmarks $\ell_i$ with $\det\Sigma_i<10^{-5}$ are not shown. The numbers next to the landmarks show the most likely class. The blue dots represent the cells of the grid map that have been explored while the red diamonds show the `fake' exploration landmarks. At time instants $t=40$,  $t=225$, and $t=335$, the landmarks $\ell_{12}$, $\ell_{14}$ ('resource center'), and $\ell_5$ and $\ell_9$ ('injured person') are detected, respectively. Mission-based planning (Algorithm \ref{alg:RRT}) was triggered at the time instants $t=225$, and $t=335$. Feasible paths were found only at $t=335$ illustrated in Figure \ref{fig:ExploitationMode}.}
  \label{fig:ExplorationMode}
\end{figure}

\begin{figure}[t]
  \centering
%\subfigure[$N/M=1/5$, Cost = $34.47$, $F=374$,  Runtime = 23.74secs]{
%\label{fig:traj15f}
%\includegraphics[width=0.45\linewidth]{figures/traj_1vs5_fast.pdf}}
%
\subfigure[$t=350$]{
    \label{fig:t350}
  \includegraphics[width=0.48\linewidth]{figures/t350m.png}}
  \subfigure[$t=380$]{
    \label{fig:t380}
  \includegraphics[width=0.48\linewidth]{figures/t380m.png}}
%    \subfigure[$t=390$]{
%    \label{fig:t390}
%  \includegraphics[width=0.48\linewidth]{figures/t390m.png}}
      \subfigure[$t=410$]{
    \label{fig:t410}
  \includegraphics[width=0.48\linewidth]{figures/t410m.png}}
  %\subfigure[$t=430$]{
  %  \label{fig:t430}
 % \includegraphics[width=0.48\linewidth]{figures/t430m.png}}
\subfigure[$t=435$]{
    \label{fig:t435}
  \includegraphics[width=0.48\linewidth]{figures/t435m.png}}
 \caption{Exploitation Mode: Figures \ref{fig:t350}-\ref{fig:t435} illustrate the robot path (cyan solid line) to accomplish the task \eqref{eq:task1} designed at time $t=335$ (green disk) when Algorithm \ref{alg:RRT} successfully designed feasible paths. %The paths are designed by Algorithm \ref{alg:RRT} over the semantic map built until the time instant $t=335$ (see Figure \ref{fig:t335}). 
 From $t=335$ until $t=380$, the robot moves towards landmark $\ell_{14}$ ('resource center'). Once this landmark is visited as per the imposed probabilistic requirement, the robot heads towards landmark $\ell_9$ ('injured person') which is visited at $t=435$ and, then, the mission terminates.} 
  \label{fig:ExploitationMode}
\end{figure}





==> files/theory.tex <==
In this section, we examine, the correctness and optimality of Algorithm \ref{alg:RRT}. First, in Theorem \ref{thm:probCompl},  we show that Algorithm \ref{alg:RRT} is probabilistically complete. In other words, given an initial semantic map $\ccalM(0)$ and a sensor model as per \eqref{eq:measModelR}, if there exists a solution to \eqref{eq:Prob2}, then Algorithm \ref{alg:RRT} will eventually find it.
%a sequence of multi-robot states $\bbp_{0:H}$ and a corresponding sequence of semantic maps $\ccalM_{0:H}$, where the metric uncertainty is updated as discussed in Section \ref{sec:updateMap}, that solve \eqref{eq:Prob2}
In Theorem \ref{thm:asOpt}, we also show that Algorithm \ref{alg:RRT} is asymptotically optimal, i.e., Algorithm \ref{alg:RRT} will eventually find the optimal solution to \eqref{eq:Prob2}, if it exists. The proofs can be found in Appendix \ref{sec:prop}.%Note that completeness and optimality guarantees hold in the presence of mobile landmarks, as well, under the assumptions discussed in Section \ref{sec:extend}.


%in Theorem \ref{thm:probCompl} and \ref{thm:asOpt}, we show that Algorithm \ref{alg:RRT} is probabilistically complete and asymptotically optimal. 

%To show completeness and optimality, we need to make the following two assumptions about the sampling strategy. First, any density function $f_{\ccalV}$ and $f_{\ccalU}$ can be used as long as they satisfy Assumptions \ref{frand} and \ref{fnew}, respectively.%\NA{It is not allowed to sample control at the same node twice, correct? To me the discrete distributions are more of a prioritization of the search of the tree -- does it have to be random?} %\BS{How do you choose amongst the different possible nodes in the set $\ccalV_k$, once $k$ is chosen?}

%We make the following assumptions for $f_{\ccalV}$:
%\begin{assumption}[Probability density function %$f_{\ccalV}$]\label{frand}
%(i) The probability density function $f_{\ccalV}(k|\ccalV):\set{1,\dots,K_n}\rightarrow[0,1]$ satisfies $f_{\ccalV}(k|\ccalV)\geq \epsilon$, $\forall$ $k\in\set{1,\dots,K_n}$ and for all $n\geq 0$, for some $\epsilon>0$ that remains constant across all iterations $n$. 
%(ii) Independent samples $k_{\text{rand}}$ can be drawn from $f_{\ccalV}$.
%\end{assumption}

%Any density function $f_{\ccalU}$ can be used to draw samples $\bbu_{\text{new}}\in\ccalU$ as long as it satisfies the following assumption.
%The density function $f_{\ccalU}$ should be designed so that it satisfies the following assumption.

%\begin{assumption}[Probability density function $f_{\ccalU}$]\label{fnew}
%(i) The distribution $f_{\ccalU}(\bbu)$ satisfies $f_{\ccalU}(\bbu)\geq \zeta$, for all $\bbu\in\ccalU$, for some  $\zeta>0$ that remains constant across all iterations $n$. (ii) Independent samples $\bbu_{\text{new}}$ can be drawn from the probability density function $f_{\ccalU}$.
%\end{assumption}


%\red{add some description}
To show completeness and optimality of Algorithm \ref{alg:RRT}, we assume that the probability mass functions $f_{\ccalV}$ and $f_{\ccalU}$ satisfy Assumptions \ref{frand} and \ref{fnew}, respectively.
\begin{theorem}[Probabilistic Completeness]\label{thm:probCompl}
If there exists a solution to \eqref{eq:Prob2}, then Algorithm \ref{alg:RRT} is probabilistically complete, i.e., the probability of finding a feasible solution, i.e., a feasible horizon $H$ and a feasible sequence of control inputs $\bbu_{0:H}$ for \eqref{eq:Prob2}, goes to $1$ as $n\to\infty$.
\end{theorem}
%If there exists a solution to (10), then Algorithm 1 is probabilistically complete, i.e., the probability of finding a feasible solution, i.e., a feasible horizon $H$ and a feasible sequence control inputs $\bbu_{0:H}$ for (10), goes to $1$ as $n_{\text{max}}\to\infty$

%\begin{theorem}[Probabilistic Completeness]\label{thm:probCompl}
%If there exists a solution to \eqref{eq:Prob2}, then Algorithm \ref{alg:RRT} is probabilistically complete, i.e., it will find with probability $1$ a path $\bbq_{0:H}$, defined as a sequence of states in $\ccalV$, i.e., $\bbq_{0:H} = \bbq(0), \bbq(1), \bbq(2), \dots, \bbq(H),$
%\begin{equation}\label{eq:path}
%\bbq_{0:H} = \bbq(0), \bbq(1), \bbq(2), \dots, \bbq(F),
%\end{equation}
%that satisfies all constraints of \eqref{eq:Prob2}, where $\bbq(h)\in\ccalV$, for all $h\in\{0,\dots,H\}$.
%\end{theorem}

\begin{theorem}[Asymptotic Optimality]\label{thm:asOpt}
Assume that there exists an optimal solution to  \eqref{eq:Prob2}. Then, Algorithm \ref{alg:RRT} is asymptotically optimal, i.e., the optimal horizon $H$ and the optimal sequence of control inputs $\bbu_{0:H}$ will be found with probability $1$, as $n\to\infty$. In other words, the path generated by Algorithm \ref{alg:RRT} satisfies
$\mathbb{P}\left(\left\{\lim_{n\to\infty} J(H,\bbu_{0:H})=J^*\right\}\right)=1,$
%\begin{equation}\label{eq:opt1}
%\mathbb{P}\left(\left\{\lim_{n\to\infty} J(F,\bbu_{0:H})=J^*\right\}\right)=1,
%\end{equation} 
where $J$ is the objective function of \eqref{eq:Prob2} and $J^*$ is the optimal cost.\footnote{Note that the horizon $H$ and $\bbu_{0:H}$ returned by Algorithm \ref{alg:RRT} depend on $n$. For simplicity of notation, we drop this dependence.}%\NA{Make $F$ or $J(F,\bbu_{0:H})$ explicitly a function of $n$?}
%, $F$ is the terminal finite horizon, $\bbq_0=\bbq_r$, $\bbu_{0:H}$ is the sequence of control inputs that generate the optimal path $\bbQ^*$,
\end{theorem}
%
%Assume that there exists an optimal solution to  \eqref{eq:Prob2}. Then, Algorithm \ref{alg:RRT} is asymptotically optimal, i.e., the optimal path  $\bbq_{0:H}^* =  \bbq(0), \bbq(1), \bbq(2), \dots, \bbq(H)$, will be found with probability $1$, as $n\to\infty$. In other words, the path generated by Algorithm \ref{alg:RRT} satisfies $\mathbb{P}\left(\left\{\lim_{n\to\infty} J(H,\bbu_{0:H})=J^*\right\}\right)=1,$

Recall from Section \ref{sec:replan} that the synthesized paths may need to be revised online by re-running Algorithm \ref{alg:RRT}. Theorems \ref{thm:probCompl}-\ref{thm:asOpt} imply that if re-planning is required at any time $t$, a feasible and the optimal path will eventually be found, if they exist. Nevertheless, the proposed control architecture cannot guarantee recursive feasibility, i.e., existence of feasible paths at future time instants when re-planning is needed. In fact, existence of feasible paths when re-planning is triggered depends on the initialization of the corresponding optimal control problem \eqref{eq:Prob2}, i.e., the online constructed map and, consequently, on the perceptual feedback which is hard to predict a-priori.
%\textcolor{red}{ADD SOME WORDS ABOUT REPLANNING}

%\begin{rem}[Density functions $f_{\ccalV}$ and $f_{\ccalU}$]
%Note that Assumptions \ref{frand}(i) and \ref{fnew}(i) also imply that the density functions $f_{\ccalV}$ and $f_{\ccalU}$ are bounded away from zero on $\set{1,\dots,K_n}$ and $\ccalU$, respectively. Also, observe that Assumptions \ref{frand} and \ref{fnew} are very flexible, since they also allow $f_{\ccalV}$ and $f_{\ccalU}$ to change with iterations $n$ of Algorithm \ref{alg:RRT}, as the tree grows.
%\end{rem}

%\begin{rem}[Sampling Strategy]
%An example of a distribution $f_{\ccalV}$ that satisfies Assumption \ref{frand} is the discrete uniform distribution $f_{\ccalV}(k|\ccalV )=\frac{1}{k}$, for all $k\in\set{1,\dots,K_n}$. Observe that the uniform function trivially satisfies Assumption \ref{frand}(ii). Also, observe that Assumption \ref{frand}(i) is also satisfied, since there exists an $\epsilon>0$ that satisfies Assumption \ref{frand}(i), which is $\epsilon =\frac{1}{|\ccalR|}$, where $\ccalR$ is a set that collects all robot configurations $\bbp$ that can be reached by the initial state $\bbp(0)$. Note that $\ccalR$ is a finite set, since the set $\ccalU$ of admissible control inputs is finite, by assumption. Similarly, uniform density functions $f_{\ccalU}$ satisfy Assumption \ref{fnew}. Note that any functions $f_{\ccalV}$ and $f_{\ccalU}$ can be employed as long as they satisfy Assumptions \ref{frand} and \ref{fnew}. Nevertheless, the selection of $f_{\ccalV}$ and $f_{\ccalU}$ affects the performance of Algorithm \ref{alg:RRT}; see the numerical experiments in Section \ref{sec:Sim}. In  Section \ref{sec:biasedSampling}, we design (nonuniform) density functions $f_{\ccalV}$ and $f_{\ccalU}$ that bias the exploration towards locations that are expected to contribute to the satisfaction of the assigned mission specification. %The latter allows us to solve large-scale active information acquisition problems.
%\end{rem} 

%Given that the optimal horizon $F$ is finite, 
%In the next theorem we show that Algorithm \ref{alg:RRT} converges exponentially fast the optimal solution of \eqref{eq:Prob2}. %with respect to iterations $n$. 
%Lemma \ref{lem:optHor} also implies that the optimal control problem \eqref{eq:Prob2} is well-defined in the sense that the optimal cost $J(F,\bbu_{0:H})$ is finite.




%According to Theorem \ref{thm:probCompl}-\ref{thm:asOpt}, Algorithm \ref{alg:RRT} can find feasible open-loop sensor control policies (including the optimal one) that satisfy $\phi$. Recall that satisfaction of $\phi$ depends on the sequence of both robot states $\bbp(t)$ and semantic maps $\ccalM(t)$. Moreover, recall also that Algorithm \ref{alg:RRT} synthesizes paths using predicted maps $\ccalM(t)$ that may differ from the maps that would be obtained after fusing collected measurements; see also Section \ref{sec:replan}. %Thus, in Theorems \ref{thm:probCompl}-\ref{thm:asOpt} $\bbq_{0:H}\models\phi$ means that the finite sequence of robot states and \textit{predicted} semantic maps satisfy $\phi$. 
%In other words, the open-loop control policies determined by Algorithm \ref{alg:RRT} that solve \eqref{eq:Prob2} are not necessarily feasible solutions to the closed-loop optimal control problem \eqref{eq:Prob1} and, therefore, re-planning may be required as the robots collect measurements and update the map; see Section \ref{sec:replan}.
%
%
%In fact, the optimal open-loop control policy that solves \eqref{eq:Prob2} is also the optimal closed-loop control policy if (i) the sensor model is linear in the hidden state dynamics and the landmark dynamics are linear, (ii) there is no process noise, and (iii) the prediction for the initial landmark positions $\hat{\bbx}(0)$ matches exactly the true initial landmark positions, i.e., $\hat{\bbx}(0)=\bbx(0)$. Condition (i) ensures that the a-posteriori covariance matrices can be computed offline as per \eqref{constr7b} and conditions (ii)-(iii) ensure the Kalman-filter prediction of the landmark state coincide with true landmark states.
%
%Also, note that in case the maps $\ccalM(t)$ are always deterministic and known, i.e., the true landmark positions and classes are known, then Theorems Theorems \ref{thm:probCompl}-\ref{thm:asOpt} still hold. In fact, \eqref{eq:Prob1} is equivalent to \eqref{eq:Prob2}  if (i) the sensor model is linear in the hidden state dynamics and the landmark dynamics are linear, (ii) there is no process noise, and (iii) the prediction for the initial landmark positions $\hat{\bbx}(0)$ matches exactly the true initial landmark positions, i.e., $\hat{\bbx}(0)=\bbx(0)$. Condition (i) ensures that the a-posteriori covariance matrices can be computed offline as per \eqref{constr7b} and conditions (ii)-(iii) ensure the Kalman-filter prediction of the landmark state coincide with the Kalman-filter update step.
%
%only (i) in the trivial case where  the map $\ccalM(t)$ is always deterministic and known, i.e., the true landmark positions and classes are known, and (ii) if the $\ccalM(t)$ is still probabilistic but is never updated using sensor measurements, i.e., constraints \ref{}

%(see e.g., line \ref{rrt:xnew})
%In the following Theorem \ref{thm:conv}, we show that Algorithm \ref{alg:RRT} converges exponentially fast to the optimal solution of Problem \ref{prob} while the exponential rate depends on the selected sampling functions. \red{will probably delete this theorem..}

%\begin{theorem}[Convergence rate bounds]\label{thm:conv}
%Let $\bbq_{0:H}^*$ denote the optimal solution to \eqref{eq:Prob2}. Then, there exist parameters $\alpha_n(\bbq_{0:H}^*)\in(0,1]$, which depend on the selected density functions $f_{\ccalV}$ and $f_{\ccalU}$, for every iteration $n$ of Algorithm \ref{alg:RRT}, such that 
%\begin{equation}\label{eq:bnd1}
%1 \geq \mathbb{P}(A^{n}(\bbq_{0:H}^*)) \geq 1-e^{-\frac{\sum_{n=1}^{n}\alpha_n(\bbq_{0:H}^*)}{2}n+H},
%\end{equation}
%if $n>H$. In \eqref{eq:bnd1}, $A^n(\bbq_{0:H}^*)$ denotes the event that Algorithm \ref{alg:RRT} constructs the path $\bbq_{0:H}^*$ within $n$ iterations.
%\end{theorem}

%\begin{rem}[Convergence rate] 
%Observe in \eqref{eq:bnd1} that $\lim_{n\to\infty}\mathbb{P}(A^n(\bbq_{0:H}^*))=1$. This means that if Problem \ref{prob} has an optimal solution, then Algorithm \ref{alg:RRT} will find it with probability $1$ as $n\to\infty$, as expected due to Theorem \ref{thm:asOpt}.  
%Note that if Problem \ref{prob} is not well-defined, i.e., if it requires an infinite sequence of control inputs (e.g., this may happen for small parameters $\delta_i$), then Algorithm \ref{alg:RRT} will never be able t
%\end{rem}



%\section{Online Execution and Re-planning}\label{sec:replan}
%\centering
%.....to be completed.....

%--here we use the semantic/metric measurements to update the map\\

%-- if ('important') inconsistencies show up with respect to the offline predicted maps, replanning is required. Explain what ('important') inconsistencies mean\\

%-- explain how we replan
